AccMPEG: Optimizing Video Encoding for Video Analytics

With more videos being recorded by edge sensors (cameras) and analyzed by computer-vision deep neural nets (DNNs), a new breed of video streaming systems has emerged, with the goal to compress and stream videos to remote servers in real time while preserving enough information to allow highly accurate inference by the server-side DNNs. An ideal design of the video streaming system should simultaneously meet three key requirements: (1) low latency of encoding and streaming, (2) high accuracy of server-side DNNs, and (3) low compute overheads on the camera. Unfortunately, despite many recent efforts, such video streaming system has hitherto been elusive, especially when serving advanced vision tasks such as object detection or semantic segmentation. This paper presents AccMPEG, a new video encoding and streaming system that meets all the three requirements. The key is to learn how much the encoding quality at each (16x16) macroblock can influence the server-side DNN accuracy, which we call accuracy gradient. Our insight is that these macroblock-level accuracy gradient can be inferred with sufficient precision by feeding the video frames through a cheap model. AccMPEG provides a suite of techniques that, given a new server-side DNN, can quickly create a cheap model to infer the accuracy gradient on any new frame in near realtime. Our extensive evaluation of AccMPEG on two types of edge devices (one Intel Xeon Silver 4100 CPU or NVIDIA Jetson Nano) and three vision tasks (six recent pre-trained DNNs) shows that AccMPEG (with the same camera-side compute resources) can reduce the end-to-end inference delay by 10-43% without hurting accuracy compared to the state-of-the-art baselines

==> abstract-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\begin{abstract}

As video-based intelligent applications proliferate, today more videos are analyzed by computer vision models (in forms of deep neural nets or DNNs) than watched by human users.
While the needs to process videos {\em en masse} spur new pipelines for video analytics, less attention has been given to the underlying video stack, which the analytics pipelines are built on. 
Current video applications inherit and customize the traditional video codecs (\eg H.264/MPEG) with handcrafted heuristics tied to particular applications. %, and a systematic understanding regarding how existing codec is largely missing.

In this work, we design and implement \name, a new video stack with the explicit design goals of 
(1) preserving high inference accuracy for a range of computer vision DNNs, and 
(2) compressing videos close-to-minimum sizes.
As we show that the optimal encoding of a video differs significantly across DNN models, achieving the two goals is impossible without a proper understanding the unique compression opportunities in each DNN model.
%on how the video encoding quality of a particular video affects the inference of a particular DNN model.
To this end, \name embodies two novel concepts. 
%In this work, we set to address two fundamental misalignment between the underlying video stack and the served applications: (1) the same video stack should apply to a variety of computer vision models, and (2) it should strike a close-to-optimal balance between video compression and computer vision accuracy by fully customizing to the need of the served applications.
%We present \name, a new video stack that achieves both objectives using several new concepts.
First, \name treats the video analytics logic as a {\em differentiable black box}, which applies to almost all modern computer vision models.
Second, for any video frame, \name calculates a new notion called {\em accuracy gradients}, which indicate where in the frame the DNN's inference result is highly sensitive to the encoding quality level and thus needs to be encoded with high quality.
%, and encodes videos using high quality only in regions of high accuracy gradients.
%\name therefore embraces the unique compression opportunities of each given analytics logic, and do so with a unified approach. 
%closer-to-optimal compression/accuracy balance than prior work.
%Our solution \name achieves (1) by treating arbitrary computer vision model as a {\em differentiable} ``black box'', and achieves (2) by encoding frames with spatially different quality assigned based on {\em accuracy gradients} which indicate how sensitive the final inference result is to the quality settings at each fine-grained region in a frame. 
%To realize these benefits in practice, we present a suite of solutions, including how to accurately infer the accuracy gradients and how to achieve that efficiently with low encoding, decoding and inference delays.
We test the effectiveness of \name in three vision tasks over a variety of real-world videos. 
Our results show that compared with the state-of-the-art baselines, \name achieves \fillme\% higher compression efficiency and \fillme\% higher accuracy at the same time. Moreover, \name's encoding/decoding delays are almost the same as the traditional codec.

%heavily influences the performance of video analytics applications.
%which is designed to enhance the video quality perceived by human viewers, rather than the performance of computer vision models. 


%creating a deeper integration between the underlying stack and the video analytics application, enabling the computer vision models to explicitly and directly guide the control of the underlying stacks. 
%As tangible results of the project, we will propose system interfaces, foundational algorithms, and practical systems of a custom stack for a wide range of video analytics tasks.

\end{abstract}


==> abstract-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\begin{abstract}

As video analytics applications proliferate, nowadays more videos are analyzed by computer vision models (in forms of deep neural nets or DNNs) than watched by human users.
To scale out video analytics, we present \name, a new video stack that provides efficient video compression and streaming for accurate inference across a wide range of computer vision DNNs.
Though there are similar efforts in the past, they optimize at some {\em task-specific} spatial granularities (\eg in object detection, what quality should a frame, object, or background be encoded in). 
Contrary to the conventional wisdom, our analysis reveals a significant yet untapped room for improving both video compression efficiency and inference accuracy, through customizing the encoding quality of individual {\em finer-grained} blocks (\eg 16 by 16 pixels) for each {\em specific DNN} (\eg a particular object detector).
To realize these potential benefits, \name makes two contributions to deeply integrate the analytics DNN in a video stack.
(1) \name treats different DNNs (even those for the same vision task) as unique {\em differentiable black boxes}, from which we derive a new abstraction called {\em accuracy gradient}, which indicates the impact of each block's encoding quality on the final DNN's inference accuracy.
(2) \name provides a suite of techniques to infer the accuracy gradients and uses them to optimize video compression and inference accuracy, all in real time.
Our evaluation of \name over three vision tasks shows that compared to the state-of-the-art baselines, \name reduces the file size by 50\% while increasing the accuracy by 4\%. 
Moreover, \name's encoding/decoding delays are almost the same as the traditional codecs.

\end{abstract}


==> abstract-v4.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\begin{abstract}

As mobile/edge applications store and analyze massive videos, they inspire many new video encoding techniques whose goal is to encode only few pixels in high quality yet still allowing computer-vision models (DNNs) running on remote servers to achieve high inference accuracy.
Yet, we argue that current solutions are fundamentally limited on two fronts.
First, they assign video quality at coarse granularities; \eg same quality is used to encode an entire bounding box, background region, or frame.
However, our analysis reveals that both video compression efficiency and inference accuracy could be significantly improved, if video quality is assigned at {\em finer-grained} granularities (\eg 16$\times$16 blocks).
Second, to make better encoding decisions, recent solutions increasingly rely on feeding online sampled video frames to the remote computer-vision DNN, but this can be hard to realize when the video sensor has sporadic network connection or privacy concerns that preclude sharing videos with remote servers in realtime. 
% Second, it is believed that making optimal encoding decisions require real-time feedback from the final computer-vision DNN, which makes it hard to encode videos in real time on video sensors that have low computing power, sporadic network connectivity, or privacy concerns that preclude sharing videos with remote servers. 

To address the limitations, we present \name, a new technique that uses a {\em local} model to optimally assign video encoding quality at a {\em macroblock} granularity.
The key idea behind \name is {\em accuracy gradients}, which indicate how much each macroblock's encoding quality can influence the final DNN's inference accuracy. 
Given {\em any} computer-vision DNN, \name treats it as a differentiable blackbox and proposes a suite of systems techniques that {\em quickly} create a cheap model to infer the given DNN's accuracy gradient per macroblock on any new frame, and based on real-time inference of accuracy gradients, encode different macroblocks with different encoding qualities.
% and (2) encode macroblock different encoding qualities at different macroblocks based on online inference of accuracy gradients.
Our evaluation of \name over three vision tasks shows that compared to the state-of-the-art baselines, \name reduces the file size by 50\% while increasing the accuracy by 4\%. 

% To address these challenges, we present \name, a new technique that optimizes video encoding for accuracy video analytics.
% \name makes two contributions that deeply integrate the computer-vision Dnn with video encoding. 
% (1) \name treats different DNNs (even those for the same vision task) as unique {\em differentiable} black boxes, from which we derive a new abstraction called {\em accuracy gradient}, which indicates the impact of each block's encoding quality on the final DNN's inference accuracy.
% Our evaluation of \name over three vision tasks shows that compared to the state-of-the-art baselines, \name reduces the file size by 50\% while increasing the accuracy by 4\%. 
% (2) \name provides a suite of techniques to infer the accuracy gradients and uses them to optimize video compression and inference accuracy, all in {\em real time}.
% Moreover, \name's encoding/decoding delays are almost the same as the traditional codecs.


% As video analytics applications proliferate, nowadays more videos are analyzed by computer vision models (in forms of deep neural nets or DNNs) than watched by human users.
% To scale out video analytics, we present \name, a new video stack that provides efficient video compression and streaming for accurate inference across a wide range of computer vision DNNs.
% Though there are similar efforts in the past, they optimize at some {\em task-specific} spatial granularities (\eg in object detection, what quality should a frame, object, or background be encoded in). 
% Contrary to the conventional wisdom, our analysis reveals a significant yet untapped room for improving both video compression efficiency and inference accuracy, through customizing the encoding quality of individual {\em finer-grained} blocks (\eg 16 by 16 pixels) for each {\em specific DNN} (\eg a particular object detector).
% To realize these potential benefits, \name makes two contributions to deeply integrate the analytics DNN in a video stack.
% (1) \name treats different DNNs (even those for the same vision task) as unique {\em differentiable black boxes}, from which we derive a new abstraction called {\em accuracy gradient}, which indicates the impact of each block's encoding quality on the final DNN's inference accuracy.
% (2) \name provides a suite of techniques to infer the accuracy gradients and uses them to optimize video compression and inference accuracy, all in real time.
% Our evaluation of \name over three vision tasks shows that compared to the state-of-the-art baselines, \name reduces the file size by 50\% while increasing the accuracy by 4\%. 
% Moreover, \name's encoding/decoding delays are almost the same as the traditional codecs.

\end{abstract}


==> abstract.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\begin{abstract}

As video-based intelligent applications proliferate, today more videos are processed by vision models (in forms of deep neural nets or DNNs) than watched by users.
While the need to analyze videos {\em en masse} inspires many efficient video analytics pipelines, less attention has been given to the underlying video stack, on top of which the analytics pipelines are built. 
Currently, video applications inherit and customize the traditional video codecs (\eg H.264/MPEG video codec and DASH/HTTP streaming protocol) using handcrafted heuristics that are tied to particular applications. %, and a systematic understanding regarding how existing codec is largely missing.

In this work, we set out to achieve two goals: (1) the same video stack should support a variety of computer vision models, and (2) it should strike a close-to-optimal balance between video compression and computer vision accuracy by fully customizing to the need of the served applications.
%In this work, we set to address two fundamental misalignment between the underlying video stack and the served applications: (1) the same video stack should apply to a variety of computer vision models, and (2) it should strike a close-to-optimal balance between video compression and computer vision accuracy by fully customizing to the need of the served applications.
We design and implement \name, a new video stack that achieves both objectives using two novel concepts.
First, \name treats the video analytics logic as a {\em differentiable black box}, which applies to almost all DNN-based computer vision models.
Second, given any video analytics logic, it calculates the {\em accuracy gradients} that measure the sensitivity of the vision inference result to the quality level at each spatial region, and then encodes videos using high quality only in regions of high accuracy gradients.
\name therefore embraces the unique compression opportunities of each given analytics logic, and do so with a unified approach. 
%closer-to-optimal compression/accuracy balance than prior work.
%Our solution \name achieves (1) by treating arbitrary computer vision model as a {\em differentiable} ``black box'', and achieves (2) by encoding frames with spatially different quality assigned based on {\em accuracy gradients} which indicate how sensitive the final inference result is to the quality settings at each fine-grained region in a frame. 
%To realize these benefits in practice, we present a suite of solutions, including how to accurately infer the accuracy gradients and how to achieve that efficiently with low encoding, decoding and inference delays.
We test the effectiveness of \name in three vision tasks over a variety of real-world videos. 
Our results show that compared with the state-of-the-art baselines, \name achieves \fillme\% higher compression efficiency and \fillme\% higher accuracy at the same time. Moreover, \name's encoding/decoding delays are almost the same as the traditional codec.

%heavily influences the performance of video analytics applications.
%which is designed to enhance the video quality perceived by human viewers, rather than the performance of computer vision models. 


%creating a deeper integration between the underlying stack and the video analytics application, enabling the computer vision models to explicitly and directly guide the control of the underlying stacks. 
%As tangible results of the project, we will propose system interfaces, foundational algorithms, and practical systems of a custom stack for a wide range of video analytics tasks.

\end{abstract}


==> discuss.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\section{Discussion: Towards a new encoding interface for video analytics}
\label{sec:discuss}


%\mypara{Encoding-invariant computer vision}


Our ultimate vision is to propose a new video stack interface with primitives designed specifically for the need of computer vision analytics.
In developing \name, it has become clear to us that the interface of existing video codecs is ill-suited. 
We identify three particular mismatches.

First, ensuring high accuracy is crucial for video analytics applications, but the primitive to enforce inference accuracy is currently missing in the traditional video codecs. 
The concept of \ag (and the \ag threshold $\AgThresh$) is one step in this direction to explicitly prioritize accuracy, but as shown in Figure~\ref{fig:eval-video-adaptation}, its effect is only ``best-effort'' (\ie accuracy is not guaranteed to be at a high level).

Second, vision analytics applications have much more highly uneven distributions of attention to data, both spatially and temporally, than human viewers. 
In many video codec today, spatially and temporally uneven encoding is functionally supported (on which \name is built) but not optimized. 
Interestingly, this trend may revive some old multimedia ideas, such as region of interest encoding and scalable video coding. 

Third, no application will achieve optimal performance without coping with the service it runs on top of. 
Video analytics applications are no exception. 
In developing \name, we found that many vision DNNs today are sometimes highly sensitive to minor pixel changes caused by codec, especially when detecting small objects. 
We envision that making vision DNNs encoding-invariant will significantly improve the effectiveness of the underlying video stack.


==> eval-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Evaluation}
\label{sec:eval}

\begin{table}
 \begin{tabular}{cccc} 
 \hline
 Name & Vision task & \# videos & \# frames \\ [0.5ex]
 \hline
 Drone & obj detect \& segment & 5 & 6213 \\ 
 \hline
 Dashcam & obj detect & 7 & 12600 \\
 \hline
 Surfing & kpt detect & 6 & 10800 \\
 \hline
 Dancing & kpt detect & 6 & 10800 \\
 \hline
\end{tabular}
 \caption{}
 \label{tab:dataset}
\end{table}


Finally, we evaluate \name along its key performance metrics:
\begin{packeditemize}
\item \name achieves better accuracy-compression tradeoffs: \fillme-\fillme\% higher accuracy at the same compression rate, or \fillme-\fillme\% lower storage cost while maintaining at least as high accuracy as the baselines.
\item \name's encoding on a single CPU is merely \fillme\% slower than H.264 and \fillme\% slower than VP8, with negligible additional delay in decoding. Compared to recent solutions, like DDS and CloudSeg, \name encoding is \fillme$\times$ faster. 
\item \name improves performance across three vision tasks and various DNNs of the same task, and achieves these improvement using the same \ag-based workflow, in which customizing the \Ag model for a given DNN takes only \fillme minutes.
\item \name offers the developers the flexibility to set file size (bandwidth usage) target while maximizing accuracy (via the high-quality area threshold $\AreaThresh$), and to prioritize accuracy stability while reduce file size (bandwidth usage) while necessary (via the \ag threshold $\AgThresh$).
\end{packeditemize}


\kt{Add a table to discuss dataset}
\kt{Autoencoder: delay, I-frame size \& accuracy}

%\mypara{Takeaway}
%Here are the takeaways from our experiments:
%\begin{itemize}
%\item in injection time, \name achieves \fillme\% less compressed video sizes than today's video codec with similar encoding delay on cpus.
%\item in consumption time, \name speeds up the inference by \fillme$\times$ than today's video codec, while achieving similar accuracy.
%\item in video streaming, \name achieves similar accuracy with \fillme\% less bandwidth and \fillme\% less inference delay.
%\end{itemize}

\subsection{Setup}
\label{subsec:eval:setup}

\mypara{Emulator}
We build an emulator to test the three phases of \name. 
In the ingestion phase, we create a video source from which \name (and the baselines) can read raw frame (\fillme$\times$\fillme) one by one. 
For fair comparison, the encoding process runs on one \fillme CPU. In particular, \name also runs the accuracy-gradient model on CPU, rather than GPU\footnote{We note that this is not the assumption behind some solutions, such as DDS and CloudSeg, and will (albeit not unfairly) show a high ingestion delay (of DDS) or consumption delay (of CloudSeg).
That said, when the video sensors do have GPU capability~\cite{??}, the delay numbers of \name will be much lower too.}.
In the consumption phase, we run the decoding on the same CPU as the ingestion phase, but to make it more realistic, the inference will be on a \fillme GPU. 
Finally, in the preparation phase, we train the accuracy-gradient model on a \fillme GPU. 


\mypara{Video analytics tasks}
We test \name on three tasks (with the default full DNN in parenthesis): object detection (FasterRCNN-ResNet50-FPN), person keypoint detection (KeypointRCNN-ResNet50-FPN), and semantic segmentation (FCN-ResNet50).
These models are retrived from torchvision model zoo~\cite{??} on \jc{which date?}.

\mypara{Setting of \name and baselines}
As mentioned in \S\ref{subsec:ag}, \name exposes two parameters and by default, we use \jc{setting of $\alpha,\beta$}.
By default, its accuracy-gradient model is trained on the same training data in COCO~\cite{??} of the full DNNs.
We compare \name with existing solutions in five categories:
\begin{packeditemize}
\item {\em Uniform quality:} The basic idea behind AWStream~\cite{awstream} and VStore~\cite{vstore} is to tune encoding parameters of the underlying codec (resolution, QP, and frame rate), though unlike \name, they use the same configuration for all frames in each time window. 
To show their fundamental limitation, we use an ``idealized'' implementation where the parameters are set such that the size reduction is maximized while its accuracy is almost same to \name.
\item {\em Spatially different quality:} DDS~\cite{dds} and EAAR~\cite{eaar} belong to this type and they share the idea of encoding different regions with different quality levels. By default, we use QP = \fillme and QP = \fillme as the low quality and high quality settings. 
\item {\em Super resolution:} We use CloudSeg~\cite{??} as an example, which simply compresses the frames in low quality (\fillme) in ingestion and use super resolution to increase its quality using a super resolution model (\fillme in this case) in consumption.
\item {\em Frame selection:} We choose Reducto~\cite{??} one of the most recent proposals along this line. We use the implementation from~\cite{??} and \jc{any other changes?}
\item Autocodec: We pick a pre-trained autocodec~\cite{??} based on \fillme architecture, which is commonly used in \fillme.
\end{packeditemize}
\jc{why these baselines?}

\jc{AUTOENCODERS ARE STILL MISSING}

\mypara{Metrics}
We compare different techniques along three key metrics: {\em size reduction}, {\em inference accuracy}, {\em ingestion delay} and {\em consumption delay}, which follows the same definition as in \S\ref{sec:back}.
In particular, the inference accuracy is calculated by comparing the full DNN output on the encoded frame and the output on the frame encoded at QP = \fillme. 

\mypara{Test videos}
We use dashcam videos~\cite{dds} and drone videos~\cite{aiskyeye} to evaluate object detection and segmentation.
\jc{explain}


\subsection{End-to-end improvement}


\begin{figure*}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    \subfloat[Object detection (Dashcam)]
    {
        \includegraphics[width=0.2\textwidth]{figs/detection_dashcam_FPN.pdf}
        \label{subfig:1}
    }
    \subfloat[Object detection (Drone)]
    {
        \includegraphics[width=0.2\textwidth]{figs/detection_drone_FPN.pdf}
        \label{subfig:2}
    }
    \subfloat[Sem. segmentation (Drone)]
    {
        \includegraphics[width=0.2\textwidth]{figs/segmentation_vis.pdf}
        \label{subfig:1}
    }
    % \subfloat[Sem. segmentation (Dashcam)]
    % {
    %     \includegraphics[width=0.22\textwidth]{figs/placeholder-eval-overall-2.pdf}
    %     \label{subfig:2}
    % }
    \subfloat[Keypoint detection (Surfing)]
    {
        \includegraphics[width=0.2\textwidth]{figs/kpt_surfing.pdf}
        \label{subfig:1}
    }
    \subfloat[Keypoint detection (Dancing)]
    {
        \includegraphics[width=0.2\textwidth]{figs/kpt_dancing.pdf}
        \label{subfig:1}
    }
    % \subfloat[Keypoint detection (Skate)]
    % {
    %     \includegraphics[width=0.22\textwidth]{figs/placeholder-eval-overall-2.pdf}
    %     \label{subfig:2}
    % }
    \caption{}
    \label{fig:eval-overall}
\end{figure*}
\mypara{Performance by task}

\jc{WHY DDS IS WORSE THAN MPEG? RPN-BBOXES ARE NOT LARGE ENOUGH TO DETECT THE OBJ EVEN IN HIGH QUALITY}


Figure~\ref{fig:eval-overall} shows the performance distribution of \name compared with various baselines on three tasks (on their default full DNN), each with two datasets.
We can see that \name outperforms the baselines: 
in compression efficiency, its encoded video is \fillme$\times$ smaller than the best baseline (\fillme) that achieve a comparable accuracy; 
in accuracy, \name is \fillme\% more accurate when compared with the the baselines (\fillme and \fillme) with similar size reduction.




\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-delay-overall.pdf}
    \includegraphics[width=0.45\columnwidth]{figs/delay.pdf}
    \includegraphics[width=0.45\columnwidth]{figs/delay2.pdf}
    \caption{}
    \label{fig:eval-delay-overall}
\end{figure}
\mypara{Delay comparison}
Figure~\ref{fig:eval-delay-overall} compares the ingestion delay and consumption delay of \name with those of the baselines. 
We can see that in both fronts, \name achieves the second lowest delay, and it is marginally slower than the simple video codec (H.264) in ingestion delay. 
Though frame selection's consumption delay is much lower than others, the same optimization (running inference on a selected set of frames) could be used in \name as well. 



\begin{figure}
    \centering
    \includegraphics[width=0.65\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    \subfloat[FasterRCNN-DC5]
    {
        \includegraphics[width=0.16\textwidth]{figs/detection_dashcam_DC5.pdf}
        \label{subfig:1}
    }
    \subfloat[FasterRCNN-FPN]
    {
        \includegraphics[width=0.16\textwidth]{figs/detection_dashcam_FPN.pdf}
        \label{subfig:2}
    }
    \subfloat[FasterRCNN-C4]
    {
        \includegraphics[width=0.16\textwidth]{figs/detection_dashcam_C4.pdf}
        \label{subfig:1}
    }
    \caption{}
    \label{fig:eval-by-model}
\end{figure}
\mypara{Performance by model}
Figure~\ref{fig:eval-by-model} shows the performance distribution of \name compared with those of various baselines when serving three object detection models. 
In running this experiment, we retrain the \name's accuracy-gradient model with the same training data as the full DNN.
The result are qualitatively similar: 
Across different full DNNs, \name achieves \fillme-\fillme\% more file size savings than the best baseline that reaches similar accuracy.


\mypara{Intuitive interpretation}


\subsection{Microbenchmarking}
\label{subsec:eval:micro}

So far we have seen that \name's end-to-end implementation outperforms the baselines. 
Next, we evaluate several key design choices. 
Throughout this section, we use \fillme as the full DNN and \fillme as the videos.


\jc{NEED TO EVALUATE THE TRAINING TIME}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\columnwidth]{figs/placeholder-eval-loss-function.pdf}
%     \caption{On dashcam videos}
%     \label{fig:eval-loss-function}
% \end{figure}
\mypara{Choice of loss function}
One important aspect in the training of accuracy-gradient model is the loss function in Eq (\ref{eq:loss-function}). 
Figure~\ref{fig:eval-loss-function} compares it with the seemingly natural baseline choices: calculating the cross entropy or the mean square error between $\AccuracyGradientModel(\HighImage)$ and $\AccuracyGradient(\LowImage)$.
As we mentioned in \S\ref{subsec:??}, these baselines perform poorly because they will be biased by the unbalanced value distribution in $\AccuracyGradient(\LowImage)$ and the resulting model tends to produce very small accuracy saliency value everywhere. 
In contrast, \name's loss function explicitly learns the high values at is robust to the value imbalance and produce more useful accuracy gradient predictions.

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/placeholder-eval-delay-breakdown.pdf}
    \includegraphics[width=0.7\columnwidth]{figs/encoding_delay.pdf}
    \caption{}
    \label{fig:eval-delay-breakdown}
\end{figure}
\mypara{Encoding delay reduction}
\name uses two techniques to speed up the accuracy gradient-based encoding. 
Figure~\ref{fig:eval-delay-breakdown} shows the incremental reduction of encoding delay by each of them. 
In each design point, the figure breakdowns the encoding delay of \name into accuracy gradient prediction and the actual encoding, and as a reference point, it also shows the encoding delay of H.264 and DDS.
To begin with, as \name uses a shallow architecture for its accuracy gradient model, the delay of accuracy gradient prediction is much smaller than prior work such as DDS that needs to actually run the final DNN. 
That said, it is sizable compared to the encoding delay.
To further reduce this delay, we sample 1 out of 30 frames, which drastically reduces the amortized delay per frame. 
As a second optimization, \name also uses the uniform color to replace the low quality encoding, which further halve the encoding delay. 
Overall, the delay is small enough to support encoding 30fps with \fillme CPUs.


\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-low-quality.pdf}
    \includegraphics[width=0.5\columnwidth]{figs/detection_qp.pdf}
    \caption{}
    \label{fig:eval-low-quality}
\end{figure}
\mypara{Effectiveness of low quality encoding}
In addition to reducing encoding delay, Figure~\ref{fig:eval-low-quality} shows another benefit of using uniform coloring as the low quality encoding. 
As illustrated in Figure~\ref{fig:uniform-color}, uniform coloring actually improves the accuracy/compression tradeoff. 
\jc{reading of the graph}


%\subsection{Sensitivity analysis}
%Lastly, we evaluate \name's sensitivity to the training data and the underlying video codec.

\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-training-data.pdf}
    \includegraphics[width=0.5\columnwidth]{figs/detection_drone_FPN_trainingset.pdf}
    % \includegraphics[width=0.4\columnwidth]{figs/detection_dashcam_FPN_trainingset.pdf}
    \caption{\name can achieve better performance with the knowledge of video content.}
    \label{fig:eval-training-data}
\end{figure}
\mypara{Training data}
Figure~\ref{fig:eval-training-data} compares \name's performance under two choices of training data: the dataset on which the final DNN is trained and a sampled \fillme-second of video from the test video.
We can see that \jc{reading of the graph}


\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figs/placeholder-eval-codec.pdf}
    
    \subfloat[H.264]
    {
        \includegraphics[width=0.3\columnwidth]{figs/detection_drone_FPN_mp4.pdf}
        \label{subfig:1}
    }
    \subfloat[H.265]
    {
        \includegraphics[width=0.3\columnwidth]{figs/detection_drone_FPN_hevc.pdf}
        \label{subfig:1}
    }
    \subfloat[VP9]
    {
        \includegraphics[width=0.3\columnwidth]{figs/detection_drone_FPN_webm.pdf}
        \label{subfig:1}
    }
    \caption{}
    \label{fig:eval-codec}
\end{figure}
\mypara{Underlying codec}
Lastly, Figure~\ref{fig:eval-codec} tests \name under different traditional codecs.
We can see that the \name shows consistent improvement on accuracy 




\subsection{\hspace{-0.2cm}Supporting adaptive streaming \kt{Rename to accuracy control and bitrate control?}}
\label{subsec:eval:adaptive}

So far, we have evaluated \name with its parameters fixed at the default values. 
As a usable video codec, \name also allows the user to set its parameters to \kt{control the accuracy and bitrate.} navigate the accuracy/compression tradeoff (as explained in \S\ref{subsec:assignment}). 
To demonstrate it, we imagine a video sensor encodes and streams the video over a bandwidth-constrained connection to a remote server for DNN analytics.
In this context, we test how well \name supports two typical policies of adaptive streaming. 

\begin{figure}
    \centering
    % \includegraphics[width=0.65\columnwidth]{figs/placeholder-eval-video-adaptation.pdf}
    \includegraphics[width=0.65\columnwidth]{figs/const_heat_bw.pdf}
    \includegraphics[width=0.65\columnwidth]{figs/const_heat_acc.pdf}
    \caption{}
    \label{fig:eval-video-adaptation}
\end{figure}
\mypara{Reducing bandwidth usage without hurting accuracy \kt{Rename this to accuracy control?}}
In the first policy, the user wants to use less bandwidth usage without hurting accuracy.
This is a good use case of setting the accuracy-gradient threshold $\AgThresh$, which allows the user to take advantages of content variation: when content is simple or contains less useful information, naturally less blocks will have high accuracy gradients, thus bandwidth usage can be lowered without affecting accuracy.
Figure~\ref{fig:eval-video-adaptation} confirms this intuition.
On this traffic video, the street is empty between \fillme and \fillme, which is implicitly leveraged by \name to reduce bandwidth usage without the user changing its parameters. 
In contrast, traditional video codecs are not aware with such bandwidth-saving opportunity, though it does has lower bandwidth usage since the video becomes easier to encode.



\begin{figure}
    \centering
    % \includegraphics[width=0.65\columnwidth]{figs/placeholder-eval-bw-adaptation.pdf}
    \includegraphics[width=0.65\columnwidth]{figs/bw_adapt_bw.pdf}
    \includegraphics[width=0.65\columnwidth]{figs/bw_adapt_acc.pdf}
    \caption{}
    \label{fig:eval-bw-adaptation}
\end{figure}
\mypara{Higher accuracy under limited bandwidth \kt{Rename this to bitrate control?}}
In the second policy, the user wants to achieve high accuracy under limited dynamic bandwidth. 
This is a good use case of setting the high-quality area threshold $\AreaThresh$, which allows user to maintain a roughly similar bandwidth usage. 
We use an offline profiling process to first create a mapping from the $\AreaThresh$ to bandwidth usage. 
Based on this profile, we then assume the user uses a typical adaptive-bitrate (ABR) logic: predicts available bandwidth using an exponential weighted moving average (over 5 seconds) and sets $\AreaThresh$ such that the expected video bitrate is slightly lower than the available bandwidth.
% The chunk length is \fillme seconds (the gap between two I-frames).
%To achieve that, ABR uses an offline profiled mapping from $\AreaThresh$
Figure~\ref{fig:eval-bw-adaptation} compares the performance of this ABR logic (in bandwidth usage and the resulting inference accuracy) when running on \name and H.264. 
The available bandwidth begins with \fillme and suddenly drops at time \fillme, and it stays there until it bounces back to \fillme at \fillme. 
We can see that while both H.264 and \name allows the ABR logic to cope with the bandwidth fluctuation, \name can maintain at a higher accuracy.



%\jc{we don't mean to eval abr logic}


%\mypara{Effect of different parameters}


%\newpage


%\kt{
%\begin{itemize}
%\item dataset
%\item setting of tasks (dnns) and codec
%\item evaluation metrics
%\item baselines: dds, neural autocodec, sr, focus, vstore
%\end{itemize}}

%\mypara{Vision task}


%\mypara{Object detection and segmentation dataset}


\begin{comment}

\mypara{Person keypoint detection dataset}
\kt{Wait after Qizheng finishes it.}

\jc{predictability experiment}

\subsection{Overall improvement}

\begin{figure}
    \centering
    \subfloat[Object detection (Highway)]
    {
        \includegraphics[width=0.22\textwidth]{figs/detection_dashcam.pdf}
        \label{subfig:1}
    }
    \subfloat[Object detection (Drone)]
    {
        \includegraphics[width=0.22\textwidth]{figs/detection_vis.pdf}
        \label{subfig:2}
    }
    
    \subfloat[Sem. segmentation (Drone)]
    {
        \includegraphics[width=0.22\textwidth]{figs/segmentation_vis.pdf}
        \label{subfig:1}
    }
    \subfloat[Sem. segmentation (Dashcam)]
    {
        \includegraphics[width=0.22\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    
    \subfloat[Keypoint detection (Kite)]
    {
        \includegraphics[width=0.22\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    \subfloat[Keypoint detection (Skate)]
    {
        \includegraphics[width=0.22\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    
    \caption{Overall filesize-accuracy tradeoff of \name and various baselines on different applications. \name saves \fillme\% filesize without hurting accuracy.}
    \label{fig:filesize-acc}

\end{figure}

\mypara{Improvement in compression efficiency} 
Figure \ref{fig:filesize-acc} demonstrates that \name consistently reduces file size by \fillme\% without hurting inference accuracy than various baselines.

\mypara{Improvement in consumption time} 
inference delay vs. accuracy

\mypara{Improvement in online analytics on streaming videos} 
\kt{are we really doing this?}

\mypara{Improvement over multiple tasks}
Improvement vs. \# of tasks

\subsection{Improvement breakdown}
how much does each technique contributing to the overall improvement

\jc{
\begin{itemize}
\item effectiveness of delay reduction (frame sampling, uniform coloring vs. low quality)
\item bandwidht adaptation
\item impact of training data
\end{itemize}}


\subsection{Microbenchmarking}


\begin{figure}
    \centering
    \subfloat[H.264]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    \subfloat[H.265]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    \subfloat[VP8]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    
    \caption{Performance of \name under different codec. The gain of \name is stable under various codec.}
    \label{fig:codec-insensitive}

\end{figure}

\begin{figure}
    \centering
    \subfloat[FasterRCNN]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    \subfloat[EfficientDet]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    \subfloat[Trasformer]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    
    \caption{Performance of \name under different genre of DNN. The gain of \name remains substantial.}
    \label{fig:dnn-insensitive}

\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/encoding-delay.pdf}
    \caption{Encoding delay between \name and H.264. \name achieves lower encoding delay without compromising accuracy.}
    \label{fig:encoding-delay}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/encoding-delay-with-gpu.pdf}
    \caption{Encoding delay of \name can be drastically decreased if equipped with low-end GPU.}
    \label{fig:encoding-delay-with-gpu}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/processing-delay.pdf}
    \caption{Processing delay per frame between \name and H.264 under various consumption demand. \name achieves lower processing delay per frame under various consumption demand.}
    \label{fig:processing-delay}
\end{figure}


\mypara{Underlying codec}
As Figure \ref{fig:codec-insensitive} demonstrates, the gain of \name is stable under various codec.

\mypara{Underlying dnn}
As Figure \ref{fig:dnn-insensitive} demonstrates, the gain of \name is substantial under various genre of DNN.

\mypara{Encoding delay}
As Figure \ref{fig:encoding-delay} demonstrates, \name achieves lower encoding delay without compromising accuracy.

\mypara{Consumption demand}
As Figure \ref{fig:processing-delay} shows, \name achieves consistently lower processing delay under various consumption demand.

\mypara{Assist with low-end GPU}
As Figure \ref{fig:encoding-delay-with-gpu} shows, the encoding delay of \name can be drastically decreased if equipped with even low-end GPU.


\end{comment}




==> eval-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    \subfloat[\centering{Object detection\\~~~~(Dashcam)}]
    {
        \includegraphics[width=0.19\textwidth]{figs/detection_dashcam_FPN.pdf}
        \label{subfig:1}
    }
    \subfloat[\centering{Object detection\\~~~~(Drone)}]
    {
        \includegraphics[width=0.19\textwidth]{figs/detection_drone_FPN.pdf}
        \label{subfig:2}
    }
    \subfloat[\centering{Semantic segmentation\\~~~~(Drone)}]
    {
        \includegraphics[width=0.19\textwidth]{figs/segmentation_vis.pdf}
        \label{subfig:1}
    }
    % \subfloat[Sem. segmentation (Dashcam)]
    % {
    %     \includegraphics[width=0.22\textwidth]{figs/placeholder-eval-overall-2.pdf}
    %     \label{subfig:2}
    % }
    \subfloat[\centering{Keypoint detection\\~~~~(Surfing)}]
    {
        \includegraphics[width=0.19\textwidth]{figs/kpt_surfing.pdf}
        \label{subfig:1}
    }
    \subfloat[\centering{Keypoint detection\\~~~~(Dancing)}]
    {
        \includegraphics[width=0.19\textwidth]{figs/kpt_dancing.pdf}
        \label{subfig:1}
    }
    % \subfloat[Keypoint detection (Skate)]
    % {
    %     \includegraphics[width=0.22\textwidth]{figs/placeholder-eval-overall-2.pdf}
    %     \label{subfig:2}
    % }
    \tightcaption{The normalized file size v.s. inference accuracy of \name and several baselines on various video genres and applications.
\name achieves high accuracy with 30-50\% file size reduction on object detection and 40\% on semantic segmentation, and 12-33\% on keypoint detection.
Ellipses show the 1-$\sigma$ range of results.}
    \label{fig:eval-overall}
\end{figure*}

\section{Evaluation}
\label{sec:eval}



Finally, we evaluate \name along its key performance metrics:
\begin{packeditemize}
\item \name achieves better accuracy compression tradeoffs: 1-5\% higher accuracy at the same compression rate, or 10-50\% lower storage cost or network usage, while maintaining at least as high accuracy as the baselines.
\item \name's encoding on a single CPU is 6x faster than VP9 (though 3.5x slower than H.264), with negligible additional delay in decoding. Compared to recent solutions, like DDS and CloudSeg, \name encoding is 50$\times$ faster. 
\item \name improves performance across three vision tasks and various DNNs of the same task, and achieves these improvements using the same \ag-based workflow; and customizing the \Ag model for a given DNN can take only 12 minutes.
\item \name offers developers the flexibility to maintain file size (bandwidth usage) at a target level while maximizing accuracy (via the high-quality area threshold $\AreaThresh$), and to prioritize accuracy stability while reduce file size (bandwidth usage) when necessary (via the \ag threshold $\AgThresh$).
\end{packeditemize}


% \kt{Add a table to discuss dataset}
% \kt{Autoencoder: delay, I-frame size \& accuracy}

%\mypara{Takeaway}
%Here are the takeaways from our experiments:
%\begin{itemize}
%\item in injection time, \name achieves \fillme\% less compressed video sizes than today's video codec with similar encoding delay on cpus.
%\item in consumption time, \name speeds up the inference by \fillme$\times$ than today's video codec, while achieving similar accuracy.
%\item in video streaming, \name achieves similar accuracy with \fillme\% less bandwidth and \fillme\% less inference delay.
%\end{itemize}



\subsection{Setup}
\label{subsec:eval:setup}


\begin{table}
{\small
\begin{tabular}{c>{\centering\arraybackslash}m{3.1cm}cc} 
\hline
Name & Vision task & \# Videos & \# Frames \\ [0.5ex]
\hline
\textsf{Drone} & object detection, semantic segmentation & 5 & 6213 \\ 
\hline
\textsf{Dashcam} & object detection & 7 & 12600 \\
\hline
\textsf{Surfing} & keypoint detection & 6 & 6598 \\
\hline
\textsf{Dance} & keypoint detection & 6 & 8711 \\
\hline
\end{tabular}
\caption{Summary of our datasets.
\vspace{-0.3cm}
}
\label{tab:dataset}
}
\end{table}


\mypara{Dataset} 
Table \ref{tab:dataset} summarizes the 4 video datasets we used to evaluate \name: 5 drone videos for object detection and semantic segmentation, 7 dashcam videos for object detection, 6 surfing videos for keypoint detection and 6 dancing videos for keypoint detection. Drone videos are sampled from VisDrone dataset \cite{aiskyeye} and other videos are obtained by searching on YouTube. We search keywords (such as ``highway dashcam hd'') in incognito mode to avoid bias induced by our personal preferences.
\jc{kuntai, please give a very brief description of each dataset and why we use them}
All used videos and collection details are available in this anonymous link~\cite{dataset-link}.

\mypara{Emulator}
We build an emulator to test each component of \name. 
In the encoding phase, we create a video source from which \name (and the baselines) can read raw frames (1280$\times$720) one by one. 
To fairly compare the encoding delay of different methods, the encoding runs on one Intel Xeon Silver 4100 CPU. 
In particular, \name also runs the accuracy-gradient model on CPU, rather than GPU\footnote{We note that this is not the assumption behind some solutions, such as DDS and CloudSeg, and will (albeit not unfairly) show a high ingestion delay (of DDS) or consumption delay (of CloudSeg).
That said, \name can be much faster when the video sensors have GPU capability~\cite{jetson}.}.
In the decoding and inference phase, we run the decoding on the same CPU, but to make it more realistic, the inference will be done on a GeForce RTX 2080 SUPER GPU. 
Finally, the preparation phase trains the \ag model on the same GPU. 


\mypara{Video analytics tasks}
We test \name on three tasks (parenthesis show the default full DNNs): object detection (FasterRCNN-FPN~\cite{ren2015faster}), person keypoint detection (KeypointRCNN-FPN~\cite{maskrcnn}), and semantic segmentation (FCN-ResNet50~\cite{long2015fully}).
We also test \name on multiple object detection models in \S\ref{subsec:eval:e2e}.

\mypara{Setting of \name and baselines}
\name introduces two parameters (\S\ref{subsec:ag}) and by default, we use $\alpha=0.5$ for object detection and semantic segmentation.
By default, its accuracy-gradient model is trained on the same training data in COCO~\cite{lin2014microsoft} of the respective full DNNs.
We compare \name with existing solutions in five categories:
\begin{packeditemize}
\item {\em Uniform quality:} The basic idea behind AWStream~\cite{awstream} is to tune encoding parameters of the underlying codec (resolution, QP, and frame rate), though unlike \name, they use the same configuration for all frames in each time window (on the timescale of minutes). (VStore~\cite{vstore} shaeres a similar idea.)
To show their limitation, we use an ``idealized'' version where the parameters are set such that the size reduction is maximized while its accuracy is almost same to \name.
\item {\em Spatially different quality:} DDS~\cite{dds} and EAAR~\cite{eaar} belong to this type and they share the idea of encoding different regions with different quality levels. By default, we use QP = (40, 30) ((34, 24) in keypoint detection) as the low quality and high quality settings. 
\item {\em Super resolution:} We use CloudSeg~\cite{cloudseg} as an example, which simply compresses the frames in low quality (640$\times$360) in ingestion and use super resolution to increase its quality using a super resolution model (\cite{carn-pytorch} in this case) in consumption.
\item {\em Frame selection:} We choose Reducto~\cite{reducto} one of the most recent proposals along this line. We use the implementation from~\cite{reducto-codebase}.
\item {\em Autoencoder}: We pick a pre-trained autoencoder~\cite{cae-codebase} (introduced in~\cite{cae}) mainly to compare its encoding delay with \name. 
\end{packeditemize}
% \jc{why these baselines?}
% \jc{AUTOENCODERS ARE STILL MISSING}

\mypara{Metrics}
Follows the definitions in \S\ref{sec:back}, we compare different techniques along four key metrics: {\em file size}, {\em inference accuracy}, and {\em encoding/decoding delays}.
In particular, the inference accuracy is calculated by comparing the full DNN's output on the encoded frame and its output on the frame encoded at highest quality\footnote{We use QP = 24 in keypoint detection (since keypoint detection DNNs needs high quality to locate the exact position of the keypoints) and QP = 30 for object detection and semantic segmentation.}. We use F1 score for the accuracy metric in object detection, IoU for semantic segmentation and distance-based accuracy  for keypoint detection. These metrics all values in [0,1], the higher the better.
Also, we normalize the file size against the file size derived from ground truth quality to enable fair comparison between different video types and lengths.

% \mypara{Test videos}
% We use dashcam videos~\cite{dds} and drone videos~\cite{aiskyeye} to evaluate object detection and segmentation.
% \jc{explain}


\subsection{End-to-end improvement}
\label{subsec:eval:e2e}


\mypara{Performance by task}
% \jc{WHY DDS IS WORSE THAN MPEG? RPN-BBOXES ARE NOT LARGE ENOUGH TO DETECT THE OBJ EVEN IN HIGH QUALITY}
Figure~\ref{fig:eval-overall} shows the performance distribution of \name compared with various baselines on the three tasks (on their perspective default full DNNs) and various datasets.
We can see that \name outperforms the baselines: 
in terms of compression efficiency, the encoded videos are 2$\times$ smaller than the best baseline (AWStream) that achieve a comparable accuracy; 
in terms of accuracy, \name is 4\% more accurate when compared to the AWStream baseline with lower size reduction.

Here, we highlight a particular contrast between \name and DDS, which is one of the state-of-the-art techniques that share the idea of assigning spatially different quality. 
As elaborated in \S\ref{subsec:analysis}, even though DDS encodes RPN-proposed regions in high quality, these regions tend to include few surrounding pixels of small objects which provides too few context for them to be detected. 
In contrast, \name can detect more objects as \ags naturally set some surrounding blocks in high quality.

We also compare \name to autoencoder for object detection on drone videos. Accuracy-wise, \name achieves 78\% accuracy but autoencoder only achieves 62\% accuracy. Moreover, \name encodes ~2.6KB per frame but autoencoder encodes 240KB~\cite{cae-codebase} per frame. Thus, we say \name has much better accuracy compression tradeoff.

% We also compare



\begin{figure}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-delay-overall.pdf}
    % \includegraphics[width=0.45\columnwidth]{figs/delay.pdf}
    % \includegraphics[width=0.45\columnwidth]{figs/delay2.pdf}
    \includegraphics[width=0.85\columnwidth]{figs/delays.pdf}
    \tightcaption{Although requiring performing inference on CPU, \name reduces the encoding delay/decoding delay by >50x compared to other inference-based baselines and achieves comparable delay compared to H.264 encoding.}
    \label{fig:eval-delay-overall}
\end{figure}
\mypara{Delay comparison}
Figure~\ref{fig:eval-delay-overall} compares the encoding and decoding delays of \name with those of the baselines. 
We can see that on both fronts, \name's delays are higher than those of a simple video codec (H.264) but with an almost negligible margin, compared to other baselines (EAAR, DDS) that also adapt quality per frame or per region. This is because \name encoding involves only a cheap DNN once every 30 frames. 
% Compared to other spatially quality differentiation approaches like EAAR and DDS, \name has more than 50$\times$ lower encoding delay reduction since we inference on a cheaper DNN less frequently.
Compared to CloudSeg and autoencoder, \name saves two orders of magnitude of decoding delay, since \name involves no DNN inference in the decoding phase, while CloudSeg and autoencoder all require DNN inference to decode each frame.
Though frame-selection approaches like Reducto have much lower encoding and deocoding delay, the same optimization (running inference on a subset of frames) can be used in \name as well. 




\begin{figure}
    \centering
    % \includegraphics[width=0.65\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    \subfloat[FasterRCNN-DC5]
    {
        \includegraphics[width=0.16\textwidth]{figs/detection_dashcam_DC5.pdf}
        \label{subfig:1}
    }
    \subfloat[FasterRCNN-FPN]
    {
        \includegraphics[width=0.16\textwidth]{figs/detection_dashcam_FPN.pdf}
        \label{subfig:2}
    }
    \subfloat[FasterRCNN-C4]
    {
        \includegraphics[width=0.16\textwidth]{figs/detection_dashcam_C4.pdf}
        \label{subfig:1}
    }
    \tightcaption{Performance of \name and several baselines on different vision applications and datasets. \name achieves better accuracy-compression tradeoffs.}
    \label{fig:eval-by-model}
\end{figure}
\mypara{Performance by model}
Figure~\ref{fig:eval-by-model} shows the performance distribution of \name (vs. baselines) when serving different object detection DNNs. 
% compared with those of various baselines when serving three object detection models. 
We pick these DNNs to represent different architectures:
% Specifically, we use different but representative architectures: 
feature pyramid network (FasterRCNN-FPN~\cite{lin2017feature}), pure convolutions (FasterRCNN-C4~\cite{ren2015faster}) and dilated convolutions (FasterRCNN-DC5~\cite{xu2017deformable}).
In running this experiment, we retrain the \name's accuracy-gradient model with the same training data as the full DNN.
The results are qualitatively similar: 
Across different full DNNs, \name achieves 25-40\% more file size savings than the best baseline that reaches similar accuracy (H.264).


% \mypara{Intuitive interpretation}
% \kt{About what...}


\subsection{Microbenchmarking}
\label{subsec:eval:micro}

So far we have seen that \name's end-to-end implementation outperforms the baselines. 
Next, we evaluate several key design choices. 
Throughout this section, we use the object detector of FasterRCNN-FPN as the full DNN and drone as the test videos.


%\jc{NEED TO EVALUATE THE TRAINING TIME}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\columnwidth]{figs/placeholder-eval-loss-function.pdf}
%     \caption{On dashcam videos}
%     \label{fig:eval-loss-function}
% \end{figure}
% \mypara{Choice of loss function}
% One important aspect in the training of accuracy-gradient model is the loss function in Eq (\ref{eq:loss-function}). 
% Figure~\ref{fig:eval-loss-function} compares it with the seemingly natural baseline choices: calculating the cross entropy or the mean square error between $\AccuracyGradientModel(\HighImage)$ and $\AccuracyGradient(\LowImage)$.
% As we mentioned in \S\ref{subsec:??}, these baselines perform poorly because they will be biased by the unbalanced value distribution in $\AccuracyGradient(\LowImage)$ and the resulting model tends to produce very small accuracy saliency value everywhere. 
% In contrast, \name's loss function explicitly learns the high values at is robust to the value imbalance and produce more useful accuracy gradient predictions.

\begin{figure}
    \centering
    % \includegraphics[width=0.7\columnwidth]{figs/placeholder-eval-delay-breakdown.pdf}
    \includegraphics[width=0.7\columnwidth]{figs/encoding_delay.pdf}
    \tightcaption{Breakdown of \name encoding delay shows that the additional delay of running the \ag model is marginal (more so after the frame sampling optimization), compared to other baselines (DDS and CloudSeg).
    \kt{Add a new figure on AccMPEG v.s. cheap object detector and segmentation. Resize the image to the same shape.}
    \jc{maybe add H.265 as a reference?}
    }
    \label{fig:eval-delay-breakdown}
\end{figure}
\mypara{Encoding delay reduction}
\name uses two techniques to speed up the accuracy-gradient-based encoding: 
(1) using a uniform color to encode the less important blocks to avoid two-pass encoding, and 
(2) running the \ag model only on sampled frames. 
Figure~\ref{fig:eval-delay-breakdown} shows their incremental reductions on encoding delay. 
The figure breaks down the encoding delay of \name into accuracy gradient prediction and the actual codec encoding, and as a reference point, it also shows the encoding delay of H.264, VP9, DDS and CloudSeg.
As \name uses the \ag model (a shallow DNN) for its accuracy gradient model, the delay of accuracy gradient prediction is much smaller than prior work such as DDS which needs to actually run the final DNN. 
That said, it is sizable compared with the encoding delay, even after saving one encoding pass by using a uniform color.
To reduce this delay, we run \ag model on 1 out of 30 frames, which drastically reduces the amortized delay per frame: \name can support encoding 30fps with 3 CPUs.
% As a second optimization, \name also uses the uniform color to replace the low quality encoding, which further halve the encoding delay. 
% Overall, the delay is small enough to support encoding 30fps with 3 CPUs.


\begin{figure}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-low-quality.pdf}
    \includegraphics[width=0.4\columnwidth]{figs/detection_qp.pdf}
    \tightcaption{Effectiveness of using the uniform color (mean pixel values) as low quality encoding, which avoids spurious results arising from low quality encoding and reduces the encoding size, while preserving enough information in the high-quality blocks to maintain high accuracy.}
    \label{fig:eval-low-quality}
\end{figure}
\mypara{Effectiveness of low quality encoding}
% In addition to reducing encoding delay, 
Next, we show the benefit of using a uniform color to encode the less important blocks in terms of accuracy and compression efficiency.
% benefit of using uniform coloring as the low quality encoding. 
Figure~\ref{fig:eval-low-quality} corroborates the intuition illustrated in Figure~\ref{fig:uniform-color}---using a uniform coloring might improves the accuracy and/or compression tradeoff: when when encode all non-high quality regions with some QP values, it may significantly increase the file size (\eg QP=32 in this example) or the final DNN sometimes is confused and return spurious detections, which hurts accuracy (\eg QP=38 in this example).
% \jc{reading of the graph}
% \kt{not sure what the message should be here...}


%\subsection{Sensitivity analysis}
%Lastly, we evaluate \name's sensitivity to the training data and the underlying video codec.

\begin{figure}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-training-data.pdf}
    \includegraphics[width=0.4\columnwidth]{figs/detection_drone_FPN_trainingset.pdf}
    % \includegraphics[width=0.4\columnwidth]{figs/detection_dashcam_FPN_trainingset.pdf}
    \tightcaption{
%    \name can achieve better performance with the knowledge of video content.
     \name improves performance under both choices of training data. 
    }
    \label{fig:eval-training-data}
\end{figure}

\mypara{Training data}
Figure~\ref{fig:eval-training-data} compares \name's performance under two choices of training data: the dataset on which the final DNN is trained (``general dataset''), and a 10x-downsampled (\ie 3 frames per second) video from the \textsf{Drone} videos (``sampled images'').
There is no clear distinction between training on general dataset and on images sampled from the test video.
As we discussed in \S\ref{subsec:loss}, training on general dataset will be more generic, but it loses the opportunity to save more file size by letting \AccuracyGradientModel adapt to test set video content.
Training on sampled images, on the other hand, may not always be possible, when the video content is confidential for instance.
%can facilitate the \AccuracyGradientModel to make better decision on test videos. However, getting similar videos to test set is not always possible (\eg when the video content is confidential). Moreover, when the test video content shifts, \AccuracyGradientModel might have poor performance.
That said, our intuition is that sampled data is slightly more advantageous as it fits the characteristics of the test videos. This also aligns with Figure~\ref{fig:eval-training-data}, the accuracy of training on sampled frame can be a bit higher than training on general dataset.

\mypara{Training time}
We use the two datasets in Figure~\ref{fig:eval-training-data} to benchmark the training time of customizing an \AccuracyGradientModel.
We first use the COCO dataset (``general dataset'') which contains 120K images, and the training takes about 6 hours (6 epochs, each scanning through the whole dataset). 
To put this number into perspective, it is several orders of magnitude faster than training a regular object detection model. 
Moreover, when trained on the small dataset (``sampled images''), which contains about 600 frames in total, the training time can be drastically reduced to about 12 minutes. 


% \jc{TALK ABOUT TRAINING TIME HERE}

\begin{figure}
    \centering
    % \includegraphics[width=0.4\columnwidth]{figs/placeholder-eval-codec.pdf}
    
    \subfloat[H.264]
    {
        \includegraphics[width=0.3\columnwidth]{figs/detection_drone_FPN_mp4.pdf}
        \label{subfig:1}
    }
    \subfloat[H.265]
    {
        \includegraphics[width=0.3\columnwidth]{figs/detection_drone_FPN_hevc.pdf}
        \label{subfig:1}
    }
    \subfloat[VP9]
    {
        \includegraphics[width=0.3\columnwidth]{figs/detection_drone_FPN_webm.pdf}
        \label{subfig:1}
    }
    \tightcaption{\name improves the accuracy-compression tradeoffs regardless of the underlying video codecs.}
    \label{fig:eval-codec}
\end{figure}
\mypara{Underlying codec}
Lastly, Figure~\ref{fig:eval-codec} tests \name under different traditional codecs.
We can see that the \name consistently reduces the file size by 24-50\% with higher accuracy compared to purely encoding through codec.


\mypara{Customization}



\mypara{Reusing}






\subsection{Supporting adaptive video streaming}
\label{subsec:eval:adaptive}

So far, we have evaluated \name with its parameters fixed at the default values. 
In this section, we show its flexibility in supporting various compression-accuracy objectives, via the setting of its parameters $\AgThresh$ and $\AreaThresh$, as explained in \S\ref{subsec:quality-assignment}. 
%As a usable video stack, \name provides two control knobs to navigate the bandwidth-accuracy tradeoffs, as explained in \S\ref{subsec:assignment}. 
To demonstrate it, we consider that a video sensor encodes and streams the video over a bandwidth-constrained connection to a remote server for DNN inference and analytics.
%In this context, we show how \name supports two typical policies of adaptive streaming, in ways that are impossible in today's video codecs.

\begin{figure}
    \centering
    % \includegraphics[width=0.65\columnwidth]{figs/placeholder-eval-video-adaptation.pdf}
    \includegraphics[width=0.48\columnwidth]{figs/const_heat_bw.pdf}
    \includegraphics[width=0.48\columnwidth]{figs/const_heat_acc.pdf}
    \tightcaption{\name with a fixed \ag threshold $\AgThresh$ vs. the traditional codec H264:
    \name automatically increases the high-quality blocks only when needed to maintain a high accuracy (between the 30$^{\textrm{th}}$ and the 50$^{\textrm{th}}$ second).
%    Comparison between \name and H.264 under accuracy-focused scenario. Black vertical lines marks the time the car enters and leaves the crossroads. \name is able to encode just enough video content to preserve high accuracy.
    }
    \label{fig:eval-video-adaptation}
\end{figure}
\mypara{Reducing bandwidth usage with high accuracy}
% \kt{Rename this to accuracy control?}
When users want to minimize bandwidth usage without hurting accuracy, it will be a good use case for setting the \ag threshold $\AgThresh$, which allows the user to take advantages of content variation: when content is simple or contains less useful information, naturally less blocks will have high accuracy gradients, thus bandwidth usage can be lowered with minimum impact on accuracy.
To show this, Figure~\ref{fig:eval-video-adaptation} runs \name and the traditional H.264 codec on a dashcam video (the link is listed in ~\cite{dataset-link}), in which the street is relatively empty from before the 30$^{\textrm{th}}$ second and after the 50$^{\textrm{th}}$ second. In these time intervals, \name can automatically save 5x bandwidth while maintaining consistently higher accuracy (in detecting traffic lights and pedestrians\jc{is it true?}). 
However, between the 30$^{\textrm{th}}$ and the 50$^{\textrm{th}}$ second (marked by the black vertical line in Figure~\ref{fig:eval-video-adaptation}), a car enters the crossroad, increasing the number of objects. 
To keep high accuracy, \name automatically encodes more blocks in high quality to maintain accuracy over 90\% of the time.
In short, with a fixed \ag threshold, \name will increase bandwidth usage {\em only} when needed.
%In contract, MPEG is of lower bandwidth usage, but the accuracy is always smaller than 90\%.



\begin{figure}
    \centering
    % \includegraphics[width=0.65\columnwidth]{figs/placeholder-eval-bw-adaptation.pdf}
    \includegraphics[width=0.48\columnwidth]{figs/bw_adapt_bw.pdf}
    \includegraphics[width=0.48\columnwidth]{figs/bw_adapt_acc.pdf}
    \tightcaption{\name vs. H.264 under a dynamic bandwidth constraint. 
    While both H.264 and \name (via setting the high-quality area threshold $\AreaThresh$) can adapt bandwidth usage, \name maintains a higher accuracy.
%    Comparison between \name and H.264  under limited dynamic bandwidth. \name achieves higher accuracy with less bandwidth fluctuation.
}
    \label{fig:eval-bw-adaptation}
\end{figure}
\mypara{Higher accuracy under bandwidth budget}
% \kt{Rename this to bitrate control?}
When users want higher accuracy under limited bandwidth, it will be a good use case for setting the high-quality area threshold $\AreaThresh$, which allows user to keep at a roughly stable bandwidth usage. 
%We use an offline profiling process to first create a mapping from bandwidth usage to $\AreaThresh$. 
%Based on this profile, we then assume that the user has the perfect knowledge of future bandwidth. 
We let the user feed the available bandwidth to \name. \name then sets $\AreaThresh$ accordingly and leverages the constant bitrate mode of H.264 codec to control bandwidth.
% The chunk length is \fillme seconds (the gap between two I-frames).
%To achieve that, ABR uses an offline profiled mapping from $\AreaThresh$
Figure~\ref{fig:eval-bw-adaptation} compares the performance between \name and the classic codec of H.264 on the same video as Figure~\ref{fig:eval-video-adaptation}, but this time, we set the available bandwidth at 2.5Mbps at the beginning and suddenly drops to 1.3Mbps at the 10$^{\textrm{th}}$ second, and it stays there until it bounces back to 2.5Mbps at the 30$^{\textrm{th}}$ second. 
We can see that while both \name and H.264 are able to stick to the bandwidth constraint, \name maintains a higher and more stable accuracy compared to H.264.

%\subsection{Offline cost analysis}



%\jc{we don't mean to eval abr logic}


%\mypara{Effect of different parameters}


%\newpage


%\kt{
%\begin{itemize}
%\item dataset
%\item setting of tasks (dnns) and codec
%\item evaluation metrics
%\item baselines: dds, neural autocodec, sr, focus, vstore
%\end{itemize}}

%\mypara{Vision task}


%\mypara{Object detection and segmentation dataset}


\begin{comment}

\mypara{Person keypoint detection dataset}
\kt{Wait after Qizheng finishes it.}

\jc{predictability experiment}

\subsection{Overall improvement}

\begin{figure}
    \centering
    \subfloat[Object detection (Highway)]
    {
        \includegraphics[width=0.22\textwidth]{figs/detection_dashcam.pdf}
        \label{subfig:1}
    }
    \subfloat[Object detection (Drone)]
    {
        \includegraphics[width=0.22\textwidth]{figs/detection_vis.pdf}
        \label{subfig:2}
    }
    
    \subfloat[Sem. segmentation (Drone)]
    {
        \includegraphics[width=0.22\textwidth]{figs/segmentation_vis.pdf}
        \label{subfig:1}
    }
    \subfloat[Sem. segmentation (Dashcam)]
    {
        \includegraphics[width=0.22\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    
    \subfloat[Keypoint detection (Kite)]
    {
        \includegraphics[width=0.22\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    \subfloat[Keypoint detection (Skate)]
    {
        \includegraphics[width=0.22\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    
    \caption{Overall accuracy compression tradeoff of \name and various baselines on different applications. \name saves \fillme\% filesize without hurting accuracy.}
    \label{fig:filesize-acc}

\end{figure}

\mypara{Improvement in compression efficiency} 
Figure \ref{fig:filesize-acc} demonstrates that \name consistently reduces file size by \fillme\% without hurting inference accuracy than various baselines.

\mypara{Improvement in consumption time} 
inference delay vs. accuracy

\mypara{Improvement in online analytics on streaming videos} 
\kt{are we really doing this?}

\mypara{Improvement over multiple tasks}
Improvement vs. \# of tasks

\subsection{Improvement breakdown}
how much does each technique contributing to the overall improvement

\jc{
\begin{itemize}
\item effectiveness of delay reduction (frame sampling, uniform coloring vs. low quality)
\item bandwidht adaptation
\item impact of training data
\end{itemize}}


\subsection{Microbenchmarking}


\begin{figure}
    \centering
    \subfloat[H.264]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    \subfloat[H.265]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    \subfloat[VP8]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    
    \caption{Performance of \name under different codec. The gain of \name is stable under various codec.}
    \label{fig:codec-insensitive}

\end{figure}

\begin{figure}
    \centering
    \subfloat[FasterRCNN]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    \subfloat[EfficientDet]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    \subfloat[Trasformer]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    
    \caption{Performance of \name under different genre of DNN. The gain of \name remains substantial.}
    \label{fig:dnn-insensitive}

\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/encoding-delay.pdf}
    \caption{Encoding delay between \name and H.264. \name achieves lower encoding delay without compromising accuracy.}
    \label{fig:encoding-delay}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/encoding-delay-with-gpu.pdf}
    \caption{Encoding delay of \name can be drastically decreased if equipped with low-end GPU.}
    \label{fig:encoding-delay-with-gpu}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/processing-delay.pdf}
    \caption{Processing delay per frame between \name and H.264 under various consumption demand. \name achieves lower processing delay per frame under various consumption demand.}
    \label{fig:processing-delay}
\end{figure}


\mypara{Underlying codec}
As Figure \ref{fig:codec-insensitive} demonstrates, the gain of \name is stable under various codec.

\mypara{Underlying dnn}
As Figure \ref{fig:dnn-insensitive} demonstrates, the gain of \name is substantial under various genre of DNN.

\mypara{Encoding delay}
As Figure \ref{fig:encoding-delay} demonstrates, \name achieves lower encoding delay without compromising accuracy.

\mypara{Consumption demand}
As Figure \ref{fig:processing-delay} shows, \name achieves consistently lower processing delay under various consumption demand.

\mypara{Assist with low-end GPU}
As Figure \ref{fig:encoding-delay-with-gpu} shows, the encoding delay of \name can be drastically decreased if equipped with even low-end GPU.


\end{comment}




==> eval.tex <==

\section{Evaluation}
\label{sec:eval}

\mypara{Takeaway}
Here are the takeaways from our experiments:
\begin{itemize}
\item in injection time, \name achieves \fillme\% less compressed video sizes than today's video codec with similar encoding delay on cpus.
\item in consumption time, \name speeds up the inference by \fillme$\times$ than today's video codec, while achieving similar accuracy.
\item in video streaming, \name achieves similar accuracy with \fillme\% less bandwidth and \fillme\% less inference delay.
\end{itemize}

\subsection{Setup}
\label{subsec:eval:setup}
\kt{
\begin{itemize}
\item dataset
\item setting of tasks (dnns) and codec
\item evaluation metrics
\item baselines: dds, neural autocodec, sr, focus, vstore
\end{itemize}}

\mypara{Vision task}
In our experiments, we evaluate two vision tasks: object detection segmentation and person keypoint detection. We use FasterRCNN-ResNet50-FPN, FCN-ResNet50 and KeypointRCNN-ResNet50-FPN from torchvision model zoo~\cite{??} as the vision model for the vision tasks listed above.

\mypara{Object detection and segmentation dataset}
We use dashcam videos~\cite{dds} and drone videos~\cite{aiskyeye} to evaluate object detection and segmentation.

\mypara{Person keypoint detection dataset}
\kt{Wait after Qizheng finishes it.}

\jc{predictability experiment}

\subsection{Overall improvement}

\begin{figure}
    \centering
    \subfloat[Object detection (Highway)]
    {
        \includegraphics[width=0.22\textwidth]{figs/detection_dashcam.pdf}
        \label{subfig:1}
    }
    \subfloat[Object detection (Drone)]
    {
        \includegraphics[width=0.22\textwidth]{figs/detection_vis.pdf}
        \label{subfig:2}
    }
    
    \subfloat[Sem. segmentation (Drone)]
    {
        \includegraphics[width=0.22\textwidth]{figs/segmentation_vis.pdf}
        \label{subfig:1}
    }
    \subfloat[Sem. segmentation (Dashcam)]
    {
        \includegraphics[width=0.22\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    
    \subfloat[Keypoint detection (Kite)]
    {
        \includegraphics[width=0.22\textwidth]{figs/keypoint_surf.pdf}
        \label{subfig:1}
    }
    \subfloat[Keypoint detection (Skate)]
    {
        \includegraphics[width=0.22\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    
    \caption{Overall filesize-accuracy tradeoff of \name and various baselines on different applications. \name saves \fillme\% filesize without hurting accuracy.}
    \label{fig:filesize-acc}

\end{figure}

\mypara{Improvement in compression efficiency} 
Figure \ref{fig:filesize-acc} demonstrates that \name consistently reduces file size by \fillme\% without hurting inference accuracy than various baselines.

\mypara{Improvement in consumption time} 
inference delay vs. accuracy

\mypara{Improvement in online analytics on streaming videos} 
\kt{are we really doing this?}

\mypara{Improvement over multiple tasks}
Improvement vs. \# of tasks

\subsection{Improvement breakdown}
how much does each technique contributing to the overall improvement

\jc{
\begin{itemize}
\item effectiveness of delay reduction (frame sampling, uniform coloring vs. low quality)
\item bandwidht adaptation
\item impact of training data
\end{itemize}}


\subsection{Microbenchmarking}


\begin{figure}
    \centering
    \subfloat[H.264]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    \subfloat[H.265]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    \subfloat[VP8]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    
    \caption{Performance of \name under different codec. The gain of \name is stable under various codec.}
    \label{fig:codec-insensitive}

\end{figure}

\begin{figure}
    \centering
    \subfloat[FasterRCNN]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    \subfloat[EfficientDet]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:2}
    }
    \subfloat[Trasformer]
    {
        \includegraphics[width=0.15\textwidth]{figs/filesize-acc.pdf}
        \label{subfig:1}
    }
    
    \caption{Performance of \name under different genre of DNN. The gain of \name remains substantial.}
    \label{fig:dnn-insensitive}

\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/encoding-delay.pdf}
    \caption{Encoding delay between \name and H.264. \name achieves lower encoding delay without compromising accuracy.}
    \label{fig:encoding-delay}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/encoding-delay-with-gpu.pdf}
    \caption{Encoding delay of \name can be drastically decreased if equipped with low-end GPU.}
    \label{fig:encoding-delay-with-gpu}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/processing-delay.pdf}
    \caption{Processing delay per frame between \name and H.264 under various consumption demand. \name achieves lower processing delay per frame under various consumption demand.}
    \label{fig:processing-delay}
\end{figure}


\mypara{Underlying codec}
As Figure \ref{fig:codec-insensitive} demonstrates, the gain of \name is stable under various codec.

\mypara{Underlying dnn}
As Figure \ref{fig:dnn-insensitive} demonstrates, the gain of \name is substantial under various genre of DNN.

\mypara{Encoding delay}
As Figure \ref{fig:encoding-delay} demonstrates, \name achieves lower encoding delay without compromising accuracy.

\mypara{Consumption demand}
As Figure \ref{fig:processing-delay} shows, \name achieves consistently lower processing delay under various consumption demand.

\mypara{Assist with low-end GPU}
As Figure \ref{fig:encoding-delay-with-gpu} shows, the encoding delay of \name can be drastically decreased if equipped with even low-end GPU.

==> intro-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}




% video analytics is popular
Video analytics applications, powered by modern computer vision, are poised to transform businesses (retail, industrial logistics, etc), technologies (intelligent assistance, video understanding, etc), and public policies (traffic management, urban planning, etc)~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero,visionzero-bellevue, msr-bellevue}.
%~\cite{??,??,??}.
Industry reports have projected that more sensor videos will be generated for analysis purposes than being watched by users~\cite{infowatch12,infowatch16}.
A key component to scale out the emerging video analytics ecosystems is a highly efficient {\em video stack}, which like in traditional video streaming, compresses (encodes) videos with low delays for a range of DNN-based video analytics tasks without hurting their inference accuracy once the videos are decoded. 
%compresses raw frames to an encoded video and feed decoded frames to deep neural nets (DNN) inference. 
%Ideally, it needs to significantly compress the size of a video stream while preserving enough information in the encoded video that still allows for highly accurate DNN inference, and do so with low encoding and decoding delays. 
% DNN can achieve the decoded video to the DNN for high accuracy with low decoding and inference delay.
%{\em injects} (\ie encodes) and {\em consumes} a video stream (\ie decodes and feeds frames to inference models) with low latency and high inference accuracy for a range of vision inference tasks.


% many prior efforts but basically limited by the same video stack
While tremendous efforts focus on efficient video analytics applications/pipelines, relatively less attention is given to the underlying video stack that these applications use.
The few works that do tune video encoding (\eg~\cite{awstream,dds}) build on widely-used classic video codecs (\eg H.264/MPEG and DASH) and try to address the different needs of DNN inference, \eg the classic codecs may encode substantial redundant information not needed by DNNs and/or drop information vital to DNN inference.
%~\cite{dds,awstream,reducto,vstore}.

Unfortunately, these video stacks use heuristics that are designed with particular video analytics tasks/DNNs in mind, so their performance falls short in other DNNs.
% rather than applicable to a broad range of applications.
In the meantime, these efforts offer little insight on how much a video could potentially be compressed without hurting the accuracy of a particular DNN.
Although both issues are not unacceptable for a point solution, developing a {\em general}, {\em near-optimal} video stack, in our view, will provide a fundamental insight about how videos should be encoded for video analytics purposes (as opposed to human perception).


%Current solutions are based on off-the-shelf video codecs (\eg H.264/MPEG and DASH/HTTP streaming protocol) originally designed to enhance human-perceived video quality.
%Recent work has highlighted potential mismatches between these codecs and DNNs' needs: the codecs may encode substantial redundant information not needed by DNNs and sometimes aggressively drop information vital to DNN inference (low inference accuracy)~\cite{dds,awstream,reducto,vstore}.
%rather than the performance of computer vision models. 
%\jc{a few examples}


% our basic observation is that the importance of pixels to the final accuracy is disproportion to the fraction of such pixels

To this end, we set out to design such a video stack. In doing so, we take a practical stance by also building our video stack on existing video codecs. 
However, we develop our solution through tackling two key questions:
\begin{packedenumerate}
\item What is the {\em optimal} compression efficiency for a given video analytics DNN that still preserves enough information to maintain high inference accuracy?
% quality level (\ie maximum compression level) that still preserves the inference accuracy of a given vision task?
%much do different levels of compressions on each pixel affect the accuracy of various vision inference tasks?
\item How can a video stack approximate the optimal compression in practice for a {\em wide} range of video analytics DNNs?
% efficiently compress each pixel at the lowest quality level that still preserves the inference accuracy?
\end{packedenumerate}
%In short, the first is about the optimal compression efficiency for DNN inference, while the second seeks to approximate it in practice.

% Our work is a step towards answering both questions.
To make the first question more concrete, we examine (\S\ref{sec:potential}) across a range of DNNs for three video analytics tasks. 
To make it more concrete, we spatially split each frame into fine-grained (16 pixels by 16 pixels) blocks and 
identify the quality-sensitive regions---a minimum set of blocks that must be encoded in high quality, such that the DNN inference produces (almost) identical results as it would on the highest quality video (\eg same detected objects). 
We show that the quality-sensitive regions on the same frame can differ significantly among the DNNs of the same task (\eg different off-the-shelf DNN object detectors). 
Moreover, the quality-sensitive regions frequently misalign with the boundaries or the bounding boxes of objects. 
In contrary to the conventional wisdom, these findings suggest that video encoding will be suboptimal if it assigns quality levels or drops frames by generic notions, such as where objects are likely located. Instead, the encoding must be deeply integrated with the needs of the particular DNN that eventually analyzes the video. 

\jc{show our accuracy is more stable than baselines}


\begin{comment}
the spatial distribution of lowest quality level across {\em fine-grained blocks} (16$\times$16 pixels) such that the inference results remain as if the whole frames are encoded in a high quality. 
Contrary to the conventional beliefs in prior work, our analysis reveals that
% Compared to similar prior attempts, our analysis is unique in two aspects.
\begin{packeditemize}
\item 
% We study the {\em spatial} distribution of minimum quality at the level of fine-grained of blocks which is much smaller than objects or bounding boxes (which are commonly used~\cite{dds,eaar}). 
the minimum set of blocks that need high quality are often misaligned with objects or bounding boxes (which are commonly used to delineate the encoding boundaries in prior work~\cite{dds,eaar}), and
% Our analysis reveals that highly quality sensitive regions (\ie encoding them at even slightly lower quality can alter the result) can be much smaller than suggested in previous studies. 
% , and that the quality sensitive regions can vary dramatically across frames.
\item 
% Our analysis spans {\em more vision tasks} (object detection, semantic segmentation, and keypoint detection) than a single one~\cite{eaar,glimpse} and reveals that 
the minimum set of blocks that need high quality varies substantially across the vision tasks and even the DNNs of the same task (which suggests the encoding cannot be agnostic to the final DNN).
% For instance, \jc{an example.}
\end{packeditemize}
\end{comment}


% we found today's codec is fundamentally ill-suited to this task

Using the measurement-driven insights, we present {\bf \name}, a new video stack 
% (including injection and consumption) 
for DNN-based vision inference.
The key idea is the new concept of {\em accuracy gradients} ({\em \ags}).
%\kt{Maybe substitude AG with AccGrad?}
% some encoding of a frame (with spatially different quality) are the gradients of the similarity between final DNN's output on that encoding and its output on the high-quality encoding. 
Intuitively, the \ag of each fine-grained spatial region captures how quality changes at the region affect the DNN's inference accuracy (\S\ref{sec:framework}).
\Ags have two unique benefits.
First, they can be calculated using only the feedforward and backpropagation operations available from {\em any} DNN model.
%, which allows us to treat each DNN as a {\em differentiable} ``black box''. 
%(\ie we treat it as a \kt{differentiable} ``black box'') and are thus applicable to a variety of DNN-based vision tasks.
Second, the knowledge of \ags naturally indicates the minimum regions that have to be preserved at high data fidelity, which can be used to assign spatially heterogeneous quality for highly efficient video compression and accurate DNN inference.
\Ags in effect serve as an interface that treats any DNN-based vision model as a {\em differentiable black box}, while preserving the necessary information to {\em customize} the encoding of each video frame for any given DNN.
% , as well as which regions regions (\eg some parts of the background) can be totally insensitive to quality, suggesting that it can be completely replaced with a fixed value or even removed, which enables more efficient video encoding and faster inference.


\begin{comment}
\name provides three operations to video analysts:
In the (offline) {\em preparation} phase, \name automatically customizes an instance of the video stack for any given DNN model and accuracy metric (loss function);
in the online {\em encoding} phase, the customized video codec takes compresses frames from a source to a compressed video; and
% source from which frames can be read and then compressed.
an on-demand {\em decoding} phase reconstructs video frames and feeds them into the DNN for inference.
% a time window in which the video will be \kt{decoded} and feed into the DNN for inference.
% \end{packeditemize}
\end{comment}

% \begin{packeditemize}
% \item {\em Preparation (offline):} The DNN model, loss function (accuracy metric) based on which \name creates a custom instance of stack for the particular DNN and loss function;
% \item {\em Injection (online):}  The video source from which frames can be read and then compressed.
% \item {\em Consumption (on demand):}  A time window in which the video will be \kt{decoded} and feed into the DNN for inference.
% \end{packeditemize}

% \kt{Maybe also emphasize that accuracy gradient can efficiently explore a large design space with just a single forwarding and backwarding?}

%In addition to the normal encoding and decoding operations, \name adds an offline preparation phase, where \name automatically customizes an instance of the video stack for any given DNN model and accuracy metric (loss function).

To realize the benefits of \ags in practice, \name addresses two challenges:
%To this end, \name presents concrete design choices to address two key challenges:
% fully realizing the benefits of accuracy gradients in practice is challenging, and our design and implementation of 
%To address them, \name presents two techniques:
\begin{packeditemize}
%\item {\em Fast accuracy-gradient estimator (\S\ref{sec:??}):} 
%\item {\em How to train an accurate light-weight model to infer \ags (\S\ref{sec:training})?} 

\item {\em How to obtain \ags on a given frame without running the eventual analytical DNN (\S\ref{sec:training})?} 
\name infers \ags of a frame by feeding it through a shallow neural network, which \name customizes for any given analytical DNN model and accuracy metric in an automated offline process.
\name also optimizes the shallow neural net to avoid pitfalls such as the imbalanced \ag value distributions.
%The \name automatically customizes offline for any given DNN model and accuracy metric (loss function).
%We also design a custom loss function to pitfalls in learning \ags that have highly imbalanced value distributions.
%For a given DNN and loss function, we train a light-weighted model (\fillme DNN) that takes a frame as input and outputs a ``heatmap'' in which the score of a region (\eg a $16\times16$ block) indicates the minimum quality at which the region should be encoded in order to achieve a similar accuracy as if it were encoded at a higher quality.
%To make this estimator run as fast as the video codec, we run it only once every \fillme frames. 
%\item {\em Reusing existing video codec (\S\ref{sec:??}):} 

\item {\em How to reduce the extra runtime overhead caused by the use of \ags (\S\ref{sec:runtime})?} 
\name supports several optimizations to cut the runtime overhead, including updating the \ags only on sampled frames and using uniform color to speed up the video encoding/decoding.
%Instead of inventing a new video codec from scratch, \name takes a pragmatic stance to reuse existing video code (\eg \fillme). 
%It spatially splits each frame into multiple versions, each containing regions to be encoded at the same quality level, and encode individual version using the off-the-shelf codec which is highly optimized to encode frames at a given quality. 

% \item {\em Spatial batching of inference (\S\ref{sec:??}):} 
% \name batches the processing of low-quality images and spatially stitches small blocks of high quality regions before feeding them into the DNN inference. 
% This optimization greatly reduces the amortized inference delay per frame.
% consumption can be greatly sped up by spatially batching the masks 
\end{packeditemize}
%We will elaborate the rationale of these design choices in \S\ref{sec:training},\ref{sec:runtime}.
The rationales behind these designs will be elaborated in \S\ref{sec:training},\ref{sec:runtime}.

Admittedly, no individual technique of \name is exactly new: it uses off-the-shelf library as its underlying video codec, and the concepts of encoding frames with spatially uneven quality levels and compressing videos in a DNN-aware manner have appeared in prior work. 
Nonetheless, as a concrete system that integrates these components based on the novel concept of accuracy gradients, \name outperforms existing solutions and generalizes to a wide range of video analytics applications.
Our evaluation shows that compared with the state-of-the-art baselines across three video analytics applications, \name reduces half of the filesize and 4\% higher accuracy on 4 sets of video in diverse genres. Moreover, \name's encoding/decoding delays are only marginally higher than the traditional codec (which vastly faster than baselines that achieve similar compression efficiency).
In addition, like traditional codecs, \name also provides tunable parameters which allow users to navigate on the new tradeoff frontier between compression and utility (accuracy).


\jc{show an example result?!}

\jc{change all full dnns to final dnns}


%\jc{accuracy stability?}

%\jc{eval summary}

%\begin{itemize}
%\item video analytics is becoming popular
%\item though efforts were made to improve performance (in accuracy, streaming delay), the video stack is largely intact. 
%\item however, video analytics results have drastically different sensitivity to the fidelity of different pixels, and only a small fraction of pixels have to preserve very high fidelity. 
%(in contrast to dds, eaar or vigil, a highly sensitive portion can be just a small part of an object/region). 
%\item existing video stack is ill-suited: (1) highly sensitive pixels are \kt{DNN-specific and} not what humans vision focus on \kt{A figure that illustrates the difference between visually-pleasing image and DNN-pleasing image}, (2) they dont change smoothly as motion vectors, and\kt{existing video stack consume all pixels in the frame, even most of them do not contribute to the inference results.}
%\item this paper presents \name, a new video stack (including encoding, decoding, and consumption) for vision inference, based on the key insight that: the highly sensitive regions can be derived based on the generic concept of {\em accuracy gradient}.
%\item for developers, \name provides an interface to specify DNN execution and loss functions, and automatically customizes the injection and consumption pipeline. 
%\item \name entails three novel techniques:
%\begin{itemize}
%\item technique \#1: accuracy gradients (and the resulting mask) can be inferred using a small model
%\item technique \#2: the mask can be smoothed so as to enable efficient encoding using existing codec
%\item technique \#3: consumption can be greatly sped up by spatially batching the masks 
%\end{itemize}
%\item additional benefits: \name can easily scale to multiple applications with one stack.
%%\item inspired by the insight, we envision a new video codec (\fillme); execution framework (\fillme)
%\item the underlying techniques are not new: still use the mpeg functionalities but add a shim layer between DNN and mpeg.
%\item design details
%\item eval summary
%\end{itemize}










==> intro-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}




% video analytics is popular
Video analytics applications, powered by modern computer vision, are poised to transform businesses (retail, industrial logistics, etc), technologies (intelligent assistance, etc), and public policies (traffic management, urban planning, etc)~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero,visionzero-bellevue, msr-bellevue}.
%~\cite{??,??,??}.
Industry reports project that more sensor videos will be generated for analysis purposes than being watched by users~\cite{infowatch12,infowatch16}.
A key component in the emerging video analytics ecosystems is a highly efficient {\em video stack}, which like in traditional video streaming, compresses (encodes) videos in real time while preserving enough information to achieve high inference accuracy for various video analytics tasks, in forms of deep neural nets (DNNs). 
%compresses raw frames to an encoded video and feed decoded frames to deep neural nets (DNN) inference. 
%Ideally, it needs to significantly compress the size of a video stream while preserving enough information in the encoded video that still allows for highly accurate DNN inference, and do so with low encoding and decoding delays. 
% DNN can achieve the decoded video to the DNN for high accuracy with low decoding and inference delay.
%{\em injects} (\ie encodes) and {\em consumes} a video stream (\ie decodes and feeds frames to inference models) with low latency and high inference accuracy for a range of vision inference tasks.


% many prior efforts but basically limited by the same video stack
% While much effort has focused on building video analytics applications/pipelines, relatively less attention is given to the underlying video stack that the applications rely on.
Prior work in this space (\eg~\cite{awstream,dds,reducto,vstore,eaar}) has observed differences between the needs of video analytics tasks (\eg object detection, segmentation) and the widely-used classic video codecs (\eg H.264/MPEG).
To address these discrepancies, current solutions try to adapt quality at the granularity specific to a {\em task}, rather than a specific DNN.
For instance, in object detection, they seek to decide which frames, objects, or bounding boxes should be encoded and in what quality (\eg~\cite{dds,reducto,awstream,vigil,eaar,glimpse}).


However, this paradigm---assigning encoding quality to task-specific granularities such as objects or frames---has two limitations. 
On one hand, it leads to suboptimal tradeoffs between compression efficiency and inference accuracy. 
Our analysis reveals that the optimal spatial quality assignments are frequently misaligned with object bounding boxes or boundaries and vary substantially across DNNs of the same task (\S\ref{subsec:analysis}).
On the other hand, each video stack is tied to one task, so a new heuristic has to be crafted for each task. 



\begin{comment}
The few works that do tune video encoding (\eg~\cite{awstream,dds}) build on widely-used classic video codecs (\eg H.264/MPEG and DASH) and try to address the different needs of DNN inference, \eg the classic codecs may encode substantial redundant information not needed by DNNs and/or drop information vital to DNN inference.
%~\cite{dds,awstream,reducto,vstore}.

Unfortunately, these video stacks use heuristics that are designed with particular video analytics tasks/DNNs in mind, so their performance falls short in other DNNs.
% rather than applicable to a broad range of applications.
In the meantime, these efforts offer little insight on how much a video could potentially be compressed without hurting the accuracy of a particular DNN. Although both issues are not unacceptable for a point solution, developing a {\em general}, {\em near-optimal} video stack, in our view, will provide a fundamental insight about how videos should be encoded for video analytics purposes (as opposed to human perception).

\end{comment}

%Current solutions are based on off-the-shelf video codecs (\eg H.264/MPEG and DASH/HTTP streaming protocol) originally designed to enhance human-perceived video quality.
%Recent work has highlighted potential mismatches between these codecs and DNNs' needs: the codecs may encode substantial redundant information not needed by DNNs and sometimes aggressively drop information vital to DNN inference (low inference accuracy)~\cite{dds,awstream,reducto,vstore}.
%rather than the performance of computer vision models. 
%\jc{a few examples}


% our basic observation is that the importance of pixels to the final accuracy is disproportion to the fraction of such pixels

Although both issues are not unacceptable for a point solution, we argue that developing a {\em general} video stack that achieves {\em near-optimal} compression-accuracy tradeoffs for a wide range of vision DNNs still offers fundamental insight into how videos should be encoded for video analytics purposes (as opposed to human perception).
Inspired by this ideal, we set out to design such a video stack by answering two key questions:
% We are driven by two key questions:

%In doing so, we are driven by two key questions
%take a practical stance by building our video stack on traditional video codecs. 
%However, we develop our solution through tackling two key questions:


\begin{packedenumerate}
\item What is the {\em optimal} compression efficiency for a given DNN while still preserving enough information to maintain high inference accuracy?
% quality level (\ie maximum compression level) that still preserves the inference accuracy of a given vision task?
%much do different levels of compressions on each pixel affect the accuracy of various vision inference tasks?
\item How can a video stack approximate the optimal compression in practice for a {\em wide} range of video analytics DNNs?
% efficiently compress each pixel at the lowest quality level that still preserves the inference accuracy?
\end{packedenumerate}
%In short, the first is about the optimal compression efficiency for DNN inference, while the second seeks to approximate it in practice.

% Our work is a step towards answering both questions.
To make the first question more concrete, we examine (\S\ref{sec:potential}) across a range of DNNs for three video analytics tasks. 
To make it more concrete, we spatially split each frame into fine-grained (16x16-pixel) blocks and 
identify the minimum set of {\em quality sensitive} blocks that must be encoded in high quality, such that the DNN inference produces (almost) identical results to its output on the highest quality video. 
Our measurements over three tasks reveal that the quality-sensitive blocks on the same frame can vary significantly across even the DNNs of the same task (\eg different object detectors).
Therefore, it is crucial to customize the encoding quality of individual blocks for each {\em specific DNN} by understanding its impact on the particular DNN's inference accuracy.

\begin{comment}
%Moreover, the quality-sensitive regions frequently misalign with the boundaries or the bounding boxes of objects. 
In contrary to the conventional wisdom, these findings suggest that video encoding will be suboptimal if it assigns quality levels or drops frames by generic notions, such as where objects are likely located. Instead, the encoding must be deeply integrated with the needs of the particular DNN that eventually analyzes the video. 
\end{comment}

% \jc{show our accuracy is more stable than baselines}


\begin{comment}
the spatial distribution of lowest quality level across {\em fine-grained blocks} (16$\times$16 pixels) such that the inference results remain as if the whole frames are encoded in a high quality. 
Contrary to the conventional beliefs in prior work, our analysis reveals that
% Compared to similar prior attempts, our analysis is unique in two aspects.
\begin{packeditemize}
\item 
% We study the {\em spatial} distribution of minimum quality at the level of fine-grained of blocks which is much smaller than objects or bounding boxes (which are commonly used~\cite{dds,eaar}). 
the minimum set of blocks that need high quality are often misaligned with objects or bounding boxes (which are commonly used to delineate the encoding boundaries in prior work~\cite{dds,eaar}), and
% Our analysis reveals that highly quality sensitive regions (\ie encoding them at even slightly lower quality can alter the result) can be much smaller than suggested in previous studies. 
% , and that the quality sensitive regions can vary dramatically across frames.
\item 
% Our analysis spans {\em more vision tasks} (object detection, semantic segmentation, and keypoint detection) than a single one~\cite{eaar,glimpse} and reveals that 
the minimum set of blocks that need high quality varies substantially across the vision tasks and even the DNNs of the same task (which suggests the encoding cannot be agnostic to the final DNN).
% For instance, \jc{an example.}
\end{packeditemize}
\end{comment}


% we found today's codec is fundamentally ill-suited to this task

Using the measurement-driven insights, we present {\bf \name}, a new video stack 
% (including injection and consumption) 
for DNN-based vision inference.
The key idea is the new concept of {\em accuracy gradients} ({\em \ags}).
%\kt{Maybe substitude AG with AccGrad?}
% some encoding of a frame (with spatially different quality) are the gradients of the similarity between final DNN's output on that encoding and its output on the high-quality encoding. 
At a high level, \ags describes for a given DNN and frame, how much the DNN's inference accuracy would be influenced by a change of quality in each spatial block (\S\ref{sec:framework}).
%fine-grained spatial region captures how quality changes at the region affect the DNN's inference accuracy (\S\ref{sec:framework}).
\Ags have two unique benefits.
First, they can be calculated using only the feedforward and backpropagation operations available from {\em any} DNN model.
%, which allows us to treat each DNN as a {\em differentiable} ``black box''. 
%(\ie we treat it as a \kt{differentiable} ``black box'') and are thus applicable to a variety of DNN-based vision tasks.
Second, the knowledge of \ags naturally indicates the minimum regions that have to be preserved at high data fidelity in order to maintain high DNN inference.
% which can be used to assign spatially heterogeneous quality for highly efficient video compression and accurate DNN inference.
Thus, \Ags in effect serves as an interface that treats any DNN-based vision model as a {\em differentiable black box}, while preserving the necessary information to {\em customize} the encoding of each video frame for any given DNN.
% , as well as which regions regions (\eg some parts of the background) can be totally insensitive to quality, suggesting that it can be completely replaced with a fixed value or even removed, which enables more efficient video encoding and faster inference.


\begin{comment}
\name provides three operations to video analysts:
In the (offline) {\em preparation} phase, \name automatically customizes an instance of the video stack for any given DNN model and accuracy metric (loss function);
in the online {\em encoding} phase, the customized video codec takes compresses frames from a source to a compressed video; and
% source from which frames can be read and then compressed.
an on-demand {\em decoding} phase reconstructs video frames and feeds them into the DNN for inference.
% a time window in which the video will be \kt{decoded} and feed into the DNN for inference.
% \end{packeditemize}
\end{comment}

% \begin{packeditemize}
% \item {\em Preparation (offline):} The DNN model, loss function (accuracy metric) based on which \name creates a custom instance of stack for the particular DNN and loss function;
% \item {\em Injection (online):}  The video source from which frames can be read and then compressed.
% \item {\em Consumption (on demand):}  A time window in which the video will be \kt{decoded} and feed into the DNN for inference.
% \end{packeditemize}

% \kt{Maybe also emphasize that accuracy gradient can efficiently explore a large design space with just a single forwarding and backwarding?}

%In addition to the normal encoding and decoding operations, \name adds an offline preparation phase, where \name automatically customizes an instance of the video stack for any given DNN model and accuracy metric (loss function).

To realize the benefits of \ags in practice, \name addresses two practical challenges:
%To this end, \name presents concrete design choices to address two key challenges:
% fully realizing the benefits of accuracy gradients in practice is challenging, and our design and implementation of 
%To address them, \name presents two techniques:
\begin{packeditemize}
%\item {\em Fast accuracy-gradient estimator (\S\ref{sec:??}):} 
%\item {\em How to train an accurate light-weight model to infer \ags (\S\ref{sec:training})?} 

\item {\em How to obtain \ags on a given frame without running the (expensive) final DNN (\S\ref{sec:training})?} 
\name infers \ags of a frame by feeding it through a shallow NN, which \name trains for any given final DNN and accuracy metric by an automated offline process.
\name also optimizes the shallow NN to avoid pitfalls such as the imbalanced \ag value distributions.
%The \name automatically customizes offline for any given DNN model and accuracy metric (loss function).
%We also design a custom loss function to pitfalls in learning \ags that have highly imbalanced value distributions.
%For a given DNN and loss function, we train a light-weighted model (\fillme DNN) that takes a frame as input and outputs a ``heatmap'' in which the score of a region (\eg a $16\times16$ block) indicates the minimum quality at which the region should be encoded in order to achieve a similar accuracy as if it were encoded at a higher quality.
%To make this estimator run as fast as the video codec, we run it only once every \fillme frames. 
%\item {\em Reusing existing video codec (\S\ref{sec:??}):} 

\item {\em How to reduce the extra runtime overhead caused by the use of \ags (\S\ref{sec:runtime})?} 
\name uses several optimizations to cut the encoding overhead, including updating the \ags only on sampled frames and using a uniform color to encode less important blocks, which improves accuracy and speeds up video encoding.
%Instead of inventing a new video codec from scratch, \name takes a pragmatic stance to reuse existing video code (\eg \fillme). 
%It spatially splits each frame into multiple versions, each containing regions to be encoded at the same quality level, and encode individual version using the off-the-shelf codec which is highly optimized to encode frames at a given quality. 

% \item {\em Spatial batching of inference (\S\ref{sec:??}):} 
% \name batches the processing of low-quality images and spatially stitches small blocks of high quality regions before feeding them into the DNN inference. 
% This optimization greatly reduces the amortized inference delay per frame.
% consumption can be greatly sped up by spatially batching the masks 
\end{packeditemize}
%We will elaborate the rationale of these design choices in \S\ref{sec:training},\ref{sec:runtime}.
The rationales behind these designs will be elaborated in \S\ref{sec:training},\ref{sec:runtime}.

Admittedly, no individual technique of \name is exactly new: it uses off-the-shelf library as its underlying video codec, and the concepts of encoding frames with spatially uneven quality levels and compressing videos in a DNN-aware manner have appeared in prior work. 
Nonetheless, as a concrete system that integrates these components based on the novel concept of accuracy gradients, \name outperforms existing solutions and automatically generalizes to various video analytics DNNs.
Our evaluation shows that compared with the state-of-the-art baselines across three video analytics applications, \name reduces half of the file size and achieves 4\% higher accuracy on four sets of video in diverse genres. Moreover, \name's encoding and decoding are only marginally slower than the traditional codecs, and are much faster than baselines that achieve similar compression efficiency.
In addition, like traditional codecs, \name also provides tunable parameters which allow users to navigate on the new compression-privacy tradeoff frontier. 
%frontier between compression and utility (accuracy).


% \jc{show an example result?!}

% \jc{change all full dnns to final dnns}


%\jc{accuracy stability?}

%\jc{eval summary}

%\begin{itemize}
%\item video analytics is becoming popular
%\item though efforts were made to improve performance (in accuracy, streaming delay), the video stack is largely intact. 
%\item however, video analytics results have drastically different sensitivity to the fidelity of different pixels, and only a small fraction of pixels have to preserve very high fidelity. 
%(in contrast to dds, eaar or vigil, a highly sensitive portion can be just a small part of an object/region). 
%\item existing video stack is ill-suited: (1) highly sensitive pixels are \kt{DNN-specific and} not what humans vision focus on \kt{A figure that illustrates the difference between visually-pleasing image and DNN-pleasing image}, (2) they dont change smoothly as motion vectors, and\kt{existing video stack consume all pixels in the frame, even most of them do not contribute to the inference results.}
%\item this paper presents \name, a new video stack (including encoding, decoding, and consumption) for vision inference, based on the key insight that: the highly sensitive regions can be derived based on the generic concept of {\em accuracy gradient}.
%\item for developers, \name provides an interface to specify DNN execution and loss functions, and automatically customizes the injection and consumption pipeline. 
%\item \name entails three novel techniques:
%\begin{itemize}
%\item technique \#1: accuracy gradients (and the resulting mask) can be inferred using a small model
%\item technique \#2: the mask can be smoothed so as to enable efficient encoding using existing codec
%\item technique \#3: consumption can be greatly sped up by spatially batching the masks 
%\end{itemize}
%\item additional benefits: \name can easily scale to multiple applications with one stack.
%%\item inspired by the insight, we envision a new video codec (\fillme); execution framework (\fillme)
%\item the underlying techniques are not new: still use the mpeg functionalities but add a shim layer between DNN and mpeg.
%\item design details
%\item eval summary
%\end{itemize}










==> intro-v4.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

% \begin{itemize}
% \item with video analytics increasingly popular, efficient video encoding is crucial.
% \item prior work in this space is driven by human vision $\neq$ computer vision $\rightarrow$ RoI-based quality assignment.
% \item despite much research, two questions remain unanswered.
% \item Q1: what should be the right granularity of quality assignment? existing work is based on coarse-grained spatial regions. they are suboptimal, because...
% \item Q2: how to decide the quality assignment in real time? especially most sensors cant run expensive dnns or send data out. yet recent work increasingly relies on real-time dnn feedback (dds, eaar, awstream). they are not practical, because...
% \item to answer these questions, we propose \name, which uses a cheap model to decide the microblock-level quality assignment and encodes video accordingly in real time. 
% accgrad is the key to make \name practical in two ways.
% \item \name seems to decide quality assignment using a cheap model while prior work needs much more expensive models. why is it possible? the problem is different (and intuitively easier). we also empirically show that a shallow dnn is sufficient
% \item \name's encoding is dnn dependent, so how to quickly customize its decision for a given dnn? key idea is accuracy gradients: accgrad of a block means how much influence does changing the quality of the block on the accuracy of the DNN. it's fast and treats dnns as only differentiable blackboxes.
% \item connection with prior work: we don't invent new tricks here, but we put them together with new insights
% \item eval highlights: better accuracy-compression tradeoffs, low overhead to encoding, fast customization per new dnn
% \item needs a summarizing list of key contributions (focus on why it's not just about vision/video encoding)
% \end{itemize}



Video analytics applications, powered by modern computer vision, are poised to transform businesses (retail, industrial logistics, etc), technologies (intelligent assistance, etc), and public policies (traffic management, urban planning, etc)~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero,visionzero-bellevue, msr-bellevue}.
Industry reports project that more sensor videos will be generated for analysis purposes than being watched by users~\cite{infowatch12,infowatch16}.
A key component in the emerging video analytics ecosystems is highly efficient {\em video compression}, which like in traditional video streaming, compresses (encodes) videos in real time while preserving enough information to achieve high inference accuracy for various video analytics tasks, in forms of deep neural nets (DNNs). 



Prior work in this space (\eg~\cite{awstream,dds,reducto,vstore,eaar}) has observed differences between the video quality requirements of video analytics tasks (\eg object detection, segmentation) and the widely used classic video codecs (\eg H.264/MPEG).
To address these discrepancies, 
the key insight is to discover those pixels that are important to final DNN inference and apply high encoding quality to them.
% Current solutions perform quality assignment through finding the region of interest of DNN and }
% \jc{``pays no attention'' is vague. please avoid such figurative terms}
To leverage this insight, the overarching trend of previous works is to evolve from finding important pixels through final-DNN-agnostic heuristics~\cite{vigil,glimpse} to finding those pixels in a final-DNN-aware manner\cite{reducto,awstream,dds,eaar,cloudseg}.\jc{``final-dnn-agnostic'' and ``final-dnn-aware'' sound awkward (and did we ever define what ``final dnn'' refers to?). actually, i dont see the need of this sentence at all. this paragraph should focus on the difference between human visual perception and dnn visual perception, NOT how one infers dnn's quality perception, right?}
Take object detection application as an example. As for object detection, previous works evolves from discovering key frames through frame difference~\cite{glimpse}, cropping out pixels that potentially contain objects through cheap DNNs~\cite{vigil} to find key frames based on extracting profile from the final DNN~\cite{reducto} and find important regions through extrapolating DNN's feedback~\cite{eaar,dds}. \jc{to put it in perspective, we should say WHY encoding videos this way doesn't make sense for human perception (or what would look more appealing to human viewers and whether that's what h264/265 optimizes for, etc)}
% \jc{the last sentence doesn't seem to be related to your argument that there are pixels that dnn doesn't care.}




Despite the rich literature in this line of research,
% \jc{paradigm seems unnecessarily grandiose} 
two research questions remain unanswered. The first question is: what should be the right {\em granularity} to find the pixels that are important to final inference accuracy? 
% \jc{i know quality assignment has been sort of hinted, but this term is used without any introduction.}
Facing this question, previous work inherently assumes that the DNN-generated\jc{no need to stress they are dnn-generated. the focus here is region-based or object-based vs. fine-grained microblock-based} {\em bounding boxes} naturally crop those important pixels out~\cite{eaar,dds}.
% \jc{the next sentence doesn't seem to logically follow the previous one. shouldn't you say why the pixels in the same bounding box don't have the same importance?}
However, this assumption implies that the pixels outside the bounding boxes are not important to accurate inference. In fact, sometimes the surrounding pixels that locate outside of the bounding box of one object are still important to help the DNN separate the boundary between object and background. If those pixels are not encoded in high quality, the boundary between the object and the background might be too blurred for DNN to confidently detect that object.
Figure~\ref{fig:object-hqblock}(a) provides an illustrative example of this.\jc{need a bit handholding here. how exactly is the example figure illustrate the point? same thing with 1(b). }
On the other hand, this assumption also implies that the pixels inside one bounding boxes are similarly important and require high encoding quality.  However, for some of the pixels inside the object bounding box, like the smooth surface of a car, compression only do little change to their RGB values. So it is safe to compress them without hurting inference accuracy.
Figure~\ref{fig:object-hqblock}(b) provides a visualization.
\jc{this paragraph is a bit too long.. shrink it later}
% This misses the opportunity to compress those regions that encoding quality do not change the pixel values. 
% On the other hand, this implies the pixels that surround the bounding boxes and the background pixels like sky pixels are of the same importance. 
% This misses the opportunity to also encode the surrounding pixels to high quality to help the DNN to draw the boundary between objects and background. Figure~\ref{fig:object-hqblock} illustrates this phenomena.

% \jc{here, we should highlight the measurement results that fine-grained quality assignments do have high potential improvements}
Based on the observation above, we desire a more {\em fine-grained} approach to better discover those important pixels.
To empirically show its potential, We also design an idealized method and demonstrate the 3x file size reduction of this method against bounding-box-based approach in \S\fillme.
\jc{missing a lot of necessary details here: what's idealized method? 3x more video compression on what tasks? what prior solutions are bounding-box-based? }

\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/object-hqblock.pdf}
    % \includegraphics[width=0.8\columnwidth]{figs/fig5_allhq.pdf}
    
    % \includegraphics[width=0.8\columnwidth]{figs/fig5_parthq.pdf}
    \includegraphics[width=0.87\columnwidth]{figs/fig5.pdf}
    
    \tightcaption{
    % Inference results on images with different regions in high quality. 
    Illustrating mismatches between optimally selected high-quality blocks and object \kt{bounding boxes}.
    (a) Some objects need surrounding pixels in high quality to be detected and (b) some objects do not need to be all in high quality to be detected. \jc{add sub (a) and (b)}}
    \label{fig:object-hqblock}
\end{figure}






% The other research question is: how to decide the quality assignment in a {\em local and DNN-aware} manner? Most of the previous works extracts some knowledge from the server-side DNN and stream it to the camera side~\cite{noscope,reducto,eaar,dds,awstream}. However, these approaches have to prevent accuracy drop by frequently upload the video in full quality to the server to flush their profile~\cite{noscope,reducto,awstream} and thus require frequent server access. This limits their use cases to only those cameras with decent server connection.
The other research question is: given that the important pixels of DNNs need to be found in a real-time DNN-aware manner~\cite{awstream,dds,eaar,reducto}, how can we achive this goal when it is {\em not feasible} for the camera to stream the video out due to connectivity (like wild-life camera~\cite{deercam}) or privacy concerns (like home camera\jc{citation?})?
Surprisingly, previous works that achieve real-time DNN-aware do not apply in this scenario because these approaches all require a decent camera-server connection to prevent the profile to be outdated~\cite{reducto,awstream} or extrapolate feedback from server side~\cite{eaar,dds}. \jc{``decent connection'' is too handwavy. maybe show some concrete numbers: how much compute it needs if it runs a dnn locally? how much bandwidth it needs if the dnn is run remotely? and what are some concrete scenarios where privacy concerns precludes any data be sent out?}
% \jc{here, we should start with (1) why dnns are increasingly used in real time to help decide video encoding, then (2) why in some cases, the client can't rely on remote dnns or run a dnn locally. right now, both are mentioned but the logic is a bit buddy.}


% \jc{need to immediately describe the new features: microblock-level quality assignment for fundamentally better accuracy-compression tradeoffs? purely local encoding without need to run dnn? and importantly, connect these new features with the the two aforementioned questions (do they offer different answers?)} 
% \jc{hmm.. i thought we wanted to start with the two challenges: (1) how to make fine-grained quality assignment in real time? (2) how to customize the compression algorithm for any given dnn quickly? and THEN explain your key idea and how it addresses both challenges?}
To answer these questions, we propose \name, a new video encoder for DNN-based inference. 
This encoder leverage a cheap DNN to discover important pixels in a microblock-level granularity for a better accuracy-compression trade-off, and perform purely local encoding without the need to access the final DNN.
The key challenge for \name is two-fold:
\begin{packeditemize}
    \item How to discover the important pixels in a real-time, fine-grained manner while still being affordable for a cheap camera?
    \item How to customize \name for any given DNN {\em quickly and automatically}?
\end{packeditemize}
The key enabler to address these two challenges is our formulation of learning {\em accuracy gradients} (\AccuracyGradient). 
At a high level, \AccuracyGradient formulates how to choose the encoding quality of each spatial blocks to reach high accuracy while maintain low bandwidth. 
This sounds like a very computer-vision problem. However, what makes \AccuracyGradient stand out is that it enables following system optimization:
\begin{packeditemize}
    \item Reduction of \AccuracyGradientModel's inference cost.
    We reduce the cost of \AccuracyGradientModel in two ways.
    First, we observe that the compute cost of convolution is proportional to the resolution of the convolution input.
    This inspires us to reduce the resolution of intermediate features to save convolution costs.
    This will not hurt the performance of \AccuracyGradientModel because the output of \AccuracyGradientModel already has a much smaller resolution compared to its input, and thus we need to reduce the resolution inside \AccuracyGradient anyway.
    Second, we save compute cost by reusing the output of \AccuracyGradientModel generated from one frame to its following frames.
    To handle the accuracy drop due to reusing, we encode a little bit more microblocks in high quality to increase the temporal redundancy of \AccuracyGradientModel's outputs.
    % Through a cheap model ==> enables cheap estimation
    % Through reusing previous quality assignment ==> temporal redundancy
    % \AccuracyGradient will generate one single importance for each microblock. 
    % Thus, we can save compute cost through letting pixels inside the microblock share the same compute. 
    % \jc{this is really cryptic. are you talking about microblock-based vs. pixel-based quality assignment? if so, please say it that way and then explain why it simplifies the problem.}
    % \item False positive tolerance for less inference. \AccuracyGradient allows a microblock to be identified with little cost on compression ratio as important as long as those important microblocks are fully discovered. 
    % Thus, we can intentionally put some extra microblocks into high quality to enhance the temporal redundancy.
    \item Quick training
    A typical training approach for \AccuracyGradientModel to maximize the final inference accuracy is to feed the encoded frames generated from \AccuracyGradientModel's output to the final DNN.
    However, this approach requires using the final DNN in every training epoch, and result in slow training.
    To cut down this overhead, we leverage the differentiability of the final DNN to prepare the ground truth for \AccuracyGradientModel before starting to train train it.
    This will reduce the training overhead by 6x.\kt{do we need to support this number in the future sections?}
    Moreover, during our whole training process, we will only access two APIs that are fundamentally built in all neural networks: the training loss API, and the inference API.
    Thus, our training approach can generalize to different DNNs from different applications at ease.
    % \item Fully differentiable for quick training. 
    % The formulation of \AccuracyGradient is fully differentiable. 
    % This enables us to derive a cheap approximation of \AccuracyGradient that makes the training orders-of-magnitude faster.
    % \item Clean API for automatic customization.
    % The formulation of \AccuracyGradient only involves two API that are implemented across all DNNs (the training loss API and the inference API).
    % As a result, instead of developing DNN-specific tricks~\cite{dds,eaar}, it can easily customize itself to new DNNs in fully automatic manner.
\end{packeditemize}



% To address these questions, we propose \name, a new video encoder for DNN-based vision inference. 

% \begin{packeditemize}
%     \item Microblock-based. 
%     Each 16x16 blocks inside the input will share the same output. 
%     Thus, we can drastically save compute cost by letting the pixels inside 16x16 blocks share the same computation.
%     \item False-positive tolerance. 
%     One block can be wrongfully identified as encoding-quality-demanding block with little extra cost of file size as long as all the quality-demanding blocks are correctly identified. 
%     This enables us to reduce the compute cost by intentionally allowing some of the blocks to be classified as quality-demanding.
%     \item Fully differentiable. 
%     Our formulation is fully differentiable. 
%     This enables us to perform quick customization through generating closed-form ground truths for \AccuracyGradient.
%     \item Access DNNs only through their {\em built-in} APIs (the training loss API and the inference result generation API). This enables us to make our solution fully automatic, without creating new heuristics for new DNNs and applications~\cite{dds,eaar}.
% \end{packeditemize}





Admittedly, not every techniques of \name is exactly new: it uses off-the-shelf libraries~\cite{h264,h265} as its underlying video codec, and the concepts of encoding frames with spatially uneven quality levels and compressing videos in a DNN-aware manner have appeared in prior work. 
Nonetheless, with a unifying formulation in mind, \name develops new techniques to further reduce the compute cost and automatically generalizes to various video analytic DNNs.



As for the performance of \name, our evaluation shows that \name reduces half of the file size and achieves 4\% higher accuracy on four sets of video and three types of applications. 
The runtime overhead of \name's encoding and decoding stages are only marginally slower than the traditional codecs, and are much faster than the baselines that achieve similar compression efficiency.
Moreover, \name can quickly customize itself to a new DNN within just \fillme.


In short, the contribution of \name can be summarized as follows:
\begin{packeditemize}
    \item DNN-aware cheap compression. We develop a set of technique to enable DNN-aware compression that is affordable on a cheap camera.
    \item Quick customization. Our compressor can be easily customized within just \fillme.
\end{packeditemize}

==> intro-v5.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

Powered by modern computer vision, video analytics applications running on edge/mobile devices are poised to transform businesses (retail, industrial logistics, home assistance, etc), and public policies (traffic management, urban planning, etc)~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero,visionzero-bellevue, msr-bellevue}.
% Industry reports project that more videos are being created for analytical purposes than being watched by human users~\cite{infowatch12,infowatch16}.
These emerging video applications use ML models to analyze massive videos from sensors, creating a new breed of video traffic that serves analytical purposes rather than is watched by users~\cite{infowatch16,VideoAnalyticsMarket,slate-video-news}.

A key component of these applications is an efficient {\em video compression}\footnote{We use video compression and video encoding interchangeably} algorithm, which greatly compresses videos in realtime while preserving enough information to allow the final video-analytics DNN (deep neural net) to perform accurate inference (\eg object detection, segmentation)~\cite{vcm-news}. 


Prior work (\eg~\cite{vigil,dds,awstream,eaar}) in this space is driven by the discrepancies between the requirements of final video-analytics DNNs (called {\em final DNN}) on video quality and the quality objectives of standard video codecs (\eg H.264/MPEG). 
Unlike human-perceived quality which degrades gracefully with lower video quality, the final DNNs have great spatial heterogeneity in how the encoding quality affects their accuracy~\cite{dds,eaar}: 
in {\em quality-sensitive} regions, any drop of encoding quality may lead to incorrect inference result or render it useless, whereas in quality-insensitive regions, lowing the encoding quality may not affect the inference output of the final DNN at all.
% \jc{say a couple of sentences to explain WHY encoding videos this way doesn't make sense for human perception (or what would look more appealing to human viewers and whether that's what h264/265 optimizes for, etc)}

%We refer to these video-analytics models (in forms of deep neural nets or DNNs) as the {\em final DNNs}.


%The intuition that drives prior work is that there are significant discrepancies between the requirements of final DNNs on video quality and the quality objectives of current video codecs (\eg H.264/MPEG).
%Prior work\jc{a few relevant citations} has shown that, unlike human-perceptual quality (measured by SSIM/VMAF), lowering the encoding quality of certain regions does not affect the accuracy of the video-analytics DNN, whereas for other regions, any drop of encoding quality can lead to incorrect inference result or render it useless. 



While several schemes have been proposed to identify the ``quality-sensitive'' regions (where the encoding quality can greatly influence the final DNN's inference accuracy), we argue that they fundamentally fall short on two fronts.

\mypara{Finer-grained quality optimization}
First, what should be the spatial granularity to assign encoding quality within a frame?
The conventional choice, which is widely used in previous solutions, is to assign quality at the {\em coarse} spatial granularities of video frames~\cite{awstream,chameleon,glimpse,noscope,cloudseg} (\ie same quality per frame) or object-associated bounding box regions~\cite{eaar,dds,vigil} (\ie high quality only in one box-shaped region per object). 
However, we argue that these {\em frame-} or {\em object}-level encoding schemes are fundamentally inefficient. 
On one hand, 
%they assume that the pixels outside the bounding boxes are not important to accurate inference, but 
some surrounding pixels outside of the bounding box of an object can still be crucial for the final DNN to confidently detect and classify the object and locate its boundary from the background.
For instance, to detect the car in Figure~\ref{fig:object-hqblock}(a), one must encode not only its final bounding box but also some neighboring pixels of the bounding box in high quality.
% If those pixels are not encoded in high quality, the boundary between the object and the background might be too blurred for DNN to confidently detect that object.
% Figure~\ref{fig:object-hqblock}(a) provides an illustrative example of this.\jc{need a bit handholding here. how exactly is the example figure illustrate the point? same thing with 1(b). }
On the other hand,
% they assume that all pixels inside one bounding boxes are similarly important and thus require high encoding quality, but this is not true either. 
some pixels inside an object bounding box (\eg the smooth surface of a car or round in Figure~\ref{fig:object-hqblock}(b)) have similar RGB values regardless of the encoding quality, 
% compression only do little change to their RGB values. 
so it is safe to compress them aggressively without hurting inference accuracy.
% Figure~\ref{fig:object-hqblock}(b) provides a visualization.


\begin{comment}
Prior work in this space (\eg~\cite{awstream,dds,reducto,vstore,eaar}) has observed differences between the video quality requirements of video analytics tasks (\eg object detection, segmentation) and the widely used classic video codecs (\eg H.264/MPEG).
To address these discrepancies, 
the key insight is to discover those pixels that are important to final DNN inference and apply high encoding quality to them.
% Current solutions perform quality assignment through finding the region of interest of DNN and }
% \jc{``pays no attention'' is vague. please avoid such figurative terms}
To leverage this insight, the overarching trend of previous works is to evolve from finding important pixels through final-DNN-agnostic heuristics~\cite{vigil,glimpse} to finding those pixels in a final-DNN-aware manner\cite{reducto,awstream,dds,eaar,cloudseg}.\jc{``final-dnn-agnostic'' and ``final-dnn-aware'' sound awkward (and did we ever define what ``final dnn'' refers to?). actually, i dont see the need of this sentence at all. this paragraph should focus on the difference between human visual perception and dnn visual perception, NOT how one infers dnn's quality perception, right?}
Take object detection application as an example. As for object detection, previous works evolves from discovering key frames through frame difference~\cite{glimpse}, cropping out pixels that potentially contain objects through cheap DNNs~\cite{vigil} to find key frames based on extracting profile from the final DNN~\cite{reducto} and find important regions through extrapolating DNN's feedback~\cite{eaar,dds}. \jc{to put it in perspective, we should say WHY encoding videos this way doesn't make sense for human perception (or what would look more appealing to human viewers and whether that's what h264/265 optimizes for, etc)}
% \jc{the last sentence doesn't seem to be related to your argument that there are pixels that dnn doesn't care.}


Despite the rich literature in this line of research,
% \jc{paradigm seems unnecessarily grandiose} 
two research questions remain unanswered. The first question is: what should be the right {\em granularity} to find the pixels that are important to final inference accuracy? 
% \jc{i know quality assignment has been sort of hinted, but this term is used without any introduction.}
Facing this question, previous work inherently assumes that the DNN-generated\jc{no need to stress they are dnn-generated. the focus here is region-based or object-based vs. fine-grained macroblock-based} {\em bounding boxes} naturally crop those important pixels out~\cite{eaar,dds}.
% \jc{the next sentence doesn't seem to logically follow the previous one. shouldn't you say why the pixels in the same bounding box don't have the same importance?}
However, this assumption implies that the pixels outside the bounding boxes are not important to accurate inference. In fact, sometimes the surrounding pixels that locate outside of the bounding box of one object are still important to help the DNN separate the boundary between object and background. If those pixels are not encoded in high quality, the boundary between the object and the background might be too blurred for DNN to confidently detect that object.
Figure~\ref{fig:object-hqblock}(a) provides an illustrative example of this.\jc{need a bit handholding here. how exactly is the example figure illustrate the point? same thing with 1(b). }
On the other hand, this assumption also implies that the pixels inside one bounding boxes are similarly important and require high encoding quality.  However, for some of the pixels inside the object bounding box, like the smooth surface of a car, compression only do little change to their RGB values. So it is safe to compress them without hurting inference accuracy.
Figure~\ref{fig:object-hqblock}(b) provides a visualization.
\jc{this paragraph is a bit too long.. shrink it later}
% This misses the opportunity to compress those regions that encoding quality do not change the pixel values. 
% On the other hand, this implies the pixels that surround the bounding boxes and the background pixels like sky pixels are of the same importance. 
% This misses the opportunity to also encode the surrounding pixels to high quality to help the DNN to draw the boundary between objects and background. Figure~\ref{fig:object-hqblock} illustrates this phenomena.

\end{comment}


In contrast to assigning quality per bounding box (\eg typically greater than $128\times128$), we empirically show that assigning quality at the finer granularity of macroblocks (16$\times$16 blocks) can potentially improve video compression as well as inference accuracy.
%we choose to {\em assign quality at the finer granularity of macroblocks (16$\times$16 blocks)}. 
By analyzing 5 common final DNN models, we show that such macroblock-level quality assignments could increase the video compression by 3$\times$ while achieving the same inference accuracy, compared to baselines based on object bounding boxes or frames.
% \jc{please add some necessary details here: what's idealized method? 3x more video compression on what tasks? what is the baseline? }

% \jc{here, we should highlight the measurement results that fine-grained quality assignments do have high potential improvements}
% Based on the observation above, we desire a more {\em fine-grained} approach to better discover those important pixels.
% To empirically show its potential, We also design an idealized method and demonstrate the 3x file size reduction of this method against bounding-box-based approach in \S\fillme.
% \jc{missing a lot of necessary details here: what's idealized method? 3x more video compression on what tasks? what prior solutions are bounding-box-based? }

\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/object-hqblock.pdf}
    % \includegraphics[width=0.8\columnwidth]{figs/fig5_allhq.pdf}
    
    % \includegraphics[width=0.8\columnwidth]{figs/fig5_parthq.pdf}
    \includegraphics[width=0.87\columnwidth]{figs/fig5.pdf}
    
    \tightcaption{
    % Inference results on images with different regions in high quality. 
    Examples of inefficiencies of object-based encoding (high quality in the object bounding box):
    % between optimally selected high-quality blocks and object \kt{bounding boxes}.
    (a) Objects not detected unless nearby pixels are in high quality; and (b) Objects still detected even if just parts are in high quality.
    % (a) Some objects need surrounding pixels in high quality to be detected and (b) some objects do not need to be all in high quality to be detected. \jc{add sub (a) and (b)}
    }
    \label{fig:object-hqblock}
\end{figure}



% \myparashort{Requirement 2: On-premise DNN-aware video encoding.}
\mypara{On-premise video encoding optimization}
Second, how to encode videos in realtime on edge devices with only sporadic network connections or privacy concerns?
The previous findings suggest that the optimal encoding must be derived from the final DNN's quality sensitivity, and recent video-analytics pipelines also invoke the final DNN every frame~\cite{dds} or periodically~\cite{awstream,eaar} to adapt the encoding parameters to realtime content. 
However, these DNN-driven workflows are incompatible with edge devices that cannot run the final DNN at line speed (30fps) and cannot send the video out to a remote server in realtime due to the lack of continuous network connections (like wild-life camera~\cite{deercam} and low-end dashcam~\cite{cheap-dashcam}]) or privacy concerns (like home camera).
% Besides cheap on-premise encoding, an ideal encoding algorithm should not require major changes on the DNN analytics.
% \jc{do we need to emphasize that we can't change anything on the final dnn algorithm? maybe if we could, there can be different design points?}


\myparashort{\name: Fine-grained on-premise encoding optimization.}
%Therefore, we choose to design a video encoder that, {\em for any given DNN}, can identify {\em in realtime} quality-sensitive macroblocks of the DNN in each frame and encode video {\em on-premise using only local compute resources}. 
We present a new video encoder \name, which explores a new design point: fine-grained quality assignment {\em per macroblock} (as opposed to per object bounding box) and {\em on-premise} quality optimization (without invoking the final DNN).
For any given DNN, \name creates a quality selector to which we can feed any frame to detect quality-sensitive macroblocks of the DNN in realtime, and then encoded in high quality to strike a desirable accuracy-compression tradeoffs.
Realizing \name in practice, however, faces two challenges:
\begin{packeditemize}
\item {\em Challenge 1: How to detect the quality-sensitive macroblocks in realtime using only local compute resource of an edge camera?}
In other words, \name's encoding overhead should be on par with only running the video codec.
%    \item How to discover the important pixels in a real-time, fine-grained manner while still being affordable for a cheap camera?
\item {\em Challenge 2: How to quickly customize \name (ideally in a few minutes or less) for any given final DNN?}
What's more, an \name trained for one final DNN should also work decently with another DNN of similar task.
%    \item How to customize \name for any given DNN {\em quickly and automatically}?
\end{packeditemize}


% The other research question is: how to decide the quality assignment in a {\em local and DNN-aware} manner? Most of the previous works extracts some knowledge from the server-side DNN and stream it to the camera side~\cite{noscope,reducto,eaar,dds,awstream}. However, these approaches have to prevent accuracy drop by frequently upload the video in full quality to the server to flush their profile~\cite{noscope,reducto,awstream} and thus require frequent server access. This limits their use cases to only those cameras with decent server connection.
% The other research question is: given that the important pixels of DNNs need to be found in a real-time DNN-aware manner~\cite{awstream,dds,eaar,reducto}, how can we achive this goal when it is {\em not feasible} for the camera to stream the video out due to connectivity (like wild-life camera~\cite{deercam}) or privacy concerns (like home camera\jc{citation?})?
% Surprisingly, previous works that achieve real-time DNN-aware do not apply in this scenario because these approaches all require a decent camera-server connection to prevent the profile to be outdated~\cite{reducto,awstream} or extrapolate feedback from server side~\cite{eaar,dds}. \jc{``decent connection'' is too handwavy. maybe show some concrete numbers: how much compute it needs if it runs a dnn locally? how much bandwidth it needs if the dnn is run remotely? and what are some concrete scenarios where privacy concerns precludes any data be sent out?}
% \jc{here, we should start with (1) why dnns are increasingly used in realtime to help decide video encoding, then (2) why in some cases, the client can't rely on remote dnns or run a dnn locally. right now, both are mentioned but the logic is a bit buddy.}


% \jc{need to immediately describe the new features: macroblock-level quality assignment for fundamentally better accuracy-compression tradeoffs? purely local encoding without need to run dnn? and importantly, connect these new features with the the two aforementioned questions (do they offer different answers?)} 
% \jc{hmm.. i thought we wanted to start with the two challenges: (1) how to make fine-grained quality assignment in realtime? (2) how to customize the compression algorithm for any given dnn quickly? and THEN explain your key idea and how it addresses both challenges?}


 

%\mypara{Our solution}
%This paper presents \name, a new video encoder that achieves both fine-grained (macroblock-level) and on-premise DNN-aware quality optimization. 
%%To answer these questions, we propose \name, a new video encoder for DNN-based inference. 
%At a high level, \name uses a cheap model (a shallow neural network) to locate quality-sensitive macroblocks without running any inference by the final DNN, and once these macroblocks are encoded in high quality, \name can achieve a better accuracy-compression trade-off than prior solutions (even if they can run inference by the final DNN).
%%for a better accuracy-compression trade-off, and perform purely local encoding without the need to access the final DNN.
%%The key challenge for \name is two-fold:
%Realizing \name in practice, however, faces two systems challenges:
%\begin{packeditemize}
%\item {\em Challenge 1:} How to reduce the quality-sensitive macroblocks in realtime using only local compute resource of an edge camera?
%In other words, \name's encoding overhead should be on par with only running the video codec.
%%    \item How to discover the important pixels in a real-time, fine-grained manner while still being affordable for a cheap camera?
%\item {\em Challenge 2:} How to quickly customize \name (ideally in a few minutes or less) for any given final DNN? 
%What's more, an \name trained for one final DNN should also work decently with another DNN of similar task.
%%    \item How to customize \name for any given DNN {\em quickly and automatically}?
%\end{packeditemize}


\mypara{Key insight}
\name addresses the challenges using the concept of {\em accuracy gradients} or \AccuracyGradient (\S\ref{sec:accgradient}).
\AccuracyGradient of a macroblock measures how much the macroblock's encoding quality influences the final DNN's inference accuracy. 
\name uses a cheap model called {\em \AccuracyGradientModel} to infer the \AccuracyGradient of each macroblock and encoding macroblocks with high (or low) \AccuracyGradient in high (or low) video quality. 
Intuitively, doing so would lead to high accuracy of the final DNN while allowing efficient video compression.
While inferring \AccuracyGradient seems like a computer vision task\footnote{Though a few similar concepts exist in computer vision, \AccuracyGradient is distinct in that it captures the impact of both each macroblock's content and its encoding quality on DNN accuracy. See more discussion in \S\ref{??}.}, it in effect enables two system optimizations crucial to \name.

To address the first challenge, \name uses a cheap shallow neural net (VGG11~\cite{vgg}) as \AccuracyGradientModel (\S\ref{sec:encoding}).
It can still detect quality-sensitive macroblocks accurately, because its task (macroblock-level quality selection) is equivalent to low-dimensional segmentation; \eg assigning high or low quality to macroblocks of a 720p frame (1280x720) is equivalent to a binary segmentation problem on an 80x45 image, which is much simpler than most vision tasks today.
%\name further saves compute cost of \AccuracyGradientModel  by slightly expanding its selected high-quality macroblocks and reusing them across adjacent frames.

Second, the conventional computer-vision approach to training an \AccuracyGradientModel 
% to detect quality-sensitive macroblocks for a given DNN 
would run numerous forward and backward propagations of an entire encoding-inference pipeline on many training images. 
In contrast, \name separates the final DNN from the training of \AccuracyGradientModel.
We leverage the fact that the \AccuracyGradients of an image can be directly derived by treating the final DNN as a differentiable blackbox. 
Thus, \name first derive the correct \AccuracyGradient per macroblock of the training images (\S\ref{sec:training}); and
it then trains \AccuracyGradientModel as a standalone (low-dimensional) segmentation model to infer these \AccuracyGradients, for which we only need fewer training iterations and training images. 

%The key enabler to address these two challenges is our formulation of learning {\em accuracy gradients} (\AccuracyGradient). 
%At a high level, \AccuracyGradient formulates how to choose the encoding quality of each spatial blocks to reach high accuracy while maintain low bandwidth. 
%This sounds like a very computer-vision problem. However, what makes \AccuracyGradient stand out is that it enables following system optimization:
%\begin{packeditemize}
%    \item Reduction of \AccuracyGradientModel's inference cost.
%    We reduce the cost of \AccuracyGradientModel in two ways.
%    First, we observe that the compute cost of convolution is proportional to the resolution of the convolution input.
%    This inspires us to reduce the resolution of intermediate features to save convolution costs.
%    This will not hurt the performance of \AccuracyGradientModel because the output of \AccuracyGradientModel already has a much smaller resolution compared to its input, and thus we need to reduce the resolution inside \AccuracyGradient anyway.
%    Second, we save compute cost by reusing the output of \AccuracyGradientModel generated from one frame to its following frames.
%    To handle the accuracy drop due to reusing, we encode a little bit more macroblocks in high quality to increase the temporal redundancy of \AccuracyGradientModel's outputs.
%    % Through a cheap model ==> enables cheap estimation
%    % Through reusing previous quality assignment ==> temporal redundancy
%    % \AccuracyGradient will generate one single importance for each macroblock. 
%    % Thus, we can save compute cost through letting pixels inside the macroblock share the same compute. 
%    % \jc{this is really cryptic. are you talking about macroblock-based vs. pixel-based quality assignment? if so, please say it that way and then explain why it simplifies the problem.}
%    % \item False positive tolerance for less inference. \AccuracyGradient allows a macroblock to be identified with little cost on compression ratio as important as long as those important macroblocks are fully discovered. 
%    % Thus, we can intentionally put some extra macroblocks into high quality to enhance the temporal redundancy.
%    \item Quick training
%    A typical training approach for \AccuracyGradientModel to maximize the final inference accuracy is to feed the encoded frames generated from \AccuracyGradientModel's output to the final DNN.
%    However, this approach requires using the final DNN in every training epoch, and result in slow training.
%    To cut down this overhead, we leverage the differentiability of the final DNN to prepare the ground truth for \AccuracyGradientModel before starting to train train it.
%    This will reduce the training overhead by 6x.\kt{do we need to support this number in the future sections?}
%    Moreover, during our whole training process, we will only access two APIs that are fundamentally built in all neural networks: the training loss API, and the inference API.
%    Thus, our training approach can generalize to different DNNs from different applications at ease.
%    % \item Fully differentiable for quick training. 
%    % The formulation of \AccuracyGradient is fully differentiable. 
%    % This enables us to derive a cheap approximation of \AccuracyGradient that makes the training orders-of-magnitude faster.
%    % \item Clean API for automatic customization.
%    % The formulation of \AccuracyGradient only involves two API that are implemented across all DNNs (the training loss API and the inference API).
%    % As a result, instead of developing DNN-specific tricks~\cite{dds,eaar}, it can easily customize itself to new DNNs in fully automatic manner.
%\end{packeditemize}



% To address these questions, we propose \name, a new video encoder for DNN-based vision inference. 

% \begin{packeditemize}
%     \item macroblock-based. 
%     Each 16x16 blocks inside the input will share the same output. 
%     Thus, we can drastically save compute cost by letting the pixels inside 16x16 blocks share the same computation.
%     \item False-positive tolerance. 
%     One block can be wrongfully identified as encoding-quality-demanding block with little extra cost of file size as long as all the quality-demanding blocks are correctly identified. 
%     This enables us to reduce the compute cost by intentionally allowing some of the blocks to be classified as quality-demanding.
%     \item Fully differentiable. 
%     Our formulation is fully differentiable. 
%     This enables us to perform quick customization through generating closed-form ground truths for \AccuracyGradient.
%     \item Access DNNs only through their {\em built-in} APIs (the training loss API and the inference result generation API). This enables us to make our solution fully automatic, without creating new heuristics for new DNNs and applications~\cite{dds,eaar}.
% \end{packeditemize}


Using four sets of video, three types of canonical vision applications, and 5 recent off-the-shelf vision DNNs, we show that \name-encoded videos are 10-50\% smaller in size and achieve 1-5\% higher inference accuracy than state-of-the-art solutions (even when they run inference by the final DNN while \name does not run the final DNN).
%reduces half of the file size and achieves 4\% higher accuracy on four sets of video and three types of applications. 
Compared to basic video encoding, the encoding speed of \name is only marginally slower than (achieving 30fps with 3 CPU cores), and are much faster than the baselines that achieve similar compression efficiency.
Moreover, an \name encoder for a new DNN can be created within only several minutes.


%Then \name encodes only these quality-sensitive macroblocks in high quality, to achieve a better accuracy-compression trade-off than prior solutions (even if they can run inference by the final DNN).



Admittedly, not all techniques of \name are exactly new: 
it uses standard video codec libraries~\cite{h264,h265} that already support region-of-interest (RoI) encoding (\ie encoding different macroblocks at different qualities), 
that different regions influence computer-vision DNN inference differently has inspired techniques to speedup DNNs themselves and improve accuracy (\eg~\cite{wang2017residual,mnih2014recurrent}), 
and as mentioned earlier, the observation that DNN has spatially heterogeneous sensitivity to encoding quality has driven this line of work.
Nonetheless, \name makes two key contributions:
%the concepts of encoding frames with spatially uneven quality levels and compressing videos in a DNN-aware manner have appeared in prior work. 
%Nonetheless, with a unifying formulation in mind, \name develops new techniques to further reduce the compute cost and automatically generalizes to various video analytic DNNs.
%In short, the contribution of \name can be summarized as follows:
\begin{packeditemize}
\item Cheap model that selects encoding quality per macroblock (improve video compression and inference accuracy) using similar compute overhead as basic video encoding. 
\item Fast creation (within several minutes) of the quality selection model for any given final DNN and graceful degradation when the final DNN changes.
\end{packeditemize}
%\begin{packeditemize}
%    \item DNN-aware cheap compression. We develop a set of technique to enable DNN-aware compression that is affordable on a cheap camera.
%    \item Quick customization. Our compressor can be easily customized within just \fillme.
%\end{packeditemize}




==> intro.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}




% video analytics is popular
Video analytics applications, powered by modern computer vision, are poised to transform businesses (retail, industrial logistics, etc), technologies (intelligent assistance, video understanding, etc), and public policies (traffic management, urban planning, etc)~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero,visionzero-bellevue, msr-bellevue}.
%~\cite{??,??,??}.
Industry reports have projected that more sensor videos will be generated for analysis purposes than being watched by users~\cite{infowatch12,infowatch16}.
A key component in scaling out the emerging ecosystem of video analytics is a highly efficient {\em video stack}, which like in traditional video streaming, should compress (encode) videos with low delays for a range of DNN-based video analytics tasks without hurting their inference accuracy once the videos are decoded. 
%compresses raw frames to an encoded video and feed decoded frames to deep neural nets (DNN) inference. 
%Ideally, it needs to significantly compress the size of a video stream while preserving enough information in the encoded video that still allows for highly accurate DNN inference, and do so with low encoding and decoding delays. 
% DNN can achieve the decoded video to the DNN for high accuracy with low decoding and inference delay.
%{\em injects} (\ie encodes) and {\em consumes} a video stream (\ie decodes and feeds frames to inference models) with low latency and high inference accuracy for a range of vision inference tasks.


% many prior efforts but basically limited by the same video stack
While most efforts focus on efficient video analytics applications/pipelines, relatively less attention is given to the video stack running beneath these applications.
For the few works that do tune video encoding (\eg~\cite{awstream,dds}), they build on widely-used classic video codecs (\eg H.264/MPEG and DASH/HTTP streaming protocol) and propose ways to bridge the potential mismatches---the classic codecs may encode substantial redundant information not needed by DNNs and/or drop information vital to DNN inference.
%~\cite{dds,awstream,reducto,vstore}.

That said, these encoding techniques use heuristics that are jointly designed with particular video analytics tasks/pipelines in mind, and thus fall short when used in other video analytics tasks.
% rather than applicable to a broad range of applications.
In the meantime, these efforts offer little idea on how much a video could be compressed without hurting the accuracy of a video analytics task.
Although both issues are not unacceptable from a pragmatic standpoint, developing a {\em general}, {\em near-optimal} video stack, in our view, will provide a fundamental insight about encoding videos for video analytics purposes (as opposed to human perception).


%Current solutions are based on off-the-shelf video codecs (\eg H.264/MPEG and DASH/HTTP streaming protocol) originally designed to enhance human-perceived video quality.
%Recent work has highlighted potential mismatches between these codecs and DNNs' needs: the codecs may encode substantial redundant information not needed by DNNs and sometimes aggressively drop information vital to DNN inference (low inference accuracy)~\cite{dds,awstream,reducto,vstore}.
%rather than the performance of computer vision models. 
%\jc{a few examples}


% our basic observation is that the importance of pixels to the final accuracy is disproportion to the fraction of such pixels

Thus, in this work, we set out to design such a video stack. In doing so, we take a practical stance by also building our video stack on existing video codecs. 
But we develop our solution through answering two key questions:
\begin{packedenumerate}
\item What is the {\em optimal} compression efficiency that still preserves enough information to maintain high DNN inference accuracy?
% quality level (\ie maximum compression level) that still preserves the inference accuracy of a given vision task?
%much do different levels of compressions on each pixel affect the accuracy of various vision inference tasks?
\item How can a video stack {\em practically} approximate the optimal compression on a {\em wide} range of video analytics applications?
% efficiently compress each pixel at the lowest quality level that still preserves the inference accuracy?
\end{packedenumerate}
The former examines the fundamental tradeoff between compression efficiency and inference accuracy, and the latter seeks to approximate it in practice.



% Our work is a step towards answering both questions.
To answer the first question, we begin with a measurement study (\S\ref{sec:potential}) to understand, across a diverse set of video analytics applications, the spatial distribution of lowest quality level across {\em fine-grained blocks} (16$\times$16 each) such that the inference results remain as if the whole frames are encoded in a high quality. 
Contrary to the conventional beliefs in prior work, our analysis reveals that
% Compared to similar prior attempts, our analysis is unique in two aspects.
\begin{packeditemize}
\item 
% We study the {\em spatial} distribution of minimum quality at the level of fine-grained of blocks which is much smaller than objects or bounding boxes (which are commonly used~\cite{dds,eaar}). 
the minimum set of blocks that need high quality are often misaligned with objects or bounding boxes (which are commonly used to delineate the encoding boundaries in prior work~\cite{dds,eaar}), and
% Our analysis reveals that highly quality sensitive regions (\ie encoding them at even slightly lower quality can alter the result) can be much smaller than suggested in previous studies. 
% , and that the quality sensitive regions can vary dramatically across frames.
\item 
% Our analysis spans {\em more vision tasks} (object detection, semantic segmentation, and keypoint detection) than a single one~\cite{eaar,glimpse} and reveals that 
the minimum set of blocks that need high quality varies substantially across the vision tasks and even the DNNs of the same task (which suggests the encoding cannot be agnostic to the final DNN).
% For instance, \jc{an example.}
\end{packeditemize}



% we found today's codec is fundamentally ill-suited to this task

Inspired by these measurement-driven insights, we then present {\em \name}, an efficient video stack 
% (including injection and consumption) 
for DNN-based vision inference tasks.
\name provides three operations to video analysts:
a {\em preparation} phase (offline) where \name takes a given DNN model and a loss function (accuracy metric) to create a custom instance of stack;
an online {\em encoding} phase takes compresses frames from a source to a compressed video; and
% source from which frames can be read and then compressed.
an on-demand {\em decoding} phase reconstructs video frames and feeds them into the DNN for inference.
% a time window in which the video will be \kt{decoded} and feed into the DNN for inference.
% \end{packeditemize}

% \begin{packeditemize}
% \item {\em Preparation (offline):} The DNN model, loss function (accuracy metric) based on which \name creates a custom instance of stack for the particular DNN and loss function;
% \item {\em Injection (online):}  The video source from which frames can be read and then compressed.
% \item {\em Consumption (on demand):}  A time window in which the video will be \kt{decoded} and feed into the DNN for inference.
% \end{packeditemize}

% \kt{Maybe also emphasize that accuracy gradient can efficiently explore a large design space with just a single forwarding and backwarding?}

The key behind \name is the new concept of {\em accuracy gradients} (\ags).
\kt{Maybe substitude AG with AccGrad?}
% some encoding of a frame (with spatially different quality) are the gradients of the similarity between final DNN's output on that encoding and its output on the high-quality encoding. 
Intuitively, the \ag of each fine-grained spatial region measures how quality change at the region affects the inference accuracy of the DNN (\S\ref{sec:framework}).
\Ags have two unique advantages.
First, they can be calculated by a feedforward and backpropagation operation on {\em any} differentiable final inference model (\ie we treat it as a \kt{differentiable} ``black box'') and are thus applicable to a variety of DNN-based vision tasks.
Second, the knowledge of \ags naturally indicates the minimum regions that have to be preserved at high data fidelity, which can be used to assign spatially heterogeneous quality for highly efficient video compression and accurate DNN inference.
% , as well as which regions regions (\eg some parts of the background) can be totally insensitive to quality, suggesting that it can be completely replaced with a fixed value or even removed, which enables more efficient video encoding and faster inference.


Nonetheless, designing a practical \ag-based video stack is challenging.
To this end, \name presents concrete design choices to address two key challenges:
% fully realizing the benefits of accuracy gradients in practice is challenging, and our design and implementation of 
%To address them, \name presents two techniques:
\begin{packeditemize}
%\item {\em Fast accuracy-gradient estimator (\S\ref{sec:??}):} 
\item {\em How to train an accurate light-weight model to infer \ags (\S\ref{sec:training})?} 
\name infers \ags using a shallow neural network. 
We also design a custom loss function to pitfalls in learning \ags that have highly imbalanced value distributions.
%For a given DNN and loss function, we train a light-weighted model (\fillme DNN) that takes a frame as input and outputs a ``heatmap'' in which the score of a region (\eg a $16\times16$ block) indicates the minimum quality at which the region should be encoded in order to achieve a similar accuracy as if it were encoded at a higher quality.
%To make this estimator run as fast as the video codec, we run it only once every \fillme frames. 
%\item {\em Reusing existing video codec (\S\ref{sec:??}):} 
\item {\em How to reduce the extra runtime overhead caused by the use of \ags (\S\ref{sec:runtime})?} 
\name supports several optimizations, including updating the \ags only on sampled frames and using uniform color to speed up multi-quality encoding.
%Instead of inventing a new video codec from scratch, \name takes a pragmatic stance to reuse existing video code (\eg \fillme). 
%It spatially splits each frame into multiple versions, each containing regions to be encoded at the same quality level, and encode individual version using the off-the-shelf codec which is highly optimized to encode frames at a given quality. 

% \item {\em Spatial batching of inference (\S\ref{sec:??}):} 
% \name batches the processing of low-quality images and spatially stitches small blocks of high quality regions before feeding them into the DNN inference. 
% This optimization greatly reduces the amortized inference delay per frame.
% consumption can be greatly sped up by spatially batching the masks 
\end{packeditemize}
We will elaborate the rationale of these design choices in \S\ref{sec:training},\ref{sec:runtime}.

Admittedly, no individual technique of \name is exactly new: it uses off-the-shelf library as its underlying video codec, and the concepts of encoding frames with spatially uneven quality levels and compressing videos in a DNN-aware manner have appeared in prior work. 
Nonetheless, as a concrete system that integrates these components based on the concept of accuracy gradients, \name outperforms existing solutions and generalizes to a wide range of video analytics applications.
Our evaluation shows that compared with the state-of-the-art baselines across three video analytics applications, \name achieves \fillme\% higher compression efficiency and \fillme\% higher accuracy on \fillme sets of video in diverse genres. Moreover, \name's encoding/decoding delays are almost the same as the traditional codec.
In addition, like traditional codecs, \name also provides parameters which operators can tune to navigate on the improved tradeoff frontier between compression and utility (accuracy).


\jc{show an example result?!}

\jc{change all full dnns to final dnns}


%\jc{accuracy stability?}

%\jc{eval summary}

%\begin{itemize}
%\item video analytics is becoming popular
%\item though efforts were made to improve performance (in accuracy, streaming delay), the video stack is largely intact. 
%\item however, video analytics results have drastically different sensitivity to the fidelity of different pixels, and only a small fraction of pixels have to preserve very high fidelity. 
%(in contrast to dds, eaar or vigil, a highly sensitive portion can be just a small part of an object/region). 
%\item existing video stack is ill-suited: (1) highly sensitive pixels are \kt{DNN-specific and} not what humans vision focus on \kt{A figure that illustrates the difference between visually-pleasing image and DNN-pleasing image}, (2) they dont change smoothly as motion vectors, and\kt{existing video stack consume all pixels in the frame, even most of them do not contribute to the inference results.}
%\item this paper presents \name, a new video stack (including encoding, decoding, and consumption) for vision inference, based on the key insight that: the highly sensitive regions can be derived based on the generic concept of {\em accuracy gradient}.
%\item for developers, \name provides an interface to specify DNN execution and loss functions, and automatically customizes the injection and consumption pipeline. 
%\item \name entails three novel techniques:
%\begin{itemize}
%\item technique \#1: accuracy gradients (and the resulting mask) can be inferred using a small model
%\item technique \#2: the mask can be smoothed so as to enable efficient encoding using existing codec
%\item technique \#3: consumption can be greatly sped up by spatially batching the masks 
%\end{itemize}
%\item additional benefits: \name can easily scale to multiple applications with one stack.
%%\item inspired by the insight, we envision a new video codec (\fillme); execution framework (\fillme)
%\item the underlying techniques are not new: still use the mpeg functionalities but add a shim layer between DNN and mpeg.
%\item design details
%\item eval summary
%\end{itemize}










==> motivate-v2-deprecated.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Background}



\kt{
\begin{itemize}
\item background on video stack
\begin{itemize}
\item high-level relevant notions: frames, blocks, motion vectors, quality objectives, etc
\item traditional goals: efficient encoding (injection), storage/streaming, and efficient consumption (decoding + rendering)
\item mention dnn-based
\end{itemize}

\item background on video analytics: object detection, keypoint detection, segmentation, etc [illustrative graphs]
\item use of codec in video analytics
\begin{itemize}
\item offline analytics
\item online streaming+analytics
\item goals: fast encoding, small file sizes (injection) + high accuracy, low decoding and inference delay (consumption).
[illustrative graphs]
\end{itemize}
\end{itemize}}

%\subsection{Background}


\kt{Stack: a whole piece of software: injection; define consumption phase}

We start with the background of typical video-related operations in video analytics applications, how these operations may affect video analytics performance, and these effects should be evaluated. 

\mypara{Video stack} 
Like video applications that serve human viewers, video-analytics applications also requires a {\em video stack} to perform two high-level operations: 
(1) {\em video ingestion} where it encodes a video stream frame-by-frame into a compressed video file for efficient storage and transmission, and (2) a {\em video consumption} where it decodes the file to individual frames/segments which are in turn fed into a DNN for vision inference.
These operations are needed for both offline analytics on archived videos (\eg~\cite{focus,vstore}) and online analytics on streamed videos (\eg~\cite{dds,awstream}).

\jc{need a double-column visualization of the whole pipeline here!}

%Video stack compresses the video frame-by-frame to reduce the file size for easy storage (injection phase), and de-compresses the video back to frames to serve their users (consumption phase). 
%Traditional video stack aims to serve human viewers. To meet the visual quality requirement of human viewers, the goal of the video stack is efficient encoding during injection phase, real-time decoding and preserving satisfying visual quality during consumption phase.

\mypara{Various encoding techniques}
So far the computer vision and video analytics are largely built on used existing video encoding/decoder (codec), such as H.264/265~\cite{??} and VP8/9~\cite{??}. 
After years of involution, these codecs embed deep understanding of human visual perception and leverage hardware accelerator, and thereby can strike a good balance between high visual quality, minimal compressed file size, and encoding/decoding delay.
%\mypara{Block-based encoding}
Typical techniques include \jc{explain some examples. in the process, introduce the notion of blocks, motion vectors, qp, etc}
Nearby pixels have redundant mutual information. Thus, traditional video codec partite pixels into blocks and encode them based on the quantization parameter (QP).

\mypara{Vision tasks under consideration} 
We consider three computer vision tasks-object detection, semantic segmentation and keypoint detection. Figure \fillme shows an example input and output of object detection (one labeled bounding box for each object), semantic segmentation (one label for each pixel) and keypoint detection (17 keypoints for each human).


\mypara{Performance objectives of video stack}
In contrast to maximizing human viewers' visual experience, however, video analytics seek high inference accuracy and low delay (especially when extracting important information from massive video feeds), thereby posing new requirements on both the video ingestion and consumption.
In particular, in the context of video analytics, the performance of a video stack should be evaluated along six metrics.
\begin{packeditemize}
\item In the ingestion phase, it needs to have low {\em encoding delay} per frame, high {\em encoding throughput} (number of frames encoded per second), and high {\em compression efficiency} (higher reduction in file size).
\item In the consumption phase, it needs to have low {\em inference delay} per frame, high {\em inference throughput} (number of frames analyzed per second), and {\em high inference accuracy}. 
\end{packeditemize}
\jc{a few words on how we calculated inference accuracy and how is it diff/similar to prior work}


\mypara{Our goal} 
In this work, we set out to design a custom video stack for video analytics applications.
In doing so, we take a pragmatic stance to optimize the existing codec, rather than creating a video codec from scratch, for two reasons.
First, these codecs have efficient (hardware-assisted) implementation and have been widely adopted in industry.
Second, there is a rich space of optimization on top of existing codec, and although recent work has taken some initial steps, there is still a substantial untapped room for improvement as we will show in the next section.
Finally, in a real video stack, we assume that one cannot run the eventual DNN inference on the original video (otherwise, one can simply store the DNN output). 

%Video stack serves video analytics in two scenarios: store the video for offline analytics and stream the video for online analytics. In these two scenarios, video stack must be able to provide video frames at a high frame rate to saturate the following analytic DNN. Moreover, video stack should also allow the following DNN to generate accurate analytic results as if the DNN is directly operating on the raw frames. Thus, the goal of video stack for video analytics is:
%{\em Encoding delay}
%{\em Encoding throughput}
%{\em Compression efficiency}
%{\em Inference delay}
%{\em Inference throughput}
%{\em Inference accuracy}
%    \item \textit{Efficient encoding}. 
%    \item \textit{Efficient decoding}.
%    \item \textit{High accuracy.}


\section{Potential for Improvement}

There has been some previous proposals to tune certain parameters of existing codec, the choice and tuning of parameters have been based on handcrafted heuristics and sometimes purpose-built. 
So before presenting our proposal, we first motivate the need for a new design in two logical steps.
\begin{packedenumerate}
\item We analyze an ``idealized'' design point, which achieve minimum file size and highest accuracy using the hindsight information of DNN inference results. 
This serves a point of comparison of idealized performance improvement. 
\item Through analyzing the source of efficiency of the idealized design point, we can crystallize the key limitations in existing solutions as well as the requirements of a ``practical'' solution to approximate the idealized performance improvement.
\end{packedenumerate}
This section will focus on compression efficiency (compressed file size) and inference accuracy, since our goal here is to understand the (near-)optimal encoding efficiency based on existing codec, rather than realizing the optimal implementation with minimum encoding delay.



%\subsection{Opportunity: block-wise quality sensitivity for better compression}





\kt{0. Methodology w/ real encoding 1. High compress efficiency. 2. The counter-intuitive part of mask a). does not align with object boundary; (have surrounding pixels, and have surrounding pixels) b). varies a lot with content and DNN model. 3. connect to related work. 4. Plot pseudo-graph}

\kt{
\begin{itemize}
\item define ``quality sensitivity'' per block: if block $i$'s quality drops from $q$ to $q'$ while all other blocks remain at $q$, how much will accuracy drop?
\item explain the methodology: dataset, methodology (block-wise enumeration). 
\item three main takeaways from the measurements:
\begin{itemize}
\item only a small fraction of blocks need high quality (despite large objects) [graphs: y = cdf, x = fraction of pixels. one line for pixels that could be in same color, and another line for minimum pixels that must be in high quality]
\item if DNN only sees a small fraction of blocks, it can still infer accurate results
\item these highly quality-sensitive blocks may not align with objects or inference results [illustrative graphs of some case studies]
\end{itemize}
\end{itemize}
}


\subsection{Idealized design point}

The basic intuition is that different parts of each frame may have different importance to the accuracy of the inference result. 
If a region is not associated to any inference result (\eg a background building far away from the detected vehicles), it could be encoded with very low quality (or even blacked out).
Likewise, when a whole frame does not contain information immediately related to the inference results, its quality can be aggressively lowered (or safely skipped). 
In other words, only a portion of the pixels are {\em quality sensitive}.


To show the effectiveness of encoding videos with spatiotemporally different quality levels, we consider a simple design point.
Given a video (originally encoded in the highest quality) and a DNN model, it first splits each frame into small blocks (by default, 16 pixels by 16 pixels), assigns each block either a high quality $\HighQuality$ or a low quality $\LowQuality$, and then encodes the frames into a low-quality video and a high-quality video, each containing only blocks assigned with the perspective quality (Figure~\ref{??} depicts an example). 
During inference time, the two videos are decoded and the blocks are put in their original positions in the frames, and the frames are then fed in the DNN for inference. 

In the idealized design point, the assignment of quality per block is such that the DNN inference accuracy is maximized while no more than $\MaxHighQualityFrac$. 
To measure its potential, we assume that the quality assignment logic can run the DNN (\eg to test its accuracy on any quality assignment). 
\jc{explain the optimization algorithm}


We acknowledge that the formulation entails three simplifying assumptions: it restricts the choice of encoding quality to two levels; there are more efficient encoding methods, such as region-of-interest encoding, for videos with a spatially different quality levels than creating two separate video files; and the $16\times16$ square blocks may not align with the optimal boundaries between regions that require different quality levels.

Nonetheless, we believe that analyzing this formulation is still valuable. 
In some sense, it generalizes the design space of several recent solutions: \jc{why it generalizes vigil, dds, awstream, glimpse, reducto}






%\mypara{Block-wise quality differentiation}
%For DNN-based analysis, the power to impact accuracy is not evenly distributed between pixels.
%Thus, we can save bandwidth by aggressively lowering the pixels that does not impact accuracy too much.
%At codec level, however, the quality of pixels are organized by blocks.
%Inside each block, the quality of pixels are the same.
%Thus, block is the minimum granularity for quality differentiation.

%\mypara{Mask}
%To quantify the compression opportunity of quality differentiation, we present a concept: \textit{mask}.
%\textit{Mask} maps each block to its corresponding encoding quality.
%
%\mypara{Potential bandwidth saving} 
%We measure the potential bandwidth saving of this opportunity on VisDrone dataset~\cite{aiskyeye} with object detection model FasterRCNN-ResNet50~[\fillme] as our backend model. 
%We use two different encoding qualities: low quality and high quality\footnote{\fillme} to encode each block.
%To determine the encoding quality of each block, our steps are:
%\kt{Substitude this into an algorithm for general vision tasks}
%\begin{packedenumerate}
%    \item Encode the whole video in high quality and collect the bounding box $b_i$ for each object $i$.
%    \item For each object, we assign a new bounding box $b'_i$, of which the center is the same with $b_i$ and the size of this bounding box is $0$.
%    \item Partition the whole frame into 16$\times$ 16 blocks.
%    \item Use highest quality to encode those blocks that overlaps with any of $b'_i$, and use lowest quality to encode other blocks.
%    \item If less than 95\% objects are detected, for those objects $j$ that are not detected, enlarge $b'_i$ by padding a constant on the left, top, right, bottom on it, and go back to step 3.
%\end{packedenumerate}


% One way to save bandwidth is to reduce the encoding quality.
% Also, the power to impact accuracy is not evenly distributed between pixels.
% It follows that we can saving bandwidth through manipulating pixel encoding quality.
% However, the pixels inside the same block (determined by the codec) will always have the same quality.
% So we instead encode

% \mypara{Heterogeneous quality sensitivity requirements} 
% Different vision models care about different parts in the video. For example, vehicle detection models care car pixels much more than human pixels; and human detection models care human pixels much more than car pixels. In terms of encoding, it means that different vision models are more sensitive to the encoding quality of some blocks more than other blocks.

% This opportunity implies that we can save bandwidth if we encode those quality-sensitive blocks in high encoding quality and those quality-insensitive blocks in low encoding quality.

% \blindtext


\subsection{Improvement analysis}

We measure the potential improvement of the idealized design point on one of our video datasets (more details in \S\ref{subsec:eval:setup}), which consists of \fillme drone camera videos (\fillme minutes in total), and use \fillme and \fillme as the high and low quality level, and \fillme as the codec. 
We choose these videos since they include a variety of scenarios (urban and rural), object classes (various vehicles and pedestrians), viewing angles, and object sizes. 
\S\ref{sec:eval} will compare various techniques on a wider range of video sources.



\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \caption{Percentage of pixels encoded in high quality v.s. accuracy. Only 2\% of the pixels need to be encoded to make accuracy more than 0.95.}
    \label{fig:percpixel-accuracy}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figs/object-hqblock.pdf}
    \caption{Inference results on images with different regions in high quality. Some objects do not need to be all in high quality to be detected, and some objects need surrounding pixels in high quality to be detected.}
    \label{fig:object-hqblock}
\end{figure}

\begin{figure}
    \centering
\includegraphics[width=0.4\columnwidth]{figs/hetero-task.pdf}
    \caption{Accuracy on different task with the same compressed video. One size does not fit for all vision tasks.}
    \label{fig:hetero-task}
\end{figure}

\begin{figure}
    \centering
\includegraphics[width=0.4\columnwidth]{figs/hetero-dnn.pdf}
    \caption{Accuracy on different object detection DNN with the same compressed video. Accurate compression for cheap model may not work on expensive model.}
    \label{fig:hetero-dnn}
\end{figure}



Our analysis of the idealized design point shows three key observations.

\vspace{0.1cm}
\noindent{\em {\bf Observation \#1:} Fractions of quality-sensitive pixels are even less than claimed by previous work.}
\vspace{0.1cm}


We first examine the {\em quality-sensitive blocks} (\ie blocks assigned with $\HighQuality$) as a fraction of all blocks in three of the canonical video analytics tasks: object detection model (\fillme), key point detection (\fillme) and semantic segmentation (\fillme).
Figure~\ref{fig:percpixel-accuracy} shows the distribution of the quality-sensitive block fraction across frames in the videos. 
Across the three tasks, we can see that only encoding \fillme-\fillme\% blocks in high quality still yield more than \fillme-\fillme\% of accuracy.

To put it in perspective, we zoom in on the object detection task and compare this idealized design with two other ways of selecting quality-sensitive blocks: one selects the blocks that overlap with one of the final detected bounding boxes, and the other one selects the blocks that overlap with one of the region proposal bounding box. 
(To show the full spectrum of their effectiveness, these strawmen are tested with a varying confidence score on the bounding boxes or the region proposals.)
Intuitively, these two strawmen assume that only regions of the difficult-be-detected objects need to be encoded in high quality, which represents the basic premise behind the state-of-the-art techniques~\cite{??,??}. 

Figure~\ref{??} shows the fraction of quality-sensitive blocks and the resulting accuracy of the idealized design and the two strawmen. 
\jc{some numbers from the graph}

A natural question therefore is what the source of improvement of the idealized design point is.
In other words, what have the strawmen missed in their assumptions.

\vspace{0.1cm}
\noindent{\em {\bf Observation \#2:} Quality-sensitive regions are not aligned with inference results (\eg objects, boundaries).}
\vspace{0.1cm}

To begin with, we observe that the quality-sensitive blocks selected by the idealized design are largely {\em not} aligned with the detected bounding boxes or region proposals. 
Figure \ref{fig:object-hqblock} uses two example frames to illustrate this observation. 
On one hand, we see in (a) that some objects cannot be detected in low quality, but do not need entirely encoded in high quality either. 
Instead, the objects can be detected at the right locations when only parts of each object are encoded in high quality.
On the other hand, we see in (b) that some objects cannot be detected even if they are entirely encoded in high quality. 
Instead, parts of the surrounding blocks have to be encoded in high quality as well.
\jc{maybe there are blocks that are not associated with any detected object, but need to be in high quality just to winnow out non-objects?}
\jc{can we plot a summarizing graph to show how prevalent such misalignments are?}


\vspace{0.1cm}
\noindent{\em {\bf Observation \#3:} Quality-sensitive regions are highly dependent to the inference task and DNN.}
\vspace{0.1cm}

Given that the detected bounding boxes or the final inference results (even if they are known) are a poor indicator of quality-sensitive blocks, what decides the quality-sensitive blocks then?
Empirically, we found that the quality-sensitive blocks are highly sensitive to the DNN and the inference task. 
To analyze this dependency, Figure~\ref{fig:??} takes three different object detection DNNs as an example and compares their accuracies on the video encoded with its corresponding quality assignment and on the  videos encoded with the other two models' quality assignments.
We see that the accuracy of a DNN drops substantially when it runs on the quality assignment of design for other models.
Zooming in, we found that although each model's quality-sensitive regions look like Figure~\ref{??}, the exact blocks that have to be encoded in high quality change across the DNNs, even though they are trained to detect same objects!
\jc{some numbers from the graph}
\jc{can the resulting map be different if you just run the idealized algorithm on the same DNN again?}
By the same token, Figure~\ref{fig:??} shows that quality drops even more obvious if one encodes the video with the same quality assignment for different inference tasks. 
\jc{some numbers from the graph}

%This compression opportunity varies a lot between different vision tasks and models.
%In other word, one mask that works perfectly for one application might result in poor accuracy in another application.
%In Figure \ref{fig:hetero-task}, accurate compression for keypoint detection does not work on object detection and semantic segmentation.
%So compression need to be designed for different applications.
%Moreover, in Figure \ref{fig:hetero-dnn}, we see that even under the same vision task, compression that works for one DNN may not work on others.




%\mypara{Takeaways} During the measurement above, we find that:
%\begin{packeditemize}
%    \item To reproduce satisfactory inference result, only a small fraction of blocks need to be encoded in high quality. From Figure \ref{fig:percpixel-accuracy}, we can see that covering only \fillme\% pixels will yield more than \fillme\% of accuracy.
%    \item Object may not align with the high-quality blocks. From Figure \ref{fig:object-hqblock}, we see that some objects do not need to be all in high quality to be detected, and some objects need surrounding pixels in high quality to be
%\end{packeditemize}
%
%\mypara{Heterogeneity between vision tasks and models}
%This compression opportunity varies a lot between different vision tasks and models.
%In other word, one mask that works perfectly for one application might result in poor accuracy in another application.
%In Figure \ref{fig:hetero-task}, accurate compression for keypoint detection does not work on object detection and semantic segmentation.
%So compression need to be designed for different applications.
%Moreover, in Figure \ref{fig:hetero-dnn}, we see that even under the same vision task, compression that works for one DNN may not work on others.
%
%\blindtext



\subsection{Mismatch of existing solutions}

\kt{
\begin{itemize}
\item{Human perception-centric quality encoding}
\begin{itemize}
\item the highly sensitive blocks are highly dependent on the task
\item existing heuristics are completely unaware of the server-side dnn structure
\item implications: need a generic way to encode videos in cognizant of the block-level sensitivity. [an illustrative example]
\end{itemize}
\item{Encoding dynamic quality sensitivity}
\begin{itemize}
\item the highly-sensitive pixels changes a lot across frames
\item today's encoding is inefficient: unnecessary motion vector, etc.  micro-block misalignment
\item implications: need a way to ``smooth'' the highly dynamic sensitive blocks [an illustrative example]
\end{itemize}
\item{Frame-wise semantics}
\begin{itemize}
\item analyzing the whole frames one by one
\item implications: putting sensitive regions together [an illustrative example]
\end{itemize}
\end{itemize}}


In general, prior work on video stack propose either new codecs or smarter ways of compressing/streaming videos over existing codecs.
In this context, we now discuss potential mismatches in both directions with respect to what an idealized video stack need.



As mentioned earlier, the idealized algorithm essentially explores a similar design space of previous work, but at a different (finer) granularity (small blocks instead of bounding boxes) and with access to the DNN (such that we can reveal the ideal improvement).
By analyzing the encoding decisions made by the idealized design, we found two 


\mypara{Limitation of existing work} 
Wrong assumptions of related work was revealed by our measurement study above. 
The vast majority of current works on quality differentiation~\cite{dds,vigil,glimpse,eaar} implicitly assumes that high quality regions should align with the objects.
However, in Figure \ref{fig:object-hqblock}, we see that high quality regions can be much smaller or much larger than the object itself.
So objects might be missed or file size might be wasted if aligning high quality regions with objects.



\mypara{Traditional video codec}
Caring about visual quality, traditional video codec pays nearly equal attention to all pixels. 
The quality-sensitive blocks, however, are highly dependent on server-side DNNs.
Traditional video codec is unable to exploit this opportunity due to its unawareness to server-side DNN.
This implies that we need a generic way to encode the videos in cognizant of block quality-sensitivity, see Figure \fillme for an illustration.

\mypara{Super resolution}
Nowadays, super resolution \cite{cloudseg,livenas} gradually becomes a new choice of video codec.
These approaches encode the video in low quality, store or stream the low quality video at server side, and then compensate the quality loss by super resolution network.

However, super resolution is fundamentally an ill-suited problem. Multiple high-quality frames may have exact same low-quality frames if compressed by the codec.
As a result, even the most compute-intensive super resolution network cannot fully recover the areas crucial to inference results. Figure \fillme shows an example.
To overcome this issue, current approaches choose to retrain the neural network online. This design choice poses too much online cost at the server side.

\mypara{Auto-encoder}
Computer vision community is actively exploring a new type of codec called auto-encoder~\cite{rate-distortion-autoencoder}. These approaches encode the video by feeding it through neural network and storing the output of that neural network. 

Unfortunately, auto-encoder that preserves high image quality is too compute-intensive for a single CPU to afford (\fillme seconds per frame).
Moreover, this approach requires another neural network as the decoder. Thus, every frame needs to be processed by the decoder at inference time and poses too much online overhead. 



\subsection{Mismatch of existing video analytics pipelines}

\kt{Benefit different vap, weaken this argument}

\kt{
\begin{itemize}
%\item approach \#1: twisting existing interface, (2) case-by-case heuristics
\item limitation \#1: fail to adapt to real-time video content (sr, awstream, vstore)
\item limitation \#2: slow costly (dds, dnn-based autocodec)
\item limitation \#3: only applies to one task (vigil, eaar, focus)
\end{itemize}}

Video analytic pipelines stream videos from the camera to the server and generate analytic results with minimum overhead as well as maintaining satisfying accuracy. However, these approaches are not suitable for video stack purpose.

\mypara{Agnostic to real-time video content} 
AWStream~\cite{awstream} and CloudSeg~\cite{cloudseg} exploit the optimal configurations~\cite{awstream} or  super resolution networks~\cite{cloudseg} derived from \textit{history video content} and count on the similarity between real-time video content and history video content.
However, in real world, the video content can change drastically. 
For example, when a car equipped with traffic camera driving on a street that human rarely appears, the system needs to adapt every time human appears to detect all of them.
These approaches are likely to have low accuracy in these scenarios.

\mypara{Too much online cost for real-time content adaptation} 
Instead, DDS~\cite{dds} choose to leverage server-side compute to adapt for video content. 
As for the online cost, however, DDS needs to run one extra inference per frame to dig out the objects that are missed, which doubles the online cost.

\mypara{Task-specific}
Vigil~\cite{vigil}, EAAR~\cite{eaar}, Focus~\cite{focus} can leverage real-time video content at relatively low cost.
Their use cases, however, are limited to object detection~\cite{vigil, eaar} and frame classification~\cite{focus} and make them not applicable for other vision tasks and applications.



==> motivate-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Background}
\label{sec:back}

\begin{comment}
\kt{
\begin{itemize}
\item background on video stack
\begin{itemize}
\item high-level relevant notions: frames, blocks, motion vectors, quality objectives, etc
\item traditional goals: efficient encoding (injection), storage/streaming, and efficient consumption (decoding + rendering)
\item mention dnn-based
\end{itemize}

\item background on video analytics: object detection, keypoint detection, segmentation, etc [illustrative graphs]
\item use of codec in video analytics
\begin{itemize}
\item offline analytics
\item online streaming+analytics
\item goals: fast encoding, small file sizes (injection) + high accuracy, low decoding and inference delay (consumption).
[illustrative graphs]
\end{itemize}
\end{itemize}}

\kt{Stack: a whole piece of software: injection; define consumption phase}
\end{comment}

We start with how a video stack is used in video analytics applications and then introduce its design space.
% and the rationale of our general design choice within it. 

%\subsection{Video stack for video analytics}

\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \includegraphics[width=0.99\columnwidth]{figs/background.pdf}
    \tightcaption{Illustration of video stack (encoding and decoding) as part of the video analytics pipelines of three applications.}
    \label{fig:background}
\end{figure}


\mypara{Video analytics applications} 
Spurred by advances in computer vision, more video applications are deployed 
%increasingly augmented with computer vision (DNN) 
to perform online/offline inference on massive video streams. 
Many video analytics applications uses a video stack to perform two basic operations: 
{\em encoding} a video stream into a compressed video file upon each frame is captured by a sensor~\cite{??,??} for efficient storage and transmission, and {\em decoding} the compressed video file to individual frames/segments which are then fed into a final DNN for vision inference.
As depicted in Figure~\ref{fig:background}, these operations are needed for both offline analytics on archived videos (\eg~\cite{focus,vstore}) and online analytics on streamed videos (\eg~\cite{dds,awstream}).
To make our discussion more concrete, this paper focuses on three typical video analytics applications: object detection (one labeled bounding box for each object), semantic segmentation (one label for each pixel) and keypoint detection (17 keypoints for each human).

%encodes the video stream into a compressed video file upon each frame is captured by a sensor~\cite{??,??}, as depicted by Figure~\ref{fig:background}, and 
%%run its {\em final DNN} on frames decoded from a compressed video (\eg MP4 format), unless running on a video sensor right after the raw video is captured)
%Thus, as shown in Figure~\ref{fig:background}, video-analytics applications need a {\em video stack} to perform two high-level operations (like video applications that serve human viewers): 
%\begin{packedenumerate}
%\item {\em Encoding} a video stream frame-by-frame into a compressed video file for efficient storage and transmission; and
%\item {\em Decoding} the compressed video file to individual frames/segments which are in turn fed into a final DNN for vision inference.
%\end{packedenumerate}


% \jc{need a double-column visualization of the whole pipeline here!}

%Video stack compresses the video frame-by-frame to reduce the file size for easy storage (injection phase), and de-compresses the video back to frames to serve their users (consumption phase). 
%Traditional video stack aims to serve human viewers. To meet the visual quality requirement of human viewers, the goal of the video stack is efficient encoding during injection phase, real-time decoding and preserving satisfying visual quality during consumption phase.



% \jc{a few words on how we calculated inference accuracy and how is it diff/similar to prior work}





\mypara{Performance objectives}
% Video analytics seek high inference accuracy and low delay (especially when extracting important information from massive video feeds), thereby posing new requirements on both the video ingestion and consumption.
% In particular, 
%In the context of video analytics, 
%The performance of a video stack for video analytics is evaluated along three metrics:
An ideal video stack for video analytics should meet four criteria:
(1) {\em high inference accuracy}, (2) {\em high compression efficiency} (file size reduction compared to the original video size), (3) {\em low encoding and decoding latency per frame}, and (4) it should {\em generalize} across a range of video analytics DNNs.
To calculate the accuracy of an inference result on an encoded frame, we obtain the ``ground truth'' results by running the final DNN on the high-quality video frames (rather than the human-annotated labels). 
This way, any inaccuracy will be due to the video stack (\eg video compression, DNN distillation), rather than errors made by the final DNN itself.
This is consistent with recent work (\eg~\cite{awstream,vigil,videostorm,chameleon,mullapudi2019online,noscope}). 
%Finally, the performance should {\em generalize} across a range of video analytics applications.

%During encoding, it should incur low {\em encoding delay} per frame
%% high {\em encoding throughput} (number of frames encoded per second), 
%and high {\em compression efficiency} (file size reduction).
%During decoding, it should incur low {\em decoding delay} per frame
%% high {\em inference throughput} (number of frames analyzed per second), 
%and {\em high inference accuracy}. 


\mypara{Design space}
The design space of a video stack for video analytics can be characterized in three aspects.
%proposes either better codecs mechanisms or smarter ways of compressing or streaming videos using existing codecs.

\begin{packeditemize}
\item{\em Choice of codec:}
Here, we refer to anything that compresses pixel matrices into a byte stream. 
Classic codcs (\eg H.264/265~\cite{??} or VP8/9~\cite{??}) are common choices in video applications.
We show in \S\ref{subsec:traditional} that if used properly, these codecs {\em could} compress video efficiently for the purposes of video analytics. 
Alternatives, such as super resolution~\cite{cloudseg} and autoencoding~\cite{??}, have yet to see wide industry adoption enjoyed by the classic codecs and they are often compute-intensive (involving DNNs) when encoding (autoencoder) or decoding (super-resolution) videos. We will evaluate them in \S\ref{sec:eval}.
%\jc{keith's paper?}

\item{\em Setting of codec parameters:}
Tuning the parameters of a video codec can influence video analytics performance. 
For instance, classic codes like H.264 allow users to set the resolution and/or quantization parameters of part of a frame, which lead to 
different tradeoffs between compression efficiency and inference accuracy.
While some prior proposals~\cite{??,??,??} fall into this category, we show in \S\ref{subsec:idealized} that they are suboptimal in many cases.
%, one can reduce the file size while still achieving high inference accuracy. 
%As shown in \S\ref{subsec:idealized}, these parameters are currently set by handcrafted heuristics, which might lead to suboptimal performance.

\item{\em Heuristics-based frame dropping/indexing:}
Another common approach is to discard frames deemed unimportant by some cheap heuristics in the encoding phase~\cite{??,??,??}. 
Since any frames discarded in this phase will not be encoded and analyzed by the final DNN, the heuristics must preserve all necessary frames, which is hard to maintain in many real-world videos~\cite{dds}.\footnote{Similar issue happens in frame indexing schemes like~\cite{focus} which indexes each frames with a set of plausible labels returned by a cheap heuristic and feeds the final model with only frames that might contain the searched label. But when cheap heuristic misses the real label of a frame, the frame will simply fall off the radar of the final analytics.}

%run cheap inference in the encoding phase to
%locate and only encode frames with important information~\cite{reducto,glimpse} or generate metadata~\cite{focus} to speed up locating of important frames.
% , the inference query can quickly locate the frames that are most promising. 
%A key assumption is that the cheap inference must avoid false negatives, \ie the labels produced by the cheap inference must include the real label; otherwise, the eventual analysis will miss. 
% However, in our analysis, we found that this is hard to guarantee, unless the ingestion phase uses an expensive model.
% Moreover, this approach still need a codec to compress videos efficiently.

\end{packeditemize}




%\begin{figure}
%    \centering
%%    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
%    \includegraphics[width=0.99\columnwidth]{figs/table.pdf}
%    \tightcaption{Comparing examples from prior work that builds on traditional codecs.}
%    % \kt{looks like our work is just spatial-different-quality version of CloudSeg... Maybe add a new dimension (No online adaptation)?}}
%    \kt{Maybe add one new dimension: require knowledge of video content}
%    \label{fig:table}
%\end{figure}


\begin{table}[]
\footnotesize
\begin{tabular}{>{\centering\arraybackslash}m{1.6cm}>{\centering\arraybackslash}m{1.8cm}>{\centering\arraybackslash}m{1.9cm}>{\centering\arraybackslash}m{1.8cm}}
 \hline
 & Spatially different quality & Final DNN not used in encoding & Applicable to different DNNs \\ \hline
DDS~\cite{dds} & \ding{52}  &  &  \\ \hline
EAAR~\cite{eaar} & \ding{52}  &  &  \\ \hline
Vigil~\cite{vigil} & \ding{52} &  &  \\ \hline
AWStream~\cite{awstream} &  &  & \ding{52} \\ \hline
CloudSeg~\cite{cloudseg} &  & \ding{52} & \ding{52} \\ \hline
VStore~\cite{vstore} &  &  & \ding{52} \\ \hline
Reducto~\cite{reducto} &  & \ding{52} &  \\ \hline
Glimpse~\cite{glimpse} &  &  &  \\ \hline
Focus~\cite{focus} &  &  &  \\ \hline
FilterForward~\cite{filterforward} &  & \ding{52} &  \\ \hline
\rowcolor[HTML]{FFFE65} 
AccMPEG & \ding{52} & \ding{52} & \ding{52}\\ \hline
\end{tabular}
    \tightcaption{Comparing examples from prior work that builds on traditional codecs.}
    % \kt{looks like our work is just spatial-different-quality version of CloudSeg... Maybe add a new dimension (No online adaptation)?}}
    \kt{Maybe add one new dimension: require knowledge of video content}
    \label{fig:table}
\end{table}

\mypara{Our design choice}
In this work, we take a pragmatic stance to build our video stack on class codecs and encode only part of regions in high quality to strike a desirable balance between high inference accuracy and compression efficiency. 
While we are not the first to explore this design choice, we identify three requirements (summarized in Figure~\ref{fig:table}) that should be satisfied in order to achieve the performance objectives regarding inference accuracy, compression efficiency, encoding/decoding latency, and generalizability.
%that influence the performance of prior efforts based on the classic codecs.
\begin{packeditemize}

\item {\em Encoding with spatially different quality:} 
%As \S\ref{subsec:idealized} shows, 
As elaborated in the next section, encoding different spatial regions with different quality has a significant room for improving inference accuracy and compression efficiency, compared to encoding frames with monolithic quality.
% this has significant room for improvement when quality is spatially assigned in an optimal manner.

\item {\em Final DNN not involved in the encoding process:} 
This important for applications where the encoding delay is critical and massive videos need to be encoded but only small portion will be eventually analyzed. 

\item {\em Minimum assumptions about the final DNN:}
%The optimization should make minimum assumptions about the final DNN model.
For instance, assumptions such as inference will be object-based may not generalize to semantics segmentation.
This is critical for the video stack generalize to different DNNs. 

\end{packeditemize}



\begin{comment}

%to enable near-optimal spatial quality assignments and accuracy inference. 
To achieve generalizability, we treat the final DNN as a differentiable model. 
% build our custom video stack on the classic codecs (H.264) but use more analytics-aware codec parameter settings and make incremental changes to the codec to enable accurate inference.
The next section will elaborate that although recent work has taken initial steps in similar directions, there is still a substantial untapped room for improvement.

For traditional codec-based solutions, we identify three key design choices that influence their performances. (Figure~\ref{fig:table} compares several examples built on traditional codecs.)
\begin{packedenumerate}
\item The final DNN should not be used in encoding process. In this particularly important if one wants to minimize the encoding delay for applications where massive videos need to be recorded but rarely analyzed. 
\item Frames should have spatially heterogeneous quality. As \S\ref{subsec:idealized} shows, this has significant room for improvement when quality is spatially assigned in an optimal manner.
\item The optimization should make minimum assumptions about the final DNN model.
For instance, assumptions such as inference will be object-based may not generalize to semantics segmentation.
\end{packedenumerate}

% \jc{need a footnote about why reducto is not general}

\end{comment}



% \jc{need to mention keith's split dnn}

%This choice is based on two complementary observations on a qualitative parallel between what information these codecs (\eg H.264) choose to preserve and what information are most needed by the DNN inference.


%\mypara{Our goal} 
%In this work, we set out to design a custom video stack for video analytics applications.
%In doing so, we take a pragmatic stance to optimize the existing codec, rather than creating a video codec from scratch, for two reasons.
%First, these codecs have efficient (hardware-assisted) implementation and have been widely adopted in industry.
%Second, there is a rich space of optimization on top of existing codec, and although recent work has taken some initial steps, there is still a substantial untapped room for improvement as we will show in the next section.
%Finally, in a real video stack, we assume that one cannot run the eventual DNN inference on the original video (otherwise, one can simply store the DNN output). 

%Video stack serves video analytics in two scenarios: store the video for offline analytics and stream the video for online analytics. In these two scenarios, video stack must be able to provide video frames at a high frame rate to saturate the following analytic DNN. Moreover, video stack should also allow the following DNN to generate accurate analytic results as if the DNN is directly operating on the raw frames. Thus, the goal of video stack for video analytics is:
%{\em Encoding delay}
%{\em Encoding throughput}
%{\em Compression efficiency}
%{\em Inference delay}
%{\em Inference throughput}
%{\em Inference accuracy}
%    \item \textit{Efficient encoding}. 
%    \item \textit{Efficient decoding}.
%    \item \textit{High accuracy.}



\section{Potential for Improvement}
\label{sec:potential}


Though previous research also tunes the parameters of traditional codecs, the choices and the settings of these parameters are based on handcrafted heuristics and often apply only to one application, which as we will see gives rise to suboptimal performance. 
To motivate for a better design, we take three logical steps:
\begin{packedenumerate}
\item We first discuss why the traditional video codec might provide a suitable mechanism for video analytics and a solid base to build our custom video stack on.
\item We then analyze an ``idealized'' design point that sets video quality with hindsight information. 
This serves as a point of comparison of idealized performance improvement. 
\item Through analyzing the improvement of the idealized design, we identify the limitations in prior solutions and how we may approximate the idealized performance improvement.
\end{packedenumerate}
In this section, our goal is to understand the impact of encoding efficiency on inference, so we focus only on the metrics of compression efficiency (compressed file size) and inference accuracy; we will discuss optimal implementation with minimum encoding/decoding delay in later sections.



%\subsection{Opportunity: block-wise quality sensitivity for better compression}





%\kt{0. Methodology w/ real encoding 1. High compress efficiency. 2. The counter-intuitive part of mask a). does not align with object boundary; (have surrounding pixels, and have surrounding pixels) b). varies a lot with content and DNN model. 3. connect to related work. 4. Plot pseudo-graph}
%
%\kt{
%\begin{itemize}
%\item define ``quality sensitivity'' per block: if block $i$'s quality drops from $q$ to $q'$ while all other blocks remain at $q$, how much will accuracy drop?
%\item explain the methodology: dataset, methodology (block-wise enumeration). 
%\item three main takeaways from the measurements:
%\begin{itemize}
%\item only a small fraction of blocks need high quality (despite large objects) [graphs: y = cdf, x = fraction of pixels. one line for pixels that could be in same color, and another line for minimum pixels that must be in high quality]
%\item if DNN only sees a small fraction of blocks, it can still infer accurate results
%\item these highly quality-sensitive blocks may not align with objects or inference results [illustrative graphs of some case studies]
%\end{itemize}
%\end{itemize}
%}


\begin{figure*}[t]
       \subfloat[Object detection]
       {
         \includegraphics[width=0.3\linewidth]{figs/measurement_detection.pdf}
         \label{fig:}
       }
       \hfill
       \subfloat[Keypoint detection]
       {
         \includegraphics[width=0.3\linewidth]{figs/placeholder-tradeoff-mpeg-idealized.pdf}
         \label{fig:}
       }
       \hfill
       \subfloat[Semantic segmentation]
       {
         \includegraphics[width=0.3\linewidth]{figs/measurement_segmentation.pdf}
         \label{fig:}
       }
    \caption{Across three analytics tasks, we see consistently (1) that in Range A, H.264 (traditional video codec) can compress videos with upto \fillme\% file reduction without affecting the inference accuracy; and (2) that in Range B, its inference accuracy drops sharply, but the encoding only selective spatial blocks in high quality can still retain high accuracy with much smaller file size.}
    \label{fig:tradeoff-mpeg-idealized}
\end{figure*}

\subsection{Why building a video stack on traditional video codecs?}
\label{subsec:traditional}

We begin with the fashionable argument that since traditional video codecs are designed to optimize human visual perception which is different from DNN models, they are fundamental ill-suited to encoding videos meant for computer vision inference.
The reality however is more nuanced and traditional video codecs are actually not entirely unsuitable.
In particular, a heuristics commonly employed by many video codecs is that it uses more bits to encode ``low frequency'' information (\eg \fillme) than ``high frequency'' information (\eg \fillme), under the assumption that they are less relevant to human perception~\cite{??}. 
Computer vision DNNs, on the other hand, also tend to learn features of low frequency, based on current theory of deep learning~\cite{??}. 
In short, though current video codec does not always preserve the exact information needed by DNN models, it does tend to use more bits to encode information more relevant to DNN inference. 

To illustrate this intuition, Figure~\ref{fig:tradeoff-mpeg-idealized} tests three models---object detection model (\fillme), key point detection (\fillme) and semantic segmentation (\fillme)---on one of our video datasets (more details in \S\ref{subsec:eval:setup}), which consists of \fillme drone camera videos (\fillme minutes in total).
%We choose these videos since they include a variety of scenarios (urban and rural), object classes (various vehicles and pedestrians), viewing angles, and object sizes. 
%\S\ref{sec:eval} will compare various techniques on a wider range of video sources.
The black line shows the encoded video size vs. inference accuracy when the video is encoded by H.264 at different quantization parameters (QP). 
In H.264/265, the QP value can be viewed as a threshold between high frequency information and low frequency information: a lower QP value means more high frequency information is preserved. 
\jc{need a graphical illustration of the high-frequency info vs. low-frequency info argument}

We can see that before QP exceeds \fillme (labeled by ``Range A''), the encoded video size decreases without affecting the inference accuracy, but as we further reduce the quality (``Range B''), accuracy does start to drop more quickly. 
The reason is that when encoding the spatial blocks in a frame, traditional codecs impose a uniform QP value (the threshold between high frequency and low frequency information), but the feature extraction of a DNN may extract features at different frequency domains at different spatial blocks, and thereby has different tolerance to QP values. 
%may have very different tolerance to the removal of high frequency information in different regions, and thereby needs different QP values at different parts of a frame.
When the QP is low enough such that all high frequency information filtered out by H.264 is not needed by the DNNs, but as QP increases, H.264 starts to filter out information that DNNs do need for feature extraction. 
%This shows that the information discarded by the codec has little impact on the features vital to these DNNs' inference accuracy.

This phenomenon can be intuitively explain by the fact that different parts of each frame may have different importance to the accuracy of the inference result. 
If a region is not associated to any inference result (\eg a background building far away from the detected vehicles), it could be encoded with very low quality (or even blacked out).
Likewise, when a whole frame does not contain information immediately related to the inference results, its quality can be aggressively lowered (or safely skipped). 
In other words, only a portion of the pixels are {\em quality sensitive}.

\jc{need to explain what high quality and low quliaty mean}

\subsection{An idealized design point}
\label{subsec:idealized}

Nonetheless, the spatial variation quality sensitivity is much more complex than the split of background and foreground. 
%To show the effectiveness of encoding videos with spatiotemporally different quality levels, 
To show it, we consider a simplified design point.
Given a video (originally encoded in the highest quality) and a DNN model, it first splits each $\OriginWidth\cdot\OriginHeight$ frame into $\GridWidth\cdot\GridHeight$ grids of 16$\times$16 blocks ($\OriginWidth=16\GridWidth,\OriginHeight=16\GridHeight$)\jc{we need a discussion on the block size}, assigns each block either a high quality $\HighQuality$ or a low quality $\LowQuality$, and then encodes the frames into a low-quality video and a high-quality video, each containing only blocks assigned with the perspective quality (Figure~\ref{??} depicts an example). 
During inference time, the two videos are decoded and the blocks are put in their original positions in the frames, and the frames are then fed in the DNN for inference. 
To measure its potential, we assume that the quality assignment logic can run the DNN (\eg to test its accuracy on any quality assignment), and we will remove this assumption in the actual video stack. 

In the idealized design point, the assignment of quality per block is such that the DNN inference accuracy is maximized while no more than $\MaxHighQualityFrac$ blocks are in high quality. 
In theory, one needs to enumerate all $2^{\GridWidth\cdot\GridHeight}$ possible quality assignments. 
So to make it tractable, we obtain a near-optimal mask with the following process.
We define a binary $\GridWidth\cdot\GridHeight$ {\em mask} to indicate the quality level assigned to each block (1 means $\HighQuality$, 0 means $\LowQuality$).
Given a mask $\Mask$, the encoding image can be expressed by $\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage$ where $\times$ is element-wise multiplication between two matrices and $\HighImage$ and $\LowImage$ are the high quality encoding and the low quality encoding of the frame. Note that the dimensions of a frame is independent of QP, so $\HighImage$ and $\LowImage$ have the same height and width.
Now let us use $\DNN:\mathbb{I}\mapsto\mathbb{O}$ to denote the DNN inference function (where $\mathbb{I}$ and $\mathbb{O}$ denote the space of input frames and the space of DNN output) and $\SimFunc:\mathbb{O}\times\mathbb{O}\mapsto\mathbb{R}$ (defined in \S\ref{sec:back}) to denote the accuracy function of the output of $\DNN$ on a compressed frame by comparing its similarity with $DNN$'s output on the high quality image. 
The optimization objective of the idealized design can be expressed as follows:
\begin{align}
\textrm{max} &~~~~\SimFunc\left(\DNN(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage),\DNN(\HighImage)\right) \label{eq:idealized-objective}\\
\textrm{s.t.} & ~~~~ \Vert\Mask\Vert \leq \MaxHighQualityFrac
\end{align}

% Then given a DNN inference function $\DNN(\cdot)$ and the accuracy function $\AccFunc(\cdot)$ (defined in \S\ref{sec:back}) that evaluates the accuracy of the output of $\DNN(\cdot)$, the optimization objective of the idealized design can be expressed as follows:
% \begin{align}
% \textrm{max} &~~~~\AccFunc\circ\DNN(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage) \label{eq:idealized-objective}\\
% \textrm{s.t.} & ~~~~ \Vert\Mask\Vert \leq \MaxHighQualityFrac
% \end{align}

\jc{Kuntai, please briefly explain how you solved it iteratively?}


\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \includegraphics[width=0.6\columnwidth]{figs/hq_percentage.pdf}
    \caption{Percentage of pixels encoded in high quality v.s. accuracy. Only 6.3\% of the pixels need to be encoded to make accuracy more than 0.9.}
    \label{fig:percpixel-accuracy}
\end{figure}

We acknowledge that the formulation entails three simplifying assumptions: it restricts the choice of encoding quality to two levels; there are more efficient encoding methods, such as region-of-interest encoding, for videos with a spatially different quality levels than creating two separate video files; and the $16\times16$ square blocks may not align with the optimal boundaries between regions that require different quality levels.
Nonetheless, we believe that analyzing this formulation is still valuable. 
In some sense, it generalizes the design space of several recent solutions: \jc{why it generalizes vigil, dds, awstream, glimpse, reducto}


To put it in perspective, we also consider two other ways of selecting which blocks to encode in high quality: one selects the blocks that overlap with one of the final detected bounding boxes, and the other one selects the blocks that overlap with one of the region proposal bounding box. 
Intuitively, these two strawmen assume that only regions of the difficult-be-detected objects need to be encoded in high quality, which represents the basic premise behind the state-of-the-art techniques~\cite{??,??}. 


Figure~\ref{fig:tradeoff-mpeg-idealized} compares the idealized design point with the two strawmen and the uniform-quality H.264 baseline. 
Here, we use \fillme and \fillme as the high and low quality level, and \fillme as the codec.
To show the full spectrum of their effectiveness, these strawmen are tested with a varying confidence score on the bounding boxes or the region proposals.
Across the three tasks, we can see that the idealized design achieves same high accuracy with \fillme\% less bits than the best of the three baselines.
Figure~\ref{fig:percpixel-accuracy} further reveals that the reduced file size (in the case of object detection) results from less blocks being selected for high quality encoding. 


%Across the three tasks, we can see that only encoding \fillme-\fillme\% blocks in high quality still yield more than \fillme-\fillme\% of accuracy.
%We measure the potential improvement of the idealized design point on one of our video datasets (more details in \S\ref{subsec:eval:setup}), which consists of \fillme drone camera videos (\fillme minutes in total), and use \fillme and \fillme as the high and low quality level, and \fillme as the codec. 
%We choose these videos since they include a variety of scenarios (urban and rural), object classes (various vehicles and pedestrians), viewing angles, and object sizes. 
%\S\ref{sec:eval} will compare various techniques on a wider range of video sources.


%\vspace{0.1cm}
%\noindent{\em {\bf Observation \#1:} }
%\vspace{0.1cm}


%We first examine the {\em quality-sensitive blocks} (\ie blocks assigned with $\HighQuality$) as a fraction of all blocks in three of the canonical video analytics tasks: object detection model (\fillme), key point detection (\fillme) and semantic segmentation (\fillme).
%Figure~\ref{fig:percpixel-accuracy} shows the distribution of the quality-sensitive block fraction across frames in the videos. 
%Across the three tasks, we can see that only encoding \fillme-\fillme\% blocks in high quality still yield more than \fillme-\fillme\% of accuracy.
%
%To put it in perspective, {\em such fractions of quality-sensitive pixels are even less than claimed by previous work.}
%We zoom in on the object detection task and compare this idealized design with two other ways of selecting quality-sensitive blocks: one selects the blocks that overlap with one of the final detected bounding boxes, and the other one selects the blocks that overlap with one of the region proposal bounding box. 
%(To show the full spectrum of their effectiveness, these strawmen are tested with a varying confidence score on the bounding boxes or the region proposals.)
%Intuitively, these two strawmen assume that only regions of the difficult-be-detected objects need to be encoded in high quality, which represents the basic premise behind the state-of-the-art techniques~\cite{??,??}. 
%
%Figure~\ref{??} shows the fraction of quality-sensitive blocks and the resulting accuracy of the idealized design and the two strawmen. 
%\jc{some numbers from the graph}


%\mypara{Block-wise quality differentiation}
%For DNN-based analysis, the power to impact accuracy is not evenly distributed between pixels.
%Thus, we can save bandwidth by aggressively lowering the pixels that does not impact accuracy too much.
%At codec level, however, the quality of pixels are organized by blocks.
%Inside each block, the quality of pixels are the same.
%Thus, block is the minimum granularity for quality differentiation.

%\mypara{Mask}
%To quantify the compression opportunity of quality differentiation, we present a concept: \textit{mask}.
%\textit{Mask} maps each block to its corresponding encoding quality.
%
%\mypara{Potential bandwidth saving} 
%We measure the potential bandwidth saving of this opportunity on VisDrone dataset~\cite{aiskyeye} with object detection model FasterRCNN-ResNet50~[\fillme] as our backend model. 
%We use two different encoding qualities: low quality and high quality\footnote{\fillme} to encode each block.
%To determine the encoding quality of each block, our steps are:
%\kt{Substitude this into an algorithm for general vision tasks}
%\begin{packedenumerate}
%    \item Encode the whole video in high quality and collect the bounding box $b_i$ for each object $i$.
%    \item For each object, we assign a new bounding box $b'_i$, of which the center is the same with $b_i$ and the size of this bounding box is $0$.
%    \item Partition the whole frame into 16$\times$ 16 blocks.
%    \item Use highest quality to encode those blocks that overlaps with any of $b'_i$, and use lowest quality to encode other blocks.
%    \item If less than 95\% objects are detected, for those objects $j$ that are not detected, enlarge $b'_i$ by padding a constant on the left, top, right, bottom on it, and go back to step 3.
%\end{packedenumerate}


% One way to save bandwidth is to reduce the encoding quality.
% Also, the power to impact accuracy is not evenly distributed between pixels.
% It follows that we can saving bandwidth through manipulating pixel encoding quality.
% However, the pixels inside the same block (determined by the codec) will always have the same quality.
% So we instead encode

% \mypara{Heterogeneous quality sensitivity requirements} 
% Different vision models care about different parts in the video. For example, vehicle detection models care car pixels much more than human pixels; and human detection models care human pixels much more than car pixels. In terms of encoding, it means that different vision models are more sensitive to the encoding quality of some blocks more than other blocks.

% This opportunity implies that we can save bandwidth if we encode those quality-sensitive blocks in high encoding quality and those quality-insensitive blocks in low encoding quality.

% \blindtext


\subsection{Improvement analysis}
\label{subsec:analysis}


A natural question therefore is what the source of improvement of the idealized design point is.
In other words, what have the strawmen missed in their assumptions.

\vspace{0.1cm}
\noindent{\em {\bf Observation \#1:} Quality-sensitive regions are not aligned with inference results (\eg objects, boundaries).}
\vspace{0.1cm}

To begin with, we observe that the quality-sensitive blocks selected by the idealized design are largely {\em not} aligned with the detected bounding boxes or region proposals. 
Figure \ref{fig:object-hqblock} uses two example frames to illustrate this observation. 
On one hand, we see in (a) that some objects cannot be detected in low quality, but do not need entirely encoded in high quality either. 
Instead, the objects can be detected at the right locations when only parts of each object are encoded in high quality.
On the other hand, we see in (b) that some objects cannot be detected even if they are entirely encoded in high quality. 
Instead, parts of the surrounding blocks have to be encoded in high quality as well.
\jc{maybe there are blocks that are not associated with any detected object, but need to be in high quality just to winnow out non-objects?}




\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figs/object-hqblock.pdf}
    
    \includegraphics[width=0.7\columnwidth]{figs/fig5_parthq.pdf}
    
    \includegraphics[width=0.7\columnwidth]{figs/fig5_allhq.pdf}
    \caption{Inference results on images with different regions in high quality. Some objects do not need to be all in high quality to be detected, and some objects need surrounding pixels in high quality to be detected.}
    \label{fig:object-hqblock}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/placeholder-obj-iou-cdf.pdf}
    \includegraphics[width=0.6\columnwidth]{figs/obj_ideal_iou_cdf.pdf}
    \caption{\kt{Over half of the selected high-quality blocks have an IoU < 60\% compared to object detection bounding boxes.}There is not strong overlap between the inference results of object detections (bounding boxes) and high-quality blocks selected by the idealized design point.}
    \label{fig:obj-iou-cdf}
\end{figure}

Figure~\ref{fig:obj-iou-cdf} shows that across all frames, there is significant misalignment between the inference results of object detections (bounding boxes) and high-quality blocks selected by the idealized design point.
\jc{more read of the graph}



\vspace{0.1cm}
\noindent{\em {\bf Observation \#2:} Quality-sensitive regions are highly dependent to the inference task and DNN.}
\vspace{0.1cm}

Given that the detected bounding boxes or the final inference results (even if they are known) are a poor indicator of quality-sensitive blocks, what decides the quality-sensitive blocks then?
Empirically, we found that the quality-sensitive blocks are highly sensitive to the DNN and the inference task. 
To analyze this dependency, we first take one DNN for each analytics task and use the idealized design to optimally select \fillme\% of spatial blocks for each DNN in each frame to encode in $\HighQuality$. 
Figure~\ref{fig:task-dependent} compares the accuracy of each DNN when fed with the frames encoded using the quality assignment designed for the model vs. the frames encoded using the quality assignments designed for the other two DNNs.
We see that the accuracy drop substantially when the quality assignment is customized for another model. 
\jc{some numbers from the graph}

Now, what about DNN models of the same task. 
Figure~\ref{fig:model-dependent} takes three different object detection DNNs as an example and compares their accuracies on the video encoded with its corresponding quality assignment and on the  videos encoded with the other two models' quality assignments.
We see that the accuracy of a DNN drops substantially when it runs on the quality assignment of design for other models.
Zooming in, we found that the exact blocks that have to be encoded in high quality change across the DNNs, even though they are trained to detect same objects!
\jc{some numbers from the graph}
\jc{can the resulting map be different if you just run the idealized algorithm on the same DNN again?}







\begin{figure}[t]
       \subfloat[Across video-analytics tasks]
       {
         \includegraphics[width=0.48\linewidth]{figs/placeholder-task-dependent.pdf}
         \label{fig:task-dependent}
       }
       \subfloat[Across models (object detection)]
       {
         \includegraphics[width=0.48\linewidth]{figs/placeholder-model-dependent.pdf}
         \label{fig:model-dependent}
       }
    \caption{The quality-sensitive regions are highly dependent to the inference task and DNN.}
    \label{fig:}
\end{figure}


\subsection{Summary of key findings}
The goal of this section was to understand the gap between existing solutions and the idealized video codec built on traditional codecs.
Using three video analytics tasks and a real-world video dataset, we show that:
\begin{packedenumerate}
\item Traditional codecs such as H.264 are qualitatively suitable for video analytics: when QP is relatively low (<\fillme), their encoding processes tend to discard higher-frequency details which are also not needed by DNN inference either. 
However, as QP increases too high (>\fillme), they start to filter out some information needed by the DNN feature extractions.
\item If one optimally assigns high quality (QP=\fillme) to a selected set of spatial blocks, we can still achieve the same high accuracy as feeding uniformly high quality video to the DNN model but with \fillme\% of spatial blocks in high quality (the rest in QP=\fillme), which gives rise to a \fillme\% reduction on video file size.
\item Achieving this potential improvement is non-trivial and inspires us to rethink the design assumptions behind prior solutions.
\begin{packeditemize}
\item The idealized quality assignments have substantial misalignment with the objects or region proposals. 
In object detection, \fillme\% of pixels assigned with high quality are not in the objects' bounding boxes and \fillme\% of pixels insight the objects' bounding boxes do not need to be in high quality.
\item The idealized quality assignments are greatly dependent not only on vision task but on the particular DNN.
On the same frame, the quality assignment generated for one DNN may result in \fillme\% lower accuracy when used to generate input frame to another DNN, even though both models detect the same objects.
\end{packeditemize}
\end{packedenumerate}

%\begin{figure}
%    \centering
%\includegraphics[width=0.4\columnwidth]{figs/hetero-task.pdf}
%    \caption{Accuracy on different task with the same compressed video. One size does not fit for all vision tasks.}
%    \label{fig:hetero-task}
%\end{figure}
%
%\begin{figure}
%    \centering
%\includegraphics[width=0.4\columnwidth]{figs/hetero-dnn.pdf}
%    \caption{Accuracy on different object detection DNN with the same compressed video. Accurate compression for cheap model may not work on expensive model.}
%    \label{fig:hetero-dnn}
%\end{figure}

%This compression opportunity varies a lot between different vision tasks and models.
%In other word, one mask that works perfectly for one application might result in poor accuracy in another application.
%In Figure \ref{fig:hetero-task}, accurate compression for keypoint detection does not work on object detection and semantic segmentation.
%So compression need to be designed for different applications.
%Moreover, in Figure \ref{fig:hetero-dnn}, we see that even under the same vision task, compression that works for one DNN may not work on others.




%\mypara{Takeaways} During the measurement above, we find that:
%\begin{packeditemize}
%    \item To reproduce satisfactory inference result, only a small fraction of blocks need to be encoded in high quality. From Figure \ref{fig:percpixel-accuracy}, we can see that covering only \fillme\% pixels will yield more than \fillme\% of accuracy.
%    \item Object may not align with the high-quality blocks. From Figure \ref{fig:object-hqblock}, we see that some objects do not need to be all in high quality to be detected, and some objects need surrounding pixels in high quality to be
%\end{packeditemize}
%
%\mypara{Heterogeneity between vision tasks and models}
%This compression opportunity varies a lot between different vision tasks and models.
%In other word, one mask that works perfectly for one application might result in poor accuracy in another application.
%In Figure \ref{fig:hetero-task}, accurate compression for keypoint detection does not work on object detection and semantic segmentation.
%So compression need to be designed for different applications.
%Moreover, in Figure \ref{fig:hetero-dnn}, we see that even under the same vision task, compression that works for one DNN may not work on others.
%
%\blindtext


\begin{comment}

\subsection{Mismatch of existing solutions}

\kt{
\begin{itemize}
\item{Human perception-centric quality encoding}
\begin{itemize}
\item the highly sensitive blocks are highly dependent on the task
\item existing heuristics are completely unaware of the server-side dnn structure
\item implications: need a generic way to encode videos in cognizant of the block-level sensitivity. [an illustrative example]
\end{itemize}
\item{Encoding dynamic quality sensitivity}
\begin{itemize}
\item the highly-sensitive pixels changes a lot across frames
\item today's encoding is inefficient: unnecessary motion vector, etc.  micro-block misalignment
\item implications: need a way to ``smooth'' the highly dynamic sensitive blocks [an illustrative example]
\end{itemize}
\item{Frame-wise semantics}
\begin{itemize}
\item analyzing the whole frames one by one
\item implications: putting sensitive regions together [an illustrative example]
\end{itemize}
\end{itemize}}


In general, prior work on video stack propose either new codecs or smarter ways of compressing/streaming videos over existing codecs.
In this context, we now discuss potential mismatches in both directions with respect to what an idealized video stack need.



As mentioned earlier, the idealized algorithm essentially explores a similar design space of previous work, but at a different (finer) granularity (small blocks instead of bounding boxes) and with access to the DNN (such that we can reveal the ideal improvement).
By analyzing the encoding decisions made by the idealized design, we found two 


\mypara{Limitation of existing work} 
Wrong assumptions of related work was revealed by our measurement study above. 
The vast majority of current works on quality differentiation~\cite{dds,vigil,glimpse,eaar} implicitly assumes that high quality regions should align with the objects.
However, in Figure \ref{fig:object-hqblock}, we see that high quality regions can be much smaller or much larger than the object itself.
So objects might be missed or file size might be wasted if aligning high quality regions with objects.



\mypara{Traditional video codec}
Caring about visual quality, traditional video codec pays nearly equal attention to all pixels. 
The quality-sensitive blocks, however, are highly dependent on server-side DNNs.
Traditional video codec is unable to exploit this opportunity due to its unawareness to server-side DNN.
This implies that we need a generic way to encode the videos in cognizant of block quality-sensitivity, see Figure \fillme for an illustration.

\mypara{Super resolution}
Nowadays, super resolution \cite{cloudseg,livenas} gradually becomes a new choice of video codec.
These approaches encode the video in low quality, store or stream the low quality video at server side, and then compensate the quality loss by super resolution network.

However, super resolution is fundamentally an ill-suited problem. Multiple high-quality frames may have exact same low-quality frames if compressed by the codec.
As a result, even the most compute-intensive super resolution network cannot fully recover the areas crucial to inference results. Figure \fillme shows an example.
To overcome this issue, current approaches choose to retrain the neural network online. This design choice poses too much online cost at the server side.

\mypara{Auto-encoder}
Computer vision community is actively exploring a new type of codec called auto-encoder~\cite{rate-distortion-autoencoder}. These approaches encode the video by feeding it through neural network and storing the output of that neural network. 

Unfortunately, auto-encoder that preserves high image quality is too compute-intensive for a single CPU to afford (\fillme seconds per frame).
Moreover, this approach requires another neural network as the decoder. Thus, every frame needs to be processed by the decoder at inference time and poses too much online overhead. 



\subsection{Mismatch of existing video analytics pipelines}

\kt{Benefit different vap, weaken this argument}

\kt{
\begin{itemize}
%\item approach \#1: twisting existing interface, (2) case-by-case heuristics
\item limitation \#1: fail to adapt to real-time video content (sr, awstream, vstore)
\item limitation \#2: slow costly (dds, dnn-based autocodec)
\item limitation \#3: only applies to one task (vigil, eaar, focus)
\end{itemize}}

Video analytic pipelines stream videos from the camera to the server and generate analytic results with minimum overhead as well as maintaining satisfying accuracy. However, these approaches are not suitable for video stack purpose.

\mypara{Agnostic to real-time video content} 
AWStream~\cite{awstream} and CloudSeg~\cite{cloudseg} exploit the optimal configurations~\cite{awstream} or  super resolution networks~\cite{cloudseg} derived from \textit{history video content} and count on the similarity between real-time video content and history video content.
However, in real world, the video content can change drastically. 
For example, when a car equipped with traffic camera driving on a street that human rarely appears, the system needs to adapt every time human appears to detect all of them.
These approaches are likely to have low accuracy in these scenarios.

\mypara{Too much online cost for real-time content adaptation} 
Instead, DDS~\cite{dds} choose to leverage server-side compute to adapt for video content. 
As for the online cost, however, DDS needs to run one extra inference per frame to dig out the objects that are missed, which doubles the online cost.

\mypara{Task-specific}
Vigil~\cite{vigil}, EAAR~\cite{eaar}, Focus~\cite{focus} can leverage real-time video content at relatively low cost.
Their use cases, however, are limited to object detection~\cite{vigil, eaar} and frame classification~\cite{focus} and make them not applicable for other vision tasks and applications.

\end{comment}



==> motivate-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Background}
\label{sec:back}

\mypara{Video analytics applications} 
Spurred by advances in computer vision, more video applications 
%increasingly augmented with computer vision (DNN) 
perform DNN-based inference on massive video streams (if not in each video's entirety). 
As depicted in Figure~\ref{fig:background}, many video analytics applications use a {\em video stack}\footnote{In this work, a video stack means a software wrapper on top of a video codec (H.264/265, VP8/9, etc) that tunes its performance for some higher-level application (video analytics tasks). In \S\ref{sec:eval}, we will evaluate our proposal's performance over various codecs and in various vision tasks.} for two basic operations: 
{\em encoding} a stream of frames into a compressed video file as the frames are captured by a video sensor~\cite{vstore} for efficient storage and transmission, and {\em decoding} the compressed video file to individual frames/segments which are then fed into a {\em final DNN} for vision inference.
These operations are needed for both offline analytics on archived videos (\eg~\cite{focus,vstore}) and online analytics on streamed videos (\eg~\cite{dds,awstream}).
To make our discussion more concrete, this paper focuses on three typical video analytics applications: object detection (one labeled bounding box for each object), semantic segmentation (one label for each pixel) and keypoint detection (17 keypoints for each human).


\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \includegraphics[width=0.99\columnwidth]{figs/background.pdf}
    \tightcaption{Illustration of a video stack (encoding and decoding) as part of the video analytics pipelines of three tasks.}
    \label{fig:background}
\end{figure}


\mypara{Performance objectives}
% Video analytics seek high inference accuracy and low delay (especially when extracting important information from massive video feeds), thereby posing new requirements on both the video ingestion and consumption.
% In particular, 
%In the context of video analytics, 
%The performance of a video stack for video analytics is evaluated along three metrics:
An ideal video stack for video analytics should meet three criteria:
\begin{packeditemize}
\item Tradeoff between {\em high inference accuracy}\footnote{To calculate the accuracy of an inference result on an encoded frame, we obtain the ``ground truth'' results by running the final DNN on the high-quality video frames (rather than using the human-annotated labels). 
Thus, any inaccuracy will be due to the video stack (\eg video compression, DNN distillation), rather than errors made by the final DNN itself.
This is consistent with recent work (\eg~\cite{awstream,vigil,videostorm,chameleon,mullapudi2019online,noscope}). } and {\em high compression efficiency} (small compressed video size);
\item {\em Low encoding and decoding latency per frame}, and 
\item It should {\em generalize} to (\ie can be automatically customized to serve) different DNNs for various vision tasks.
\end{packeditemize}
%Finally, the performance should {\em generalize} across a range of video analytics applications.


\mypara{Design space}
To put our design into perspective, we first sketch the space of various potential design points.
\begin{packeditemize}
\item {\em Choice of codec:}
One option is to re-use a traditional codec (\eg H.264/265~\cite{1218189}, VP9~\cite{6737765}) and tune its parameters (\eg quantization parameters). 
There are also alternative NN-based codecs (\eg super resolution~\cite{cloudseg}, autoencoder~\cite{rate-distortion-autoencoder}), but they have yet to see the wide industry adoption enjoyed by the traditional codecs, and they usually have compute-intensive encoding (\eg autoencoder) and decoding (\eg super-resolution).
In this work, we take a pragmatic stance to build our video stack on traditional codecs, like most work in this space.


\item {\em Quality adaptation granularity:}
To cope with the dynamics of video content, prior work tries to adapt quality by saving only a subset of frames (\eg~\cite{glimpse,reducto,awstream}), assigning different quality to different frames (\eg~~\cite{awstream,vstore,chameleon}), and/or assigning a higher quality to only object bounding boxes or region proposals (\eg~~\cite{vigil,dds,eaar}).
In this work, we assign quality for each fine-grained blocks (16x16 pixels), which as shown in the next section could lead to much better compression efficiency and inference accuracy than the aforementioned granularities.


\item {\em Integration with final DNN:}
Using the final DNN's output (or intermediate features) does help to identify regions of interest (\eg~\cite{eaar,dds}), but it potentially adds a prohibitive overhead to encoding (especially for archived videos most of which will not be analyzed).
On other other hand, using cheap heuristics that are agnostic to the final DNN has been shown to produce suboptimal compression efficiency and/or low inference accuracy~\cite{dds}.
In this work, we design a shallow NN to infer a (near-)optimal quality assignment, which as we will see is a much simpler task than the actual final inference.

\end{packeditemize}


\begin{comment}

\subsection{Design space}

Before diving to specific designs, we first sketch the broader design space of the video stacks for video analytics purposes.
In particular, we identify three dimensions that characterize this design space.

\kt{What Codec?}\myparaq{What control knobs}
One choice to use customized codec, such as super resolution~\cite{cloudseg} and autoencoder~\cite{rate-distortion-autoencoder}, but they have yet to see the wide industry adoption enjoyed by the classic codec, and they usually have high encoding/decoding delays, due to compute-intensive encoding (\eg autoencoder) and decoding (\eg super-resolution).
In this work, we take a pragmatic stance to build our video stack on classic codecs and explore a specific parameter: {\em assigning different quality level to each fine-grained spatial region}. 
%It can encode any selected regions in a low quality level. 
When using the lowest quality level, it in effect blacks out the region or a whole frame (\ie frame is discarded). 
In theory, this knob is more flexible than most prior work, which can be subsumed under different settings of this control knob, such as frame dropping~\cite{glimpse,reducto,filterforward}, spatial quality adaptation~\cite{dds,eaar,awstream,chameleon,vigil}.


%One can choose to use one of the classic codecs (\eg H.264/265~\cite{??} or VP8/9~\cite{??}) and tune the configuration parameters it exposes. 
%Alternatives (\eg super resolution~\cite{cloudseg} and autoencoding~\cite{??}) have yet to see the wide industry adoption enjoyed by the classic codec, and they usually have higher encoding/decoding delays than the classic codec-based solutions, due to compute-intensive encoding (autoencoder) and decoding (super-resolution).



%Thus, the classic codecs {\em could} compress video very efficiently for video analytics purposes.


\myparaq{How often to update encoding}
One can update the parameter setting (quality assignment) at a coarse timescale using history frames~\cite{awstream,chameleon}. 
However, as noted in a recent work~\cite{dds}, movements of objects or camera angles can mount to changes that require a different optimal encoding scheme every handful of frames. 
In this work, we try to determine the parameter setting (quality assignment) based on the real-time content of each frame~\cite{dds,reducto}, which better adapts to the dynamic video content and could lead to more desirable accuracy-compression tradeoffs. 


%One can either update the parameter setting at a coarse timescale using history frames~\cite{awstream,chameleon}, or determine the parameter setting based on the real-time content of each frame~\cite{dds,reducto}.
%In this work, we explore the latter option, which could lead to more desirable accuracy-compression tradeoffs, since it better adapts to the dynamic video content. 
%As noted in a recent work~\cite{dds}, movements of objects or camera angles can mount to changes that require a different optimal encoding scheme every handful of frames. 




\myparaq{How to involve the final DNN}
Depending on how the final DNN is used, there are two ways of adapting quality assignment per frame.
On one hand, one can use a cheap heuristics to filter out pixels deemed unimportant for the final task~\cite{reducto,glimpse,vigil}. 
However, awareness of the task (\eg object detection) does not equal awareness of the final DNN (\eg a specific object detector DNN).
As shown in \S\ref{sec:eval}, such heuristics may drop too many pixels for the DNN to maintain high accuracy (\eg objects cannot be detected without enough context) and/or drop too few pixels to waste bandwidth (\eg a DNN can still detect some object when only part of its pixels are encoded).\footnote{Similar issue happens in frame indexing schemes like~\cite{focus} which indexes each frames with a set of plausible labels returned by a cheap heuristic and feeds the final model with only frames that might contain the searched label. But when cheap heuristic misses the real label of a frame, the frame will simply fall off the radar of the final analytics.}
%The issue is that any pixels/frames discarded in this phase will not be encoded and analyzed by the final DNN, so the heuristics must preserve all necessary frames, which is hard to achieve in many real-world videos
Realizing this limitations, recent works instead try to run the final DNN on almost every frame while keeping intermediate results like regions proposals for future use~\cite{dds,eaar}. 
Though region proposals are popular, they may not be available in other DNN models in general. 
Moreover, running the final DNN adds a significant overhead to the encoding phase. (In fairness, they target settings where every frame will analyzed by the final DNN, so the additional cost is justifiable.)


In this work, we explore the following design point. 
We train a light-weight model for a specific final DNN (rather than the task), such that the model returns a near-optimal spatial quality assignment for each frame---only minimum regions are assigned and encoded in high quality yet the final DNN still achieves high accuracy.
As we will show in the next section, encoding with spatially different quality levels still has a significant, {\em untapped} room for improving inference accuracy and compression efficiency.
To our best knowledge, we are the first to explore this design choice. 

\end{comment}




%but it requires extra computation per-frame to determine the quality assignment. 
%To avoid inflating the encoding delay when ingesting the video, many techniques use a cheap heuristics to determine which frames or pixels are unimportant~\cite{reducto,glimpse,vigil}. 
%
%To our best knowledge, there is currently no solution to distill a dnn-based spatial quality assignment logic. filterforward does temporal
%
%
%to avoid inflating the encoding delay when ingesting the video
%
%
%
%DNN not involved vs. DNN directly used vs. assumed DNN's goal
%
%Some techniques run the final DNN (to extract the features or region proposals) on almost every frame~\cite{dds,eaar}, which adds a significant overhead to the encoding phase. (In fairness, they target settings where every frame will analyzed by the final DNN, so the additional cost is justifiable.)
%
%
%In short, we explore spatially different quality assignment, which could be much better than existing solutions, let along frame dropping schemes. update it every frame, in a DNN-aware manner.

\section{Potential for Improvement}
\label{sec:potential}


% Given our design goal (spatial quality assignment per frame over traditional codecs), 
In this section, we follow three steps to motivate the potential improvements of our design choice. 
%Though previous research also tunes the parameters of traditional codecs, the choices and the settings of these parameters are based on handcrafted heuristics and often apply only to one application, which as we will see gives rise to suboptimal performance. 
%To motivate for a better design, we take three logical steps:
\begin{packedenumerate}
\item We first show that the traditional video codecs are not a qualitative mismatch with video analytics. %and a solid base to build our custom video stack on.
\item We then analyze an ``idealized'' design point that optimally assigns video quality in the traditional codecs.
This serves as a point of comparison of optimal improvements. 
\item Through analyzing the idealized quality assignments, we identify where existing solutions fall short.
\end{packedenumerate}
In this section, our goal is to understand the impact of encoding efficiency on DNN inference, so we focus only on compression efficiency (compressed file size) and accuracy; we will discuss encoding/decoding delay in later sections.



%\subsection{Opportunity: block-wise quality sensitivity for better compression}





%\kt{0. Methodology w/ real encoding 1. High compress efficiency. 2. The counter-intuitive part of mask a). does not align with object boundary; (have surrounding pixels, and have surrounding pixels) b). varies a lot with content and DNN model. 3. connect to related work. 4. Plot pseudo-graph}
%
%\kt{
%\begin{itemize}
%\item define ``quality sensitivity'' per block: if block $i$'s quality drops from $q$ to $q'$ while all other blocks remain at $q$, how much will accuracy drop?
%\item explain the methodology: dataset, methodology (block-wise enumeration). 
%\item three main takeaways from the measurements:
%\begin{itemize}
%\item only a small fraction of blocks need high quality (despite large objects) [graphs: y = cdf, x = fraction of pixels. one line for pixels that could be in same color, and another line for minimum pixels that must be in high quality]
%\item if DNN only sees a small fraction of blocks, it can still infer accurate results
%\item these highly quality-sensitive blocks may not align with objects or inference results [illustrative graphs of some case studies]
%\end{itemize}
%\end{itemize}
%}


% \begin{figure*}[t]
%       \subfloat[Object detection]
%       {
%          \includegraphics[width=0.25\linewidth]{figs/measurement_detection.pdf}
%          \label{fig:}
%       }
%       \hfill
%       \subfloat[Keypoint detection]
%       {
%          \includegraphics[width=0.25\linewidth]{figs/measurement_keypoint.pdf}
%          \label{fig:}
%       }
%       \hfill
%       \subfloat[Semantic segmentation]
%       {
%          \includegraphics[width=0.25\linewidth]{figs/measurement_segmentation.pdf}
%          \label{fig:}
%       }
%     \tightcaption{Across three analytics tasks, we see (1) that in Range A, H.264 (traditional video codec) can compress videos with upto 75\% file reduction without affecting the inference accuracy; and (2) that in Range B, its inference accuracy drops sharply, but the encoding only selective spatial blocks in high quality can still retain high accuracy with much smaller file size.}
%     \label{fig:tradeoff-mpeg-idealized}
% \end{figure*}

\begin{figure}[t]
       \subfloat[Object detection]
       {
         \includegraphics[width=0.32\columnwidth]{figs/measurement_detection.pdf}
         \label{fig:}
       }
       \subfloat[Semantic seg.]
       {
         \includegraphics[width=0.32\columnwidth]{figs/measurement_segmentation.pdf}
         \label{fig:}
       }
       \subfloat[Keypoint detection]
       {
         \includegraphics[width=0.32\columnwidth]{figs/measurement_keypoint.pdf}
         \label{fig:}
       }
    \tightcaption{In three analytics tasks, as encoding quality drops, traditional video codec (H.264) can compress videos by upto 50\%, after which inference accuracy starts to drop sharply. 
    However, encoding only selective spatial blocks (``ideal'') in high quality still retains high accuracy with smaller file size.}
    \label{fig:tradeoff-mpeg-idealized}
\end{figure}

%\subsection{Why building a video stack on traditional video codecs?}
\subsection{Why are traditional codecs a good idea?}
\label{subsec:traditional}

A frequently invoked argument has been that because traditional video codecs are designed for human visual perception rather than computer vision DNNs, they are ill-suited to encoding videos for DNN inference.
The reality, however, is more nuanced than that, and traditional video codecs may not be a bad idea after all.
% A specific heuristics commonly employed by 
Traditional codecs typically use more bits to encode ``low frequency'' information (\eg local brightness) than ``high frequency'' information (\eg fine textures on objects), since high-frequency information is less relevant to human perception~\cite{h264}. 
In the meantime, current theory of deep learning suggests that computer vision DNNs also tend to learn low-frequency features~\cite{xu2019training,xu2019frequency,wang2016cnnpack}
%, based on current theory of deep learning. 
% Thus, although traditional video codecs do not keep the exact data needed by DNN models, they do qualitatively 
Therefore, traditional codecs do tend to use more bits to encode information more relevant to DNN inference. 
%not always preserve the exact information needed by DNN models, it does tend to use more bits to encode information more relevant to DNN inference. 

To illustrate this intuition, Figure~\ref{fig:tradeoff-mpeg-idealized} tests three models---object detection model~\cite{ren2015faster}, key point detection~\cite{maskrcnn} and semantic segmentation~\cite{long2015fully}---on two of our video datasets (more details in \S\ref{subsec:eval:setup}), which consists of 5 drone camera videos (4 minutes in total).
%We choose these videos since they include a variety of scenarios (urban and rural), object classes (various vehicles and pedestrians), viewing angles, and object sizes. 
%\S\ref{sec:eval} will compare various techniques on a wider range of video sources.
The H.264 line (red) shows the encoded video size vs. inference accuracy when the video is encoded by H.264 using different quantization parameters (QP in \{31, 32, 34, 36, 40, 44\} for object detection and semantic segmentation, and QP in \{24, 26, 28, 32, 36, 42, 48\} for keypoint detection). 
In H.264/265, the QP value intuitively serves as a threshold between high frequency information (which will be discarded) and low frequency information (which will be preserved). 
%a lower QP value means more high frequency information is preserved. 
%\jc{need a graphical illustration of the high-frequency info vs. low-frequency info argument}
% We can see that until QP exceeds 36 \kt{kpt detection} (``Range A''), 
We see that as quality drops (QP increases) the encoded video size decreases without hurting the inference accuracy much, but as we further reduce the quality, accuracy starts to drop more sharply. 


This is because when encoding the spatial blocks in a frame, traditional codecs impose the same QP value everywhere in a frame, 
%(the threshold between high frequency and low frequency information), 
but the DNNs may need features at different frequencies in different spatial blocks. %, and therefore exhibit different tolerance to QP values. 
%may have very different tolerance to the removal of high frequency information in different regions, and thereby needs different QP values at different parts of a frame.
%When the QP is low enough such that all high frequency information filtered out by H.264 is not needed by the DNNs, but as QP increases, H.264 starts to filter out information that DNNs do need for feature extraction. 
%This shows that the information discarded by the codec has little impact on the features vital to these DNNs' inference accuracy.
%This phenomenon can be intuitively explain by the fact that different parts of each frame may have different importance to the accuracy of the inference result. 
If a region is not related to the inference result (\eg a background building far away from the detected vehicles), it could be encoded with very low quality (high QP).
% , \ie can tolerate a high QP value.
But for regions related to the inference result, sufficient low-frequency information must be preserved.
Of course, such accuracy-compression tradeoffs of traditional video codecs have been observed before, but our interpretation is still valuable---it is not that computer vision and human vision are looking for qualitatively different information; rather, the difference is simply that computer vision needs spatially heterogeneous quality (QP) assignments.


% has more spatially heterogeneous tolerance to quality levels than human vision.
% This naturally indicates that the key to best utilize traditional codecs is an optimal spatial assignment of quality level (QP).

%Likewise, when a whole frame does not contain information immediately related to the inference results, its quality can be aggressively lowered (or safely skipped). 
%In other words, only a portion of the pixels are {\em quality sensitive}.

%\jc{need to explain what high quality and low quliaty mean}

\subsection{An idealized design point}
\label{subsec:idealized}

Next, we analyze the optimal spatial quality assignments and their performance.
To make the discussion more concrete, we split each $\OriginWidth\cdot\OriginHeight$ frame into $\GridWidth\cdot\GridHeight$ grids of 16x16 blocks ($\OriginWidth=16\GridWidth,\OriginHeight=16\GridHeight$) and assign each block either a high quality or a low quality. % (this aligns with previous work~\cite{eaar,dds}).
We now consider this problem: what is the best quality assignment for these 16x16 blocks that maximizes the accuracy subject to no more than $\MaxHighQualityFrac$ blocks encoded in high quality.
Formally, it searches for a binary mask $\Mask$ of size $\GridWidth\cdot\GridHeight$ ($\Mask_{x,y}=1$ means block $x,y$ is in high quality), such that 

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\textrm{max} &~~~~\SimFunc\left(\DNN(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage),\DNN(\HighImage)\right) \label{eq:idealized-objective}\\
\textrm{s.t.} & ~~~~ \Vert\Mask\Vert \leq \MaxHighQualityFrac
\end{align}
}
where $\HighImage$ and $\LowImage$ are the high-quality encoding and the low-quality encoding of each frame\footnote{The dimension of a frame is the same for different QP values, so $\HighImage$ and $\LowImage$ have the same dimension.}, $\DNN:\mathbb{I}\mapsto\mathbb{O}$ returns the DNN inference result ($\mathbb{I}$ and $\mathbb{O}$ are the spaces of input frames and DNN output), and $\SimFunc:\mathbb{O}\times\mathbb{O}\mapsto\mathbb{R}$ (defined in \S\ref{sec:back}) returns the accuracy of $\DNN$'s output on a compressed frame by comparing its similarity with $\DNN$'s output on the high quality image $\DNN(\HighImage)$. 


This formulation involves two simplifying assumptions: the 16x16 blocks may be suboptimal boundaries between quality levels, and it restricts the encoding to only two quality levels.
That being said, we believe that analyzing this formulation is still valuable for two reasons.
First, the block granularity of 16x16 is on par with the block sizes employed in H.264 and H.265, which means more fine-grained blocks will not have much impact on the encoded video size. 
Second, the use of two quality levels does subsume many recent solutions (\eg~\cite{vigil, dds, awstream, glimpse, reducto}) which use two or fewer quality levels.


To search for the ideal solution, we consider an idealized design point that can run the final DNN ($\DNN(\cdot)$) as many times as needed (\ie it is idealized, not practical).
Figure~\ref{fig:tradeoff-mpeg-idealized} shows that the accuracy-compression tradeoffs of the idealized assignment 
% (with QP = 30 \kt{kpt detection also}) 
achieve 9-26\% higher accuracy than the traditional codec tradeoffs at the same compression rate. 
% Figure~\ref{fig:percpixel-accuracy} illustrates the reason behind 
A closer investigation reveals the reason behind the idealized assignments' superior tradeoffs: encoding only 6.3\% 16x16 grids still allows it to hit 90\% accuracy.

As a reference point, we also show two other heuristics for selecting the high-quality blocks: ``Object-based'' heuristics selects all blocks that overlap with some of the final DNN's detected bounding boxes (note that this is not practical either), and ``DDS'' is a recently proposed solution~\cite{dds} that selects the region proposals for which the final DNN has low confidence.
The two heuristics embody a popular assumption underlying most prior work that uses spatially different quality levels: only regions directly associated with the inference results (either the bounding box or region proposals that have not been confirmed) need to be encoded in high quality.
However, Figure~\ref{fig:tradeoff-mpeg-idealized} shows a substantial performance gap between these heuristics and the idealized assignments. 
% \jc{refer to fig 3 if new lines are added}
%Intuitively, these two strawmen assume that only regions of the difficult-be-detected objects need to be encoded in high quality, which represents the basic premise behind the state-of-the-art techniques~\cite{??,??}. 

% \jc{need to say something about other applications}

\begin{comment}
\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \includegraphics[width=0.4\columnwidth]{figs/hq_percentage.pdf}
    \caption{Percentage of pixels encoded in high quality v.s. accuracy. Only 6.3\% of the pixels need to be encoded to make accuracy more than 0.9.
    \jc{add a line for dds and object-based.}
    \kt{Object will cover a fixed size of high quality pixels}
    }
    \label{fig:percpixel-accuracy}
\end{figure}
\end{comment}

% compares the idealized design point with the two strawmen and the uniform-quality H.264 baseline. 
%Here, we use \fillme and \fillme as the high and low quality level, and \fillme as the codec.
%To show the full spectrum of their effectiveness, these strawmen are tested with a varying confidence score on the bounding boxes or the region proposals.
%Across the three tasks, we can see that the idealized design achieves same high accuracy with \fillme\% less bits than the best of the three baselines.
%Figure~\ref{fig:percpixel-accuracy} further reveals that the reduced file size (in the case of object detection) results from less blocks being selected for high quality encoding. 




\begin{comment}

introduce an idealized design point to help us understand the optimal spatial quality assignment.
In theory, the best 


The idealized design uses searches for a near optimal quality assignment, and  with the access to ground truth


Nonetheless, the spatial variation quality sensitivity is much more complex than the split of background and foreground. 
%To show the effectiveness of encoding videos with spatiotemporally different quality levels, 
To show it, we consider a simplified design point.
Given a video (originally encoded in the highest quality) and a DNN model, it first splits each $\OriginWidth\cdot\OriginHeight$ frame into $\GridWidth\cdot\GridHeight$ grids of 16$\times$16 blocks ($\OriginWidth=16\GridWidth,\OriginHeight=16\GridHeight$)\jc{we need a discussion on the block size}, assigns each block either a high quality $\HighQuality$ or a low quality $\LowQuality$, and then encodes the frames into a low-quality video and a high-quality video, each containing only blocks assigned with the perspective quality (Figure~\ref{??} depicts an example). 
During inference time, the two videos are decoded and the blocks are put in their original positions in the frames, and the frames are then fed in the DNN for inference. 
To measure its potential, we assume that the quality assignment logic can run the DNN (\eg to test its accuracy on any quality assignment), and we will remove this assumption in the actual video stack. 

In the idealized design point, the assignment of quality per block is such that the DNN inference accuracy is maximized while no more than $\MaxHighQualityFrac$ blocks are in high quality. 
In theory, one needs to enumerate all $2^{\GridWidth\cdot\GridHeight}$ possible quality assignments. 
So to make it tractable, we obtain a near-optimal mask with the following process.
We define a binary $\GridWidth\cdot\GridHeight$ {\em mask} to indicate the quality level assigned to each block (1 means $\HighQuality$, 0 means $\LowQuality$).
Given a mask $\Mask$, the encoding image can be expressed by $\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage$ where $\times$ is element-wise multiplication between two matrices and $\HighImage$ and $\LowImage$ are the high quality encoding and the low quality encoding of the frame. Note that the dimensions of a frame is independent of QP, so $\HighImage$ and $\LowImage$ have the same height and width.
Now let us use $\DNN:\mathbb{I}\mapsto\mathbb{O}$ to denote the DNN inference function (where $\mathbb{I}$ and $\mathbb{O}$ denote the space of input frames and the space of DNN output) and $\SimFunc:\mathbb{O}\times\mathbb{O}\mapsto\mathbb{R}$ (defined in \S\ref{sec:back}) to denote the accuracy function of the output of $\DNN$ on a compressed frame by comparing its similarity with $DNN$'s output on the high quality image. 
The optimization objective of the idealized design can be expressed as follows:
\begin{align}
\textrm{max} &~~~~\SimFunc\left(\DNN(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage),\DNN(\HighImage)\right) \label{eq:idealized-objective}\\
\textrm{s.t.} & ~~~~ \Vert\Mask\Vert \leq \MaxHighQualityFrac
\end{align}

% Then given a DNN inference function $\DNN(\cdot)$ and the accuracy function $\AccFunc(\cdot)$ (defined in \S\ref{sec:back}) that evaluates the accuracy of the output of $\DNN(\cdot)$, the optimization objective of the idealized design can be expressed as follows:
% \begin{align}
% \textrm{max} &~~~~\AccFunc\circ\DNN(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage) \label{eq:idealized-objective}\\
% \textrm{s.t.} & ~~~~ \Vert\Mask\Vert \leq \MaxHighQualityFrac
% \end{align}

\jc{Kuntai, please briefly explain how you solved it iteratively?}


\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \includegraphics[width=0.6\columnwidth]{figs/hq_percentage.pdf}
    \caption{Percentage of pixels encoded in high quality v.s. accuracy. Only 6.3\% of the pixels need to be encoded to make accuracy more than 0.9.}
    \label{fig:percpixel-accuracy}
\end{figure}

We acknowledge that the formulation entails three simplifying assumptions: it restricts the choice of encoding quality to two levels; there are more efficient encoding methods, such as region-of-interest encoding, for videos with a spatially different quality levels than creating two separate video files; and the $16\times16$ square blocks may not align with the optimal boundaries between regions that require different quality levels.
Nonetheless, we believe that analyzing this formulation is still valuable. 
In some sense, it generalizes the design space of several recent solutions: \jc{why it generalizes vigil, dds, awstream, glimpse, reducto}


To put it in perspective, we also consider two other ways of selecting which blocks to encode in high quality: one selects the blocks that overlap with one of the final detected bounding boxes, and the other one selects the blocks that overlap with one of the region proposal bounding box. 
Intuitively, these two strawmen assume that only regions of the difficult-be-detected objects need to be encoded in high quality, which represents the basic premise behind the state-of-the-art techniques~\cite{??,??}. 


Figure~\ref{fig:tradeoff-mpeg-idealized} compares the idealized design point with the two strawmen and the uniform-quality H.264 baseline. 
Here, we use \fillme and \fillme as the high and low quality level, and \fillme as the codec.
To show the full spectrum of their effectiveness, these strawmen are tested with a varying confidence score on the bounding boxes or the region proposals.
Across the three tasks, we can see that the idealized design achieves same high accuracy with \fillme\% less bits than the best of the three baselines.
Figure~\ref{fig:percpixel-accuracy} further reveals that the reduced file size (in the case of object detection) results from less blocks being selected for high quality encoding. 


\end{comment}

%Across the three tasks, we can see that only encoding \fillme-\fillme\% blocks in high quality still yield more than \fillme-\fillme\% of accuracy.
%We measure the potential improvement of the idealized design point on one of our video datasets (more details in \S\ref{subsec:eval:setup}), which consists of \fillme drone camera videos (\fillme minutes in total), and use \fillme and \fillme as the high and low quality level, and \fillme as the codec. 
%We choose these videos since they include a variety of scenarios (urban and rural), object classes (various vehicles and pedestrians), viewing angles, and object sizes. 
%\S\ref{sec:eval} will compare various techniques on a wider range of video sources.


%\vspace{0.1cm}
%\noindent{\em {\bf Observation \#1:} }
%\vspace{0.1cm}


%We first examine the {\em quality-sensitive blocks} (\ie blocks assigned with $\HighQuality$) as a fraction of all blocks in three of the canonical video analytics tasks: object detection model (\fillme), key point detection (\fillme) and semantic segmentation (\fillme).
%Figure~\ref{fig:percpixel-accuracy} shows the distribution of the quality-sensitive block fraction across frames in the videos. 
%Across the three tasks, we can see that only encoding \fillme-\fillme\% blocks in high quality still yield more than \fillme-\fillme\% of accuracy.
%
%To put it in perspective, {\em such fractions of quality-sensitive pixels are even less than claimed by previous work.}
%We zoom in on the object detection task and compare this idealized design with two other ways of selecting quality-sensitive blocks: one selects the blocks that overlap with one of the final detected bounding boxes, and the other one selects the blocks that overlap with one of the region proposal bounding box. 
%(To show the full spectrum of their effectiveness, these strawmen are tested with a varying confidence score on the bounding boxes or the region proposals.)
%Intuitively, these two strawmen assume that only regions of the difficult-be-detected objects need to be encoded in high quality, which represents the basic premise behind the state-of-the-art techniques~\cite{??,??}. 
%
%Figure~\ref{??} shows the fraction of quality-sensitive blocks and the resulting accuracy of the idealized design and the two strawmen. 
%\jc{some numbers from the graph}


%\mypara{Block-wise quality differentiation}
%For DNN-based analysis, the power to impact accuracy is not evenly distributed between pixels.
%Thus, we can save bandwidth by aggressively lowering the pixels that does not impact accuracy too much.
%At codec level, however, the quality of pixels are organized by blocks.
%Inside each block, the quality of pixels are the same.
%Thus, block is the minimum granularity for quality differentiation.

%\mypara{Mask}
%To quantify the compression opportunity of quality differentiation, we present a concept: \textit{mask}.
%\textit{Mask} maps each block to its corresponding encoding quality.
%
%\mypara{Potential bandwidth saving} 
%We measure the potential bandwidth saving of this opportunity on VisDrone dataset~\cite{aiskyeye} with object detection model FasterRCNN-ResNet50~[\fillme] as our backend model. 
%We use two different encoding qualities: low quality and high quality\footnote{\fillme} to encode each block.
%To determine the encoding quality of each block, our steps are:
%\kt{Substitude this into an algorithm for general vision tasks}
%\begin{packedenumerate}
%    \item Encode the whole video in high quality and collect the bounding box $b_i$ for each object $i$.
%    \item For each object, we assign a new bounding box $b'_i$, of which the center is the same with $b_i$ and the size of this bounding box is $0$.
%    \item Partition the whole frame into 16$\times$ 16 blocks.
%    \item Use highest quality to encode those blocks that overlaps with any of $b'_i$, and use lowest quality to encode other blocks.
%    \item If less than 95\% objects are detected, for those objects $j$ that are not detected, enlarge $b'_i$ by padding a constant on the left, top, right, bottom on it, and go back to step 3.
%\end{packedenumerate}


% One way to save bandwidth is to reduce the encoding quality.
% Also, the power to impact accuracy is not evenly distributed between pixels.
% It follows that we can saving bandwidth through manipulating pixel encoding quality.
% However, the pixels inside the same block (determined by the codec) will always have the same quality.
% So we instead encode

% \mypara{Heterogeneous quality sensitivity requirements} 
% Different vision models care about different parts in the video. For example, vehicle detection models care car pixels much more than human pixels; and human detection models care human pixels much more than car pixels. In terms of encoding, it means that different vision models are more sensitive to the encoding quality of some blocks more than other blocks.

% This opportunity implies that we can save bandwidth if we encode those quality-sensitive blocks in high encoding quality and those quality-insensitive blocks in low encoding quality.

% \blindtext


\subsection{Improvement analysis}
\label{subsec:analysis}


Therefore, a natural question is: why encoding similar number of blocks allows the idealized quality assignment to achieve higher accuracy than the baselines?
%the source of improvement of the idealized design point is.
%In other words, what have the strawmen missed in their assumptions.

\vspace{0.1cm}
\noindent{\em {\bf Observation \#1:} Quality-sensitive blocks are not aligned with inference results (\eg objects, boundaries).}
\vspace{0.1cm}

% To begin with, 
We observe that the quality-sensitive blocks selected by the idealized design are {\em not} strictly aligned with the detected bounding boxes or region proposals. 
Figure~\ref{fig:object-hqblock} shows two illustrative examples.
(a) shows that the high quality sometimes is needed at the surrounding blocks to provide enough context for Conv layers to extract sufficient reliable features. 
(b) shows that the high quality blocks do not always need to cover the whole object.
% The object cannot be detected in low quality, but does not need to be entirely encoded in high quality either. 
Instead, an object can be detected at the right locations even when only parts of the object is encoded in high quality.
% inference to be accurate.
% Even when completely encoded in high quality, those small objects cannot be detected because their sounding pixels are in low quality for Conv layers to extract sufficient reliable features. 
%On the other hand, we see in (b) that some objects cannot be detected even if they are entirely encoded in high quality. 
% Instead, some surrounding blocks must be encoded in high quality as well.
%\jc{maybe there are blocks that are not associated with any detected object, but need to be in high quality just to winnow out non-objects?}
We then test this observation on all frames in Figure~\ref{fig:tradeoff-mpeg-idealized}(a), and calculate the intersection-over-union between the optimally selected high-quality blocks and the detected bounding boxes. 
Figure~\ref{fig:obj-iou-cdf} shows that on more than half of the frames, the IoU is less than 0.5, indicating non-trivial misalignments. 

%that across all frames, there is significant misalignment between the inference results of object detections (bounding boxes) and high-quality blocks selected by the idealized design point.
%\jc{more read of the graph}



\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/object-hqblock.pdf}
    % \includegraphics[width=0.8\columnwidth]{figs/fig5_allhq.pdf}
    
    % \includegraphics[width=0.8\columnwidth]{figs/fig5_parthq.pdf}
    \includegraphics[width=0.87\columnwidth]{figs/fig5.pdf}
    
    \tightcaption{
    % Inference results on images with different regions in high quality. 
    Illustrating mismatches between optimally selected high-quality blocks and object regions.
    (a) Some objects need surrounding pixels in high quality to be detected and (b) some objects do not need to be all in high quality to be detected. \jc{add sub (a) and (b)}}
    \label{fig:object-hqblock}
\end{figure}

\begin{figure}
    \centering
%    \includegraphics[width=0.5\columnwidth]{figs/placeholder-obj-iou-cdf.pdf}
    \includegraphics[width=0.4\columnwidth]{figs/obj_ideal_iou_cdf.pdf}
    \tightcaption{\kt{Over half of the selected high-quality blocks have an IoU < 60\% compared to object detection bounding boxes.}There is not strong overlap between the inference results of object detections (bounding boxes) and high-quality blocks selected by the idealized design point.}
    \label{fig:obj-iou-cdf}
\end{figure}



% We have seen that the final inference results (even if they are known) are a poor indicator of the optimal quality assignment, what decides the quality-sensitive blocks then?

\vspace{0.1cm}
\noindent{\em {\bf Observation \#2:} Quality-sensitive blocks are highly dependent to the inference task and DNN.}
\vspace{0.1cm}


Empirically, we found that the optimal quality assignments are highly dependent on the final DNNs and the task. 
To show this dependency, Figure~\ref{fig:task-dependent} takes the segmentation and object detection DNNs, gets their perspective optimal quality assignments (with QP = 30) on the same set of videos, and tests the performance of each quality assignment in the other task's DNN. 
We see that accuracy drops substantially when the quality assignment is tested on a different DNN than it was customized on.
% \jc{some numbers from the graph}
Figure~\ref{fig:model-dependent} zooms in on one task (object detection), and shows that if one re-uses the quality assignment designed for one DNN to encode the video and feeds it to another DNN, the accuracy will be significantly lower, even though they are both object detectors trained to detect the same classes of objects!
% \jc{can the resulting map be different if you just run the idealized algorithm on the same DNN again?}

%first take one DNN for each analytics task and use the idealized design to optimally select \fillme\% of spatial blocks for each DNN in each frame to encode in $\HighQuality$. 
%Figure~\ref{fig:task-dependent} compares the accuracy of each DNN when fed with the frames encoded using the quality assignment designed for the model vs. the frames encoded using the quality assignments designed for the other two DNNs.
%We see that the accuracy drop substantially when the quality assignment is customized for another model. 
%\jc{some numbers from the graph}


%takes three different object detection DNNs as an example and compares their accuracies on the video encoded with its corresponding quality assignment and on the  videos encoded with the other two models' quality assignments.
%We see that the accuracy of a DNN drops substantially when it runs on the quality assignment of design for other models.
%Zooming in, we found that the exact blocks that have to be encoded in high quality change across the DNNs, even though they are trained to detect same objects!
%\jc{some numbers from the graph}








\begin{figure}[t]
    %   \subfloat[Across video-analytics tasks]
    %   {
    %      \includegraphics[width=0.48\linewidth]{figs/placeholder-task-dependent.pdf}
    %      \label{fig:task-dependent}
    %   }
    %   \subfloat[Across models (object detection)]
    %   {
    %      \includegraphics[width=0.48\linewidth]{figs/placeholder-model-dependent.pdf}
    %      \label{fig:model-dependent}
    %   }
    \centering
       \subfloat[Across vision tasks]
       {
         \includegraphics[height=0.25\linewidth]{figs/multi_app.pdf}
         \label{fig:task-dependent}
       }
       \subfloat[Across models (object detection)]
       {
         \includegraphics[height=0.25\linewidth]{figs/multi_DNN.pdf}
         \label{fig:model-dependent}
       }
    \tightcaption{The quality-sensitive regions are highly dependent to the inference task and DNN. }
    \label{fig:}
\end{figure}


\subsection{Summary of key findings}
The goal of this section is to understand the idealized way of using traditional codecs and where existing solutions fall short. 
%the gap between existing solutions and on traditional codecs.
Using three video analytics tasks and real-world videos, we show that:
\begin{packedenumerate}
\item Traditional codecs such as H.264 are qualitatively suitable for video analytics: when QP is relatively low (<36), their encoding processes tend to discard higher-frequency details which are also not needed by DNN inference either. 
However, as QP grows (>36), they start to filter out information needed by the DNN feature extractions.
\item If one optimally assigns high quality (QP=30) to a selected set of spatial blocks, we can achieve the same high accuracy as if feeding the high quality video to the DNN but encoding only 6.3\% of spatial blocks in high quality (the rest in QP=50). 
% , which gives rise to a 70\% reduction on video file size.
\item Achieving this potential improvement inspires us to rethink the design assumptions behind prior solutions.
\begin{packeditemize}
\item The idealized quality assignments are not strictly aligned with the objects or region proposals. 
In object detection, for instance, the IoU between pixels assigned with high quality and those assigned with bounding boxes is smaller than 50\% most of the time.
% \fillme\% of pixels assigned with high quality are not in the objects' bounding boxes and \fillme\% of pixels in the objects' bounding boxes do not need to be in high quality.
\item The idealized quality assignments are greatly dependent not only on the vision task but on the specific DNN.
At the same frame, the quality assignment generated for one DNN may result in 12\% lower accuracy when used to generate input frame to another DNN.
\end{packeditemize}
\end{packedenumerate}

%\begin{figure}
%    \centering
%\includegraphics[width=0.4\columnwidth]{figs/hetero-task.pdf}
%    \caption{Accuracy on different task with the same compressed video. One size does not fit for all vision tasks.}
%    \label{fig:hetero-task}
%\end{figure}
%
%\begin{figure}
%    \centering
%\includegraphics[width=0.4\columnwidth]{figs/hetero-dnn.pdf}
%    \caption{Accuracy on different object detection DNN with the same compressed video. Accurate compression for cheap model may not work on expensive model.}
%    \label{fig:hetero-dnn}
%\end{figure}

%This compression opportunity varies a lot between different vision tasks and models.
%In other word, one mask that works perfectly for one application might result in poor accuracy in another application.
%In Figure \ref{fig:hetero-task}, accurate compression for keypoint detection does not work on object detection and semantic segmentation.
%So compression need to be designed for different applications.
%Moreover, in Figure \ref{fig:hetero-dnn}, we see that even under the same vision task, compression that works for one DNN may not work on others.




%\mypara{Takeaways} During the measurement above, we find that:
%\begin{packeditemize}
%    \item To reproduce satisfactory inference result, only a small fraction of blocks need to be encoded in high quality. From Figure \ref{fig:percpixel-accuracy}, we can see that covering only \fillme\% pixels will yield more than \fillme\% of accuracy.
%    \item Object may not align with the high-quality blocks. From Figure \ref{fig:object-hqblock}, we see that some objects do not need to be all in high quality to be detected, and some objects need surrounding pixels in high quality to be
%\end{packeditemize}
%
%\mypara{Heterogeneity between vision tasks and models}
%This compression opportunity varies a lot between different vision tasks and models.
%In other word, one mask that works perfectly for one application might result in poor accuracy in another application.
%In Figure \ref{fig:hetero-task}, accurate compression for keypoint detection does not work on object detection and semantic segmentation.
%So compression need to be designed for different applications.
%Moreover, in Figure \ref{fig:hetero-dnn}, we see that even under the same vision task, compression that works for one DNN may not work on others.
%
%\blindtext


\begin{comment}

\subsection{Mismatch of existing solutions}

\kt{
\begin{itemize}
\item{Human perception-centric quality encoding}
\begin{itemize}
\item the highly sensitive blocks are highly dependent on the task
\item existing heuristics are completely unaware of the server-side dnn structure
\item implications: need a generic way to encode videos in cognizant of the block-level sensitivity. [an illustrative example]
\end{itemize}
\item{Encoding dynamic quality sensitivity}
\begin{itemize}
\item the highly-sensitive pixels changes a lot across frames
\item today's encoding is inefficient: unnecessary motion vector, etc.  micro-block misalignment
\item implications: need a way to ``smooth'' the highly dynamic sensitive blocks [an illustrative example]
\end{itemize}
\item{Frame-wise semantics}
\begin{itemize}
\item analyzing the whole frames one by one
\item implications: putting sensitive regions together [an illustrative example]
\end{itemize}
\end{itemize}}


In general, prior work on video stack propose either new codecs or smarter ways of compressing/streaming videos over existing codecs.
In this context, we now discuss potential mismatches in both directions with respect to what an idealized video stack need.



As mentioned earlier, the idealized algorithm essentially explores a similar design space of previous work, but at a different (finer) granularity (small blocks instead of bounding boxes) and with access to the DNN (such that we can reveal the ideal improvement).
By analyzing the encoding decisions made by the idealized design, we found two 


\mypara{Limitation of existing work} 
Wrong assumptions of related work was revealed by our measurement study above. 
The vast majority of current works on quality differentiation~\cite{dds,vigil,glimpse,eaar} implicitly assumes that high quality regions should align with the objects.
However, in Figure \ref{fig:object-hqblock}, we see that high quality regions can be much smaller or much larger than the object itself.
So objects might be missed or file size might be wasted if aligning high quality regions with objects.



\mypara{Traditional video codec}
Caring about visual quality, traditional video codec pays nearly equal attention to all pixels. 
The quality-sensitive blocks, however, are highly dependent on server-side DNNs.
Traditional video codec is unable to exploit this opportunity due to its unawareness to server-side DNN.
This implies that we need a generic way to encode the videos in cognizant of block quality-sensitivity, see Figure \fillme for an illustration.

\mypara{Super resolution}
Nowadays, super resolution \cite{cloudseg,livenas} gradually becomes a new choice of video codec.
These approaches encode the video in low quality, store or stream the low quality video at server side, and then compensate the quality loss by super resolution network.

However, super resolution is fundamentally an ill-suited problem. Multiple high-quality frames may have exact same low-quality frames if compressed by the codec.
As a result, even the most compute-intensive super resolution network cannot fully recover the areas crucial to inference results. Figure \fillme shows an example.
To overcome this issue, current approaches choose to retrain the neural network online. This design choice poses too much online cost at the server side.

\mypara{Auto-encoder}
Computer vision community is actively exploring a new type of codec called auto-encoder~\cite{rate-distortion-autoencoder}. These approaches encode the video by feeding it through neural network and storing the output of that neural network. 

Unfortunately, auto-encoder that preserves high image quality is too compute-intensive for a single CPU to afford (\fillme seconds per frame).
Moreover, this approach requires another neural network as the decoder. Thus, every frame needs to be processed by the decoder at inference time and poses too much online overhead. 



\subsection{Mismatch of existing video analytics pipelines}

\kt{Benefit different vap, weaken this argument}

\kt{
\begin{itemize}
%\item approach \#1: twisting existing interface, (2) case-by-case heuristics
\item limitation \#1: fail to adapt to real-time video content (sr, awstream, vstore)
\item limitation \#2: slow costly (dds, dnn-based autocodec)
\item limitation \#3: only applies to one task (vigil, eaar, focus)
\end{itemize}}

Video analytic pipelines stream videos from the camera to the server and generate analytic results with minimum overhead as well as maintaining satisfying accuracy. However, these approaches are not suitable for video stack purpose.

\mypara{Agnostic to real-time video content} 
AWStream~\cite{awstream} and CloudSeg~\cite{cloudseg} exploit the optimal configurations~\cite{awstream} or  super resolution networks~\cite{cloudseg} derived from \textit{history video content} and count on the similarity between real-time video content and history video content.
However, in real world, the video content can change drastically. 
For example, when a car equipped with traffic camera driving on a street that human rarely appears, the system needs to adapt every time human appears to detect all of them.
These approaches are likely to have low accuracy in these scenarios.

\mypara{Too much online cost for real-time content adaptation} 
Instead, DDS~\cite{dds} choose to leverage server-side compute to adapt for video content. 
As for the online cost, however, DDS needs to run one extra inference per frame to dig out the objects that are missed, which doubles the online cost.

\mypara{Task-specific}
Vigil~\cite{vigil}, EAAR~\cite{eaar}, Focus~\cite{focus} can leverage real-time video content at relatively low cost.
Their use cases, however, are limited to object detection~\cite{vigil, eaar} and frame classification~\cite{focus} and make them not applicable for other vision tasks and applications.

\end{comment}









==> motivate-v4.tex <==

\section{Motivation}
\label{sec:motivation}

\begin{itemize}
    \item Video analytic applications on edge devices is pervasive.
    \item While deploying video analytic applciations to edge devices, we found a largely-ignored use case: edge devices can only access server resources upon incidents.
    \item Previous work compress videos based on bounding boxes to deliver high encoding quality regions. This misses opportunities to further discriminate the quality of pixels inside and outside the bounding boxes. We show the high potential gain of this opportunity
\end{itemize}

Nowadays, more and more videos captured on edge devices are generated for analytic purposes instead of watched by human viewers. 
This trend reveals a new research opportunity: compressing videos to maintain accurate analytic results rather than maintaining visual quality. 

Previous works found that: different from human beings that care about the overall visual quality, some pixels are much more important than the others for DNNs to generate accurate analytic results.
For example, the pixels on the objects, like car pixels and human pixels, are much more important than background pixels like tree pixels and building pixels for those object detection DNNs.
Moreover, the pixels that are important to inference accuracy are constantly changing based on video contents.
For example, when a car quickly drives across the traffic camera, the corresponding car pixels, which are important for DNN to detect the car, are also quickly moving.
Based on these two observations, previous works find important pixels by streaming the video to the server-side DNN, and get the server-side DNN feedback in real-time~\cite{dds,eaar}.




Despite the high compression efficiency, these approaches heavily rely on a high quality camera-server connection (the bandwidth requirement is about 1 Mbps\footnote{We calculate this based on the encoding of DDS~\cite{dds}. We encode this video~\cite{trafficcam-example} in low quality (QP 40), calculate the bandwidth for it, and then double the bandwidth to estimate the bandwidth usage of high quality and low quality video streams.}) in order to stream the video stream in real time.
This makes these approaches not applicable on the cameras that prefer not to stream their videos out, like the cameras with no LTE connection (like wild-life camera~\cite{deercam} and cheap dashcam~\cite{cheap-dashcam}) or privacy concerns (like home camera~\cite{HOA-homecam,forbes-homecam}).
% \mypara{Design for future analysis} 
% \jc{i would replace ``retrospective'' with a different word. ``retrospective'' sounds like you don't even know what model will be used to analyzed the video.}
% When deploying these algorithms to edge devices, these works all assume that the edge devices have the access to the server and performs edge-cloud optimization jointly. However, we will show that there are a lot of usecases where the cameras are disconnected from the server and have to archive the video and wait for retrospective analysis. To tackle these usecases, we desire an algorithm that can perform \textbf{cheap and local} encoding.
% \jc{``cheap and local'' can be misleading. vigil, glimpse, focus, all have ``cheap and local'' processing. how about start with why dnns are increasingly used to decide encoding quality in real time, and then say there is currently no ``cheap and local'' way to do that?}
In these scenarios, we desire a {\em cheap and DNN-aware} approach that deliver equal or even higher compression efficiency than previous works~\cite{dds,eaar} while being affordable for a cheap camera.






Moreover, these approaches also generate the important pixels by filtering the {\em bounding boxes} generated from the neural network.
However, we observe that the important pixels do not align with the bounding box boundaries.
Some of the pixels outside the bounding boxes are still helpful for the neural network to separate the object from the boundary and some of the pixels inside the bounding box are also not important.
For example, in Figure~\ref{fig:object-hqblock}(a), the boundary pixels of the object must be encoded to make the object detected, in Figure~\ref{fig:object-hqblock}(b), the car door pixels are less important than the car wheel pixels and the car window pixels and can be encoded in low quality.
We also perform measurements (see \S\ref{subsec:microblock}) to show that we will have 3x file size reduction compared to only encoding the pixels of the object in high quality in an ideal scenario.
% \mypara{Design for efficient compression} 
% \jc{this seems to be about finer-grained encoding can improve accuracy and compression? if so, say it that way.}
% On the technical side, current algorithms perform spatial compression by looking at the boxes generated from DNN's intermediate output such as region proposals~\cite{dds,eaar}. However, we will show that the pixels that need to be encoded into high quality are \textbf{not} aligned with the object boundary. Based on this observation, we need to assign encoding quality for each microblock (the minimum encoding unit for the video codec to operate on) based on the need of server-side DNN.



\subsection{Design space}

\mypara{Design space}
To put our design into perspective, we first sketch the space of various potential design points.
\begin{packeditemize}
\item {\em Choice of codec:}
One option is to re-use a traditional codec (\eg H.264/265~\cite{1218189}, VP9~\cite{6737765}) and tune its parameters (\eg quantization parameters). 
There are also alternative NN-based codecs (\eg super resolution~\cite{cloudseg}, autoencoder~\cite{rate-distortion-autoencoder}), but they have yet to see the wide industry adoption enjoyed by the traditional codecs, and they usually have compute-intensive encoding (\eg autoencoder) and decoding (\eg super-resolution).
In this work, we take a pragmatic stance to build our video stack on traditional codecs, like most work in this space.


\item {\em Quality adaptation granularity:}
To cope with the dynamics of video content, prior work tries to adapt quality by saving only a subset of frames (\eg~\cite{glimpse,reducto,awstream}), assigning different quality to different frames (\eg~~\cite{awstream,vstore,chameleon}), and/or assigning a higher quality to only object bounding boxes or region proposals (\eg~~\cite{vigil,dds,eaar}).
In this work, we assign quality for each fine-grained blocks (16x16 pixels), which as shown in the next section could lead to much better compression efficiency and inference accuracy than the aforementioned granularities.


\item {\em Integration with final DNN:}
Using the final DNN's output (or intermediate features) does help to identify regions of interest (\eg~\cite{eaar,dds}), but it potentially adds a prohibitive overhead to encoding (especially for archived videos most of which will not be analyzed).
On other other hand, using cheap heuristics that are agnostic to the final DNN has been shown to produce suboptimal compression efficiency and/or low inference accuracy~\cite{dds}.
In this work, we design a shallow NN to infer a (near-)optimal quality assignment, which as we will see is a much simpler task than the actual final inference.

\end{packeditemize}

\subsection{Deploy camera for future analysis}



\begin{table}
{\small
\begin{tabular}{cc} 
\hline
Name & Runtime (ms) \\ [0.5ex]
\hline
Ours & 20 \\ 
\hline
TinyYoLo & 40\\
\hline
\end{tabular}

\caption{Comparison between runtime on our model and a cheap object detector like TinyYoLo.
\label{tab:tinyyolo}
\vspace{-0.3cm}
}
\label{tab:dataset}
}
\end{table}




Due to poor connectivity, power constraint or privacy concerns, it may be not feasible for the camera to stream the videos out.
Here are three example scenarios that the cameras are not able to access the internet.
\begin{packeditemize}
    \item {\em Wildlife camera}. 
    Wildlife cameras play a more and more important role in learning and protecting the animals~\cite{newyorktime-wildlifecam}.
    However, these cameras typically will be placed in the wild for several days to record enough data for future analytics.
    For example, deer cameras need to sample videos on its own for 10 days and then be retrieved back for future analysis~\cite{deercam}.
    Thus, limited by lacking of sufficient power and LTE connectivity, these cameras have to archive the video for future analytics.
    \item {\em Dashcam for personal use}. 
    A cheap dashcam is only \$50~\cite{cheap-dashcam}. 
    To equip with 4G connectivity, however, one need to purchase a \$150 LTE module~\cite{4GModule}, a SIM card and an expensive plan that provides sufficient bandwidth for video streaming. 
    Thus, the most economic option is to purchase a cheap dashcam, archive the videos and analyse these videos when needed.
    \item {\em Home camera.}
    Nowadays, people are more and more concerned about the privacy issue of home cameras~\cite{forbes-homecam,HOA-homecam}.
    The best way for the camera to maintain private is to avoid streaming the video out from the camera and archive the videos on the camera side for future anlaytics.
\end{packeditemize}


As a result, to serve these cameras, the challenge is: how to compress the video locally while still yields high compression efficiency?


One alternative approach is to leverage a cheap object detection algorithm to detect potential object of interests and encode the object of interests only.
However, the typical cheap object detector (such as TinyYoLO) is still much expensive compared with our approach for the camera to afford (the runtime of TinyYoLo is 2x compared to our approach as listed in Table~\ref{tab:tinyyolo}), and the overall file size-accuracy trade-off is poor (we will show this in \S\fillme).


That being said, our approach can still work under typical video streaming scenarios. To better support video streaming scenario, we also develop the bandwidth adaptation algorithm (see \S\label{sec:bandwidth-adaptation}) to cope with the dynamic bandwidth change and different user needs.

\subsection{Microblock-based encoding for efficient compression}
\label{subsec:microblock}

% On the other hand, videos need to be efficiently compressed to efficiently utilize limited storage/network resources.

% Previous works on video compression can be coarsely classified into two types:
% \begin{itemize}
%     \item Uniform spatial quality.
%     \item Box-based spatial quality differentiation
% \end{itemize}

% However, in the following measurements we show that this misses two opportunities with high compression potential.

% \jc{you need to introduce how you identified quality-sensitive microblocks. maybe we need a simpler methodology than the one we used before?}


In this part, we demonstrate the potential gain if we encode the videos without aligning the pixels in high quality with object boundaries.
We use 16x16 microblock as our basic encoding unit, the same as modern codecs such as H.264~\cite{h264} and H.265~\cite{h265}.



\mypara{Finding quality-sensitive blocks} 
We use an idealized heuristic to find the quality-sensitive blocks.
Initially, for each undetected element (an element can be an object, a pixel or a keypoint), we assign this element to one random microblock that overlaps with this element, and encode this block in high quality. 
We then iterate on each quality assignment 10 times according to the following rule: for each undetected element, we pick its corresponding block, enlarge this block by 16 pixels and then encode this enlarged block in high quality.

\begin{figure}[t]
       \subfloat[Object detection]
       {
         \includegraphics[width=0.32\columnwidth]{figs/measurement_detection.pdf}
         \label{fig:}
       }
       \subfloat[Semantic seg.]
       {
         \includegraphics[width=0.32\columnwidth]{figs/measurement_segmentation.pdf}
         \label{fig:}
       }
       \subfloat[Keypoint detection]
       {
         \includegraphics[width=0.32\columnwidth]{figs/measurement_keypoint.pdf}
         \label{fig:}
       }
    \tightcaption{In three analytics tasks, as encoding quality drops, traditional video codec (H.264) can compress videos by upto 50\%, after which inference accuracy starts to drop sharply. 
    However, encoding only selective spatial blocks (``ideal'') in high quality still retains high accuracy with smaller file size.}
    \label{fig:tradeoff-mpeg-idealized}
\end{figure}

\mypara{Performance analysis}
Figure~\ref{fig:tradeoff-mpeg-idealized} shows that the accuracy-compression tradeoffs of the idealized assignment 
% (with QP = 30 \kt{kpt detection also}) 
achieve 9-26\% higher accuracy than the traditional codec tradeoffs at the same compression rate. 
% Figure~\ref{fig:percpixel-accuracy} illustrates the reason behind 
A closer investigation reveals the reason behind the idealized assignments' superior tradeoffs: encoding only 6.3\% 16x16 grids still allows it to hit 90\% accuracy.

As a reference point, we also show two other heuristics for selecting the high-quality blocks: ``Object-based'' heuristics selects all blocks that overlap with some of the final DNN's detected bounding boxes (note that this is not practical either), and ``DDS'' is a recently proposed solution~\cite{dds} that selects the region proposals for which the final DNN has low confidence.
The two heuristics embody a popular assumption underlying most prior work that uses spatially different quality levels: only regions directly associated with the inference results (either the bounding box or region proposals that have not been confirmed) need to be encoded in high quality.
However, Figure~\ref{fig:tradeoff-mpeg-idealized} shows a substantial performance gap between previous works and the idealized assignments. 

%the source of improvement of the idealized design point is.
%In other words, what have the strawmen missed in their assumptions.

\vspace{0.1cm}
\noindent{\em {\bf Observation:} Quality-sensitive blocks are not aligned with inference results (\eg objects, boundaries, key points).}
\vspace{0.1cm}

% To begin with, 
We observe that the quality-sensitive blocks selected by the idealized design are {\em not} strictly aligned with the detected bounding boxes or region proposals. 
Figure~\ref{fig:object-hqblock} shows two illustrative examples.
(a) shows that the high quality sometimes is needed at the surrounding blocks to provide enough context for Conv layers to extract sufficient reliable features. 
(b) shows that the high quality blocks do not always need to cover the whole object.
% The object cannot be detected in low quality, but does not need to be entirely encoded in high quality either. 
Instead, an object can be detected at the right locations even when only parts of the object is encoded in high quality.
% inference to be accurate.
% Even when completely encoded in high quality, those small objects cannot be detected because their sounding pixels are in low quality for Conv layers to extract sufficient reliable features. 
%On the other hand, we see in (b) that some objects cannot be detected even if they are entirely encoded in high quality. 
% Instead, some surrounding blocks must be encoded in high quality as well.
%\jc{maybe there are blocks that are not associated with any detected object, but need to be in high quality just to winnow out non-objects?}
We then test this observation on all frames in Figure~\ref{fig:tradeoff-mpeg-idealized}(a), and calculate the intersection-over-union between the optimally selected high-quality blocks and the detected bounding boxes. 
Figure~\ref{fig:obj-iou-cdf} shows that on more than half of the frames, the IoU is less than 0.5, indicating non-trivial misalignments. 

%that across all frames, there is significant misalignment between the inference results of object detections (bounding boxes) and high-quality blocks selected by the idealized design point.
%\jc{more read of the graph}





\begin{figure}
    \centering
%    \includegraphics[width=0.5\columnwidth]{figs/placeholder-obj-iou-cdf.pdf}
    \includegraphics[width=0.4\columnwidth]{figs/obj_ideal_iou_cdf.pdf}
    \tightcaption{\kt{Over half of the selected high-quality blocks have an IoU < 60\% compared to object detection bounding boxes.}There is not strong overlap between the inference results of object detections (bounding boxes) and high-quality blocks selected by the idealized design point.}
    \label{fig:obj-iou-cdf}
\end{figure}



% We have seen that the final inference results (even if they are known) are a poor indicator of the optimal quality assignment, what decides the quality-sensitive blocks then?

% \vspace{0.1cm}
% \noindent{\em {\bf Observation \#2:} Quality-sensitive blocks are highly dependent to the inference task and DNN. \kt{remove this observation?}}
% \vspace{0.1cm}


% Empirically, we found that the optimal quality assignments are highly dependent on the final DNNs and the task. 
% To show this dependency, Figure~\ref{fig:task-dependent} takes the segmentation and object detection DNNs, gets their perspective optimal quality assignments (with QP = 30) on the same set of videos, and tests the performance of each quality assignment in the other task's DNN. 
% We see that accuracy drops substantially when the quality assignment is tested on a different DNN than it was customized on.
% % \jc{some numbers from the graph}
% Figure~\ref{fig:model-dependent} zooms in on one task (object detection), and shows that if one re-uses the quality assignment designed for one DNN to encode the video and feeds it to another DNN, the accuracy will be significantly lower, even though they are both object detectors trained to detect the same classes of objects!
% \jc{can the resulting map be different if you just run the idealized algorithm on the same DNN again?}

%first take one DNN for each analytics task and use the idealized design to optimally select \fillme\% of spatial blocks for each DNN in each frame to encode in $\HighQuality$. 
%Figure~\ref{fig:task-dependent} compares the accuracy of each DNN when fed with the frames encoded using the quality assignment designed for the model vs. the frames encoded using the quality assignments designed for the other two DNNs.
%We see that the accuracy drop substantially when the quality assignment is customized for another model. 
%\jc{some numbers from the graph}


%takes three different object detection DNNs as an example and compares their accuracies on the video encoded with its corresponding quality assignment and on the  videos encoded with the other two models' quality assignments.
%We see that the accuracy of a DNN drops substantially when it runs on the quality assignment of design for other models.
%Zooming in, we found that the exact blocks that have to be encoded in high quality change across the DNNs, even though they are trained to detect same objects!
%\jc{some numbers from the graph}








% \begin{figure}[t]
%     %   \subfloat[Across video-analytics tasks]
%     %   {
%     %      \includegraphics[width=0.48\linewidth]{figs/placeholder-task-dependent.pdf}
%     %      \label{fig:task-dependent}
%     %   }
%     %   \subfloat[Across models (object detection)]
%     %   {
%     %      \includegraphics[width=0.48\linewidth]{figs/placeholder-model-dependent.pdf}
%     %      \label{fig:model-dependent}
%     %   }
%     \centering
%       \subfloat[Across vision tasks]
%       {
%          \includegraphics[height=0.25\linewidth]{figs/multi_app.pdf}
%          \label{fig:task-dependent}
%       }
%       \subfloat[Across models (object detection)]
%       {
%          \includegraphics[height=0.25\linewidth]{figs/multi_DNN.pdf}
%          \label{fig:model-dependent}
%       }
%     \tightcaption{The quality-sensitive regions are highly dependent to the inference task and DNN. }
%     \label{fig:}
% \end{figure}


% \subsection{Summary of key findings}
% The goal of this section is to understand the idealized way of using traditional codecs and where existing solutions fall short. 
% %the gap between existing solutions and on traditional codecs.
% Using three video analytics tasks and real-world videos, we show that:
% \begin{packedenumerate}
% \item Traditional codecs such as H.264 are qualitatively suitable for video analytics: when QP is relatively low (<36), their encoding processes tend to discard higher-frequency details which are also not needed by DNN inference either. 
% However, as QP grows (>36), they start to filter out information needed by the DNN feature extractions.
% \item If one optimally assigns high quality (QP=30) to a selected set of spatial blocks, we can achieve the same high accuracy as if feeding the high quality video to the DNN but encoding only 6.3\% of spatial blocks in high quality (the rest in QP=50). 
% % , which gives rise to a 70\% reduction on video file size.
% \item Achieving this potential improvement inspires us to rethink the design assumptions behind prior solutions.
% \begin{packeditemize}
% \item The idealized quality assignments are not strictly aligned with the objects or region proposals. 
% In object detection, for instance, the IoU between pixels assigned with high quality and those assigned with bounding boxes is smaller than 50\% most of the time.
% % \fillme\% of pixels assigned with high quality are not in the objects' bounding boxes and \fillme\% of pixels in the objects' bounding boxes do not need to be in high quality.
% \item The idealized quality assignments are greatly dependent not only on the vision task but on the specific DNN.
% At the same frame, the quality assignment generated for one DNN may result in 12\% lower accuracy when used to generate input frame to another DNN.
% \end{packeditemize}
% \end{packedenumerate}







% \subsubsection{Encoding region inside the box with lower quality}

% \begin{itemize}
%     \item Large objects does not need to be encoded on high quality.
%     \item Introduce the heuristic algorithm. 
% \end{itemize}

% \begin{itemize}
%     \item We need more generalizable solution.
% \end{itemize}

% \subsubsection{Encoding region outside the box with higher quality}


% \begin{itemize}
%     \item Some objects also need surrounding pixels to be high quality to be detected.
%     \item Introduce the heuristic algorithm: enlarge those undetected objects.
%     \item Introduce the baselines
%     \item Demonstrate the eval figures and how to read it.
% \end{itemize}


==> motivate-v5.tex <==

\section{Motivation}
\label{sec:motivation}



\kt{
\begin{packeditemize}
    \item Three performence dimensions: high accuracy, low delay and low camera compute
\end{packeditemize}
}






We begin by motivating the two requirements that drive our design: the need for fine-grained quality optimization (\S\ref{subsec:macroblock}) and on-premise encoding using only local compute resource (\S\ref{subsec:local}).
As will be elaborated, prior work falls short on either requirement.
% These two goals lead to a new design point of a {\em cheap, local and DNN-aware} encoding algorithm, which we will explore in the next few sections.



% Nowadays, more and more videos captured on edge devices are generated for analytic purposes instead of watched by human viewers. 
% Different from human viewers that care about the {\em overall} visual quality, a {\em small fraction} of pixels are much more important than the others for DNNs to generate accurate analytic results.
% The conventional wisdom assumes that these pixels lie in a subset of objects.
% However, we revisit this assumption in \S\ref{subsec:macroblock} and show that it will actually lead to sub-optimal file size-accuracy trade-off.



% From the deployment side, previous works~\cite{dds,awstream,reducto,eaar} optimize the overall bandwidth-accuracy trade-off based on server-side compute.
% In fact, we will show in \S\ref{subsec:local} that a lot of cameras prefer not to stream their video out. 
% To facilitate the video analytics on these cameras, the key is to design a cheap and accurate encoding algorithm {\em without accessing the server online}.




\subsection{Optimizing video encoding for DNNs}

\kt{mention online and offline video streaming }



\mypara{Video analytics applications} 
Spurred by advances in computer vision, more video applications 
%increasingly augmented with computer vision (DNN) 
perform DNN-based inference on massive video streams. 
As depicted in Figure~\ref{fig:background}, many video analytics applications rely on efficient video-compression algorithms to encode the incoming video streams, and these videos will be analyzed by computer-vision algorithms, in forms of deep neural nets (DNNs).
These encoded videos fetched for future on-demand queries or streamed for online analytics by a compute-intensive video-analytics DNN (called {\em final DNN}) running on a more powerful (cloud) server.
To make our discussion more concrete, this paper focuses on three typical video analytics applications: object detection (one labeled bounding box for each object), semantic segmentation (one label for each pixel) and keypoint detection (17 keypoints for each human).

\kt{Add new para here}

\mypara{Video encoding for video analytics}

To better serve video analytics applications, we need an efficient video compression algorithm that reduces the file size without hurting the accuracy of the derived analytic results.
This is because reducing file size will reduce the network bandwidth requirement for video-streaming-based analytics, and will reduce the storage burden when the video is offline archived for future inference.
However, traditional video codecs (like H.264~\cite{h264} and H.265~\cite{h265}) are optimized for human perception rather than inference accuracy.
This gives us research opportunity.



\mypara{DNN-aware encoding optimization}
In many video-analytics applications, each DNN takes a non-trivial amount of time and effort to train\footnote{About 40\% companies take one month or longer to put their models into production~\cite{ml-deployment-time}, and the deployment time of their models is increasing year-on-year~\cite{ML_trends}. Moreover, 78\% of AI/ML projects stall at some stage before deployment~\cite{stall}.}, and many applications apply one DNN to analyze each video stream\footnote{Wildlife Insights mainly consumes wild life videos for species  detection~\cite{wildlife-application} and intuVision Traffic focuses on detecting cars and other vehicles for traffic videos}.
Therefore, we consider the setting where the DNN is known before we encode the incoming video streams and thus the encoding can be optimized for a given DNN. 
Same assumption is used in recent work (\eg~\cite{noscope,eaar,dds,awstream,elf}).
That said, the encoded videos should still work well for other DNNs of similar video analytics purposes (\eg among different object detectors). 


% As depicted in Figure~\ref{fig:background}, many video analytics applications rely on video compression algorithm\footnote{In this work, a video stack means a software wrapper on top of a video codec (H.264/265, VP8/9, etc) that tunes its performance for some higher-level application (video analytics tasks). In \S\ref{sec:eval}, we will evaluate our proposal's performance over various codecs and in various vision tasks.} for two basic operations: 
% {\em encoding} a stream of frames into a compressed video file as the frames are captured by a video sensor~\cite{vstore} for efficient storage and transmission, and {\em decoding} the compressed video file to individual frames/segments which are then fed into a {\em final DNN} for vision inference.
% These operations are needed for both offline analytics on archived videos (\eg~\cite{focus,vstore}) and online analytics on streamed videos (\eg~\cite{dds,awstream}).




\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \includegraphics[width=0.8\columnwidth]{figs/background.pdf}
    \tightcaption{Illustration of a video codec (video encoding and decoding) as part of the video analytics pipelines of three tasks.}
    \label{fig:background}
\end{figure}


% , and 
% \item It should {\em generalize} to (\ie can be automatically customized to serve) different DNNs for various vision tasks.

%Finally, the performance should {\em generalize} across a range of video analytics applications.


\begin{figure*}[t]
\centering
       \subfloat[\centering{Object detection\\~~~(FasterRCNN-FPN)}]
       {
         \includegraphics[width=0.35\columnwidth]{figs/measurement_detection_FPN.pdf}
         \label{fig:}
       }
       \subfloat[\centering{Object detection\\~~~(FasterRCNN-DC5)}]
       {
         \includegraphics[width=0.35\columnwidth]{figs/measurement_detection_DC5.pdf}
         \label{fig:}
       }
       \subfloat[\centering{Object detection\\~~~(FasterRCNN-C4)}]
       {
         \includegraphics[width=0.35\columnwidth]{figs/measurement_detection_C4.pdf}
         \label{fig:}
       }
       \subfloat[\centering{Segmentation\\~~~~~~~~(FCN)}]
       {
         \includegraphics[width=0.35\columnwidth]{figs/measurement_segmentation.pdf}
         \label{fig:}
       }
       \subfloat[\centering{Keypoint detection\\~~~~(KeypointRCNN)}]
       {
         \includegraphics[width=0.35\columnwidth]{figs/measurement_keypoint.pdf}
         \label{fig:}
       }
    \tightcaption{Across three analytics tasks (each evaluated on one dataset from Table~\ref{tab:dataset}), encoding selected macroblocks (``MB'') in high quality achieves better accuracy-compression tradeoffs than encoding object bounding boxes (``Object'') or whole frames (``Frame'') in high quality. The results are based on RoI encoding of H.264. \jc{kuntai, change H.264 to ``frame''}
    % as encoding quality drops, traditional video codec (H.264) can compress videos by upto 50\%, after which inference accuracy starts to drop sharply. 
    % However, encoding only selective spatial blocks (``ideal'') in high quality still retains high accuracy with smaller file size.
    }
    \label{fig:tradeoff-mpeg-idealized}
\end{figure*}



\subsection{Performance objectives}

\kt{end to end delay}

% Video analytics seek high inference accuracy and low delay (especially when extracting important information from massive video feeds), thereby posing new requirements on both the video ingestion and consumption.
% In particular, 
%In the context of video analytics, 
%The performance of a video stack for video analytics is evaluated along three metrics:
An ideal video stack for video analytics should meet three performance goals: High compression rate (small compressed video size) while achieving  high inference accuracy \footnote{To calculate the accuracy of an inference result on an encoded frame, we obtain the ``ground truth'' results by running the final DNN on the high-quality video frames (rather than using the human-annotated labels). 
Thus, any inaccuracy will be due to the video stack (\eg video compression, DNN distillation), rather than errors made by the final DNN itself.
This is consistent with recent work (\eg~\cite{awstream,vigil,videostorm,chameleon,mullapudi2019online,noscope}).}
{\em (accurate compression)}
on the decoded video; low encoding, decoding and streaming delay (\em low delay); and low camera-side compute overhead (\em low camera cost).



\begin{table}
{\footnotesize
\begin{tabular}{c|c|c|c} 
\hline
Approach & \thead{Efficient\\compression} & \thead{Low\\delay} & \thead{Low\\camera cost} \\
\hline
Autoencoder\cite{rate-distortion-autoencoder} &   \cmark         & $\times$      & $\times$ \\
\hline
\thead{AWStream\cite{awstream}\\Reducto\cite{reducto}}     & \thead{$\times$}    & \cmark      &  \cmark  \\
\hline
CloudSeg~\cite{cloudseg} & $\times$ & $\times$ & \cmark\\
\hline
Vigil\cite{vigil}       & $\times$     & \cmark      & $\times$  \\
\hline
Glimpse\cite{glimpse}     & \thead{$\times$}   & \cmark     & \cmark  \\
\hline
\thead{EAAR\cite{eaar}\\DDS\cite{dds}}         & \thead{\cmark}    & $\times$      & \thead{\cmark} \\
\hline
\name 
\textbf{(Ours)}      &  \thead{\cmark}     & \cmark       & \thead{\cmark} \\
\hline
\end{tabular}
\vspace{0.5cm}
\tightcaption{Comparison between the design choices of previous works and ours along three performance criteria. \name achieves three criteria simultaneously, while other approaches for short in some of the criteria.}
\label{tab:design}
\vspace{-0.3cm}
}
\end{table}






However, as shown in Table \ref{tab:design}, previous works are not able to hit three performance criteria simultaneously:
\kt{categorize with performance metrics}
\begin{packeditemize}
    \item {\em DNN-based video codecs} (like Autoencoder\cite{rate-distortion-autoencoder} and CloudSeg~\cite{cloudseg}) train heavy DNN-based decoder at the server side, and thus creates high decoding delay.
    \item {\em Cheap on-camera heuristics} \cite{reducto,awstream,vigil,glimpse} 
    leverages cheap on-camera algorithms to perform cheap filtering (like Glimpse~\cite{glimpse} and Reducto~\cite{reducto}), adjust video encoding parameters (like AWStream~\cite{awstream}) or crop out region of interest~\cite{vigil}.
    However, bounded by the camera compute, their approach is too cheap to be always accurate. Thus, when the video content changes (like when a kid suddenly run across the street), their camera-side heuristics will become inaccurate and result in inefficient compression.
    \item {\em Server-driven approaches} (like DDS~\cite{dds} and EAAR~\cite{eaar}) collect server-side feedback to guide the camera-side video compression.
    These approaches, however, need to communicate with the server during their encoding, and thus creates high encoding delay.
\end{packeditemize}
Thus, we desire an approach that achieves all three performance criteria. The key challenges are two-fold:
\begin{packeditemize}
    \item How to further compress the video without hurting inference accuracy (\ie how to improve compression efficiency)? We answer this question in \S\ref{subsec:macroblock}.
    \item 
\end{packeditemize}








\subsection{Macroblock-based encoding for efficient compression}
\label{subsec:macroblock}


% \begin{itemize}
%     \item - start with the observation (best encoding doesn't align with object bounding boxes or any traditional notions of regions) and a few examples, and why.

% \item - introduce MB-based encoding

% \item - introduce the oracle design of MB-based encoding and show it's potential over object/box-based encodings.
% \end{itemize}




% In this part, we demonstrate the potential gain if we encode the videos without aligning the pixels in high quality with object boundaries.
% We use 16x16 macroblock as our basic encoding unit, the same as modern codecs such as H.264~\cite{h264} and H.265~\cite{h265}.




Different from human viewers that care about the {\em overall} visual quality, there are only a {\em small fraction} of pixels who encoding quality might affect inference accuracy. 
We call these pixels {\em quality-sensitive} pixels.
% Previous work assume that these quality-sensitive pixels
% lie in a subset of {\em objects} generated from DNNs inference results or region proposals.
Prior work either encodes the whole frame in one uniform quality, \ie {\em frame-based} optimization~\cite{glimpse,reducto,awstream}, or encodes the bounding boxes in high quality (background in low quality), \ie {\em object-based} optimization~\cite{dds,eaar,vigil}.


However, our observation is that: {\em quality-sensitive pixels are not aligned with objects.}
% We observe that the quality-sensitive blocks selected by the idealized design are {\em not} strictly aligned with the detected bounding boxes or region proposals. 
Figure~\ref{fig:object-hqblock} shows two illustrative examples:
% (a) shows that the high quality sometimes is needed at the surrounding blocks to provide enough context for Conv layers to extract sufficient reliable features. 
% \kt{this is not a real example. Case 1(a) typically happens on very small objects and thus are not visually pleasing to show.}
\begin{packeditemize}
    \item Figure~\ref{fig:object-hqblock}(a) shows that for the car to be detected, some surrounding pixels outside of the object's bounding box must be encoded in high encoding quality so that the object detection DNN can discern the boundary between the object and the background\footnote{Note that uniformly enlarging the bounding boxes to cover those surrounding pixels might include many unimportant pixels; empirically, we found the quality-sensitive pixels can sometime have an IoU < 10\% with the bounding box itself, as shown in Figure~\ref{fig:obj-iou-cdf}.}.
    \item Figure~\ref{fig:object-hqblock}(b) shows that not all pixels within an object's bounding box are equally important for accurate inference: the door of the car do not need to be encoded in high quality because there is little pixel change between high and low quality and the wheels and the windows of the car are already in high quality.
\end{packeditemize}
% (a) shows that the high quality sometimes is needed at the surrounding pixels to help the neural networks separate the objects out from the background.
% (b) shows that the high quality blocks do not always need to cover the whole object.
% % The object cannot be detected in low quality, but does not need to be entirely encoded in high quality either. 
% Instead, an object can be detected at the right locations even when only parts of the object is encoded in high quality.


\mypara{Macroblock-level optimization}
The misalignments between quality-sensitive pixels and object bounding boxes suggest that frames or object bounding boxes are not the right {\em spatial granularity} for quality optimization in video analytics.
% We observe that instead of using pixel as the minimum encoding granularity, modern codecs usually use {\em macroblock}, a block of $16\times16$ pixels~\cite{h264}, to encode the videos.
% Thus, we follow this practice and use macroblock as our minimum encoding quality.
In contrast, we choose to assign quality at the {\em macroblock} (a $16\times16$ pixel block) granularity.
Fortunately, standard video codecs like H.264~\cite{h264} already support encoding different macroblocks in different quality levels (quantization parameters, QP in short) through region-of-interest (RoI) encoding.

\mypara{Potential improvement} 
Before presenting our design of macroblock-level quality optimization, we first measure its potential improvement in compression rate and inference accuracy using an idealized macroblock-level quality assignment algorithm.
% We consider an idealized algorithm which makes the assumption that the inference output of the image in high encoding quality (\ie the ground truth) is already known.
% This algorithm is designed to find those quality-sensitive macroblocks.
% In this algorithm, we make an idealized assumption: the ground truth results (the inference results delivered from encoding the whole frame into high encoding quality) is already known.
We first perform inference on low-quality encoding, and we assign each undetected/misclassified element (which means an object in object detection, a pixel in segmentation, or a keypoint in keypoint detection) a macroblock that overlaps with the element, and encode this macroblock in high quality. 
We then iterate the following process 10 times: each time, we expand the macroblock of each undetected/misclassified element in four directions by one macroblock and encode the expanded region in high quality, until the element is correctly detected.\footnote{Note that this idealized algorithm addresses the cases in Figure~\ref{fig:object-hqblock}: it may expand the high quality region beyond the object's bounding box Figure~\ref{fig:object-hqblock}(a), and it may stop expanding the high-quality region before reaching the bounding box if object is already detected.} 
Here, we assume the high quality and low quality are QP 30 and QP 46, respectively.
% After that, we remove the corresponding high quality block for those elements that still remain undetected.
% Intuitively, to make a small object to be detected, this algorithm may expand the high quality block {\em beyond} the object bounding box (like the object in Figure~\ref{fig:object-hqblock}(a)).
% On the other hand, when the object only requires part of it in high quality to be detected, this algorithm may stop expanding the high quality block even it is still inside the object bounding box (like the case in Figure~\ref{fig:object-hqblock}(b)).

We evaluate the performance (in accuracy and compression) of the idealized macroblock-level quality optimization on three datasets (``drone'' for object detection and semantic segmentation, ``surfing'' for keypoint detection; more details in Table~\ref{tab:dataset}). 
As a reference, we consider an object-based baseline that only encodes the ground-truth bounding boxes in high quality\footnote{In semantic segmentation, the ground truth bounding box are those covering the non-background pixel, and in keypoint detection, the ground truth bounding boxes are human bounding boxes.} in high quality, and a frame-based baseline that only encodes the whole frame in a uniform quality (we scan different QP values to show the spectrum of performance).
Figure~\ref{fig:tradeoff-mpeg-idealized} shows that the accuracy-compression tradeoffs of the idealized assignment 
% (with QP = 30 \kt{kpt detection also}) 
achieve 9-26\% higher accuracy than the frame-based encoding and the object-based encoding at the same compression rate. 
This potential improvement is not specific to one DNN model: similar improvements are obtained across three object detection models (Figure~\ref{fig:tradeoff-mpeg-idealized}(a-c)).
% Figure~\ref{fig:percpixel-accuracy} illustrates the reason behind 



% \mypara{Object-based encoding algorithm}
% Our object-based algorithm will only encode the ground truth elements\footnote{We use the pixels that are classified as non-background as the elements in semantic segmentation, and the ground truth human bounding boxes as the elements in keypoint detection.} in high quality.

% \mypara{Frame-based encoding algorithm}
% We encode the whole frame with uniform spatial quality in this algorithm.

% \mypara{Measurement setup}
% We perform our measurements based on three object detection models 
% % (FasterRCNN-C4~\cite{faster-rcnn}, FasterRCNN-DC5~\cite{dc5}, FasterRCNN-FPN~\cite{fpn}, implemented in Detectron2~\cite{detectron2})
% , one semantic segmentation model 
% % (FCN-ResNet101~\cite{fcn-resnet101})
% and one keypoint detection model 
% % (KeypointRCNN~\cite{maskrcnn}, implemented  in Detectron2~\cite{detectron2})
% .
% We use surfing videos for keypoint detection, and drone videos for object detection and semantic segmentation. Please refer to \S\ref{subsec:eval:setup} for details on our datasets and models.


% \mypara{Performance analysis}
% Figure~\ref{fig:tradeoff-mpeg-idealized} shows that the accuracy-compression tradeoffs of the idealized assignment 
% % (with QP = 30 \kt{kpt detection also}) 
% achieve 9-26\% higher accuracy than the frame-based encoding and the object-based encoding at the same compression rate. 
% % Figure~\ref{fig:percpixel-accuracy} illustrates the reason behind 
% A closer investigation reveals the reason behind the idealized assignments' superior tradeoffs: encoding only 6.3\% 16x16 macroblocks still allows it to hit 90\% accuracy.

% As a reference point, we also show two other heuristics for selecting the high-quality blocks: ``Object-based'' heuristics selects all blocks that overlap with some of the final DNN's detected bounding boxes (note that this is not practical either), and ``DDS'' is a recently proposed solution~\cite{dds} that selects the region proposals for which the final DNN has low confidence.
% The two heuristics embody a popular assumption underlying most prior work that uses spatially different quality levels: only regions directly associated with the inference results (either the bounding box or region proposals that have not been confirmed) need to be encoded in high quality.
% However, Figure~\ref{fig:tradeoff-mpeg-idealized} shows a substantial performance gap between previous works and the idealized assignments. 

%the source of improvement of the idealized design point is.
%In other words, what have the strawmen missed in their assumptions.

% To begin with, 

% inference to be accurate.
% Even when completely encoded in high quality, those small objects cannot be detected because their sounding pixels are in low quality for Conv layers to extract sufficient reliable features. 
%On the other hand, we see in (b) that some objects cannot be detected even if they are entirely encoded in high quality. 
% Instead, some surrounding blocks must be encoded in high quality as well.
%\jc{maybe there are blocks that are not associated with any detected object, but need to be in high quality just to winnow out non-objects?}

A closer investigation reveals the reason behind the idealized assignments' superior tradeoffs: encoding only 6.3\% 16x16 macroblocks still allows it to hit 90\% accuracy. 
Not surprisingly, this small fraction of quality-sensitive pixels are not well aligned with the ground truth bounding boxes.
% To further reveal the nonalignment between the high quality macroblocks choosed by our macroblock-based encoding algorithm and the object based algorithm, 
In Figure~\ref{fig:obj-iou-cdf}, we calculate the intersection-over-union between the high quality macroblocks selected by these two approaches, and we found that more than half of the frames, the IoU is less than 0.2, indicating non-trivial misalignments. 
% plot the CDF across three different applications.
% Figure~\ref{fig:obj-iou-cdf} shows that on more than half of the frames, the IoU is less than 0.2, indicating non-trivial misalignments. 

%that across all frames, there is significant misalignment between the inference results of object detections (bounding boxes) and high-quality blocks selected by the idealized design point.
%\jc{more read of the graph}





\begin{figure}[t]
       \subfloat[\centering{Obj. detection\\(FasterRCNN-FPN)}]
       {
         \includegraphics[width=0.3\columnwidth]{figs/IoU_FPN.pdf}
         \label{fig:}
       }
       \subfloat[\centering{Obj. detection\\(FasterRCNN-DC5)}]
       {
         \includegraphics[width=0.3\columnwidth]{figs/IoU_DC5.pdf}
         \label{fig:}
       }
       \subfloat[\centering{Obj. detection\\(FasterRCNN-C4)}]
       {
         \includegraphics[width=0.3\columnwidth]{figs/IoU_C4.pdf}
         \label{fig:}
       }
       
    \vspace{-0.1cm}
    \tightcaption{On three different object detection DNNs, the overlap between the high quality blocks chosen by the idealized macroblock-based algorithm and the object bounding boxes is smaller than 20\% on over half of the frames.
    \jc{kuntai, increase the font to same size as fig 3.}}
    \label{fig:obj-iou-cdf}
\end{figure}











\subsection{\hspace{-0.3cm}Local DNN-aware encoding optimization}
\label{subsec:local}

The previous measurements show substantial improvements if the encoding optimization is aware of the quality-sensitive pixels (macroblocks) of the final DNN.
Indeed, recent techniques (though not macroblock-level optimization) have increasingly made the encoding optimization DNN-aware (\eg~\cite{dds,eaar,reducto,awstream,elf}). 
However, so far they have relied on DNNs that run on remote servers to which the edge cameras are connected with a reliable network connection\footnote{For instance, the bandwidth requirement for DDS to optimize this example video~\cite{trafficcam-example} (with low quality of QP 40 and high quality of QP30) is at least .} to stream videos to the server (in realtime or periodically).
% the encoding decision needs to find those quality-sensitive pixels not only at a {\em macroblock} level, but also be aware of the final DNN. 
% Previous works achieve this awareness by running inference on the final DNN at the server side~\cite{dds,eaar,reducto,awstream}.
% As a result, these approaches heavily rely on a high quality camera-server connection (the bandwidth requirement is roughly about 1 Mbps\footnote{We calculate this based on the encoding of DDS~\cite{dds}. We encode this video~\cite{trafficcam-example} in low quality (QP 40), calculate the bandwidth for it, and then double the bandwidth to estimate the bandwidth usage of high quality and low quality video streams.}) to stream the video to the server.

\myparaq{Why not server-driven encoding optimization}
\kt{reason: high delay}
Unfortunately, these online DDN-driven workflows will not work well on edge cameras (though not all cameras) that only have sporadic network connections (any network disconnection will block the encoding process or queue up many raw frames creating much memory stress on edge cameras) or privacy concerns which preclude videos be shared in realtime with remote servers.
Examples of these issues include:
\begin{packeditemize}
    \item {\em Wildlife camera:} Widely used in learning animal activities in the wild~\cite{newyorktime-wildlifecam}, wildlife cameras are often placed in places with no LTE signal (thus cannot communicate with remote analytics models in realtime) for days to record enough data for future analytics~\cite{deercam}.
    While frame-dropping schemes are effective, the main contributor to video size is the video frames where the objects of interest are present which are not easy to compress without sacrificing accuracy.
    % Wildlife cameras play a more and more important role in learning and protecting the animals~\cite{newyorktime-wildlifecam}.
    % However, these cameras typically will be placed in the wild with no LTE signal for several days to record enough data for future analytics (like deer cameras~\cite{deercam}).
    % Thus, due to poor LTE connectivity, these cameras cannot stream their video out to the server.
    % One may question that a simple frame dropping technique for wild camera is already enough. However, the main file size of wildlife camera videos lies on the frames with animals as the background is relatively stationary and very easy to compress for modern codec.
    \item {\em Low-end dashcam:} 
    A cheap dashcam is only \$50~\cite{cheap-dashcam}, but adding LTE connectivity to it needs a \$150 LTE module~\cite{4GModule}, or alternatively, a \$200+ LTE-capable camera~\cite{??}, not to mention the cellular data plan needed to provide a reliable network connection.
    In contrast, a more economic option is to use a cheap dashcam and encode videos locally.
    \item {\em Home camera:}
    With a growing market of home cameras and rising concerns about their privacy issues~\cite{forbes-homecam,HOA-homecam}, the best way is to not stream the video out from the camera until the user issues a query of certain analytics task.
    % Nowadays, people are more and more concerned about the privacy issue of home cameras~\cite{forbes-homecam,HOA-homecam}.
    % The best way for the camera to maintain private is to not streaming the video out from the camera unless the user grants permission.
\end{packeditemize}

% However, sometimes the cameras prefer not to stream the video out\footnote{Analysts can still fetch their videos out when they need to analyze them.} and thus the encoding must be done purely at the camera side.
% This is because the cameras may {\em lack of reliable network connection} to support video streaming, or do not have the permission to stream the video out due to {\em privacy issue}.
% We list out three categories of cameras that fall into these two cases:


% like the cameras with no LTE connection (like wild-life camera~\cite{deercam} and cheap dashcam~\cite{cheap-dashcam}) or privacy concerns (like home camera~\cite{HOA-homecam,forbes-homecam}).
% \mypara{Design for future analysis} 
% \jc{i would replace ``retrospective'' with a different word. ``retrospective'' sounds like you don't even know what model will be used to analyzed the video.}
% When deploying these algorithms to edge devices, these works all assume that the edge devices have the access to the server and performs edge-cloud optimization jointly. However, we will show that there are a lot of usecases where the cameras are disconnected from the server and have to archive the video and wait for retrospective analysis. To tackle these usecases, we desire an algorithm that can perform \textbf{cheap and local} encoding.
% \jc{``cheap and local'' can be misleading. vigil, glimpse, focus, all have ``cheap and local'' processing. how about start with why dnns are increasingly used to decide encoding quality in real time, and then say there is currently no ``cheap and local'' way to do that?}













% \mypara{Design space}
% To put our design into perspective, we first sketch the space of various potential design points.
% \begin{packeditemize}
% \item {\em Choice of codec:}
% One option is to re-use a traditional codec (\eg H.264/265~\cite{1218189}, VP9~\cite{6737765}) and tune its parameters (\eg quantization parameters). 
% There are also alternative NN-based codecs (\eg super resolution~\cite{cloudseg}, autoencoder~\cite{rate-distortion-autoencoder}), but they have yet to see the wide industry adoption enjoyed by the traditional codecs, and they usually have compute-intensive encoding (\eg autoencoder) and decoding (\eg super-resolution).
% In this work, we take a pragmatic stance to build our video stack on traditional codecs, like most work in this space.


% \item {\em Quality adaptation granularity:}
% To cope with the dynamics of video content, prior work tries to adapt quality by saving only a subset of frames (\eg~\cite{glimpse,reducto,awstream}), assigning different quality to different frames (\eg~~\cite{awstream,vstore,chameleon}), and/or assigning a higher quality to only object bounding boxes or region proposals (\eg~~\cite{vigil,dds,eaar}).
% In this work, we assign quality for each fine-grained blocks (16x16 pixels), which as shown in the next section could lead to much better compression efficiency and inference accuracy than the aforementioned granularities.


% \item {\em Integration with final DNN:}
% Using the final DNN's output (or intermediate features) does help to identify regions of interest (\eg~\cite{eaar,dds}), but it potentially adds a prohibitive overhead to encoding (especially for archived videos most of which will not be analyzed).
% On other other hand, using cheap heuristics that are agnostic to the final DNN has been shown to produce suboptimal compression efficiency and/or low inference accuracy~\cite{dds}.
% In this work, we design a shallow NN to infer a (near-)optimal quality assignment, which as we will see is a much simpler task than the actual final inference.
% \end{packeditemize}




% Due to poor connectivity, power constraint or privacy concerns, it may be not feasible for the camera to stream the videos out.
% Here are three example scenarios that the cameras are not able to access the internet.


















\begin{table}
{\footnotesize
\begin{tabular}{c|c|c} 
\hline
Name & \multicolumn{2}{c}{Frames per second}\\
\hline
& Raspberry Pi 4 & CPU Server \\
\hline
Encoding & 3.40 & 22.07\\ 
\hline
\thead{Cheap object detector\\ (MobileNet-SSD)~\cite{SSD}} & 0.21 & 8.45\\ 
\hline
\thead{Compute-intensive\\object detector\\ (FasterRCNN-C4)~\cite{faster-rcnn}} & OOM & 0.05\\
\hline
\end{tabular}
\vspace{0.5cm}
\tightcaption{Performance comparison between the running speed (frames per second) of video encoding, cheap object detector and compute-intensive object detector on a Raspberry Pi 4 and on a server CPU. Raspberry Pi 4 has Broadcom BCM2711, Quad core Cortex-A72 (ARM v8) 64-bit SoC @ 1.5GHz with 4GB memory; the server CPU is Intel(R) Xeon(R) Platinum 8163 CPU @ 2.50GHz.)}
\label{tab:tinyyolo}
\vspace{-0.3cm}
}
\end{table}






\mypara{Strawmen for on-premise encoding optimization}
There are a few strawmen that try to leverage limited compute power on the camera, but none of them can compress videos aggressively without sacrificing accuracy (Table~\ref{tab:tinyyolo}:
\begin{packeditemize}
    \item One strawman is to run the above DNN-driven workflows on the camera, but most final DNNs are too memory-/compute-intensive for an edge camera to run locally.
    \item One can also run a cheap object detector on the camera~\cite{vigil} to identify regions that likely contain objects. 
    However, cheap object detector, like TinyYolo~\cite{yolo} and MobileNet-SSD can be inaccurate (as we show in \S\ref{sec:eval}) and is already too slow to run on a camera at the line speed.
    \item Frame dropping~\cite{glimpse, reducto} is also an option and is widely used in some prior work, but similar to frame-level quality optimization, it falls short when objects of interest are almost always present in a dynamic scene (which makes it hard to detect arrivals of new objects).
    % However, these approaches cannot efficiently drop frames when the video contains moving objects.
    \item Finally, one can use autoencoders (deep-learning-based video codecs trained to optimize human perception or accuracy of a DNN), but these autoencoders are orders of magnitude more expensive than the standard video codes (used in \name): the fastest encoder runs at similar speed on GPU as H264 on CPU~\cite{rippel2019learned} (we will also evaluate autoencoder in \S\ref{sec:eval}).
    % (\eg~\cite{rate-distortion-autoencoder})  is too heavy for the camera to afford and the accuracy remains to be low 
\end{packeditemize}

% In these scenarios, we desire a {\em cheap and DNN-aware encoding} that encodes {\em purely by the camera itself} (we call this property {\em local}) and delivers higher compression efficiency through macroblock-level encoding.


% The recent effort on new video codec for DNN inference purposes like super resolution~\cite{cloudseg} and auto-encoder~\cite{rate-distortion-autoencoder} may seem to be a good choice at the first glance. 
% However, the accuracy of super-resolution-based approach is low if there is no camera-server connection available (see Figure~\ref{fig:eval-overall}) and the encoding delay of auto-encoder is more than 4 seconds per single frame (see Figure~\ref{fig:eval-delay-overall}).
% One may also use a cheap object detector to crop out some regions of interest and save them at the camera side~\cite{vigil}.
% The cheap object detector, however, falls short in accuracy when handling challenging contents (as we will show in \S\ref{sec:eval}) and is still too heavy for a cheap camera to afford (cheap camera can only run TinyYoLo~\cite{yolo} in \fillme frames per second, as shown in Table~\ref{tab:tinyyolo}).
% Thus, none of them can hit high accuracy while still maintaining local encoding.




\mypara{Summary}
Table~\ref{tab:design} summarizes the prior solutions in three dimensions. 
In short, previous work optimizes encoding quality at either frame-based or object-based, and thus fails to exploit the potential of macroblock-based optimization.
Moreover, none of them achieve can optimize encoding in a DNN-aware manner using only local compute resource.

% To further visualize the limitations of prior work, we illustrate the design choices of previous works along each design dimensions in Table~\ref{tab:design}. From ths table, we can see that none of the prior work hits macroblock-level granularity, cheap local encoding and real-time DNN awareness simultaneously.




% One alternative approach is to leverage a cheap object detection algorithm to detect potential object of interests and encode the object of interests only.
% However, the typical cheap object detector (such as TinyYoLO) is still much expensive compared with our approach for the camera to afford (the runtime of TinyYoLo is 2x compared to our approach as listed in Table~\ref{tab:tinyyolo}), and the overall file size-accuracy trade-off is poor (we will show this in \S\fillme).




==> motivate-v6.tex <==

\section{Motivation}
\label{sec:motivation}


We begin by motivating the three performance metrics for video encoding that drive our design (low accuracy, low encoding and streaming delay, and low compute overhead on the camera side).
% : high inference accuracy ({\em high accuracy}), low encoding delay and streaming delay ({\em low delay}), and low camera-side compute overhead ({\em low camera cost}). 
We then elaborate on why prior solutions inherently improve two performance criteria at the expense of the remaining one.
% These two goals lead to a new design point of a {\em cheap, local and DNN-aware} encoding algorithm, which we will explore in the next few sections.



% Nowadays, more and more videos captured on edge devices are generated for analytic purposes instead of watched by human viewers. 
% Different from human viewers that care about the {\em overall} visual quality, a {\em small fraction} of pixels are much more important than the others for DNNs to generate accurate analytic results.
% The conventional wisdom assumes that these pixels lie in a subset of objects.
% However, we revisit this assumption in \S\ref{subsec:macroblock} and show that it will actually lead to sub-optimal file size-accuracy trade-off.



% From the deployment side, previous works~\cite{dds,awstream,reducto,eaar} optimize the overall bandwidth-accuracy trade-off based on server-side compute.
% In fact, we will show in \S\ref{subsec:local} that a lot of cameras prefer not to stream their video out. 
% To facilitate the video analytics on these cameras, the key is to design a cheap and accurate encoding algorithm {\em without accessing the server online}.




\subsection{Optimizing video encoding for DNNs}


Spurred by advances in computer vision, more video applications analyze massive video streams using deep neural nets (DNNs). 

\mypara{Distributed video analytics} 
As accurate analytics require compute-intensive DNNs that cheap video sensors cannot afford, 
the video need to be {\em compressed} by {\em video encoder}, and then sent to the remote server for highly accurate DNN-based analytics (Figure~\ref{fig:background}).
We refer to the server-side DNN as the {\em final DNN}.
% As depicted in Figure~\ref{fig:background}, video analytics applications rely on efficient video-compression algorithms to encode the incoming video, and these videos will be analyzed by computer-vision algorithms, in forms of deep neural nets (DNNs). 
To make our discussion more concrete, we focus on three typical video analytics tasks: object detection (one labeled bounding box for each object), semantic segmentation (one label for each pixel), and keypoint detection (17 keypoints for each human). 
% That said, our approach can also benefit retrospective analytics.

A common component of these distributed video-analytics applications is the video encoding algorithm, which is critical for both live and retrospective analytics:
\begin{packeditemize}
    \item {\em Live analytics:} The video stream is continuously encoded and sent to a remote server which runs the final DNN to analyze the video in an online fashion~\cite{dds,eaar,vigil,glimpse,reducto,elf,awstream,noscope,videostorm}.
    \item {\em Retrospective analytics:} The encoded video will be first saved on camera's local disk, and an operator can choose to fetch part of the archived video for DNN-based analytics~\cite{chameleon,blazeit,focus}.
\end{packeditemize}


% \kt{Add new para here}

% \mypara{Video encoding for video analytics}
% To better serve video analytics applications, we need an efficient video compression algorithm that reduces the file size without hurting the accuracy of the derived analytic results.
% This is because reducing file size will reduce the network bandwidth requirement for video-streaming-based analytics, and will reduce the storage burden when the video is offline archived for future inference.
% However, traditional video codecs (like H.264~\cite{h264} and H.265~\cite{h265}) are optimized for human perception rather than inference accuracy.
% This gives us research opportunity.



% \mypara{DNN-aware encoding optimization}
% In many video-analytics applications, each DNN takes a non-trivial amount of time and effort to train\footnote{About 40\% companies take one month or longer to put their models into production~\cite{ml-deployment-time}, and the deployment time of their models is increasing year-on-year~\cite{ML_trends}. Moreover, 78\% of AI/ML projects stall at some stage before deployment~\cite{stall}.}, and many applications apply one DNN to analyze each video stream\footnote{Wildlife Insights mainly consumes wild life videos for species  detection~\cite{wildlife-application} and intuVision Traffic focuses on detecting cars and other vehicles for traffic videos}.
% Therefore, we consider the setting where the DNN is known before we encode the incoming video streams and thus the encoding can be optimized for a given DNN. 
% Same assumption is used in recent work (\eg~\cite{noscope,eaar,dds,awstream,elf}).
% That said, the encoded videos should still work well for other DNNs of similar video analytics purposes (\eg among different object detectors). 


% As depicted in Figure~\ref{fig:background}, many video analytics applications rely on video compression algorithm\footnote{In this work, a video stack means a software wrapper on top of a video codec (H.264/265, VP8/9, etc) that tunes its performance for some higher-level application (video analytics tasks). In \S\ref{sec:eval}, we will evaluate our proposal's performance over various codecs and in various vision tasks.} for two basic operations: 
% {\em encoding} a stream of frames into a compressed video file as the frames are captured by a video sensor~\cite{vstore} for efficient storage and transmission, and {\em decoding} the compressed video file to individual frames/segments which are then fed into a {\em final DNN} for vision inference.
% These operations are needed for both offline analytics on archived videos (\eg~\cite{focus,vstore}) and online analytics on streamed videos (\eg~\cite{dds,awstream}).




\begin{figure}
    \centering
%    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \includegraphics[width=0.8\columnwidth]{figs/background.pdf}
    \tightcaption{Illustration of video encoding as part of the video analytics pipelines of three tasks.\kt{replot this figure}}
    \label{fig:background}
\end{figure}


% , and 
% \item It should {\em generalize} to (\ie can be automatically customized to serve) different DNNs for various vision tasks.

%Finally, the performance should {\em generalize} across a range of video analytics applications.


% \begin{figure*}[t]
% \centering
%       \subfloat[\centering{Object detection\\~~~(FasterRCNN-FPN)}]
%       {
%          \includegraphics[width=0.35\columnwidth]{figs/measurement_detection_FPN.pdf}
%          \label{fig:}
%       }
%       \subfloat[\centering{Object detection\\~~~(FasterRCNN-DC5)}]
%       {
%          \includegraphics[width=0.35\columnwidth]{figs/measurement_detection_DC5.pdf}
%          \label{fig:}
%       }
%       \subfloat[\centering{Object detection\\~~~(FasterRCNN-C4)}]
%       {
%          \includegraphics[width=0.35\columnwidth]{figs/measurement_detection_C4.pdf}
%          \label{fig:}
%       }
%       \subfloat[\centering{Segmentation\\~~~~~~~~(FCN)}]
%       {
%          \includegraphics[width=0.35\columnwidth]{figs/measurement_segmentation.pdf}
%          \label{fig:}
%       }
%       \subfloat[\centering{Keypoint detection\\~~~~(KeypointRCNN)}]
%       {
%          \includegraphics[width=0.35\columnwidth]{figs/measurement_keypoint.pdf}
%          \label{fig:}
%       }
%     \tightcaption{Across three analytics tasks (each evaluated on one dataset from Table~\ref{tab:dataset}), encoding selected macroblocks (``MB'') in high quality achieves better accuracy-compression tradeoffs than encoding object bounding boxes (``Object'') or whole frames (``Frame'') in high quality. The results are based on RoI encoding of H.264. \jc{kuntai, change H.264 to ``frame''}
%     % as encoding quality drops, traditional video codec (H.264) can compress videos by upto 50\%, after which inference accuracy starts to drop sharply. 
%     % However, encoding only selective spatial blocks (``ideal'') in high quality still retains high accuracy with smaller file size.
%     }
%     \label{fig:tradeoff-mpeg-idealized}
% \end{figure*}



% Video analytics seek high inference accuracy and low delay (especially when extracting important information from massive video feeds), thereby posing new requirements on both the video ingestion and consumption.
% In particular, 
%In the context of video analytics, 
%The performance of a video stack for video analytics is evaluated along three metrics:
\mypara{Performance objectives}
An ideal video encoding algorithm for distributed video analytics should meet three goals: 
\begin{packeditemize}
\item {\em High accuracy:}
The encoded video must preserve enough information for the final DNN to extract nearly identical analytic results as running the final DNN on the uncompressed video.\footnote{To calculate the accuracy of an inference result on an encoded frame, we obtain the ``ground truth'' results by running the final DNN on the high-quality video frames (rather than using the human-annotated labels). 
Thus, any inaccuracy will be due to the video stack (\eg video compression, DNN distillation), rather than errors made by the final DNN itself.
This is consistent with recent work (\eg~\cite{awstream,vigil,videostorm,chameleon,mullapudi2019online,noscope}).}
% \item The delay spent on encoding the video (encoding delay) and streaming the video to the server (streaming delay) should be low ({\em low delay}).

\item {\em Low delay:} The delay spent on encoding the video (encoding delay) and streaming the video to the server (streaming delay) should be low.

\item {\em Low camera cost:} The encoding algorithm should be cheap enough to run at a line speed of 30 frames per second on a low-end camera such as \fillme.
% (see Table~\ref{tab:tinyyolo} for the runtime of several baseline algorithms on Raspberry Pi 4 and the CPU server).
\end{packeditemize}



% \begin{table}
% {\footnotesize
% \centering
% \begin{tabular}{c|c|c|c} 
% \hline
% Approach & \thead{High\\Accuracy} & \thead{Low\\delay} & \thead{Low\\camera cost} \\
% \hline
% \thead{Cheap camera-side\\heuristics\\\cite{vigil,glimpse,reducto,awstream,cinet,elf}}     & \thead{$\times$}    & \cmark      &  \cmark  \\
% \hline
% \thead{Server-driven\\approaches\\\cite{dds,eaar,cloudseg}}         & \thead{\cmark}    & $\times$      & \thead{\cmark} \\
% \hline
% \thead{Autoencoder\\\cite{rate-distortion-autoencoder,NLAM}} &   \cmark         & \cmark      & $\times$ \\
% \hline
% \name 
% \textbf{(Ours)}      &  \thead{\cmark}     & \cmark       & \thead{\cmark} \\
% \hline
% \end{tabular}
% \vspace{0.5cm}
% \tightcaption{Comparison between the design choices of previous works and ours along three performance objectives. \name achieves three objectives simultaneously, while other approaches fall short in one of these objectives. \kt{Replot this figure in a triangle manner}}
% \label{tab:design}
% \vspace{-0.3cm}
% }
% \end{table}




\subsection{Limitation of previous work}
\label{subsec:challenge}


However, as shown in Figure \ref{fig:design}, previous works inherently trade one of the three criteria mentioned for the other two.

% \begin{packeditemize}
    % \item {\em Low accuracy.} 
\mypara{Low accuracy}
Some previous works deploy cheap on-camera heuristics ~\cite{vigil,glimpse,reducto,awstream,cinet,elf} to compress the video.
However, bounded by camera's limited compute power, these approaches will become inaccurate when video content changes. 

To put this into perspective, let's take Reducto~\cite{reducto} (an approach that filters out frames that do not significantly differ from their preceding frames) as an example and assume that one car equipped with a dashcam is driving on a highway.
Initially, there is no other car on the highway.
In this case, all frames differ a lot from their preceding frames (since the car is driving at a high speed) but no object of interest occurs.
Thus, Reducto picks an aggressive filter that filters out nearly all frames.
However, when a new car suddenly appears, Reducto will still rely on the aggressive filter and drop all the frames containing the new car. As a result, Reducto completely fails to detect this car and gets zero accuracy.
    
    % \item {\em High delay.}
\mypara{High delay}
Some previous work explores server-side compute to optimize the encoding~\cite{dds,eaar,cloudseg}. Thus, these approaches requires extra time to connect to server for encoding, and thus creates extra delay.

    % \item {\em High camera cost.} 

\mypara{High camera-side compute cost}
Some previous works compress the video at the camera side by using DNN-based autoencoder~\cite{rate-distortion-autoencoder,NLAM}. \kt{the autoencoder that VCM benchmarks is cited here.}
However, these encoders require performing {\em expensive 3D} convolutions on videos for more than {\em 30 times} (in comparison, a middle-end object detector backbone ResNet34~\cite{resnet} only performs {\em 2D} convolution for {\em 34 times}), which is way too compute-intensive for a cheap camera to afford.
% \end{packeditemize}
% \begin{packeditemize}
%     \item {\em DNN-based video codecs} (like Autoencoder\cite{rate-distortion-autoencoder} and CloudSeg~\cite{cloudseg}) train heavy DNN-based decoder at the server side, and thus creates high decoding delay.
%     \item {\em Cheap on-camera heuristics} \cite{reducto,awstream,vigil,glimpse} 
%     leverages cheap on-camera algorithms to perform cheap filtering (like Glimpse~\cite{glimpse} and Reducto~\cite{reducto}), adjust video encoding parameters (like AWStream~\cite{awstream}) or crop out region of interest~\cite{vigil}.
%     However, bounded by the camera compute, their approach is too cheap to be always accurate. Thus, when the video content changes (like when a kid suddenly run across the street), their camera-side heuristics will become inaccurate and result in inefficient compression.
%     \item {\em Server-driven approaches} (like DDS~\cite{dds} and EAAR~\cite{eaar}) collect server-side feedback to guide the camera-side video compression.
%     These approaches, however, need to communicate with the server during their encoding, and thus creates high encoding delay.
% \end{packeditemize}
Thus, we desire a new encoding that achieves all three performance objectives. 

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/previous-work}
    \tightcaption{``Impossible trinity'' among three performance objectives. Previous work achieves two of the objectives with the cost of the remaining one.}
    \label{fig:design}
\end{figure}

% Specifically, the encoding algorithm should be {\em local} (\ie the encoding is performed on camera only to minimize the encoding delay); {\em cheap} (to reduce camera-side cost) yet still {\em aware of server-side DNN} (to maintain high accuracy while still able to compress the video to reduce the streaming delay)? 

% The challenges of developing such an algorithm are three-fold:
% \begin{packeditemize}
%     \item How to identify a encoding problem that can potentially be solved by a cheap algorithm?
%     \item How to reduce the overall runtime of the cheap algorithm on camera side?
%     \item How to quickly obtain a change of server-side DNN (ideally within several minutes)?
% \end{packeditemize}







 








% \subsection{On-camera DNN-aware encoding optimization}
% \label{subsec:local}

% Recent techniques have increasingly made the encoding optimization DNN-aware (\eg~\cite{dds,eaar,reducto,awstream,elf}) in order to let the server-side DNN achieve high accuracy.
% However, so far they have relied on DNNs that run on remote servers to which the edge cameras are connected with a reliable network connection\footnote{For instance, the bandwidth requirement for DDS to optimize this example video~\cite{trafficcam-example} (with low quality of QP 40 and high quality of QP30) is at least .} to stream videos to the server (in realtime or periodically).
% % the encoding decision needs to find those quality-sensitive pixels not only at a {\em macroblock} level, but also be aware of the final DNN. 
% % Previous works achieve this awareness by running inference on the final DNN at the server side~\cite{dds,eaar,reducto,awstream}.
% % As a result, these approaches heavily rely on a high quality camera-server connection (the bandwidth requirement is roughly about 1 Mbps\footnote{We calculate this based on the encoding of DDS~\cite{dds}. We encode this video~\cite{trafficcam-example} in low quality (QP 40), calculate the bandwidth for it, and then double the bandwidth to estimate the bandwidth usage of high quality and low quality video streams.}) to stream the video to the server.

% \myparaq{Why not server-driven encoding optimization}
% \kt{reason: high delay}
% Previous works~\cite{dds,eaar} leverages server-driven approach to optimize the encoding for a better trade-off between file size and accuracy.
% However, it requires the camera to stream the video to the server and wait for its response to obtain server-side information and finish encoding.
% Thus, the encoding delay of this approach will be high.
% % Unfortunately, these online DDN-driven workflows will not work well on edge cameras (though not all cameras) that only have sporadic network connections (any network disconnection will block the encoding process or queue up many raw frames creating much memory stress on edge cameras) or privacy concerns which preclude videos be shared in realtime with remote servers.
% % Examples of these issues include:
% % \begin{packeditemize}
% %     \item {\em Wildlife camera:} Widely used in learning animal activities in the wild~\cite{newyorktime-wildlifecam}, wildlife cameras are often placed in places with no LTE signal (thus cannot communicate with remote analytics models in realtime) for days to record enough data for future analytics~\cite{deercam}.
% %     While frame-dropping schemes are effective, the main contributor to video size is the video frames where the objects of interest are present which are not easy to compress without sacrificing accuracy.
% %     % Wildlife cameras play a more and more important role in learning and protecting the animals~\cite{newyorktime-wildlifecam}.
% %     % However, these cameras typically will be placed in the wild with no LTE signal for several days to record enough data for future analytics (like deer cameras~\cite{deercam}).
% %     % Thus, due to poor LTE connectivity, these cameras cannot stream their video out to the server.
% %     % One may question that a simple frame dropping technique for wild camera is already enough. However, the main file size of wildlife camera videos lies on the frames with animals as the background is relatively stationary and very easy to compress for modern codec.
% %     \item {\em Low-end dashcam:} 
% %     A cheap dashcam is only \$50~\cite{cheap-dashcam}, but adding LTE connectivity to it needs a \$150 LTE module~\cite{4GModule}, or alternatively, a \$200+ LTE-capable camera~\cite{??}, not to mention the cellular data plan needed to provide a reliable network connection.
% %     In contrast, a more economic option is to use a cheap dashcam and encode videos locally.
% %     \item {\em Home camera:}
% %     With a growing market of home cameras and rising concerns about their privacy issues~\cite{forbes-homecam,HOA-homecam}, the best way is to not stream the video out from the camera until the user issues a query of certain analytics task.
% %     % Nowadays, people are more and more concerned about the privacy issue of home cameras~\cite{forbes-homecam,HOA-homecam}.
% %     % The best way for the camera to maintain private is to not streaming the video out from the camera unless the user grants permission.
% % \end{packeditemize}

% % However, sometimes the cameras prefer not to stream the video out\footnote{Analysts can still fetch their videos out when they need to analyze them.} and thus the encoding must be done purely at the camera side.
% % This is because the cameras may {\em lack of reliable network connection} to support video streaming, or do not have the permission to stream the video out due to {\em privacy issue}.
% % We list out three categories of cameras that fall into these two cases:


% % like the cameras with no LTE connection (like wild-life camera~\cite{deercam} and cheap dashcam~\cite{cheap-dashcam}) or privacy concerns (like home camera~\cite{HOA-homecam,forbes-homecam}).
% % \mypara{Design for future analysis} s
% % \jc{i would replace ``retrospective'' with a different word. ``retrospective'' sounds like you don't even know what model will be used to analyzed the video.}
% % When deploying these algorithms to edge devices, these works all assume that the edge devices have the access to the server and performs edge-cloud optimization jointly. However, we will show that there are a lot of usecases where the cameras are disconnected from the server and have to archive the video and wait for retrospective analysis. To tackle these usecases, we desire an algorithm that can perform \textbf{cheap and local} encoding.
% % \jc{``cheap and local'' can be misleading. vigil, glimpse, focus, all have ``cheap and local'' processing. how about start with why dnns are increasingly used to decide encoding quality in real time, and then say there is currently no ``cheap and local'' way to do that?}













% \mypara{Design space}
% To put our design into perspective, we first sketch the space of various potential design points.
% \begin{packeditemize}
% \item {\em Choice of codec:}
% One option is to re-use a traditional codec (\eg H.264/265~\cite{1218189}, VP9~\cite{6737765}) and tune its parameters (\eg quantization parameters). 
% There are also alternative NN-based codecs (\eg super resolution~\cite{cloudseg}, autoencoder~\cite{rate-distortion-autoencoder}), but they have yet to see the wide industry adoption enjoyed by the traditional codecs, and they usually have compute-intensive encoding (\eg autoencoder) and decoding (\eg super-resolution).
% In this work, we take a pragmatic stance to build our video stack on traditional codecs, like most work in this space.


% \item {\em Quality adaptation granularity:}
% To cope with the dynamics of video content, prior work tries to adapt quality by saving only a subset of frames (\eg~\cite{glimpse,reducto,awstream}), assigning different quality to different frames (\eg~~\cite{awstream,vstore,chameleon}), and/or assigning a higher quality to only object bounding boxes or region proposals (\eg~~\cite{vigil,dds,eaar}).
% In this work, we assign quality for each fine-grained blocks (16x16 pixels), which as shown in the next section could lead to much better compression efficiency and inference accuracy than the aforementioned granularities.


% \item {\em Integration with final DNN:}
% Using the final DNN's output (or intermediate features) does help to identify regions of interest (\eg~\cite{eaar,dds}), but it potentially adds a prohibitive overhead to encoding (especially for archived videos most of which will not be analyzed).
% On other other hand, using cheap heuristics that are agnostic to the final DNN has been shown to produce suboptimal compression efficiency and/or low inference accuracy~\cite{dds}.
% In this work, we design a shallow NN to infer a (near-)optimal quality assignment, which as we will see is a much simpler task than the actual final inference.
% \end{packeditemize}




% Due to poor connectivity, power constraint or privacy concerns, it may be not feasible for the camera to stream the videos out.
% Here are three example scenarios that the cameras are not able to access the internet.


















\begin{table}
{\footnotesize
\centering
\begin{tabular}{c|c|c|c|c} 
\hline
Name & \multicolumn{4}{c}{Frames per second}\\
\hline
& \thead{Raspberry\\Pi 4} & \thead{Jetson Nano\\(CPU)} & \thead{Jetson Nano\\(GPU)} & \thead{CPU\\Server} \\
\hline
H.264 Encoding & 3.40 & 3.57 & 3.57 & 22.07\\ 
\hline
H.265 Encoding & 0.58 & 0.39 & 0.39 & \\ 
\hline
VP9 Encoding & 0.41 & 0.54 & 0.54 & \\ 
\hline
\thead{Cheap object detector\\ (MobileNet-SSD)\\\cite{SSD}} & 0.081 & 0.11 & 16.53 & 8.45\\ 
\hline
\thead{Compute-intensive\\object detector\\ (FasterRCNN)\\\cite{faster-rcnn}} & 0.027 & 0.032 & 0.20 & 0.05\\
\hline
\thead{AccMPEG} & 0.15 & 0.15 & 18.52
& ?\\
\hline
\end{tabular}
\vspace{0.5cm}
\tightcaption{Performance comparison between the running speed (frames per second) of video encoding, cheap object detector and compute-intensive object detector on a Raspberry Pi 4 and on a server CPU\footnote{Raspberry Pi 4 has Broadcom BCM2711, Quad core Cortex-A72 (ARM v8) 64-bit SoC @ 1.5GHz with 4GB memory; the server CPU is Intel() Xeon(R) Platinum 8163 CPU @ 2.50GHz.)}.}
\label{tab:tinyyolo}
}
\end{table}






% \mypara{Strawmen for on-premise encoding optimization}
% There are a few strawmen that try to leverage limited compute power on the camera, but none of them can compress videos aggressively without sacrificing accuracy
% \begin{packeditemize}
%     \item One strawman is to run the above DNN-driven workflows on the camera, but most final DNNs are too memory-/compute-intensive for an edge camera to run locally.
%     \item One can also run a cheap object detector on the camera~\cite{vigil} to identify regions that likely contain objects. 
%     However, cheap object detector, like TinyYolo~\cite{yolo} and MobileNet-SSD can be inaccurate (as we show in \S\ref{sec:eval}) and is already too slow to run on a camera at the line speed (a Raspberry Pi 4 can barely run cheap objector in \fillme ms, as shown in Table \ref{tab:tinyyolo}).
%     \item Frame dropping~\cite{glimpse, reducto} is also an option and is widely used in some prior work, but similar to frame-level quality optimization, it falls short when objects of interest are almost always present in a dynamic scene (which makes it hard to detect arrivals of new objects).
%     % However, these approaches cannot efficiently drop frames when the video contains moving objects.
%     \item Finally, one can use autoencoders (deep-learning-based video codecs trained to optimize human perception or accuracy of a DNN), but these autoencoders are orders of magnitude more expensive than the standard video codes (used in \name): the fastest encoder runs at similar speed on GPU as H264 on CPU~\cite{rippel2019learned} (we will also evaluate autoencoder in \S\ref{sec:eval}).
%     % (\eg~\cite{rate-distortion-autoencoder})  is too heavy for the camera to afford and the accuracy remains to be low 
% \end{packeditemize}

% % In these scenarios, we desire a {\em cheap and DNN-aware encoding} that encodes {\em purely by the camera itself} (we call this property {\em local}) and delivers higher compression efficiency through macroblock-level encoding.


% % The recent effort on new video codec for DNN inference purposes like super resolution~\cite{cloudseg} and auto-encoder~\cite{rate-distortion-autoencoder} may seem to be a good choice at the first glance. 
% % However, the accuracy of super-resolution-based approach is low if there is no camera-server connection available (see Figure~\ref{fig:eval-overall}) and the encoding delay of auto-encoder is more than 4 seconds per single frame (see Figure~\ref{fig:eval-delay-overall}).
% % One may also use a cheap object detector to crop out some regions of interest and save them at the camera side~\cite{vigil}.
% % The cheap object detector, however, falls short in accuracy when handling challenging contents (as we will show in \S\ref{sec:eval}) and is still too heavy for a cheap camera to afford (cheap camera can only run TinyYoLo~\cite{yolo} in \fillme frames per second, as shown in Table~\ref{tab:tinyyolo}).
% % Thus, none of them can hit high accuracy while still maintaining local encoding.




% \mypara{Summary}
% Table~\ref{tab:design} summarizes the prior solutions in three dimensions. 
% In short, previous work all queries server-side DNN to achieve accurate compression. None of them can optimize encoding in a DNN-aware manner using only camera-side compute.

% % To further visualize the limitations of prior work, we illustrate the design choices of previous works along each design dimensions in Table~\ref{tab:design}. From ths table, we can see that none of the prior work hits macroblock-level granularity, cheap local encoding and real-time DNN awareness simultaneously.




% % One alternative approach is to leverage a cheap object detection algorithm to detect potential object of interests and encode the object of interests only.
% % However, the typical cheap object detector (such as TinyYoLO) is still much expensive compared with our approach for the camera to afford (the runtime of TinyYoLo is 2x compared to our approach as listed in Table~\ref{tab:tinyyolo}), and the overall file size-accuracy trade-off is poor (we will show this in \S\fillme).




==> motivation.tex <==

\section{Motivation}

\kt{
\begin{itemize}
\item background on video stack
\begin{itemize}
\item high-level relevant notions: frames, blocks, motion vectors, quality objectives, etc
\item traditional goals: efficient encoding (injection), storage/streaming, and efficient consumption (decoding + rendering)
\item mention dnn-based
\end{itemize}

\item background on video analytics: object detection, keypoint detection, segmentation, etc [illustrative graphs]
\item use of codec in video analytics
\begin{itemize}
\item offline analytics
\item online streaming+analytics
\item goals: fast encoding, small file sizes (injection) + high accuracy, low decoding and inference delay (consumption).
[illustrative graphs]
\end{itemize}
\end{itemize}}

\subsection{Background}

\kt{Stack: a whole piece of software: injection; define consumption phase}


\mypara{Video stack} Video stack compresses the video frame-by-frame to reduce the file size for easy storage (injection phase), and de-compresses the video back to frames to serve their users (consumption phase). 

Traditional video stack aims to serve human viewers. To meet the visual quality requirement of human viewers, the goal of the video stack is efficient encoding during injection phase, real-time decoding and preserving satisfying visual quality during consumption phase.

\mypara{Block-based encoding}
Nearby pixels have redundant mutual information. Thus, traditional video codec partite pixels into blocks and encode them based on the quantization parameter (QP).

\mypara{Vision tasks under consideration} 
We consider three computer vision tasks-object detection, semantic segmentation and keypoint detection. Figure \fillme shows an example input and output of object detection (one labeled bounding box for each object), semantic segmentation (one label for each pixel) and keypoint detection (17 keypoints for each human).

\mypara{Video stack in video analytics} 
Video stack serves video analytics in two scenarios: store the video for offline analytics and stream the video for online analytics. In these two scenarios, video stack must be able to provide video frames at a high frame rate to saturate the following analytic DNN. Moreover, video stack should also allow the following DNN to generate accurate analytic results as if the DNN is directly operating on the raw frames. Thus, the goal of video stack for video analytics is:
\begin{packeditemize}
    \item \textit{Efficient encoding}. 
    \item \textit{Efficient decoding}.
    \item \textit{High accuracy.}
\end{packeditemize}

\subsection{Opportunity: block-wise quality sensitivity for better compression}

\kt{0. Methodology w/ real encoding 1. High compress efficiency. 2. The counter-intuitive part of mask a). does not align with object boundary; (have surrounding pixels, and have surrounding pixels) b). varies a lot with content and DNN model. 3. connect to related work. 4. Plot pseudo-graph}

\kt{
\begin{itemize}
\item define ``quality sensitivity'' per block: if block $i$'s quality drops from $q$ to $q'$ while all other blocks remain at $q$, how much will accuracy drop?
\item explain the methodology: dataset, methodology (block-wise enumeration). 
\item three main takeaways from the measurements:
\begin{itemize}
\item only a small fraction of blocks need high quality (despite large objects) [graphs: y = cdf, x = fraction of pixels. one line for pixels that could be in same color, and another line for minimum pixels that must be in high quality]
\item if DNN only sees a small fraction of blocks, it can still infer accurate results
\item these highly quality-sensitive blocks may not align with objects or inference results [illustrative graphs of some case studies]
\end{itemize}
\end{itemize}
}

\mypara{Block-wise quality differentiation}
For DNN-based analysis, the power to impact accuracy is not evenly distributed between pixels.
Thus, we can save bandwidth by aggressively lowering the pixels that does not impact accuracy too much.
At codec level, however, the quality of pixels are organized by blocks.
Inside each block, the quality of pixels are the same.
Thus, block is the minimum granularity for quality differentiation.

\mypara{Mask}
To quantify the compression opportunity of quality differentiation, we present a concept: \textit{mask}.
\textit{Mask} maps each block to its corresponding encoding quality.

\mypara{Potential bandwidth saving} 
We measure the potential bandwidth saving of this opportunity on VisDrone dataset~\cite{aiskyeye} with object detection model FasterRCNN-ResNet50~[\fillme] as our backend model. 
We use two different encoding qualities: low quality and high quality\footnote{\fillme} to encode each block.
To determine the encoding quality of each block, our steps are:
\kt{Substitude this into an algorithm for general vision tasks}
\begin{packedenumerate}
    \item Encode the whole video in high quality and collect the bounding box $b_i$ for each object $i$.
    \item For each object, we assign a new bounding box $b'_i$, of which the center is the same with $b_i$ and the size of this bounding box is $0$.
    \item Partition the whole frame into 16$\times$ 16 blocks.
    \item Use highest quality to encode those blocks that overlaps with any of $b'_i$, and use lowest quality to encode other blocks.
    \item If less than 95\% objects are detected, for those objects $j$ that are not detected, enlarge $b'_i$ by padding a constant on the left, top, right, bottom on it, and go back to step 3.
\end{packedenumerate}


% One way to save bandwidth is to reduce the encoding quality.
% Also, the power to impact accuracy is not evenly distributed between pixels.
% It follows that we can saving bandwidth through manipulating pixel encoding quality.
% However, the pixels inside the same block (determined by the codec) will always have the same quality.
% So we instead encode

% \mypara{Heterogeneous quality sensitivity requirements} 
% Different vision models care about different parts in the video. For example, vehicle detection models care car pixels much more than human pixels; and human detection models care human pixels much more than car pixels. In terms of encoding, it means that different vision models are more sensitive to the encoding quality of some blocks more than other blocks.

% This opportunity implies that we can save bandwidth if we encode those quality-sensitive blocks in high encoding quality and those quality-insensitive blocks in low encoding quality.

% \blindtext

\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figs/percpixel-accuracy.pdf}
    \caption{Percentage of pixels encoded in high quality v.s. accuracy. Only 2\% of the pixels need to be encoded to make accuracy more than 0.95.}
    \label{fig:percpixel-accuracy}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figs/object-hqblock.pdf}
    \caption{Inference results on images with different regions in high quality. Some objects do not need to be all in high quality to be detected, and some objects need surrounding pixels in high quality to be detected.}
    \label{fig:object-hqblock}
\end{figure}

\begin{figure}
    \centering
\includegraphics[width=0.4\columnwidth]{figs/hetero-task.pdf}
    \caption{Accuracy on different task with the same compressed video. One size does not fit for all vision tasks.}
    \label{fig:hetero-task}
\end{figure}

\begin{figure}
    \centering
\includegraphics[width=0.4\columnwidth]{figs/hetero-dnn.pdf}
    \caption{Accuracy on different object detection DNN with the same compressed video. Accurate compression for cheap model may not work on expensive model.}
    \label{fig:hetero-dnn}
\end{figure}


\mypara{Takeaways} During the measurement above, we find that:
\begin{packeditemize}
    \item To reproduce satisfactory inference result, only a small fraction of blocks need to be encoded in high quality. From Figure \ref{fig:percpixel-accuracy}, we can see that covering only \fillme\% pixels will yield more than \fillme\% of accuracy.
    \item Object may not align with the high-quality blocks. From Figure \ref{fig:object-hqblock}, we see that some objects do not need to be all in high quality to be detected, and some objects need surrounding pixels in high quality to be
\end{packeditemize}

\mypara{Heterogeneity between vision tasks and models}
This compression opportunity varies a lot between different vision tasks and models.
In other word, one mask that works perfectly for one application might result in poor accuracy in another application.
In Figure \ref{fig:hetero-task}, accurate compression for keypoint detection does not work on object detection and semantic segmentation.
So compression need to be designed for different applications.
Moreover, in Figure \ref{fig:hetero-dnn}, we see that even under the same vision task, compression that works for one DNN may not work on others.

\blindtext

\mypara{Limitation of existing work} 
Wrong assumptions of related work was revealed by our measurement study above. 
The vast majority of current works on quality differentiation~\cite{dds,vigil,glimpse,eaar} implicitly assumes that high quality regions should align with the objects.
However, in Figure \ref{fig:object-hqblock}, we see that high quality regions can be much smaller or much larger than the object itself.
So objects might be missed or file size might be wasted if aligning high quality regions with objects.



\subsection{Mismatch of today's video codec}

\kt{
\begin{itemize}
\item{Human perception-centric quality encoding}
\begin{itemize}
\item the highly sensitive blocks are highly dependent on the task
\item existing heuristics are completely unaware of the server-side dnn structure
\item implications: need a generic way to encode videos in cognizant of the block-level sensitivity. [an illustrative example]
\end{itemize}
\item{Encoding dynamic quality sensitivity}
\begin{itemize}
\item the highly-sensitive pixels changes a lot across frames
\item today's encoding is inefficient: unnecessary motion vector, etc.  micro-block misalignment
\item implications: need a way to ``smooth'' the highly dynamic sensitive blocks [an illustrative example]
\end{itemize}
\item{Frame-wise semantics}
\begin{itemize}
\item analyzing the whole frames one by one
\item implications: putting sensitive regions together [an illustrative example]
\end{itemize}
\end{itemize}}

\mypara{Traditional video codec}
Caring about visual quality, traditional video codec pays nearly equal attention to all pixels. 
The quality-sensitive blocks, however, are highly dependent on server-side DNNs.
Traditional video codec is unable to exploit this opportunity due to its unawareness to server-side DNN.
This implies that we need a generic way to encode the videos in cognizant of block quality-sensitivity, see Figure \fillme for an illustration.

\mypara{Super resolution}
Nowadays, super resolution \cite{cloudseg,livenas} gradually becomes a new choice of video codec.
These approaches encode the video in low quality, store or stream the low quality video at server side, and then compensate the quality loss by super resolution network.

However, super resolution is fundamentally an ill-suited problem. Multiple high-quality frames may have exact same low-quality frames if compressed by the codec.
As a result, even the most compute-intensive super resolution network cannot fully recover the areas crucial to inference results. Figure \fillme shows an example.
To overcome this issue, current approaches choose to retrain the neural network online. This design choice poses too much online cost at the server side.

\mypara{Auto-encoder}
Computer vision community is actively exploring a new type of codec called auto-encoder~\cite{rate-distortion-autoencoder}. These approaches encode the video by feeding it through neural network and storing the output of that neural network. 

Unfortunately, auto-encoder that preserves high image quality is too compute-intensive for a single CPU to afford (\fillme seconds per frame).
Moreover, this approach requires another neural network as the decoder. Thus, every frame needs to be processed by the decoder at inference time and poses too much online overhead. 



\subsection{Mismatch of existing video analytics pipelines}

\kt{Benefit different vap, weaken this argument}

\kt{
\begin{itemize}
%\item approach \#1: twisting existing interface, (2) case-by-case heuristics
\item limitation \#1: fail to adapt to real-time video content (sr, awstream, vstore)
\item limitation \#2: slow costly (dds, dnn-based autocodec)
\item limitation \#3: only applies to one task (vigil, eaar, focus)
\end{itemize}}

Video analytic pipelines stream videos from the camera to the server and generate analytic results with minimum overhead as well as maintaining satisfying accuracy. However, these approaches are not suitable for video stack purpose.

\mypara{Agnostic to real-time video content} 
AWStream~\cite{awstream} and CloudSeg~\cite{cloudseg} exploit the optimal configurations~\cite{awstream} or  super resolution networks~\cite{cloudseg} derived from \textit{history video content} and count on the similarity between real-time video content and history video content.
However, in real world, the video content can change drastically. 
For example, when a car equipped with traffic camera driving on a street that human rarely appears, the system needs to adapt every time human appears to detect all of them.
These approaches are likely to have low accuracy in these scenarios.

\mypara{Too much online cost for real-time content adaptation} 
Instead, DDS~\cite{dds} choose to leverage server-side compute to adapt for video content. 
As for the online cost, however, DDS needs to run one extra inference per frame to dig out the objects that are missed, which doubles the online cost.

\mypara{Task-specific}
Vigil~\cite{vigil}, EAAR~\cite{eaar}, Focus~\cite{focus} can leverage real-time video content at relatively low cost.
Their use cases, however, are limited to object detection~\cite{vigil, eaar} and frame classification~\cite{focus} and make them not applicable for other vision tasks and applications.



==> overview-v2.tex <==

\section{Overview of \name}

We present \name, a new encoder that achieves local macroblock-level encoding optimization on edge cameras.
% To cope with the challenge above, we present \name, a cheap, local and DNN-aware video encoder. 
% \name trains 
% we present {\em \name}, which uses
% a cheap model to detect quality-sensitive macroblocks of a given DNN in realtime and assigns high encoding quality to these blocks only.
This section begins with the overall workflow of \name and its key insight.

% To be concrete, the performance criteria of \name are:
% \begin{packeditemize}
%     \item {\em Small file size with high accuracy.} \name needs to reduce the file size while maintaining high accuracy.
%     \item {\em On-premise fast encoding.} \name needs to have similar encoding delay as basic video encoding on camera's CPUs.
%     \item {\em Quick training.} \name need to finish training its model to new video anlaytic DNN within several minutes.
% \end{packeditemize}



% In this section, we begin with the overall workflow of \name. 
% After that, we introduce the key idea of \name that enables us to meet the performance criteria.
% We then discuss the design rationales behind \name.


% Based on the design goal above, the challenge is: how to assign encoding quality to each microblock on the cameras in a {\em cheap, local and DNN-aware} manner? 
% To be concrete, the performance requirements are:
% \begin{packeditemize}
%     \item {\em Small file size with high accuracy.} The desired algorithm needs to reduce the file size while maintaining high accuracy.
%     \item {\em On-premise fast encoding.} The desired algorithm needs to have similar encoding delay as basic video encoding on camera's CPUs.
%     \item {\em Quick customization.} The desired algorithm need to adapt to new server-side vision model within tens of minutes.
% \end{packeditemize}

% % Previous works, however, all achieve DNN-awareness through camera-server connection. One category of previous works focusing on exploiting real-time feedbacks from server-side DNN~\cite{eaar,dds}. As a result, these works assume the server is nearly always within reach and can only handle server disconnection for several seconds through client-side tracking. The other category of previous works instead maintain a profile~\cite{awstream,reducto} or maintain a server-side decompressor~\cite{cloudseg} and update them periodically to cope with the change of video content. However, to perform these updates, these systems require the camera to stream the video in quality as the ground truth to the server and thus requires good internet connection (the bandwdidth requirement for the camera-server connection is about 2.5Mbps\footnote{We calculate this number based on a traffic camera video from youtube~\cite{trafficcam-example}.}).

% The difficulty that lies behind being cheap, local and DNN-aware is that this assumptions requires the camera to be aware of server-side DNN as well as encoding without a server. 
% How can the camera be aware of server-side DNN without even looking it at encoding stage?





% \subsection{Design rationales behind \name}
% \label{subsec:rationale}


% To address this difficulty, our insight is that: learning the quality assignment for the server-side DNN is order-of-magnitude easier than what the server-side DNN actually do (we will explain this in \S\fillme). Based on this observation, we formalize this learning problem as learning {\em accuracy gradient} (\AccuracyGradient for short), train a cheap model that generates \AccuracyGradient, and then deploy this model to the camera.

% We design \name to address the challenge above. \name trains a DNN in an automatic manner that assign encoding quality (high quality or low quality) to each microblock offline, and then use this DNN to guide the encoding process. 









\subsection{Workflow of \name}


\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{figs/overall-workflow.pdf}
    \tightcaption{Architecture and three phases of \name. \kt{Maybe replot this figure? The reading flow of this figure is not pretty linear...}}
    \label{fig:workflow}
    \vspace{-3mm}
\end{figure}

As depicted in Figure~\ref{fig:workflow}, the key component of \name is the cheap {\em quality selector}.
\begin{packeditemize}
\item {\em Training the quality selector (\S\ref{sec:training}):}
For a given final DNN, \name offers a routine to train the quality selector for the DNN. 
Users need to provide the final DNN's inference function $\DNN(\HighImage)$, which takes as input an image $\HighImage$ and returns the inference results.
They also need to provide the accuracy function $\SimFunc(x,y)$, which takes an inference output $x$ and the ground truth $y$ as input and calculate the accuracy of $x$ against $y$.
Both $\DNN(\HighImage)$ and $\SimFunc(x,y)$ must be differentiable, but this is already the common case as modern DNN training already requires them to be differentiable.
By default, the quality selector is trained on a sampled subset of images in COCO dataset~\cite{coco} (\S\ref{subsec:??}). 
\item {\em Online encoding (\S\ref{sec:encoding}):}
The trained quality selector is deployed on the edge camera.
\name then feeds each incoming frame to the quality selector to detect the quality-sensitive macroblocks of a given final DNN, and it then applies
% The analyst can use the thresholds of $\AgThresh$ or $\AreaThresh$ ({\footnotesize{\bf \texttt{param}}}) to decide the quality assignment according to \S\ref{subsec:quality-assignment}.
% By setting the parameters, users can select tradeoff between accuracy and compression efficiency (file size). 
%The encoded video will then be saved together with a metafile that includes the quality assignment information.
% \name will then apply 
region-of-interest encoding to encode only these quality-sensitive macroblocks in high quality.
\end{packeditemize}


% To address this difficulty, we present \name, a new video encoder for video analytic applications.
% \name trains a cheap model {\em offline} (hereinafter \AccuracyGradientModel) that determines the quality-sensitive macroblocks based on final DNN and deploy it to the camera side.
% Upon encoding, the camera runs \AccuracyGradientModel to determine which macroblocks should be in high quality and encode the video correspondingly.

% Figure~\ref{fig:workflow} depicts \name's workflow and the three APIs:

% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{ag\_model = prepare(dnn\_func,acc\_func)}}\\
% {\bf \texttt{encoded\_video = ingest(ag\_model,*raw\_frame,param)}}\\
% {\bf \texttt{result = consume(encoded\_video,dnn)}}
% \vspace{0.1cm}
% }






% \mypara{Creating \AccuracyGradientModel}
% At this stage, \name offers an \AccuracyGradientModel pretrained on COCO dataset~\cite{coco} for different analytic tasks. Optionally, the analyst can choose to retrain or customize the \AccuracyGradientModel through three APIs:
% \begin{packeditemize}
%     \item The accuracy function $\SimFunc(x,y)$. This function receives the inference results $x$, the ground truths $y$ and calculate the accuracy of $x$ against $y$ in a differentiable manner. Analyst can choose to use the negative training loss of the final DNN, or implement customized accuracy function.
%     \item The inference function $\DNN(\HighImage)$. This function receives the input $\HighImage$ and generates the corresponding inference results $\DNN(\HighImage)$.
%     \item A dataset iterator $D$. \name will use $D$ as the training set and update $\AccuracyGradientModel$. 
% \end{packeditemize}
% We will further discuss the training details and training cost reduction techniques in \S\ref{sec:training}.
% After training, \name deploys the \AccuracyGradientModel on the camera side and wait for online encoding.


% The analyst provides \name the final DNN with its accuracy function ({\footnotesize{\bf \texttt{acc\_func}}}), and \name trains a customized {\em \AccuracyGradientModel} ({\footnotesize{\bf \texttt{ag\_model}}}), which will predict the \ags on any new frame. 
% %(similarity between DNN outputs on the high-quality frame and on the low-quality encoding)
% %The accuracy function takes DNN's outputs on the high quality encoding and on the low quality encoding of a frame as input, and returns the similarity between them (which indicates accuracy as defined in \S\ref{??}).
% %the accuracy of running the DNN on the encoded frame with respect to the result of running the DNN on the high quality image as the ``ground truth''. 
% Optionally, the operator also provides a dataset to {\em finetune} the \AccuracyGradientModel; otherwise, \name can directly use the pretrain
% We evaluate these choices in \S\ref{subsec:eval:micro}.
% %As elaborated in \S\ref{??}, the choice of training data involves a tradeoff between accuracy-gradient model performance and real-time overhead. 

% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{ag\_model = prepare(dnn\_func,acc\_func)}}
% }

\mypara{Key challenges}
The key is how to make the quality selector fast and easily customized for each given DNN:
\begin{packeditemize}
\item {\em Challenge 1: How to detect the quality-sensitive macroblocks in realtime using only local compute resource of an edge camera?}
In other words, \name's encoding overhead should be on par with only running the video codec.
%    \item How to discover the important pixels in a real-time, fine-grained manner while still being affordable for a cheap camera?
\item {\em Challenge 2: How to quickly customize \name (ideally in a few minutes or less) for any given final DNN?}
What's more, an \name trained for one final DNN should also work decently with another DNN of similar task.
%    \item How to customize \name for any given DNN {\em quickly and automatically}?
\end{packeditemize}



% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{encoded\_video = encode(ag\_model,*frame,param)}}
% }

\begin{comment}
\mypara{On-demand decoding}
Finally, when the user decide to analyze the video, \name decodes the video to frames and then feed them to the final DNN.
%and use the quality assignment information in the metafile to overlay the decoded high quality blocks on the low quality one. 
%The resulting frames are 
% and then feed them to the DNN for inference whenever needed.
%As an further optimization to reduce inference time, the DNN can also use the quality sensitivity information in the metafile to filter out regions that are very unlikely to have useful information (\eg background).

% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{*frame = decode(encoded\_video)}}
% \vspace{0.1cm}
% }

% Though the workflow sketched in Figure~\ref{fig:workflow} is functionally sufficient,
% %to encode videos with spatially different quality based on the notion of accuracy gradients, 
% two challenges remain: 
% (1) how to learn an accurate \AccuracyGradientModel (\S\ref{sec:training}); and (2) how to use it in real time for high accuracy and low encoding/decoding overhead (\S\ref{sec:runtime}).
% We will address them in the next two sections.



\mypara{Challenge} The core challenge of designing \name is: how to find a machine learning problem that achieve high compression efficiency while enabling a series of system optimization?

\end{comment}


\subsection{Key idea: Accuracy Gradients}

The key idea of \name is the concept of {\em Accuracy Gradients} (\AccuracyGradient).
Intuitively the \AccuracyGradient of a macroblock measures how much the macroblock's encoding quality influences the final DNN's inference accuracy.

Here, we first formally define \AccuracyGradient and how \name uses it, then explain the formulation that leads us to it, and finally explain the rationale behind why \AccuracyGradient enables \name to address the two aforementioned challenges.

\mypara{Defining \AccuracyGradient} 
We split each $\OriginWidth\cdot\OriginHeight$ frame into $\GridWidth\cdot\GridHeight$ grids of 16x16 blocks ($\OriginWidth=16\GridWidth,\OriginHeight=16\GridHeight$).
Given a frame whose high-quality encoding and low-quality encoding are $\HighImage$ and $\LowImage$ respectively, \AccuracyGradient at the macroblock $x,y$ is defined as:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\AccuracyGradient_{x,y} = \sum_{(i,j)\in block_{x,y}}\bigg\Vert\frac{\partial \SimFunc\big(\DNN(\LowImage), \DNN(\HighImage)\big)}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_1. \label{eq:acc-gradients}
% \bigg\Vert\frac{\partial{\AccuracyFunc\circ \DNN(\textbf{V}), gt)}}{\partial \textbf{V}} \bigg|_{i,j}\bigg\Vert_2 \label{eq:acc-gradients}
\end{align}
}
where $\SimFunc(x, y)$ measures the accuracy of inference results $x$ against ground truth $y$, $\HighImage$ and $\LowImage$ are the high-quality encoding and the low-quality encoding of each frame\footnote{The dimension of a frame is the same for different QP values, so $\HighImage$ and $\LowImage$ have the same dimension.} and $\DNN$ is the inference function of the final DNN.

\mypara{Quality selector based on \AccuracyGradient}
Since calculating the real \AccuracyGradients requires running the final DNN $\DNN$, \name trains a cheap model \AccuracyGradientModel that predicts the \AccuracyGradient per macroblock in a given frame.
Based on \ag matrix of a frame, \name then uses one of two parameters to decide which blocks in a frame should be encoded in high quality: 
\begin{packeditemize}
\item {\em \Ag threshold ($\AgThresh$)} means all blocks $(x,y)$ with $\AccuracyGradient_{x,y}\geq\AgThresh$ will be encoded in high quality.
%\name picks a subset of blocks whose \ags based on Eq (\ref{eq:acc-gradients}) are over $\AgThresh$.
\item {\em High-quality area threshold ($\AreaThresh$)} sets the maximum number of high-quality blocks, by simply picking the top $\AreaThresh$ blocks with the highest \ags.
%\name picks the top $\AreaThresh$ blocks with the highest \ags.
\end{packeditemize} 
After a set of blocks are selected, \name then 
% the block-padding scale $\PadThresh$ to 
expands these selected blocks to each direction by $\PadThresh$ (by default 4) blocks (if they are not already selected). 
% We will further explain the rationales in \S\fillme.

Both $\AgThresh$ and $\AreaThresh$ allow users to navigate \name's accuracy-compression tradeoffs (lower $\AgThresh$ or higher $\AreaThresh$ increases the accuracy at the expense of encoding more blocks).
However, they have very different practical implications.\footnote{At a high level, the effects of $\AgThresh$ and $\AreaThresh$ in \name are analogous to variable bitrate (VBR) and constant bitrate (CBR) encoding (one adapts to content and one maintains constant bitrate).
However, we acknowledge that $\AgThresh$ and $\AreaThresh$ in our design do not directly tie to a target accuracy or fixed bitrate, which we will discuss in \S\ref{sec:discuss}.
Nonetheless, we will demonstrate how they can help adaptive streaming in \S\ref{subsec:eval:adaptive}.}
\begin{packeditemize}
\item When the \ag threshold $\AgThresh$ is set to a fixed value, \name will assign high quality to {\em all} low \ag blocks.
In effect, it {\em adapts the compression rate to content}, \eg when content is simple, it will compress more aggressively.
\item When the high-quality area threshold $\AreaThresh$ is set to a fixed value, \name will assign high quality to a {\em fixed} number of blocks.
As a result, it {\em adapts the accuracy to a target compression rate}.
\end{packeditemize} 


\subsection{Rationale of Accuracy Gradients}
\label{subsec:rationales}

\mypara{Why \AccuracyGradient improves accuracy-compression tradeoffs}
The above quality assignment process based on \AccuracyGradient (Equation~\ref{eq:acc-gradients}) in effect approximates the optimal solution of the following problem.
Let us use $\AccuracyGradientModel$ as the input a high quality image $\HighImage$ and returns as output a $[0,1]$-valued mask of size $\GridWidth\cdot\GridHeight$, $\Mask=\AccuracyGradientModel(\HighImage)$. 
The element inside the mask $\Mask_{x,y}=1$ means block $x,y$ is completely in high quality and $\Model(\Mask_{x,y})=0$ means block $x,y$ is completely in low quality.
Then the optimization goal is to maximize accuracy with less elements of $\Mask$ being 1: 

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\max_{\AccuracyGradientModel} &~~~~\SimFunc\bigg(\DNN \big(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage \big),\DNN(\HighImage)\bigg) - \lambda  \frac{\big\Vert \Mask \big\Vert_1}{numel \big(\Mask\big)}
\label{eq:idealized-objective}
\end{align}
}
where $\AllOnes$ refers to a matrix where all the elements are one, $\times$ refer to pixel-wise multiplication\footnote{The multiplication operation here will first resize the left operand back to size $\OriginWidth\cdot\OriginHeight$ and then apply pixel-wise multiplication.}, $\big\Vert \Mask \big\Vert_1 / {numel \big(\Mask\big)}$ counts percentage of macroblocks inside $\Mask$ encoded in high quality and $\lambda$ navigates the trade-off between accuracy and percentage of macroblocks in high quality.
We will elaborate how \AccuracyGradients optimize Equation~\ref{eq:idealized-objective} in \S\ref{subsec:bandwidth-adaptation}.
% (we will specify how we navigate this trade-off in \S\ref{subsec:bandwidth-adaptation}).

\begin{comment}

\subsection{Key enabler: accuracy gradients}


\mypara{Formulation} We first formulate quality assignment problem into an optimization problem.
To make the discussion more concrete, we split each $\OriginWidth\cdot\OriginHeight$ frame into $\GridWidth\cdot\GridHeight$ grids of 16x16 blocks ($\OriginWidth=16\GridWidth,\OriginHeight=16\GridHeight$) and assign each block either a high quality or a low quality. % (this aligns with previous work~\cite{eaar,dds}).
Our goal is to find a model $\AccuracyGradientModel$ that generates a $[0,1]$-valued mask of size $\GridWidth\cdot\GridHeight$ by feeding the high quality image $\HighImage$ into $\AccuracyGradientModel$, \ie $\Mask=\AccuracyGradientModel(\HighImage)$, where the element inside the mask $\Mask_{x,y}=1$ means block $x,y$ is completely in high quality and $\Model(\Mask_{x,y}=0$ means block $x,y$ is completely in low quality. The optimization goal is to minimize the number of blocks in high quality as well as maximize the inference accuracy\footnote{This formulation involves two simplifying assumptions: the 16x16 blocks may be suboptimal boundaries between quality levels, and it restricts the encoding to only two quality levels.
That being said, we believe that analyzing this formulation is still valuable for two reasons.
First, the block granularity of 16x16 is on par with the block sizes employed in H.264 and H.265, which means more fine-grained blocks will not have much impact on the encoded video size. 
Second, the use of two quality levels does subsume many recent solutions (\eg~\cite{vigil, dds, awstream, glimpse, reducto}) which use two or fewer quality levels.}:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\max_{\AccuracyGradientModel} &~~~~\SimFunc\bigg(\DNN \big(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage \big),\DNN(\HighImage)\bigg) - \lambda  \frac{\big\Vert \Mask \big) \big\Vert_1}{numel \big(\Mask\big)}
\label{eq:idealized-objective}
\end{align}
}
where $\SimFunc(x, y)$ measures the accuracy of inference results $x$ against ground truth $y$, $\HighImage$ and $\LowImage$ are the high-quality encoding and the low-quality encoding of each frame\footnote{The dimension of a frame is the same for different QP values, so $\HighImage$ and $\LowImage$ have the same dimension.}, $\AllOnes$ refers to a matrix where all the elements are one, $\times$ refer to pixel-wise multiplication\footnote{The multiplication operation here will actually resize the left operand back to size $\OriginWidth\cdot\OriginHeight$ and then apply pixel-wise multiplication.}, $\DNN$ is the server-side DNN that generates the DNN inference result, $\big\Vert \Mask \big\Vert_1 / {numel \big(\Mask\big)}$ counts percentage of macroblocks inside $\Mask$ encoded in high quality and $\lambda$ navigates the trade-off between accuracy and percentage of macroblocks in high quality (we will specify how we navigate this trade-off in \S\ref{subsec:bandwidth-adaptation}).


\mypara{Accuracy gradients} To efficiently solve the problem above, we develop a novel concept called accuracy gradient (\AccuracyGradient in short), defined as:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\AccuracyGradient_{x,y} = \sum_{(i,j)\in block_{x,y}}\bigg\Vert\frac{\partial \SimFunc\big(\DNN(\LowImage), \DNN(\HighImage)\big)}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_1. \label{eq:acc-gradients}
% \bigg\Vert\frac{\partial{\AccuracyFunc\circ \DNN(\textbf{V}), gt)}}{\partial \textbf{V}} \bigg|_{i,j}\bigg\Vert_2 \label{eq:acc-gradients}
\end{align}
}
\kt{I rewrite the formulation here to enable the half splitting trick }Based on this concept, in order to maximize Equation~\ref{eq:idealized-objective}, we only need to let our \AccuracyGradientModel learns \AccuracyGradient (we will show the connection between Equation~\ref{eq:idealized-objective} and \ref{eq:acc-gradients} in \S\fillme)












\subsection{\Ag-based quality assignment}
\label{subsec:quality-assignment}

Given the matrix of \ags of a frame, \name then uses one of two parameters to decide which blocks in a frame should be encoded in high quality: 
\begin{packeditemize}
\item {\em \Ag threshold $\AgThresh$} means all blocks $(x,y)$ with $\AccuracyGradient_{x,y}\geq\AgThresh$ will be encoded in high quality.
%\name picks a subset of blocks whose \ags based on Eq (\ref{eq:acc-gradients}) are over $\AgThresh$.
\item {\em High-quality area threshold $\AreaThresh$} sets the maximum number of high-quality blocks, by simply picking the top $\AreaThresh$ blocks with the highest \ags.
%\name picks the top $\AreaThresh$ blocks with the highest \ags.
\end{packeditemize} 
After a set of blocks are selected, \name then 
% the block-padding scale $\PadThresh$ to 
expands these selected blocks to each direction by $\PadThresh$ (by default 4) blocks (if they are not already selected). We will further explain the rationales in \S\fillme.

Both $\AgThresh$ and $\AreaThresh$ allow users to navigate \name's accuracy-compression tradeoffs (lower $\AgThresh$ or higher $\AreaThresh$ increases the accuracy at the expense of encoding more blocks).
However, they have very different practical implications.
\begin{packeditemize}
\item When the \ag threshold $\AgThresh$ is set to a fixed value, \name will assign high quality to {\em all} low \ag blocks.
In effect, it {\em adapts the compression rate to content}, \eg when content is simple, it will compress more aggressively.
\item When the high-quality area threshold $\AreaThresh$ is set to a fixed value, \name will assign high quality to a {\em fixed} number of blocks.
As a result, it {\em adapts the accuracy to a target compression rate}.
\end{packeditemize} 
At a high level, the effects of $\AgThresh$ and $\AreaThresh$ in \name are analogous to variable bitrate (VBR) and constant bitrate (CBR) encoding (one adapts to content and one maintains constant bitrate).
However, we acknowledge that $\AgThresh$ and $\AreaThresh$ in our design do not directly tie to a target accuracy or fixed bitrate, which we will discuss in \S\ref{sec:discuss}.
Nonetheless, we will demonstrate how they can help adaptive streaming in \S\ref{subsec:eval:adaptive}.

%while minimizing compressed video size. 
%In contrast, the high-quality area threshold $\AreaThresh$ can be used to {\em control compressed video size} while maximizing accuracy. 

%\jc{can't control directy, but effective}

% In practice, we found tuning them result in a similar frontier of accuracy/compression tradeoffs, so we expose $\AgThresh$ as a tunable parameter to users (just as QP in MPEG/H.264) and empirically set $\PadThresh$ at 2 by default.


%it is straightforward to derive the optimal quality assignment on the given frame.
%\jc{Kuntai, please give the derivation}
%Recall that only $c$-many blocks will be encoded in high quality, we just need to pick $c$-many blocks with largest accuracy gradient value, encode them in high quality and encode remaining blocks in low quality.



















\subsection{Design rationales}


\end{comment}




\mypara{Why \AccuracyGradientModel can be cheap} 
% A natural question is that why a cheap \AccuracyGradientModel exists. This is because learning \AccuracyGradient has three properties that makes it much easier than traditional server-side DNN tasks like semantic segmentation:
A cheap \AccuracyGradientModel can be learned due to three reasons that make it easier to learn than semantic segmentation, a typical computer-vision task:
\begin{packeditemize}
    \item {\em Small output space:} %\kt{I name it to small output space cuz coarse granularity sounds like we are not doing fine-grained encoding}
    \AccuracyGradientModel returns one label per macroblock (all pixels in a 16x16 macroblock share the same DNN output). 
    The benefit is that, in contrast to traditional convolutional operations which scan the image pixel by pixel, \AccuracyGradientModel logically only needs to scan the image macroblock by macroblock (which has a compute saving of upto 256x on convolutional operations).
    Moreover, compared to the common multi-class segmentation tasks, the task of \AccuracyGradientModel is essentially {\em binary} classification (classifying each macroblock as high quality or low quality), which further reduces the complexity of \AccuracyGradientModel. 
    {\em  This property also enables us to reduce the cost of \AccuracyGradientModel.} (More details in \S\ref{subsec:architecture}).
    % So we can let these pixels generate {\em one} feature, and then apply future compute to this one feature to get the output of this 16x16 macroblock. Ideally, this means that we can save {\em 256x} compute cost compared to traditional segmentation task.
%   {\em  This property also enables us to reduce the cost of \AccuracyGradientModel.} 
    % \item {\em Binary segmentation:} Quality assignment task is essentially a binary classification (classifying each macroblock as high quality or low quality), while traditional semantic segmentation is multi-class classification (classify each pixel to a class label). The former is easier than the latter. This wisdom is also used by other works ~\cite{dds}. 
    \item {\em Boundary expansion tolerance:}
    While accurate image segmentation must return precise boundaries along objects, our formulation~\ref{eq:idealized-objective} relaxes this constraints. 
    Slightly expanding the high-quality regions has little impact on the accuracy of the final DNN, though the compressed file size will slightly increase\footnote{Due to intra-frame encoding in modern codecs, the compressed video size grows sublinearly with more high-quality regions, which is favorable to \name.}.
    {\em This property enables us to inference on \AccuracyGradient less frequently.} (More details in \S\fillme.)
    % One of the central challenge of image segmentation task is to accuracy sketch the object boundary~\cite{crf}. 
    % However, our formulation~\ref{eq:idealized-objective} makes this less of an issue.
    % This is because our formulation permits \AccuracyGradientModel to slightly expand the object boundary\footnote{Expanding the object boundary will only make the percentage of high pixels (i.e. $\big\Vert \Mask \big\Vert_1 / {numel \big(\Mask\big)}$) marginally larger, and thus have little impact on the value of overall objective~\ref{eq:idealized-objective}.} to make the object boundary much smoother and easier to learn.
    % However, when maxmizing Equation~\ref{eq:idealized-objective}, we can encode some extra blocks into high quality as long as those important microblocks that might hurt accuracy if compressed can be segmented out. So when it comes to a microblock that the DNN is not sure whether it is on the boundary or not, the DNN can safely put this microblock in high quality.
    % \item False positive tolerance. Also, as long as the important microblocks are segmented out to make the accuracy high, it is OK to segment out some other microblocks since they will only cause little bit of extra file size. Accordingly, when it comes to a microblock that the DNN is not sure whether it is part of the object or not, it can safely put this microblock in high quality.
\end{packeditemize}


These observations suggest that a shallow NN is enough for \AccuracyGradientModel. 
% to exploit the opportunity behind the optimization objective~\ref{eq:idealized-objective} and thus have a preferable file size-accuracy trade-off.
This is empirically validated in Figure~\ref{fig:architecture-loss} which shows cheap \AccuracyGradientModel can predict \AccuracyGradients almost as accurately as a much more expensive one
(see \S\ref{subsec:architecture}).
% support that a cheap model can already have similar performance compared to the compute-intensive models in \S\ref{subsec:architecture}







\mypara{Why training \AccuracyGradientModel can be fast}
Training a \AccuracyGradientModel that optimizes Equation~\ref{eq:idealized-objective} can be prohibitively expensive for two reasons:
(1) it requires running numerous forward/backward propagations on the end-to-end pipeline of $\DNN$, $\AccuracyGradientModel$, and $\AccuracyFunc$, and (2) similar training typically requires a large set of images~\cite{??,??}. 
% Directly training through objective~\ref{eq:idealized-objective} can be expensive.
% This is because this formulation requires passing through the heavy server-side DNN {\em in every training epoch}.
Fortunately, \AccuracyGradient can be directly derived from the final DNN $\DNN$ (Equation~\ref{eq:acc-gradients}) using one forward-backward propagation. 
This allows us to separate the compute-intensive $\DNN$ from the end-to-end training and instead focus the computation on training of \AccuracyGradientModel.
% By leveraging the \AccuracyGradient to train \AccuracyGradientModel, however, we only need to access the server-side DNN {before} training starts to generate ground truths.
% The afterward training process of \AccuracyGradientModel is then completely irrelevant to server-side DNNs.
Empirically, this can save about {\em 15x} overhead on accessing the heavy server-side DNNs since the \AccuracyGradientModel typically takes 15 training epochs to converge (see Figure~\ref{fig:architecture-loss} for the convergence speed).








% Thus, the overall training overhead of \AccuracyGradientModel is minor. We will further develop training cost reduction technique in \S\ref{sec:training}.




==> overview-v3.tex <==

\section{Overview of \name}
\label{sec:overview}

% We present \name, a new encoder that achieves local macroblock-level encoding optimization on edge cameras.
% This section begins with the overall workflow of \name and its key insight.


% To cope with the challenge above, we present \name, a cheap, local and DNN-aware video encoder. 
% \name trains 
% we present {\em \name}, which uses
% a cheap model to detect quality-sensitive macroblocks of a given DNN in realtime and assigns high encoding quality to these blocks only.

% To be concrete, the performance criteria of \name are:
% \begin{packeditemize}
%     \item {\em Small file size with high accuracy.} \name needs to reduce the file size while maintaining high accuracy.
%     \item {\em On-premise fast encoding.} \name needs to have similar encoding delay as basic video encoding on camera's CPUs.
%     \item {\em Quick training.} \name need to finish training its model to new video anlaytic DNN within several minutes.
% \end{packeditemize}



% In this section, we begin with the overall workflow of \name. 
% After that, we introduce the key idea of \name that enables us to meet the performance criteria.
% We then discuss the design rationales behind \name.


% Based on the design goal above, the challenge is: how to assign encoding quality to each microblock on the cameras in a {\em cheap, local and DNN-aware} manner? 
% To be concrete, the performance requirements are:
% \begin{packeditemize}
%     \item {\em Small file size with high accuracy.} The desired algorithm needs to reduce the file size while maintaining high accuracy.
%     \item {\em On-premise fast encoding.} The desired algorithm needs to have similar encoding delay as basic video encoding on camera's CPUs.
%     \item {\em Quick customization.} The desired algorithm need to adapt to new server-side vision model within tens of minutes.
% \end{packeditemize}

% % Previous works, however, all achieve DNN-awareness through camera-server connection. One category of previous works focusing on exploiting real-time feedbacks from server-side DNN~\cite{eaar,dds}. As a result, these works assume the server is nearly always within reach and can only handle server disconnection for several seconds through client-side tracking. The other category of previous works instead maintain a profile~\cite{awstream,reducto} or maintain a server-side decompressor~\cite{cloudseg} and update them periodically to cope with the change of video content. However, to perform these updates, these systems require the camera to stream the video in quality as the ground truth to the server and thus requires good internet connection (the bandwdidth requirement for the camera-server connection is about 2.5Mbps\footnote{We calculate this number based on a traffic camera video from youtube~\cite{trafficcam-example}.}).

% The difficulty that lies behind being cheap, local and DNN-aware is that this assumptions requires the camera to be aware of server-side DNN as well as encoding without a server. 
% How can the camera be aware of server-side DNN without even looking it at encoding stage?





% \subsection{Design rationales behind \name}
% \label{subsec:rationale}


% To address this difficulty, our insight is that: learning the quality assignment for the server-side DNN is order-of-magnitude easier than what the server-side DNN actually do (we will explain this in \S\fillme). Based on this observation, we formalize this learning problem as learning {\em accuracy gradient} (\AccuracyGradient for short), train a cheap model that generates \AccuracyGradient, and then deploy this model to the camera.

% We design \name to address the challenge above. \name trains a DNN in an automatic manner that assign encoding quality (high quality or low quality) to each microblock offline, and then use this DNN to guide the encoding process. 









% \subsection{Workflow of \name}


\begin{figure}
    \centering
    \includegraphics[width=1.9\columnwidth]{figs/overall-workflow.pdf}
    \tightcaption{Overview of \name}
    \label{fig:workflow}
    \vspace{-3mm}
\end{figure}

We present \name, a new encoder that achieves local macroblock-level encoding optimization on edge cameras.
As depicted in Figure~\ref{fig:workflow}, the key component of \name is the cheap {\em quality selector}.
\begin{packeditemize}
\item {\em Training the quality selector (\S\ref{sec:training}):}
For a given final DNN, \name offers a routine to train the quality selector for the DNN. 
Users need to provide the final DNN's inference function $\DNN(\HighImage)$, which takes as input an image $\HighImage$ and returns the inference results.
They also need to provide the accuracy function $\SimFunc(x,y)$, which takes an inference output $x$ and the ground truth $y$ as input and calculate the accuracy of $x$ against $y$.
Both $\DNN(\HighImage)$ and $\SimFunc(x,y)$ must be differentiable, but this is already the common case as modern DNN training already requires them to be differentiable.
By default, the quality selector is trained on a sampled subset of images in COCO dataset~\cite{coco} (\S\ref{subsec:??}). 
\item {\em Online encoding (\S\ref{sec:encoding}):}
The trained quality selector is deployed on the edge camera.
\name then feeds each incoming frame to the quality selector to detect the quality-sensitive macroblocks of a given final DNN, and it then applies
% The analyst can use the thresholds of $\AgThresh$ or $\AreaThresh$ ({\footnotesize{\bf \texttt{param}}}) to decide the quality assignment according to \S\ref{subsec:quality-assignment}.
% By setting the parameters, users can select tradeoff between accuracy and compression efficiency (file size). 
%The encoded video will then be saved together with a metafile that includes the quality assignment information.
% \name will then apply 
region-of-interest encoding to encode only these quality-sensitive macroblocks in high quality.
\end{packeditemize}


% To address this difficulty, we present \name, a new video encoder for video analytic applications.
% \name trains a cheap model {\em offline} (hereinafter \AccuracyGradientModel) that determines the quality-sensitive macroblocks based on final DNN and deploy it to the camera side.
% Upon encoding, the camera runs \AccuracyGradientModel to determine which macroblocks should be in high quality and encode the video correspondingly.

% Figure~\ref{fig:workflow} depicts \name's workflow and the three APIs:

% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{ag\_model = prepare(dnn\_func,acc\_func)}}\\
% {\bf \texttt{encoded\_video = ingest(ag\_model,*raw\_frame,param)}}\\
% {\bf \texttt{result = consume(encoded\_video,dnn)}}
% \vspace{0.1cm}
% }






% \mypara{Creating \AccuracyGradientModel}
% At this stage, \name offers an \AccuracyGradientModel pretrained on COCO dataset~\cite{coco} for different analytic tasks. Optionally, the analyst can choose to retrain or customize the \AccuracyGradientModel through three APIs:
% \begin{packeditemize}
%     \item The accuracy function $\SimFunc(x,y)$. This function receives the inference results $x$, the ground truths $y$ and calculate the accuracy of $x$ against $y$ in a differentiable manner. Analyst can choose to use the negative training loss of the final DNN, or implement customized accuracy function.
%     \item The inference function $\DNN(\HighImage)$. This function receives the input $\HighImage$ and generates the corresponding inference results $\DNN(\HighImage)$.
%     \item A dataset iterator $D$. \name will use $D$ as the training set and update $\AccuracyGradientModel$. 
% \end{packeditemize}
% We will further discuss the training details and training cost reduction techniques in \S\ref{sec:training}.
% After training, \name deploys the \AccuracyGradientModel on the camera side and wait for online encoding.


% The analyst provides \name the final DNN with its accuracy function ({\footnotesize{\bf \texttt{acc\_func}}}), and \name trains a customized {\em \AccuracyGradientModel} ({\footnotesize{\bf \texttt{ag\_model}}}), which will predict the \ags on any new frame. 
% %(similarity between DNN outputs on the high-quality frame and on the low-quality encoding)
% %The accuracy function takes DNN's outputs on the high quality encoding and on the low quality encoding of a frame as input, and returns the similarity between them (which indicates accuracy as defined in \S\ref{??}).
% %the accuracy of running the DNN on the encoded frame with respect to the result of running the DNN on the high quality image as the ``ground truth''. 
% Optionally, the operator also provides a dataset to {\em finetune} the \AccuracyGradientModel; otherwise, \name can directly use the pretrain
% We evaluate these choices in \S\ref{subsec:eval:micro}.
% %As elaborated in \S\ref{??}, the choice of training data involves a tradeoff between accuracy-gradient model performance and real-time overhead. 

% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{ag\_model = prepare(dnn\_func,acc\_func)}}
% }

\mypara{Key challenges}
The key is how to make the quality selector fast and easily customized for each given DNN:
\begin{packeditemize}
\item {\em Challenge 1: How to detect the quality-sensitive macroblocks in realtime using only local compute resource of an edge camera?}
In other words, \name's encoding overhead should be on par with only running the video codec.
%    \item How to discover the important pixels in a real-time, fine-grained manner while still being affordable for a cheap camera?
\item {\em Challenge 2: How to quickly customize \name (ideally in a few minutes or less) for any given final DNN?}
What's more, an \name trained for one final DNN should also work decently with another DNN of similar task.
%    \item How to customize \name for any given DNN {\em quickly and automatically}?
\end{packeditemize}



% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{encoded\_video = encode(ag\_model,*frame,param)}}
% }

\begin{comment}
\mypara{On-demand decoding}
Finally, when the user decide to analyze the video, \name decodes the video to frames and then feed them to the final DNN.
%and use the quality assignment information in the metafile to overlay the decoded high quality blocks on the low quality one. 
%The resulting frames are 
% and then feed them to the DNN for inference whenever needed.
%As an further optimization to reduce inference time, the DNN can also use the quality sensitivity information in the metafile to filter out regions that are very unlikely to have useful information (\eg background).

% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{*frame = decode(encoded\_video)}}
% \vspace{0.1cm}
% }

% Though the workflow sketched in Figure~\ref{fig:workflow} is functionally sufficient,
% %to encode videos with spatially different quality based on the notion of accuracy gradients, 
% two challenges remain: 
% (1) how to learn an accurate \AccuracyGradientModel (\S\ref{sec:training}); and (2) how to use it in real time for high accuracy and low encoding/decoding overhead (\S\ref{sec:runtime}).
% We will address them in the next two sections.



\mypara{Challenge} The core challenge of designing \name is: how to find a machine learning problem that achieve high compression efficiency while enabling a series of system optimization?

\end{comment}


\section{Key idea: Accuracy Gradients}

The key idea of \name is the concept of {\em Accuracy Gradients} (\AccuracyGradient).
Intuitively the \AccuracyGradient of a macroblock measures how much the macroblock's encoding quality influences the final DNN's inference accuracy.

Here, we first formally define \AccuracyGradient and how \name uses it, then explain the formulation that leads us to it, and finally explain the rationale behind why \AccuracyGradient enables \name to address the two aforementioned challenges.

\subsection{What \AccuracyGradient?}

We split each $\OriginWidth\cdot\OriginHeight$ frame into $\GridWidth\cdot\GridHeight$ grids of 16x16 blocks ($\OriginWidth=16\GridWidth,\OriginHeight=16\GridHeight$).
Given a frame whose high-quality encoding and low-quality encoding are $\HighImage$ and $\LowImage$ respectively, \AccuracyGradient at the macroblock $x,y$ is defined as:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\AccuracyGradient_{x,y} = \sum_{(i,j)\in block_{x,y}}\bigg\Vert\frac{\partial \SimFunc\big(\DNN(\LowImage), \DNN(\HighImage)\big)}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_1. \label{eq:acc-gradients}
% \bigg\Vert\frac{\partial{\AccuracyFunc\circ \DNN(\textbf{V}), gt)}}{\partial \textbf{V}} \bigg|_{i,j}\bigg\Vert_2 \label{eq:acc-gradients}
\end{align}
}
where $\SimFunc(x, y)$ measures the accuracy of inference results $x$ against ground truth $y$, $\HighImage$ and $\LowImage$ are the high-quality encoding and the low-quality encoding of each frame\footnote{The dimension of a frame is the same for different QP values, so $\HighImage$ and $\LowImage$ have the same dimension.} and $\DNN$ is the inference function of the final DNN.




% \mypara{Why \AccuracyGradient improves accuracy-compression tradeoffs}

\mypara{\AccuracyGradient-based quality selection}
Since calculating the real \AccuracyGradients requires running the final DNN $\DNN$, \name trains a cheap model \AccuracyGradientModel that predicts the \AccuracyGradient per macroblock in a given frame.
Based on \ag matrix of a frame, \name then uses one of two parameters to decide which blocks in a frame should be encoded in high quality: 
\begin{packeditemize}
\item {\em \Ag threshold ($\AgThresh$)} means all blocks $(x,y)$ with $\AccuracyGradient_{x,y}\geq\AgThresh$ will be encoded in high quality.
%\name picks a subset of blocks whose \ags based on Eq (\ref{eq:acc-gradients}) are over $\AgThresh$.
\item {\em High-quality area threshold ($\AreaThresh$)} sets the maximum number of high-quality blocks, by simply picking the top $\AreaThresh$ blocks with the highest \ags.
%\name picks the top $\AreaThresh$ blocks with the highest \ags.
\end{packeditemize} 
After a set of blocks are selected, \name then 
% the block-padding scale $\PadThresh$ to 
expands these selected blocks to each direction by $\PadThresh$ (by default 4) blocks (if they are not already selected). 

% \mypara{Quality selector based on \AccuracyGradient}


\subsection{How \AccuracyGradients navigate accuracy- compression tradeoffs (near-)optimally}

% We will further explain the rationales in \S\fillme.

The above \AccuracyGradient-based quality assignment process in effect approximates the optimal tradeoffs between accuracy and compression. 
To explain the intuition, we consider $\Mask$ as a 0/1-valued binary mask of size $\GridWidth\cdot\GridHeight$ and the following optimization problem, 

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\max_{\Mask} &~~~~\SimFunc\bigg(\DNN \big(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage \big),\DNN(\HighImage)\bigg) \\
s.t.&~~~~ \big\Vert \Mask \big\Vert_1 \leq c
\label{eq:idealized-objective}
\end{align}
}
where $\AllOnes$ refers to a matrix where all the elements are one, $\times$ refer to pixel-wise multiplication\footnote{The multiplication operation here will first resize the left operand back to size $\OriginWidth\cdot\OriginHeight$ and then apply pixel-wise multiplication.}, and $c$ is a positive integer. 
The optimization problem maximizes the accuracy when the macroblock $x,y$ is encoded in high (or low) quality if $\Mask_{x,y}=1$ (or $0$)\footnote{\jc{need a note to explain why there's no extra encoding artifact}}, while no more than $c$ macroblocks are encoded in high quality.

The solution to maximize Equation~\ref{eq:idealized-objective} can be approximated by the solution to minimize $\sum_{x,y}(1-\Mask_{x,y}) \cdot \AccuracyGradient_{x,y}$.\footnote{
Maximizing Equation~\ref{eq:idealized-objective} is equivalent to minimizing 
% (where $\Image=\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage$) is equivalent to the following (note that the first term of Eq~\ref{eq:objective} is a constant to $\Mask$). Thus, the first objective can be rewritten as:

{
\tiny
\vspace{-0.2cm}
\begin{align}
& \SimFunc(\DNN(\AllOnes\times\HighImage), \DNN(\HighImage))-\SimFunc(\DNN(\Image), \DNN(\HighImage)) 
= \bigg\langle\frac{\partial \SimFunc(\DNN(\Image'), \DNN(\HighImage))}{\partial \Image'},(\AllOnes\times\HighImage - \Image)\bigg \rangle_{\textrm{F}}  \nonumber\\
\approx & \bigg\langle\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage},(\AllOnes\times\HighImage - \Image)\bigg\rangle_{\textrm{F}}
= \bigg\langle\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage},(\AllOnes-\Mask)\times(\HighImage-\LowImage)\bigg\rangle_{\textrm{F}}, \nonumber
\end{align}
}
where $\Image=\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage$, $\langle\cdot,\cdot\rangle_{\textrm{F}}$ is the Frobenius inner product. 
The first transition uses Lagrange's Mean Value Theorem, where $\Image'$ lies between $\HighImage$ and $\Image$. 
Since the values in each macroblock of $\Mask$ are identical, the last term can be rewritten as the sum of the following over all macroblocks:
% In Equation (\ref{eq:temp}), since the value of $\Mask$ is identical inside each block, each block $(x,y)$ contributes the following value to Eq (\ref{eq:temp}):

{\tiny
\vspace{-0.2cm}
\begin{align}
& (1-\Mask_{x,y})\bigg\langle\sum_{(i,j)\in block_{x,y}} \frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}, (\HighImage_{i,j}-\LowImage_{i,j})\bigg\rangle_{\textrm{F}}\nonumber\\
\leq & \delta \cdot (1-\Mask_{x,y}) \cdot \sum_{(i,j)\in block_{x,y}} \bigg\Vert\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_1 \nonumber
= \delta \cdot (1-\Mask_{x,y}) \cdot \AccuracyGradient_{x,y}. \nonumber
\label{eq:temp3}
\end{align}
}
where $\delta$ denotes the maximum absolute value in $\HighImage_{i,j}-\LowImage_{i,j}$.
}
Intuitively, if at most $c$ macroblocks should be encoded in high quality, it should be the macroblocks with the highest $\AccuracyGradient_{x,y}$.
Therefore, $\AgThresh$ and $\AreaThresh$ allow users to navigate the near-optimal accuracy-compression tradeoffs: 
% lower $\AgThresh$ or higher $\AreaThresh$ increases the accuracy at the expense of encoding more blocks.
lowering $\AgThresh$ or raising $\AreaThresh$ encodes more macroblocks but these macroblocks are the ones that likely lead to the most improvement in accuracy.


We also note that $\AgThresh$ and $\AreaThresh$ have different practical implications.\footnote{At a high level, the effects of $\AgThresh$ and $\AreaThresh$ in \name are analogous to variable bitrate (VBR) and constant bitrate (CBR) encoding (one adapts to content and one maintains constant bitrate).
We will demonstrate how they can help adaptive streaming in \S\ref{subsec:eval:adaptive}.
That said, we will explore for future work how to use $\AgThresh$ and $\AreaThresh$ to precisely control the accuracy or bitrate.}
\begin{packeditemize}
\item When the \ag threshold $\AgThresh$ is set to a fixed value, \name will assign high quality to {\em all} low \ag macroblocks.
In effect, it {\em adapts the compression rate to content}, \eg when content is simple, it will compress more aggressively.
\item When the high-quality area threshold $\AreaThresh$ is set to a fixed value, \name will assign high quality to a {\em fixed} number of macroblocks.
As a result, it {\em adapts the accuracy to a target compression rate}.
\end{packeditemize} 


\begin{comment}

Let us use $\AccuracyGradientModel$ as the input a high quality image $\HighImage$ and returns as output a $[0,1]$-valued mask of size $\GridWidth\cdot\GridHeight$, $\Mask=\AccuracyGradientModel(\HighImage)$. 
The element inside the mask $\Mask_{x,y}=1$ means block $x,y$ is completely in high quality and $\Model(\Mask_{x,y})=0$ means block $x,y$ is completely in low quality.
Then the optimization goal is to maximize accuracy with less elements of $\Mask$ being 1: 

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\max_{\AccuracyGradientModel} &~~~~\SimFunc\bigg(\DNN \big(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage \big),\DNN(\HighImage)\bigg) - \lambda  \frac{\big\Vert \Mask \big\Vert_1}{numel \big(\Mask\big)}
\label{eq:idealized-objective}
\end{align}
}
where $\AllOnes$ refers to a matrix where all the elements are one, $\times$ refer to pixel-wise multiplication\footnote{The multiplication operation here will first resize the left operand back to size $\OriginWidth\cdot\OriginHeight$ and then apply pixel-wise multiplication.}, $\big\Vert \Mask \big\Vert_1 / {numel \big(\Mask\big)}$ counts percentage of macroblocks inside $\Mask$ encoded in high quality and $\lambda$ navigates the trade-off between accuracy and percentage of macroblocks in high quality.
We will elaborate how \AccuracyGradients optimize Equation~\ref{eq:idealized-objective} in \S\ref{subsec:bandwidth-adaptation}.
% (we will specify how we navigate this trade-off in \S\ref{subsec:bandwidth-adaptation}).




\subsection{Key enabler: accuracy gradients}


\mypara{Formulation} We first formulate quality assignment problem into an optimization problem.
To make the discussion more concrete, we split each $\OriginWidth\cdot\OriginHeight$ frame into $\GridWidth\cdot\GridHeight$ grids of 16x16 blocks ($\OriginWidth=16\GridWidth,\OriginHeight=16\GridHeight$) and assign each block either a high quality or a low quality. % (this aligns with previous work~\cite{eaar,dds}).
Our goal is to find a model $\AccuracyGradientModel$ that generates a $[0,1]$-valued mask of size $\GridWidth\cdot\GridHeight$ by feeding the high quality image $\HighImage$ into $\AccuracyGradientModel$, \ie $\Mask=\AccuracyGradientModel(\HighImage)$, where the element inside the mask $\Mask_{x,y}=1$ means block $x,y$ is completely in high quality and $\Model(\Mask_{x,y}=0$ means block $x,y$ is completely in low quality. The optimization goal is to minimize the number of blocks in high quality as well as maximize the inference accuracy\footnote{This formulation involves two simplifying assumptions: the 16x16 blocks may be suboptimal boundaries between quality levels, and it restricts the encoding to only two quality levels.
That being said, we believe that analyzing this formulation is still valuable for two reasons.
First, the block granularity of 16x16 is on par with the block sizes employed in H.264 and H.265, which means more fine-grained blocks will not have much impact on the encoded video size. 
Second, the use of two quality levels does subsume many recent solutions (\eg~\cite{vigil, dds, awstream, glimpse, reducto}) which use two or fewer quality levels.}:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\max_{\AccuracyGradientModel} &~~~~\SimFunc\bigg(\DNN \big(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage \big),\DNN(\HighImage)\bigg) - \lambda  \frac{\big\Vert \Mask \big) \big\Vert_1}{numel \big(\Mask\big)}
\label{eq:idealized-objective}
\end{align}
}
where $\SimFunc(x, y)$ measures the accuracy of inference results $x$ against ground truth $y$, $\HighImage$ and $\LowImage$ are the high-quality encoding and the low-quality encoding of each frame\footnote{The dimension of a frame is the same for different QP values, so $\HighImage$ and $\LowImage$ have the same dimension.}, $\AllOnes$ refers to a matrix where all the elements are one, $\times$ refer to pixel-wise multiplication\footnote{The multiplication operation here will actually resize the left operand back to size $\OriginWidth\cdot\OriginHeight$ and then apply pixel-wise multiplication.}, $\DNN$ is the server-side DNN that generates the DNN inference result, $\big\Vert \Mask \big\Vert_1 / {numel \big(\Mask\big)}$ counts percentage of macroblocks inside $\Mask$ encoded in high quality and $\lambda$ navigates the trade-off between accuracy and percentage of macroblocks in high quality (we will specify how we navigate this trade-off in \S\ref{subsec:bandwidth-adaptation}).


\mypara{Accuracy gradients} To efficiently solve the problem above, we develop a novel concept called accuracy gradient (\AccuracyGradient in short), defined as:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\AccuracyGradient_{x,y} = \sum_{(i,j)\in block_{x,y}}\bigg\Vert\frac{\partial \SimFunc\big(\DNN(\LowImage), \DNN(\HighImage)\big)}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_1. \label{eq:acc-gradients}
% \bigg\Vert\frac{\partial{\AccuracyFunc\circ \DNN(\textbf{V}), gt)}}{\partial \textbf{V}} \bigg|_{i,j}\bigg\Vert_2 \label{eq:acc-gradients}
\end{align}
}
\kt{I rewrite the formulation here to enable the half splitting trick }Based on this concept, in order to maximize Equation~\ref{eq:idealized-objective}, we only need to let our \AccuracyGradientModel learns \AccuracyGradient (we will show the connection between Equation~\ref{eq:idealized-objective} and \ref{eq:acc-gradients} in \S\fillme)












\subsection{\Ag-based quality assignment}
\label{subsec:quality-assignment}

Given the matrix of \ags of a frame, \name then uses one of two parameters to decide which blocks in a frame should be encoded in high quality: 
\begin{packeditemize}
\item {\em \Ag threshold $\AgThresh$} means all blocks $(x,y)$ with $\AccuracyGradient_{x,y}\geq\AgThresh$ will be encoded in high quality.
%\name picks a subset of blocks whose \ags based on Eq (\ref{eq:acc-gradients}) are over $\AgThresh$.
\item {\em High-quality area threshold $\AreaThresh$} sets the maximum number of high-quality blocks, by simply picking the top $\AreaThresh$ blocks with the highest \ags.
%\name picks the top $\AreaThresh$ blocks with the highest \ags.
\end{packeditemize} 
After a set of blocks are selected, \name then 
% the block-padding scale $\PadThresh$ to 
expands these selected blocks to each direction by $\PadThresh$ (by default 4) blocks (if they are not already selected). We will further explain the rationales in \S\fillme.

Both $\AgThresh$ and $\AreaThresh$ allow users to navigate \name's accuracy-compression tradeoffs (lower $\AgThresh$ or higher $\AreaThresh$ increases the accuracy at the expense of encoding more blocks).
However, they have very different practical implications.
\begin{packeditemize}
\item When the \ag threshold $\AgThresh$ is set to a fixed value, \name will assign high quality to {\em all} low \ag blocks.
In effect, it {\em adapts the compression rate to content}, \eg when content is simple, it will compress more aggressively.
\item When the high-quality area threshold $\AreaThresh$ is set to a fixed value, \name will assign high quality to a {\em fixed} number of blocks.
As a result, it {\em adapts the accuracy to a target compression rate}.
\end{packeditemize} 
At a high level, the effects of $\AgThresh$ and $\AreaThresh$ in \name are analogous to variable bitrate (VBR) and constant bitrate (CBR) encoding (one adapts to content and one maintains constant bitrate).
However, we acknowledge that $\AgThresh$ and $\AreaThresh$ in our design do not directly tie to a target accuracy or fixed bitrate, which we will discuss in \S\ref{sec:discuss}.
Nonetheless, we will demonstrate how they can help adaptive streaming in \S\ref{subsec:eval:adaptive}.

%while minimizing compressed video size. 
%In contrast, the high-quality area threshold $\AreaThresh$ can be used to {\em control compressed video size} while maximizing accuracy. 

%\jc{can't control directy, but effective}

% In practice, we found tuning them result in a similar frontier of accuracy/compression tradeoffs, so we expose $\AgThresh$ as a tunable parameter to users (just as QP in MPEG/H.264) and empirically set $\PadThresh$ at 2 by default.


%it is straightforward to derive the optimal quality assignment on the given frame.
%\jc{Kuntai, please give the derivation}
%Recall that only $c$-many blocks will be encoded in high quality, we just need to pick $c$-many blocks with largest accuracy gradient value, encode them in high quality and encode remaining blocks in low quality.



















\subsection{Design rationales}


\end{comment}




\subsection{Rationales of \AccuracyGradient and \AccuracyGradientModel}
\label{subsec:rationales}


While \AccuracyGradient is computer-vision concept, it is the key to addressing the two challenges (\S\ref{sec:overview}) of \name by allowing \AccuracyGradientModel to be cheap and trained quickly.

\mypara{Why \AccuracyGradientModel can be cheap} 
% A natural question is that why a cheap \AccuracyGradientModel exists. This is because learning \AccuracyGradient has three properties that makes it much easier than traditional server-side DNN tasks like semantic segmentation:
A cheap \AccuracyGradientModel can be learned due to three reasons that make it easier to learn than semantic segmentation, a typical computer-vision task:
\begin{packeditemize}
    \item {\em Small output space:} %\kt{I name it to small output space cuz coarse granularity sounds like we are not doing fine-grained encoding}
    \AccuracyGradientModel returns one label per macroblock (all pixels in a 16x16 macroblock share the same DNN output). 
    The benefit is that, in contrast to traditional convolutional operations which scan the image pixel by pixel, \AccuracyGradientModel logically only needs to scan the image macroblock by macroblock (which has a compute saving of upto 256x on convolutional operations).
    Moreover, compared to the common multi-class segmentation tasks, the task of \AccuracyGradientModel is essentially {\em binary} classification (classifying each macroblock as high quality or low quality), which further reduces the complexity of \AccuracyGradientModel. 
    {\em  This property also enables us to reduce the cost of \AccuracyGradientModel.} (More details in \S\ref{subsec:architecture}).
    % So we can let these pixels generate {\em one} feature, and then apply future compute to this one feature to get the output of this 16x16 macroblock. Ideally, this means that we can save {\em 256x} compute cost compared to traditional segmentation task.
%   {\em  This property also enables us to reduce the cost of \AccuracyGradientModel.} 
    % \item {\em Binary segmentation:} Quality assignment task is essentially a binary classification (classifying each macroblock as high quality or low quality), while traditional semantic segmentation is multi-class classification (classify each pixel to a class label). The former is easier than the latter. This wisdom is also used by other works ~\cite{dds}. 
    \item {\em Boundary expansion tolerance:}
    While accurate image segmentation must return precise boundaries along objects, our formulation~\ref{eq:idealized-objective} relaxes this constraints. 
    Slightly expanding the high-quality regions has little impact on the accuracy of the final DNN, though the compressed file size will slightly increase\footnote{Due to intra-frame encoding in modern codecs, the compressed video size grows sublinearly with more high-quality regions, which is favorable to \name.}.
    {\em This property enables us to inference on \AccuracyGradient less frequently.} (More details in \S\fillme.)
    % One of the central challenge of image segmentation task is to accuracy sketch the object boundary~\cite{crf}. 
    % However, our formulation~\ref{eq:idealized-objective} makes this less of an issue.
    % This is because our formulation permits \AccuracyGradientModel to slightly expand the object boundary\footnote{Expanding the object boundary will only make the percentage of high pixels (i.e. $\big\Vert \Mask \big\Vert_1 / {numel \big(\Mask\big)}$) marginally larger, and thus have little impact on the value of overall objective~\ref{eq:idealized-objective}.} to make the object boundary much smoother and easier to learn.
    % However, when maxmizing Equation~\ref{eq:idealized-objective}, we can encode some extra blocks into high quality as long as those important microblocks that might hurt accuracy if compressed can be segmented out. So when it comes to a microblock that the DNN is not sure whether it is on the boundary or not, the DNN can safely put this microblock in high quality.
    % \item False positive tolerance. Also, as long as the important microblocks are segmented out to make the accuracy high, it is OK to segment out some other microblocks since they will only cause little bit of extra file size. Accordingly, when it comes to a microblock that the DNN is not sure whether it is part of the object or not, it can safely put this microblock in high quality.
\end{packeditemize}


These observations suggest that a shallow NN is enough for \AccuracyGradientModel. 
% to exploit the opportunity behind the optimization objective~\ref{eq:idealized-objective} and thus have a preferable file size-accuracy trade-off.
This is empirically validated in Figure~\ref{fig:architecture-loss} which shows cheap \AccuracyGradientModel can predict \AccuracyGradients almost as accurately as a much more expensive one
(see \S\ref{subsec:architecture}).
% support that a cheap model can already have similar performance compared to the compute-intensive models in \S\ref{subsec:architecture}







\mypara{Why training \AccuracyGradientModel can be fast}
Training a \AccuracyGradientModel that optimizes Equation~\ref{eq:idealized-objective} can be prohibitively expensive for two reasons:
(1) it requires running numerous forward/backward propagations on the end-to-end pipeline of $\DNN$, $\AccuracyGradientModel$, and $\AccuracyFunc$, and (2) similar training typically requires a large set of images~\cite{??,??}. 
% Directly training through objective~\ref{eq:idealized-objective} can be expensive.
% This is because this formulation requires passing through the heavy server-side DNN {\em in every training epoch}.
Fortunately, \AccuracyGradient can be directly derived from the final DNN $\DNN$ (Equation~\ref{eq:acc-gradients}) using one forward-backward propagation. 
This allows us to separate the compute-intensive $\DNN$ from the end-to-end training and instead focus the computation on training of \AccuracyGradientModel.
% By leveraging the \AccuracyGradient to train \AccuracyGradientModel, however, we only need to access the server-side DNN {before} training starts to generate ground truths.
% The afterward training process of \AccuracyGradientModel is then completely irrelevant to server-side DNNs.
Empirically, this can save about {\em 15x} overhead on accessing the heavy server-side DNNs since the \AccuracyGradientModel typically takes 15 training epochs to converge (see Figure~\ref{fig:architecture-loss} for the convergence speed).








% Thus, the overall training overhead of \AccuracyGradientModel is minor. We will further develop training cost reduction technique in \S\ref{sec:training}.




==> overview.tex <==

\section{A video stack framework for video analytics}

\subsection{Design space}

\kt{
\begin{itemize}
\item injection: to achieve dnn-awareness, heavy processing, low-quality stream, or cheap model? 
\item codec: use existing mpeg or autocodec or some intermediate feature? 
\item execution: complete frame decoding? temporal batching? spatial batch?
\item \name chooses ``cheap model + mpeg + spatial batching''
\item why is it better than baselines (nn-based codec, SR, autocodec, dds)
\end{itemize}}

A video stack consist of three phases: offline preparation, online injection and on-demand consumption.

\begin{packeditemize}
    \item Traditional codec with vision applications as filter. Most of this kind of works~\cite{dds,vigil,glimpse,eaar} use vision application to feed areas critical to DNN inference to codec, and others~\cite{awstream,vstore} use vision application to filter out the sub-optimal configuration of the codec.
    \item Super resolution. CloudSeg~\cite{cloudseg} and LiveNAS~\cite{livenas} send a low quality video first and forward the video to a super resolution network to recover the video quality.
    \item Auto encoder. Instead of using traditional video codec, recent works from computer vision community~\cite{rate-distortion-autoencoder} start to use DNN as encoder and decoder to encode the video.
\end{packeditemize}






\subsection{Accuracy decomposition on video analytic system}
\kt{
\begin{itemize}
\item definition of accuracy gradient 
\begin{itemize}
\item why is it what we want
\item how could it be used to improve injection and consumption
\item why is it generic
\end{itemize}
\item an example
\item difference to conceptions (like attention) in vision
\end{itemize}
}

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/attn-acc.pdf}
    \caption{Contrasting accuracy gradient and attention mechanism. Attention mechanism might highlight those pixels that may of interest but do not contribute to the inference results.}
    \label{fig:attn-acc}
\end{figure}

\mypara{Formulation}
The overall goal of a video analytic system is to maximize the accuracy of the inference result:
\begin{equation}
Acc(G(\textbf{V}))
\label{eq:goal}
\end{equation}
where $\textbf{V}$ is the video forwarded to the DNN by the video analytic system, $Acc$ is the accuracy function, the higher the better, $G$ is the server-side DNN application and $\textbf{V}$ is the compressed video.

The inference result on high quality image are of a fixed accuracy, which means
$$
Acc(G(\textbf{high}))
$$
is a constant, where $\textbf{high}$ is the video generated under unlimited cost (\textit{i.e.} the highest quality video).

Thus, maximizing the overall accuracy
$$
Acc(G(\textbf{V}))
$$
is equivalent to minimizing the constant minus the overall accuracy:
$$
Acc(G(\textbf{high})) - Acc(G(\textbf{V})).
$$
% For simplicity, let
% $$
% f(\textbf{V}) = Acc(G(\textbf{V}), gt),
% $$
% So we are maximizing
% $$
% f(\textbf{high}) - f(\textbf{V}).
% $$
The neural network $G$ is differentiable. Assume that $Acc$ is differentiable, according to Lagrange mean value theorem, we have
$$
Acc(G(\textbf{high})) - Acc(G(\textbf{V})) = \sum(Acc\circ G)'(\textbf{X})\times(\textbf{high}-\textbf{V}),
$$
where $\sum$ means summing up all the elements in a matrix, $(Acc\circ G)'$ is the derivative of the function composition of $Acc$ and $G$, $\textbf{X}$ is a value lies between $\textbf{high}$ and $\textbf{V}$, and $\times$ is element-wise multiplication between matrices.

Now we approximate $f'(\textbf{X})$ by $f'(\textbf{high})$. We have
$$
f(\textbf{high}) - f(\textbf{V}) \approx \sum(f'(\textbf{high})\times(\textbf{high}-\textbf{V})).
$$
So maximizing the overall accuracy can be approximated by minimizing
$$
\sum(f'(\textbf{high})\times(\textbf{high}-\textbf{V})).
$$
Inside the sum above, each pixel $(i, j)$ will contribute
$$
f'(\textbf{high})_{i,j} \times (\textbf{high}_{i,j} - \textbf{V}_{i,j}).
$$
Now we assume that compress the video will always hurt the accuracy, which means
$$
f'(\textbf{high})_{i,j} \times (\textbf{high}_{i,j} - \textbf{V}_{i,j}) < 0.
$$
So we see, to maximize overall accuracy, pixel change 
$$|\textbf{high}_{i,j} - \textbf{V}_{i,j}|$$ 
should be small when the corresponding gradient  
$$|f'(\textbf{high})_{i,j}|$$ is large.

\mypara{Takeaway} Maximizing overall accuracy of a video analytic system can be approximated by minimizing the product of \textbf{accuracy gradient}
$$
\bigg\Vert\frac{\partial{Acc(G(\textbf{V}), gt)}}{\partial \textbf{V}} \bigg|_{i,j}\bigg\Vert_2
$$
and \textbf{\textbf{pixel change}} between high quality video and compressed video
$$
|\textbf{high}_{i,j} - \textbf{V}_{i,j}|
$$
at each pixel. Pixel change should be small when accuracy gradient is large.

\mypara{Accuracy gradient versus attention mechanism}
More and more DNN-based vision algorithms leverage attention mechanism\cite{??,??} for efficiency and effectiveness.
Attention mechanism focuses on where to spend more \textit{compute resource} to \textit{prevent accuracy loss} \textit{inside} the neural network.
Thus, pixels that are likely to resemble an object \textit{but not} will not be highlighted by 
As shown in Figure \ref{fig:attn-acc}, a muffin that looks like a dog may wrongfully highlighted by attention mechanism but won't be highlighted by accuracy gradient.


\mypara{Accuracy gradient versus region proposal}
Recent works~\cite{dds,eaar} leverages region proposal to seek for regions that potentially contain objects. 
However, region proposal will produce \textit{all} regions that may contain objects, including those regions that may contain objects that are not of interest.
In contrast, those objects that are not of interest will not contribute to accuracy calculation. Thus, the accuracy gradient of those objects will be 0.

\mypara{Accuracy gradient versus saliency}


\subsection{Instantiate accuracy gradient in \name}

In \name, we use two qualities to encode the video.

$$
\frac{
    \partial Acc(
        G(
            \textbf{high}\times \textbf{M}
            +
            \textbf{low}\times (\textbf{1}-\textbf{M}))
        ),
        G(\textbf{high})
    )
}{
    \partial \textbf{M}
}\bigg|_{\textbf{M}=\textbf{0}}
$$

The meaning of the notations above is:
\begin{packeditemize}
    \item $Acc(x, target):$ A differentiable function that can measure the accuracy of certain inference result $x$ to a given target $target$.
    \item $\textbf{1}:$ a all-1 matrix.
    \item $\textbf{0}:$ a all-0 matrix.
    \item $G(\textbf{x}):$ The server-side DNN model that generates inference results from the video $\textbf{x}$.
    \item $\textbf{high}:$ The high-quality version of the video.
    \item $\textbf{low}:$ The low-quality version of the video.
    \item $\textbf{M}:$ The mask that linearly combines low-quality video $\textbf{low}$ and high-quality video $\textbf{high}$ at each pixel. For that pixel $p$, $M_p=0$ will let that pixel be in low-quality, and $M_p=1$ in high quality.
    \item $gen:$ Generate final analytic results from inference results. For example, in object detection, we need to attach class label to the object and discard this object with low confidence score.
\end{packeditemize}

Moreover, to get the accuracy gradient for each 16$\times$16 block, we sum up the gradient of the pixel value for each pixel inside the block.

\mypara{Why accuracy gradient better} 
The expression answers that standing at the low-quality video, what is the \textit{accuracy-wise optimal} direction of which pixel should we encode in high quality. 
This formulation exploits the following opportunity that no previous works have been explored:
\begin{packeditemize}
    \item Not all pixels on the object require high quality. For example, there is no need to encode those pixels on object that do not change too much if encoded in high quality.
    \item Pixels near the object may also require high quality. \kt{example}
    \item When we cannot encode every pixel in high quality, which pixels should we focus on first. \kt{example of encoding a small object first cuz it has high accuracy gradient.}
\end{packeditemize}

\blindtext

\mypara{Generalizability of accuracy gradient}
The formulation above is agnostic to DNN architecture (versus DDS~\cite{dds} and EAAR~\cite{eaar} that assume the existence of region proposal network) and application (versus the object detection assumption in Vigil~\cite{vigil} and the classification assumption in Focus~\cite{focus}) in the formulation of accuracy gradient. This makes the formulation above generalizable and clean.

\mypara{Difference between attention mechanism} Attention mechanism [\fillme] is a kind of mechanism that entails which area requires more \textbf{compute}. Typically, attention can coarsely crop out the position and the boundary of the object, but it is completely agnostic to encoding and unaware of accuracy.

\subsection{Workflow and API of \name}

\mypara{Offline preparation}
During offline preparation, \name trains a cheap neural network on the same training set of the analytic model to calculate the accuracy gradient per block. To train this neural network, the API for developer is:
\begin{itemize}
    \item Training set of the original model.
    \item Training loss. We use this loss as a differentiable accuracy measurement to derive accuracy gradient.
\end{itemize}

\mypara{Online injection}
During online injection, \name takes the video as the input and generate the compressed video by using traditional codec to encode only quality-sensitive blocks. In this part, the API for developer is:
\begin{packeditemize}
    \item The video to compress.
    \item Desired compression codec.
\end{packeditemize}

% \subsection{API of \name}

% \kt{
% \begin{itemize}
% \item \name is a shim layer between mpeg and dnn.
% \item Preparation api:
% \item injection api: 
% \item consumption api:
% \item example of object detection on a video stream (vs. traditional ffmpeg)
% \end{itemize}}

% \name is a layer lies between traditional video codec (e.g. H.264) and DNN. It 

%\subsection{Why existing solutions are insufficient}
%\begin{itemize}
%\item neural network for video codec
%\item super resolution
%\item autocodec
%\item dds
%\end{itemize}

%\blindtext

==> related.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\section{Related work}
\label{sec:related}

\mypara{Video analytics pipelines}
There is an extensive literature on video analytics pipelines that try to balance analytics cost and DNN inference accuracy. 
Some discard frames before they are saved or analyzed~\cite{glimpse,reducto,fvc,filterforward}, and \name as a video stack is complementary to these frame-discarding heuristics. 
The most relevant to \name are those that encode videos in an analytics-aware fashion.
However, they either use uniform quality across consecutive frames~\cite{awstream,videostorm,chameleon,vstore} or only differentiate quality based on the regions of objects~\cite{vigil,dds,eaar}, which we have shown suboptimal when objects are relatively small and reducing bandwidth usage when the objects are quite large.
In contrast, \name uses a different primitive which identifies the sensitivity of accuracy to the quality level at each part of a video, thereby directly linking the encoding optimization with inference accuracy.


\jc{emphasize on model agnostic}

\jc{mentione video streaming!}

\mypara{Video encoding}
We share the general goal of improving video compression efficiency with the decades-long literature on video encoding and streaming. 
Recent work in video encoding also leverages the effectiveness of deep learning by training DNN-based autoencoders (\eg~\cite{theis2017lossy,cae,rate-distortion-autoencoder}) that generate ever more realistic looking frames with less encoded bits.
While most work focuses on optimizing human perception measured by SSIM or PSNR, a growing body of work also develops learning-based encoders that optimize the accuracy of computer vision tasks (\eg~\cite{hu2020towards,haris2018task}).
That said, unlike \name, minimizing the encoding delay is not one of the primary goals of these techniques.
% In this sense, they are orthogonal to \name, which optimizes compression efficiency for video analytics.


\mypara{Video management systems}
% \name is related to systems and database literature on efficient video processing pipelines that store and analyze videos for various vision/video applications.
The systems/database communities also developed video-based query execution frameworks to reduce the video inference delay and storage size, via better indexing and more efficient execution of queries (\eg~\cite{focus,noscope,scanner}).
In this sense, their optimizations are complementary to this work: \name provides a lower-level video stack on which videos can be efficiently stored/streamed and the frames picked by a query can be quickly decoded and analyzed.


% \mypara{Attention mechanism}
% Lastly, the notion of calculating the gradients of DNN inference results is not new and has been used to understand DNN inference and improve DNN inference accuracy.
% As mentioned in \S\ref{??}, our notion of accuracy gradients differ in several key aspects. \jc{Kuntai, please elaborate}


%\jc{cite pku work}

==> technical-backup.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{\hspace{-0.2cm}Towards a new video stack for video analytics}
\label{sec:framework}

The previous section shows a substantial room for improvement by allocating quality level based on how much impact each fine-grained region has on the final DNN inference. 
A natural question then is how to build a concrete system to realize the benefits.
In this section, we begin with an optimization framework for such a video stack  and introduce the key ideas behind our design. 


% \tightsubsection{\hspace{-0.2cm}Framework for optimal quality assignment}

\subsection{Accuracy gradients}
\label{subsec:ag}

The idealized algorithm introduced in \S\ref{subsec:idealized} requires running the final DNN multiple times on different encoded videos. 
To make it practical, one needs to determine the quality assignment without running the DNN; instead, it needs to ``derive'' the quality assignment per frame from the pixels of each frame. 

%Formally, this problem can be framed in the following optimization problem.
%\jc{kuntai, please fill the formulation in here. please start from the formula of the idealized design point}
\mypara{Optimization framework}
To do so, we first rewrite the objective of the idealized algorithm in Eq (\ref{eq:idealized-objective}) (let $\Image=\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage,$ be the optimal solution) to minimizing the following value (the first term is independent on $\Mask$):
{\small
\begin{align}
& \SimFunc(\DNN(\AllOnes\times\HighImage), \DNN(\HighImage))-\SimFunc(\DNN(\Image), \DNN(\HighImage)) \label{eq:objective}\\
= & \bigg\langle\frac{\partial \SimFunc(\DNN(\Image'), \DNN(\HighImage))}{\partial \Image'},(\AllOnes\times\HighImage - \Image)\bigg \rangle_{\textrm{F}} \label{eq:lagrange}\\
\approx & \bigg\langle\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage},(\AllOnes\times\HighImage - \Image)\bigg\rangle_{\textrm{F}} \nonumber \\
= & \bigg\langle\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage},(\AllOnes-\Mask)\times(\HighImage-\LowImage)\bigg\rangle_{\textrm{F}}, \label{eq:temp}
\end{align}
}
where $\langle\cdot,\cdot\rangle_{\textrm{F}}$ is the Frobenius inner product. 
Here, Eq (\ref{eq:lagrange}) uses Lagrange mean value theorem, and $\Image'$ lies between $\HighImage$ and $\Image$. In Equation (\ref{eq:temp}), since the value of $\Mask$ is identical inside each block, each block $(x,y)$ contributes the following value to Eq (\ref{eq:temp}):
{\small
\begin{align}
& (1-\Mask_{x,y})\bigg\langle\sum_{(i,j)\in block_{x,y}} \frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}, (\HighImage_{i,j}-\LowImage_{i,j})\bigg\rangle_{\textrm{F}}\nonumber\\
\leq & \delta \cdot (1-\Mask_{x,y}) \cdot \sum_{(i,j)\in block_{x,y}} \bigg\Vert\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_2, \label{eq:temp3}
\end{align}
}
where $\delta$ denotes the maximum element in $\HighImage_{i,j}-\LowImage_{i,j}$.
This upper bound holds when the gradient of $\SimFunc(\DNN(\Image), \DNN(\HighImage))$ at $\Image$ is non-negative all pixels in the block, which is a reasonable assumption since changing pixel values closer to the high quality encoding will likely make the inference result more similar to $\DNN(\Image)$.
% Now we assume lowering the encoding quality at every pixel will always lower the accuracy, thus Equation (\ref{eq:temp2}) is bounded by:
% \begin{align}
% &(1-\Mask_{x,y}) \nonumber\\
% \times&\bigg(\sum_{(i,j)\in block_{x,y}} \bigg\Vert\frac{\partial \SimFunc(\DNN(\Image), \DNN(\HighImage))}{\partial \Image}\bigg|_{i,j}\bigg\Vert_2\bigg) \nonumber\\
% \times& \bigg(\sum_{(i,j)\in block_{x,y}}\big\Vert\HighImage_{i,j}-\LowImage_{i,j}\big\Vert_2\bigg)
% \label{eq:temp3}
% \end{align}


\mypara{Accuracy gradient and its rationale} 
From Eq (\ref{eq:temp3}), we can see that the key to approximating the optimal solution is knowing the following value, which we call {\em accuracy gradients} or {\em \ag}, at each block $(x,y)$:
{\small
\begin{align}
\AccuracyGradient(\LowImage)_{x,y} = \sum_{(i,j)\in block_{x,y}}\bigg\Vert\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_2 \label{eq:acc-gradients}
% \bigg\Vert\frac{\partial{\AccuracyFunc\circ \DNN(\textbf{V}), gt)}}{\partial \textbf{V}} \bigg|_{i,j}\bigg\Vert_2 \label{eq:acc-gradients}
\end{align}
}
% which is essentially the gradients of the accuracy evaluation function at the point of specific encoding $\Image$. 
%Given its importance, we call it the {\em accuracy gradients} or {\em \ag}.
%Since the calculation of \ag in Eq (\ref{eq:acc-gradients}) still runs the DNN inference on the frame, 
In \S\ref{sec:training}, we will train a light-weight NN model to infer the \ag value per block.
% \jc{question: is the accuracy gradient matrix same size of the grids or the image?}
The rationale of \ags is three-fold.
\begin{packeditemize}
\item \Ags naturally indicate which block should be in high quality. 
Intuitively, if a block $(x,y)$ has a high value $\AccuracyGradient(\LowImage)_{x,y}$, then in order to minimize Eq (\ref{eq:objective}), $\Mask_{x,y}$ should be set to 0.
%The quality assignments based on the accuracy gradients preserve similar performance improvement as the idealized algorithm in \S\ref{subsec:idealized}. 
%Figure~\ref{??} shows the quality assignment based on the idealized algorithm and the assignment based on accuracy gradients. 
%We can see that in both assignments, \fillme
%\jc{maybe a visualization?}
\item \ag is amenable to inference. Ideally, we want to directly infer the binary masks returned by the idealized algorithm. 
However, these masks can flip between 0 and 1 frequently across neighboring blocks, making it hard to infer at times. 
%The idealized algorithm can sometimes be very sensitive to \fillme, which gives rise to the quality assignment that changes frequently even between neighboring blocks, which can be prohibitively difficult to train the accuracy-gradient model on.
In contrast, we empirically found that the \ag matrix is relatively ``smoother'' and thus easier to approximate with a small model as we will see in the next section.
\item \ag may appear similar to the popular notion of saliency map in the computer vision. 
While they generally look for regions with more influence on the DNN output, \ags indicate the how much increasing each block's quality brings the DNN output closer to the DNN output on the high quality encoding, which is exactly what we want.
%\item In addition, assigning quality by blocks still aligns with the (microblocks) used in classic codecs (H.264/265).
%\jc{why not pixel level? our blocks align with the basic spatial units (microblocks) used in classic codecs like H.264/265.}
\end{packeditemize}


\subsection{Quality assignment}
\label{subsec:quality-assignment}

Once the \ag matrix of a frame is known, \name then uses one of two parameters to decide which blocks should be in high quality in the frame: 
\begin{packeditemize}
\item {\em \Ag threshold $\AgThresh$:} \name picks a subset of blocks whose \ags based on Eq (\ref{eq:acc-gradients}) are over $\AgThresh$.
\item {\em High-quality area threshold $\AreaThresh$:} \name picks the top $\AreaThresh$ blocks with the highest \ags.
\end{packeditemize} 
After a set of blocks are selected, \name then 
% the block-padding scale $\PadThresh$ to 
expands these selected blocks to each direction by $\PadThresh$ (by default 2) blocks (if they are not already selected).

Both $\AgThresh$ and $\AreaThresh$ can control the tradeoffs between inference accuracy and compression efficiency: lower $\AgThresh$ or higher $\AreaThresh$ increases the accuracy at the expense of potentially encoding more blocks.
But they have different practical implications.
On one hand, when the \ag threshold $\AgThresh$ is set to a fixed value, \name will assign high quality to {\em all} high \ag blocks.
Consequently, the system will {\em adapt the compression rate to content}: when content is simple, it will compress more aggressively.
On the other hand, when the high-quality area threshold $\AreaThresh$ is set to a fixed value, \name will assign high quality to a {\em fixed} number of blocks.
As a result, the system will {\em adapt the accuracy to a target bitrate}.
At a high level, the functions of $\AgThresh$ and $\AreaThresh$ in \name are somewhat similar to variable bitrate (VBR) and constant bitrate (CBR) in classic encoding (one is more content adaptive and one achieves constant bitrate).
However, we acknowledge that in our current implementation, $\AgThresh$ and $\AreaThresh$ do not directly tie to a target accuracy or fixed bitrate, which we will discuss in \S\ref{sec:discuss}.
Nonetheless, we will demonstrate how the current design can still help adaptive streaming in \S\ref{subsec:eval:adaptive}.

%while minimizing compressed video size. 
%In contrast, the high-quality area threshold $\AreaThresh$ can be used to {\em control compressed video size} while maximizing accuracy. 

%\jc{can't control directy, but effective}

% In practice, we found tuning them result in a similar frontier of accuracy/compression tradeoffs, so we expose $\AgThresh$ as a tunable parameter to users (just as QP in MPEG/H.264) and empirically set $\PadThresh$ at 2 by default.


%it is straightforward to derive the optimal quality assignment on the given frame.
%\jc{Kuntai, please give the derivation}
%Recall that only $c$-many blocks will be encoded in high quality, we just need to pick $c$-many blocks with largest accuracy gradient value, encode them in high quality and encode remaining blocks in low quality.



\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{figs/overall-workflow.pdf}
    \tightcaption{Architecture and three phases of \name.}
    \label{fig:workflow}
\end{figure}

\subsection{Workflow of \name}

Figure~\ref{fig:workflow} depicts \name's workflow and the three APIs:

\vspace{0.1cm}
{\footnotesize
\noindent
{\bf \texttt{agm = prepare(dnn\_func,acc\_func)}}\\
{\bf \texttt{encoded\_video = ingest(agm,*raw\_frame,param)}}\\
{\bf \texttt{result = consume(encoded\_video,dnn)}}
\vspace{0.1cm}
}

\mypara{Preparation}
The analyst provides \name the final DNN with its accuracy function ({\bf \texttt{acc\_func}}), and \name trains an {\em \ag model} ({\bf \texttt{agm}}) that predicts the \ags on any new frame. 
%(similarity between DNN outputs on the high-quality frame and on the low-quality encoding)
%The accuracy function takes DNN's outputs on the high quality encoding and on the low quality encoding of a frame as input, and returns the similarity between them (which indicates accuracy as defined in \S\ref{??}).
%the accuracy of running the DNN on the encoded frame with respect to the result of running the DNN on the high quality image as the ``ground truth''. 
Optionally, the operator also provides a training dataset to train the \ag model; otherwise, \name will learn the \ag model on a pre-determined number of video frames from the real video stream. We elaborate this in \S\ref{subsec:training-data}.
%As elaborated in \S\ref{??}, the choice of training data involves a tradeoff between accuracy-gradient model performance and real-time overhead. 

\mypara{Encoding} 
\name runs the trained \ag model on each input frame to get the \ag per block and uses the thresholds of $\AgThresh$ or $\AreaThresh$ ({\bf \texttt{param}}) to decide the quality assignment according to \S\ref{subsec:quality-assignment}.
Through tuning the parameters, the user can vary the tradeoff between accuracy and compression efficiency (file size). 
%The encoded video will then be saved together with a metafile that includes the quality assignment information.
A straightforward implementation would encode two videos, incurring twice the encoding overheads, but \S\ref{sec:runtime} will discuss how \name reduces the additional overhead. 

\mypara{Decoding}
\name decodes the video frames 
%and use the quality assignment information in the metafile to overlay the decoded high quality blocks on the low quality one. 
%The resulting frames are 
and then feed them to the DNN for inference. 
%As an further optimization to reduce inference time, the DNN can also use the quality sensitivity information in the metafile to filter out regions that are very unlikely to have useful information (\eg background).

Though the workflow sketched in Figure~\ref{fig:workflow} is functionally sufficient,
%to encode videos with spatially different quality based on the notion of accuracy gradients, 
two challenges remain: 
(1) how to learn an accurate \ag model; and (2) how to use it in real time for high accuracy and low encoding/decoding overhead.
We will address them in the next two sections.


%\begin{itemize}
%\item why the idealized design is impractical => automatically generating the quality assignment 
%\item an optimization framework for accuracy/compression tradeoffs
%\item key notion: a saliency map based on accuracy gradients
%\item why is it unique (diff to traditional saliency). aware of hq-lq diff
%\item why accuracy gradients naturally give rise to the three opportunities.
%\item walk-through an example (with API)
%\item challenges: (1) how to learn an accurate generator of accuracy gradients; and (2) how to use it in real time for high accuracy and low encoding/decoding overhead
%\item intuitively, why this problem is much simpler than final DNN. 
%\end{itemize}





%\section{Design of \name}


\section{Learning accuracy gradients in \name}
\label{sec:training}

First, it may be tempting to use an off-the-shelf background detector, a region proposal network or a segmentation network as the \ag model. 
However, the \ag of a block indicates how much the inference result would change if the pixels in the block change from low quality encoding to high quality encoding, so  a small \ag does not necessarily mean the block is in the background (maybe part of an object that can be detected under both high and low quality).


\begin{comment}
However, the goal of an \ag model differ in several aspects.
%First, the goal of an \ag model may look similar to that of a background detector, a region proposal network or a segmentation network. However, they differ in several key aspects.
First, an \ag model's output is per block, not per pixel, which has implications.
The \ag of a block indicates how much the inference result would change if the pixels in the block change from low quality encoding to high quality encoding. 
In other words, it captures both the importance of a region to the inference results and the magnitude of pixel value changes between different quality levels.
Thus, a low accuracy gradient does not necessarily mean the block is in the background (\eg part of an object that can be detected under both high and low quality).
In short, the accuracy-gradient model cannot directly reuse off-the-shelf models.
\end{comment}

%\jc{give a few examples, back ref to section 3}

Next, we discuss the design choices of \name's model architecture, loss function, and training data.


\subsection{Model architecture}

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/vgg11.pdf}
    \caption{Schematic architecture of our \ag model. \kt{ugly. Plan to redraw it.}}
    \label{fig:vgg11}
\end{figure}

\kt{Maybe also illustrate some reasons of why cheap neural network suffice (compared to why this architecture)?}

We use a custom DNN based on VGG11 as the architecture of the \ag model~\cite{??}. 
Figure~\ref{fig:vgg11} shows the model architecture.
% \jc{a few highlights on the model?}
The choice of this architecture is based on two reasons.

On one hand, this model is much more compact than the alternatives that are still based on fully convolutional (FC) feature extractors.
To put it into perspective, our \ag model has \fillme FLOPs, an \fillme orders of magnitude reduction compared to the typical cheap convolutional models (such as ResNet18 and MobileNet), which contain \fillme FLOPs.
%\jc{any other metrics}
In addition, since the architecture in Figure~\ref{fig:??} consists only of FC operations (and batch normalization and activation), its computational overhead is proportional to the size of the input frame (\ie $4\times$ faster when the frame size reduces by $2\times$ in each dimension). 
\jc{if we use it to optimize mask generation cost, we should echo it here!}

On the other hand, we have intuitive reasons (in addition to the empirical results in \S\ref{sec:eval}) to believe this architecture suffices to learn the task.
Inferring \ags is functionally similar to running semantic segmentation on a low resolution image, to which FC operation is a natural fit as demonstrated in prior research~\cite{??,??}.
Moreover, compared to traditional segmentation tasks (where each label can be one of hundreds of classes), our task essentially assigns a binary label to each block: ultimately, the \ag model output is not evaluated by how accurately each \ag is inferred, but whether the right set of blocks are selected to encode in high quality.\footnote{At first glance, it does appear that the \ag model needs to approximate a highly complex mathematically procedure: after all calculating \ags in Eq (\ref{eq:acc-gradients}) involves the full DNN.
However, we believe this is not far fetched.
The matrix of \ag is mathematically the saliency of a DNN, and there is recent work in deep learning (\eg~\cite{dabkowski2017real}) that proposes relatively shallow models that quickly infer saliency of an arbitrary differentiable image classifier.
An intuitive explanation is that saliency inference is often used for purposes that do not depend on precise estimation of saliency on each pixel (\eg DNN interpretation or video encoding in our case), so they are inherently more tolerant to error than the task of the final DNN.
}
%our quality assignment only depends on whether accuracy gradient of a block is over a given threshold.

We acknowledge that it is possible to design a custom DNN architecture for our \ag model and train it from scratch.
Nonetheless, our goal here is not to choose the ``optimal'' architecture; rather, we want the \ag model to be light-weight and accurate enough to identify which regions should be in high quality.
In designing the model, \name takes a pragmatic choice of fine-tuning a pretrained VGG11 model~\cite{pre-train model link}  which can be faster and more data efficient than training a clean-slate model in practice.


% \jc{why not customized model architecture?}


%On the other hand, any smaller model will have a CNN feature extractor smaller than most of the common ones, so one has to customize the model architecture and train the model from scratch. 
% \jc{1. it's easier than detection, etc
% 2. it's functionally similar to segmentation on a low-resolution image, and FC is known to be a good fit to segmentation.}
% \jc{explain please?}









\subsection{Loss function}

In training the \ag model, \name uses the following loss function:
% \jc{equation}
{\small
\begin{align}
    \sum_{\lambda\in \Lambda} CrossEntropy(\AccuracyGradientModel(\RawImage), \mathbbm{1}(\AccuracyGradient(\LowImage) > \lambda)) \label{eq:loss-function}
\end{align}
}
where $\AccuracyGradientModel$ is the trained \ag model, $\mathbbm{1}(\cdot)$ is the indicator function, $\RawImage$ is the original frame representation (\eg raw pixels) available before we encode the frame, and $\Lambda$ is a set of threshold values with a logarithmic scale (in our experiment, we used 0.1, 0.01, 0.001, etc).
While using cross entropy loss is common in deep learning, this particular form of loss function entails two design choices.

First, using thresholds ($\lambda$) efficiently tackles the imbalanced value distribution in $\AccuracyGradient(\LowImage)$.
$\AccuracyGradient(\LowImage)$ contains mostly low values (close to 0) while the more useful large values are large ones, so if we use the traditional cross entropy loss (or mean square error) between $\AccuracyGradientModel$ and $\AccuracyGradient$ as the objective function, the resulting model will tend to produce mostly zeros. 
In fact, the values in $\AccuracyGradient(\LowImage)$ roughly follow a log-normal distribution, 
%so in order to learn values at each percentile of the distribution, 
we set a series of thresholds $\lambda$ with a logarithmic gap between them, so that it explicitly teaches the $\AccuracyGradientModel$ model  to learn \ag values at each scale. 
We note that though the use of these threshold  is motivated by the log-normal-like shape of \ag values, it is generally effective at tackling the imbalanced \ag values distributions.
%and does not depend on whether \ag values strictly follow a log-normal distribution. 
% We have found them to be effective at tackling the imbalance of saliency values.
\jc{kuntai, why not just log the values first and then train it with normal cross entropy? is it because there are lots of zeros?}

Second, while a natural choice would be to minimize the loss between $\AccuracyGradientModel(\LowImage)$ and $\AccuracyGradient(\LowImage)$, we choose to use $\RawImage$ as the input to $\AccuracyGradientModel$ for two reasons.
(1) The high quality image of $\RawImage$ preserves more information (high frequency and low frequency) than $\LowImage$, which allows $\AccuracyGradientModel$ to learn more better features.
(2) In the encoding step, $\RawImage$ is naturally available and does not require additional encoding, whereas to get the $\LowImage$ would require one additional encoding.



% \jc{why $\AccuracyGradientModel$ is applied on $\HighImage$. To get more features}

% To see the reason behind this choice, let us first consider some other seemingly reasonable ones.

% 1. MSE
% $$
% \Vert \AccuracyGradientModel(\HighImage), \AccuracyGradient(\LowImage) \Vert_2^2
% $$
% \jc{accuracy gradient values are highly unbalanced, so MSE will tend to generate a all-zero mask, because most elements are small. in contrast, crossentropy will use $\lambda$ to filter out ??}

% 2. Cross entropy loss

% \begin{align*}
%     CrossEntropy(\AccuracyGradientModel(\HighImage), \AccuracyGradient(\LowImage))
% \end{align*}

% How to choose the threshold $\lambda$?
% The gradients in $\AccuracyGradient(\HighImage)$ follows a normal distribution in the logscale space.


% \jc{this is the place to show your lessons learned from prior tries of various loss functions}

\jc{explain why not training a binary mask generator directly?}

% \jc{emphasize that we give more penalty to false negative than false positive}

%\begin{itemize}
%\item problem formulation: what to learn. how is it diff to region-proposal, background detection, etc
%\item problem 1: choice of labels (or loss function)
%\item strawman: \fillme. why it should work and why it didn't work
%\item our solution: 
%\item problem 2: choice of model architecture
%\item why not a custom model
%\item why vgg? any connection with classification
%\item choice of training data: same as the dnn (or user-defined)
%\end{itemize}


\subsection{Training data}
\label{subsec:training-data}

\name provides two options to obtain the training data of the accuracy-gradient model $\AccuracyGradientModel$. 
% Like in any ML models, the training data can affect both the accuracy and the generalizability of the accuracy-gradient model. \jc{this is not about generalizability!}
% In designing \name, we provide two options of obtaining the training data.

First, the operator who provides the full DNN may share its training dataset (in many cases, this is a public dataset such as COCO or ImageNet.)
This way, the $\AccuracyGradientModel$ can be trained on the same images that the final DNN was trained on.
The reasoning of this choice is as follows.
Hypothetically, if the $\AccuracyGradientModel$ has a comparable complexity of the final DNN, then in theory, if $\AccuracyGradientModel$ is trained on the same dataset as the final DNN, it can very closely approximate the process of \ag calculation of Eq (\ref{eq:acc-gradients}).
Thus when $\AccuracyGradientModel$ is based on a compact model, any error made by $\AccuracyGradientModel$ is likely caused by the model architecture, rather than any training data biases.
Of course, this reasoning is no rigorous proof, but in lack of a dataset customized for training \ag model, we believe this is a reasonable choice (as shown in \S\ref{sec:eval}). 
%We show that the resulting model performs reasonably among videos that the final DNN works well.  

%A natural choice of training data is the same dataset used to train the DNN used for final inference. 
%In theory, this choice maximizes generalizability, because \jc{what's the rationale?}

The other choice of training data, sometimes used in prior work (~\cite{reducto,noscope}), is to train the \ag model based on the frames sampled from the test video steam. 
A benefit of this approach is that these sampled frames might share a similar data distribution with the real video stream. 
We will show the effectiveness of both choices in \S\ref{subsec:eval:micro}.
%In practice, if training data of the full DNN is available, these two approach can be combined: one can first train $\AccuracyGradientModel$ on the operator-provided dataset in the preparation phase, and then fine-tune it with sampled frames from the test video streams. 
%\jc{a sentence to summarize the takeaway from eval}





\section{Using accuracy gradients in \name}
\label{sec:runtime}

% Even if one successfully trains the accuracy gradient model, the challenge still remains when deploying it as part of a video stack.
% This section will introduce how \name addresses these issues. 


%\mypara{Speeding up encoding}
% Compared to the traditional video encoding, 
If we naively apply \ag model in video encoding, each frame would involve one light-weight DNN (\ag model) inference and two encoding passes, compared to only one encoding pass in the traditional codec. 
Likewise, the decoding will involve two decoding processes per frame, instead of one.
In fairness, the computational cost of \name is still much lower than some prior work, which runs a large DNN inference on each frame~\cite{dds} or a few times every tens of seconds~\cite{awstream}, and it is not uncommon for video analytics pipelines to run a light-weight object detector~\cite{vigil,canel2019scaling}, vision feature extractor~\cite{reducto}, object tracker~\cite{glimpse}, or super-resolution~\cite{cloudseg} on each frame. 
Nonetheless, the increased computational overheads compared to traditional codecs hinder \name's deployment in resource-constrained devices.
% 's use as a generic video stack and can hinder its deployment in resource-constrained devices.
\name reduces the additional computational cost in two ways.

\subsection{Persistence of accuracy gradients}

\kt{Mention enlargement}

First, \name runs the \ag model only on sampled frames, rather than all frames. 
The intuition behind it is that although the \ag values do vary across frames, the quality assignment derived from it changes at a much longer timescale. 
Figure~\ref{fig:assignment-persistence} confirms this intuition: most blocks will be selected in \fillme\% of frames in each 1-second window. 


\begin{figure}
    \centering
    \includegraphics[width=0.65\columnwidth]{figs/placeholder-assignment-persistence.pdf}
    
    \includegraphics[width=0.65\columnwidth]{figs/persistance.pdf}
    \caption{Most high-quality blocks persist for over \fillme consecutive frames. \kt{More than 90\% of the frames have persistence greater than 30.}}
    \label{fig:assignment-persistence}
\end{figure}


% \jc{show some empirical evidence that the per-frame masks do evolve slowly}

We speculate that the relatively slow pace of change 
% in quality accuracy-gradient matrix 
results from the conservative predictions of the \ag model. % and the relatively coarse granularity of grids.
% of the grids than pixels.
% While regions that must be encoded in high quality do move over time (\eg a moving object), we empirically found that the 
First, the \ag values generated by the \ag model change smoothly across neighboring blocks.
As a side effect, many blocks surrounding the high-\ag blocks also have substantial predicted \ag values, which means slightly more regions are encoded in high quality.
% the inferred accuracy gradient matrices tend to encode slightly more regions in high quality.
% so even when a block is not assigned to high quality, it is 
% In addition, since the training process (introduced in \S\ref{??}) gives more penalty to false negatives (\fillme) than to false positives (\fillme). 
% As a consequence, the inferred accuracy gradient matrices tend to encode slightly more regions in high quality.
These conservative estimates might lead to slightly inflated file sizes, but it does make it possible to reuse an accuracy-gradient matrix across neighboring frames.



\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/placeholder-uniform-color.pdf}
    
    \includegraphics[width=0.95\columnwidth]{figs/fig10.pdf}
    \caption{\kt{Using low quality to encode the background may introduce spurious objects, while encoding with uniform color will not.}Using uniform color to encode most of the blocks actually improves accuracy compared to using low quality which misleads the DNN to infer spurious results.}
    \label{fig:uniform-color}
\end{figure}

\subsection{Uniformly colored encoding}

Besides reducing inference frequency of the \ag generator, \name also explores the extreme design point of using uniform color as the low quality encoding.
It does obviate the need to encode each frame twice (only high quality blocks need to be encoded), but at first sight, this should hurt high accuracy, because the low-quality region provides no information outside the regions encoded in high quality, and the uniform coloring may appear ``unnatural'' to the DNN feature extractors and cause low accuracy.\footnote{We acknowledge that the two encodings could be combined if RoI encoder is used (though the file size of RoI-encoded video will still be more than setting all non-high quality blocks in uniform coloring. We did not use it since it is no longer readily supported in many off-the-shelf codec implementation~\cite{??}.}

However, these arguments ignore several properties of DNNs. 
First, many vision tasks, such as object detection, do handle partially observed objects; \eg if only half of a bus appears in the frame, an object detector still has enough features to detect it. 
% We have seen empirical evidence in our experiments too.
%that when an object is only partially encoded in high quality, object detection models can still detect them.

Second, using a single color to encode parts of a frame does not necessarily reduce accuracy.
Vision features extracted by FC layers are ``localized'', \ie changing the value of a pixel in theory does not change another region's FC-extracted features.
(This pattern may hold in the recent transformer-based vision models, but we have not verified it yet.)
However, setting non-high quality blocks in the uniform color {\em could} still have two adverse effects: 
(1) it may change the result of the batch normalization operation (normalizing the feature values) which does take the whole image into account, and 
(2) it may still affect nearby FC-extracted features.
Somewhat surprisingly, we found that setting the non-high quality blocks in the mean pixel value (rather than an arbitrary color such as black) can effectively mitigate these issues, since batch normalization will not be affected and it effectively ``smooth'' the transition to high quality blocks (see Figure~\ref{fig:uniform-color}).
This uniform color value can be kept with negligible overhead. 
% the uniform color is chosen in a way that \jc{kuntai, is this about normalization?}. \jc{also needs to mention that the uniform color can be retrieved from the encoded image so no additional meta data is needed}
% \kt{We do need to record the metadata (the mask). But for each frame, the mask only contain 45*60 booleans, and the mask is the same for 30 frames. The storage size is ~0.1KB per frame.}

Third, there is in fact a tradeoff between using a low quality vs. uniform color to encode the non-high quality blocks.
Using a low quality to encode these regions might cause the DNN to output ``spurious'' inference results.
In contrast, since the high-quality blocks picked by \name already contain enough blocks for DNN to make pretty accurate inference. 
Setting the background in uniform color does not incur much cost on accuracy.

We acknowledge that using the uniform color may {\em not} apply to all cases. 
For instance, \jc{give a failure case}
That said, our design choice is driven by the empirical observations of the DNNs under our study and we hope it can inform future designs to improve its generalizability. 

\jc{need to mention ROI encoding!}


%\subsection{Quality assignment based on accuracy gradients}
%
%\jc{threshold + enlargement}

%\jc{need to talk about how to deal adapt to bandwidth}



%\begin{itemize}
%\item solution (not running it per frame)
%\item choice of quality: we explore an extreme design point of uni-color background
%\item benefits: low bw for same acc, speed-up encoding/decoding \& inference
%\end{itemize}


%\mypara{Mitigating the effect of hard boundaries} 
%\begin{itemize}
%\item problem 1: inference accuracy over the black background can be low. example/reason(cnn)
%\item solution (smoothing?)
%\end{itemize}


\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{figs/placeholder-example.pdf}
    
    \includegraphics[width=0.95\columnwidth]{figs/walkthough.pdf}
    \caption{A walkthrough of the output of each stage in \name. }
    \label{fig:example}
\end{figure}


% \subsection{Putting the components together}

Finally, we proceed to put the different design components together. 
Figure~\ref{fig:example} shows a concrete example to walk through the input and output of each step.


%\begin{itemize}
%\item challenges remain in two aspects
%\item problem 1: inference accuracy over the black background can be low. example/reason(cnn)
%\item solution (smoothing?)
%\item problem 2: overhead of running the generator per frame. 
%\item solution (not running it per frame)
%\item choice of quality: we explore an extreme design point of uni-color background
%\item benefits: low bw for same acc, speed-up encoding/decoding \& inference
%\end{itemize}

%\newpage

==> technical-v2.tex <==



\section{Online encoding}
\label{sec:encoding}

% \begin{itemize}
%     \item The architecture and the compute overhead of \AccuracyGradientModel
%     \item Encoding based on \AccuracyGradientModel
%     \item Bandwidth adaptation
% \end{itemize}

In this section, we discuss the technical details of the encoding stage of \name. 
We first introduce the architecture of our \AccuracyGradientModel and the techniques to reduce its computation cost.
We then introduce the technique to let \name use \AccuracyGradientModel less frequently.
After that, we introduce one technique to further reduce the file size generated by \name.
Last, we introduce the bandwidth adaptation algorithm for \name.




\subsection{Model architecture}
\label{subsec:architecture}

% \begin{itemize}
%     \item Mention the architecture
%     \item Mention how cheap it is
%     \item Mention why it is easier than simple segmentation
% \end{itemize}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\columnwidth]{figs/vgg11.pdf}
%     \tightcaption{Schematic architecture of our \AccuracyGradientModel, where ``conv'' is convolution and ``pool'' is max pooling. \jc{maybe drop this graph. doesn't add much value}}
%     \label{fig:vgg11}
% \end{figure}

% It is important to notice that the \ag of a block indicates how much the inference result would be changed by a change of the block's encoding quality.
% Thus, 
% It is important to notice that the high-\ag blocks (as shown in \S\ref{subsec:analysis}) can be frequently misaligned with detection results (the bounding boxes or edges of objects).
% As a result, we do not design the \AccuracyGradientModel based on region-proposal networks or cheap object detector (which are used in prior work that will be compared against in \S\ref{sec:eval}).
% Instead, we use a custom shallow NN based on VGG11 as the architecture of the \AccuracyGradientModel. 

As \AccuracyGradientModel learns to assign a label (high encoding quality or low encoding quality) to each microblock, which is similar to semantic segmentation task, which learns to assign a label to each pixel,
we design the architecture of \AccuracyGradientModel based on the architecture of semantic segmentation models~\cite{long2015fully} with a pretrained feature extraction backbone~\cite{vgg}. We freeze the pretrained feature extraction backbone parameters.

\mypara{Pooling optimization} To further save compute cost, we leverage the low resolution opportunity mentioned in \S\ref{subsec:rationale}. Specifically, we put 4 layers that performs 2x downsample through max pooling inside our model architecture as illustrated in Figure~\ref{fig:vgg11}. After each max pooling, the width and the height of the output will be reduced by half,and thus reduce the compute of all following layers. This technique will reduce the compute cost from 10, 683 GFLOPs to 146 GFLOPs, a 73x cost reduction.



\mypara{Compute cost of \AccuracyGradientModel} To put the compute cost of \AccuracyGradientModel into perspective, our model is much more compact than other commonly-used feature extractors.
To put it into perspective, our \AccuracyGradientModel has 160 GFLOPs, an 3.5x reduction compared to the typical cheap convolutional models (such as ResNet50), which contain 550 GFLOPs.
%\jc{any other metrics}
In addition, since the architecture in Figure~\ref{fig:vgg11} consists only of FC operations (in addition to a few batch normalization and activation), its computational overhead is proportional to the size of the input frame (\eg $4\times$ faster when the frame size is reduced by $2\times$ in each dimension). 




\mypara{Cheap \AccuracyGradientModel suffices} 
To show that a cheap \AccuracyGradientModel already suffices to accurately learn \AccuracyGraident,
we evaluate the impact of different compute complexity of \AccuracyGradientModel on the training performance against training epochs (we use cross validation loss as the performance metrics here).
We use different feature extractor (VGG11, VGG13, VGG16 and VGG19) with different compute cost ( $1.0\times$, $1.4\times$, $1.9\times$ and $2.4\times$ compute cost compared to \AccuracyGradientModel respectively) pretrained on image net.
In Figure~\ref{fig:architecture-loss}, we see that our model (the $1.0\times$ curve) is good enough to deliver good performance. The cross validation loss will just be marginally better even when granting \name $2.4\times$ more compute.



% On the other hand, 
% we have intuitive reasons (in addition to the empirical results in \S\ref{sec:eval}) to believe this architecture suffices to learn the task.


% Second, we use this model,
% % this architecture suffices to learn \ag values, 
% because inferring \ags is functionally similar to running semantic segmentation on a low resolution image, to which FC operation is a natural fit~\cite{long2015fully}.
% Moreover, compared to traditional segmentation tasks (where each label can be one of hundreds of classes), our task essentially assigns a binary label to each block: ultimately, the \AccuracyGradientModel output is not evaluated by how accurately each \ag is inferred, but whether the right set of blocks are selected to encode in high quality.\footnote{At first glance, it does appear that the \AccuracyGradientModel needs to approximate a highly complex mathematical procedure: after all calculating \ags in Eq (\ref{eq:acc-gradients}) involves the full DNN.
% However, we believe this is not far fetched.
% The matrix of \ag is mathematically the saliency of a DNN, and there is recent work in deep learning (\eg~\cite{dabkowski2017real}) that proposes relatively shallow models that quickly infer saliency of an arbitrary differentiable image classifier.
% An intuitive explanation is that saliency inference is often used for purposes that do not depend on precise estimation of saliency on each pixel (\eg DNN interpretation or video encoding in our case), so they are inherently more tolerant to error than the task of the final DNN.
% }






% As \AccuracyGradientModel generates a quality assignment to every microblock, this task shares the same output format as semantic segmentation, where it  generates a class label to every pixel. Thus, we use a fully-convolutional network architecture~\cite{long2015fully} based on pretrained VGG-11 backbone~\cite{vgg}.
% Figure~\ref{fig:vgg11} shows the model architecture.
% % \jc{a few highlights on the model?}





\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/training-curve-vs-arch.pdf}
    \tightcaption{Cross validation loss versus compute cost (we denote the compute cost of VGG-11 as $1.0x$). We can see that \AccuracyGradient is easy enough for a cheap architecture (VGG-11) to learn and an architecture with compute cost $2.4x$ (VGG-19) will only increase the gain marginally.
    \jc{add a line of a much smaller model doesn't work}}
    \label{fig:architecture-loss}
\end{figure}





%our quality assignment only depends on whether accuracy gradient of a block is over a given threshold.

% We acknowledge that it is possible to design a custom DNN architecture for our \AccuracyGradientModel and train it from scratch.
% That being said, our goal here is not to choose the ``optimal'' architecture; rather, \name takes a pragmatic choice of fine-tuning a pretrained VGG11~\cite{pytorch-model-zoo}, which can be done more efficiently than training a custom DNN model from scratch.
% We will evaluate its inference and training cost in \S\ref{sec:eval}.

% rather, we want a light-weight \AccuracyGradientModel that is accurate enough to identify which regions should be in high quality.
% In designing the model, \name takes a pragmatic choice of fine-tuning a pretrained VGG11 model~\cite{pre-train model link}  which can be faster and more data efficient than training a clean-slate model in practice.


% \jc{why not customized model architecture?}


%On the other hand, any smaller model will have a CNN feature extractor smaller than most of the common ones, so one has to customize the model architecture and train the model from scratch. 
% \jc{1. it's easier than detection, etc
% 2. it's functionally similar to segmentation on a low-resolution image, and FC is known to be a good fit to segmentation.}
% \jc{explain please?}



\subsection{Saving inference cost through sampling}


\mypara{Frame sampling for cheap inference} \name runs the \AccuracyGradientModel only once every 30 frames (rather than each frame) and use the output from that one frame to encode all 30 frames.
The intuition here is that although the \ags do vary across frames, the quality assignment derived from it changes at much longer timescales. 
Figure~\ref{fig:assignment-persistence} shows that even if \name assigns quality per frame, on more than 90\% of the frames, the quality assignment of 90\% of the blocks remains the same in the next 30 frames. 

\mypara{Padding} 
In order to make the quality-sensitive macroblocks generated by \AccuracyGradientModel temporally  smoother,
we leverage the boundary distortion tolerance mentioned in \S\ref{subsec:rationale} and put those macroblocks that are at most 4 macroblocks away to the quality-sensitive blocks in high quality, \ie $\PadThresh=4$.
Figure~\ref{fig:assignment-persistence} shows that even if \name assigns quality per frame, on more than 90\% of the frames, the quality assignment of 90\% of the blocks remains the same in the next 30 frames. 
The intuition is that even if the important microblock moved due to object motion, it will not move too far away and thus it will still locate near the original micriblock.
We acknowledge that re-using quality assignment can be problematic when objects move quickly and that these conservative estimates might lead to slightly inflated file sizes (as shown in the Dance dataset in Figure \ref{fig:eval-overall}). 



\begin{figure}
    \centering
    % \includegraphics[width=0.65\columnwidth]{figs/placeholder-assignment-persistence.pdf}
    
    \includegraphics[width=0.4\columnwidth]{figs/persistance.pdf}
    \tightcaption{The high quality blocks generated by more than 90\% of the frames can persist for over 30 consecutive frames.}
    \label{fig:assignment-persistence}
\end{figure}









\subsection{Uniform colored background}
\label{subsec:uniform}

After encoding the quality-sensitive macroblocks to high quality, a direct thought is to encode these macroblocks in high quality and encode the background in low quality through region-of-interest encoding.
% Besides reducing inference frequency of the \ag generator, 
However, we empirically find that this approach falls into a sub-optimal trade-off since the accuracy gain provided by low-quality background cannot compensate the large extra file size from it.
Moreover, we found that in some cases encoding the background in low encoding quality may sometimes hurt the accuracy instead (as shown in Figure~\ref{fig:uniform-color}).


\begin{figure}
    \centering
    % \includegraphics[width=0.9\columnwidth]{figs/placeholder-uniform-color.pdf}
    
    \includegraphics[width=0.95\columnwidth]{figs/fig10.pdf}
    \tightcaption{Using low quality to encode may sometimes mislead the DNN to infer spurious objects while encoding the background in uniform color will not.}
    \label{fig:uniform-color}
\end{figure}



\begin{figure}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-low-quality.pdf}
    \includegraphics[width=0.4\columnwidth]{figs/detection_qp.pdf}
    \tightcaption{\name lies on a better file size-accuracy trade-off compared to encoding background in QP=32 and QP=38.}
    \label{fig:eval-low-quality}
\end{figure}




Based on these observations, \name instead use uniform color (RGB=(123.675,116.28,103.53), the mean value of COCO normalization~\cite{pytorch-model-zoo}) to encode the background.
To evaluate the performance impact of this design choice, we show in Figure~\ref{fig:eval-low-quality} that the file size-accuracy trade-off of \name with uniform color as background, and \name with background in different encoding quality (QP=32 and QP=38).
We see that \name lies on a better trade-off compared to using low quality as the background.
% At first sight, it seems to hurt accuracy, 
% % but at first sight, this should hurt high accuracy, 
% because the low-quality regions now provide no useful information outside the regions encoded in high quality.
% % , and the uniform coloring may appear ``unnatural'' to the DNN feature extractors and cause low accuracy.
% However, it ignores several favorable properties of DNNs. 

% First, many vision models, such as object detectors, naturally handle partially observed objects; \eg if half of a bus appears in the frame, an object detector still has enough features to detect it. 
% % We have seen empirical evidence in our experiments too.
% %that when an object is only partially encoded in high quality, object detection models can still detect them.
% Second, using a single color to encode parts of a frame does not necessarily reduce accuracy.
% Vision features extracted by FC layers are ``localized'', \ie changing the value of a pixel in theory does not change another region's FC-extracted features.
% (This pattern may hold in the recent transformer-based vision models, but we have not verified it yet.)
% That said, using a uniform color still may change the result of the batch normalization operation (which normalizes the feature matrices of the whole image).
% % has two adverse effects: 
% % (1) it may change the result of the batch normalization operation (which normalizes the feature matrices of the whole image); and % which does take the whole image into account, and 
% % (2) it may still affect nearby FC-extracted features.
% Somewhat surprisingly, we found that setting the non-high quality blocks in the {\em mean} pixel value (rather than an arbitrary color such as black) can effectively alleviate these issues, since batch normalization will not be affected. %, and it effectively ``smoothes'' the transition to high quality blocks (see Figure~\ref{fig:uniform-color}).
% (This uniform color value can be stored with negligible overhead.)
% % the uniform color is chosen in a way that \jc{kuntai, is this about normalization?}. \jc{also needs to mention that the uniform color can be retrieved from the encoded image so no additional meta data is needed}
% % \kt{We do need to record the metadata (the mask). But for each frame, the mask only contain 45*60 booleans, and the mask is the same for 30 frames. The storage size is ~0.1KB per frame.}
% Third, using low quality to encode non-high quality regions often cause DNN to output ``spurious'' inference results (see Figure~\ref{fig:uniform-color}).
% In contrast, using a uniform color avoids such false positives. % the high-quality blocks picked by \name already contain enough blocks for DNN to make pretty accurate inference. 


\begin{comment}

there is in fact a tradeoff between using a low quality vs. uniform color to encode the non-high quality blocks.
Using a low quality to encode these regions might cause the DNN to output ``spurious'' inference results.
In contrast, since the high-quality blocks picked by \name already contain enough blocks for DNN to make pretty accurate inference. 
Setting the background in uniform color does not incur much cost on accuracy.
\end{comment}

We acknowledge that using the uniform color may {\em not} apply to all cases. 
% For instance, \jc{give a failure case}
That said, our design choice is driven by the observations of the set of DNNs under our study and we hope it can inspire future designs to improve its generalizability. 

% \jc{need to mention ROI encoding!}


%\subsection{Quality assignment based on accuracy gradients}
%
%\jc{threshold + enlargement}

%\jc{need to talk about how to deal adapt to bandwidth}



%\begin{itemize}
%\item solution (not running it per frame)
%\item choice of quality: we explore an extreme design point of uni-color background
%\item benefits: low bw for same acc, speed-up encoding/decoding \& inference
%\end{itemize}


%\mypara{Mitigating the effect of hard boundaries} 
%\begin{itemize}
%\item problem 1: inference accuracy over the black background can be low. example/reason(cnn)
%\item solution (smoothing?)
%\end{itemize}


\begin{figure}
    \centering
    % \includegraphics[width=0.95\columnwidth]{figs/placeholder-example.pdf}
    
    \includegraphics[width=0.95\columnwidth]{figs/walkthough.pdf}
    \tightcaption{Walkthrough of each stage in \name.}
    \label{fig:example}
    \vspace{-1mm}
\end{figure}




% \jc{show some empirical evidence that the per-frame masks do evolve slowly}

% We speculate that the relatively slow pace of change 
% in quality accuracy-gradient matrix 
% results from the conservative predictions of the \AccuracyGradientModel. % and the relatively coarse granularity of grids.
% of the grids than pixels.
% While regions that must be encoded in high quality do move over time (\eg a moving object), we empirically found that the 
% We speculate that the relatively slow pace of change results from the conservative quality assignment by \name. 
% First, empirically we found that the \ag values generated by the \AccuracyGradientModel change smoothly across neighboring blocks.
% As a side effect, many blocks surrounding the high-\ag blocks also have high \ag values, which means slightly more regions are encoded in high quality.
% Second, \name adds $\gamma$ (by default, 3) blocks to each direction of a high-\ag block, which helps (though to a less extent than the first one) to stabilize the quality assignment.
% % the inferred accuracy gradient matrices tend to encode slightly more regions in high quality.
% % so even when a block is not assigned to high quality, it is 
% % In addition, since the training process (introduced in \S\ref{??}) gives more penalty to false negatives (\fillme) than to false positives (\fillme). 
% % As a consequence, the inferred accuracy gradient matrices tend to encode slightly more regions in high quality.
% We acknowledge that re-using quality assignment can be problematic when objects move quickly and that these conservative estimates might lead to slightly inflated file sizes (as shown in the Dance dataset in Figure \ref{fig:eval-overall}). 
% Nonetheless, it does make it possible to reuse an accuracy-gradient matrix across neighboring frames.

% \mypara{Frame dropping} Different from frame dropping technique~\cite{reducto} that skip running server-side models on some of the frames, our frame sampling technique will still encode all frames. Thus, as long as 






\subsection{Bandwidth adaptation}
\label{subsec:bandwidth-adaptation}

We show the flexibility of \name in supporting various compression-accuracy objectives, via the setting of its parameters $\AgThresh$ and $\AreaThresh$, as explained in \S\ref{subsec:quality-assignment}. 
%As a usable video stack, \name provides two control knobs to navigate the bandwidth-accuracy tradeoffs, as explained in \S\ref{subsec:assignment}. 
To demonstrate it, we consider that a video sensor encodes and streams the video over a bandwidth-constrained connection to a remote server for DNN inference and analytics.

\mypara{Reducing bandwidth usage with high accuracy}
% \kt{Rename this to accuracy control?}
When users want to minimize bandwidth usage without hurting accuracy, it will be a good use case for setting the \ag threshold $\AgThresh$, which allows the user to take advantages of content variation: when content is simple or contains less useful information, naturally less blocks will have high accuracy gradients, thus bandwidth usage can be lowered with minimum impact on accuracy.

\mypara{Higher accuracy under bandwidth budget}
% \kt{Rename this to bitrate control?}
When users want higher accuracy under limited bandwidth, it will be a good use case for setting the high-quality area threshold $\AreaThresh$, which allows user to keep at a roughly stable bandwidth usage. 
%We use an offline profiling process to first create a mapping from bandwidth usage to $\AreaThresh$. 
%Based on this profile, we then assume that the user has the perfect knowledge of future bandwidth. 
We let the user feed the available bandwidth to \name. \name then sets $\AreaThresh$ accordingly and leverages the constant bitrate mode of H.264 codec to control bandwidth.




\section{Offline customization}

In this section, we show the techniques in the offline customization phase of \name.
We first specify how we generate the ground truth for \AccuracygradientModel. 
Then we show the loss function to train the \AccuracyGradientModel.
At last we show how \name customize itself to a new server-side DNN.

\subsection{Problem formulation}

We first formulate quality assignment problem into an optimization problem.
To make the discussion more concrete, we split each $\OriginWidth\cdot\OriginHeight$ frame into $\GridWidth\cdot\GridHeight$ grids of 16x16 blocks ($\OriginWidth=16\GridWidth,\OriginHeight=16\GridHeight$) and assign each block either a high quality or a low quality. % (this aligns with previous work~\cite{eaar,dds}).
Our goal is to find a model $\AccuracyGradientModel$ that generates a $[0,1]$-valued mask of size $\GridWidth\cdot\GridHeight$ by feeding the high quality image $\HighImage$ into $\AccuracyGradientModel$, \ie $\Mask=\AccuracyGradientModel(\HighImage)$, where the element inside the mask $\Mask_{x,y}=1$ means block $x,y$ is completely in high quality and $\Mask_{x,y}=0$ means block $x,y$ is completely in low quality. The optimization goal is to minimize the number of blocks in high quality as well as maximize the inference accuracy:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\max_{\AccuracyGradientModel} &~~~~\SimFunc\bigg(\DNN \big(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage \big),\DNN(\HighImage)\bigg) \label{eq:idealized-objective}\\
s.t.&~~~~ \big\Vert \Mask \big\Vert_1 \leq c
\end{align}
}
where $\SimFunc(x, y)$ measures the accuracy of inference results $x$ against ground truth $y$, $\HighImage$ and $\LowImage$ are the high-quality encoding and the low-quality encoding of each frame\footnote{The dimension of a frame is the same for different QP values, so $\HighImage$ and $\LowImage$ have the same dimension.}, $\AllOnes$ refers to a matrix where all the elements are one, $\times$ refer to pixel-wise multiplication\footnote{The multiplication operation here will actually resize the left operand back to size $\OriginWidth\cdot\OriginHeight$ and then apply pixel-wise multiplication.}, $\DNN$ is the server-side DNN that generates the DNN inference result, $\big\Vert \Mask \big\Vert_1 $ counts the number of high quality macroblocks inside $\Mask$ and $c$ constraints the number of macroblocks in high quality to save bandwidth.

Now, maximizing Equation~\ref{eq:idealized-objective} can be approximated by 





\subsection{Ground truth generation through accuracy gradient}


Training based on the Objective~\ref{eq:idealized-objective} requires accessing the final heavy DNN (the $G$ term inside Objective~\ref{eq:idealized-objective}) in every training epoch.
As our model typically takes 15 epochs to converge, we denote the overhead comes from the final DNN as $15\times$.
To reduce this $15\times$ overhead, we perform the following transformation.

\mypara{Detach final DNN $G$ from \AccuracyGradientModel}First, we replace the constraint $\Mask=\AccuracyGradientModel(\HighImage)$ in Objective~\ref{eq:idealized-objective} into one new objective:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\min_{\AccuracyGradientModel}&~~~~ Loss\big(\AccuracyGradientModel(\HighImage), \Mask\big),
\label{eq:separate_objective}
\vspace{-0.2cm}
\end{align}
}
where $Loss$ is a loss function that measures the distance between $\AccuracyGradientModel(\HighImage)$ (we will specify the concrete form of loss in \S\ref{subsec:loss}).
Thus, the overall objective can be written as:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\max_{\Mask} &~~~~\SimFunc\bigg(\DNN \big(\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage \big),\DNN(\HighImage)\bigg) \nonumber\\
\min_{\AccuracyGradientModel}&~~~~ Loss\big(\AccuracyGradientModel(\HighImage), \Mask\big).
\label{eq:idealized-objective}
\end{align}
}
\mypara{Ground truth generation of \Mask}
To get a closed-form approximation of \Mask, notice that $\textrm{max}  ~~ \SimFunc(\DNN(\Image), \DNN(\HighImage))$ (where $\Image=\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage$)
is equivalent to the following (note that the first term of Eq~\ref{eq:objective} is a constant to $\Mask$). Thus, the first objective can be rewritten as:



% To this end, we first rewrite the objective of the idealized algorithm in Eq (\ref{eq:idealized-objective}) $\textrm{max}  ~~ \SimFunc(\DNN(\Image), \DNN(\HighImage))$ (where $\Image=\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage$)
% as follows: (note that the first term of Eq~\ref{eq:objective} a constant to $\Mask$):

{\footnotesize
\vspace{-0.2cm}
\begin{align}
\textrm{min} ~~~~ & \SimFunc(\DNN(\AllOnes\times\HighImage), \DNN(\HighImage))-\SimFunc(\DNN(\Image), \DNN(\HighImage)) \label{eq:objective}\\
= & \bigg\langle\frac{\partial \SimFunc(\DNN(\Image'), \DNN(\HighImage))}{\partial \Image'},(\AllOnes\times\HighImage - \Image)\bigg \rangle_{\textrm{F}} \label{eq:lagrange}\\
\approx & \bigg\langle\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage},(\AllOnes\times\HighImage - \Image)\bigg\rangle_{\textrm{F}} \label{eq:relax} \\
= & \bigg\langle\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage},(\AllOnes-\Mask)\times(\HighImage-\LowImage)\bigg\rangle_{\textrm{F}}, \label{eq:temp}
\end{align}
}
where $\langle\cdot,\cdot\rangle_{\textrm{F}}$ is the Frobenius inner product. 
Eq (\ref{eq:lagrange}) uses Lagrange's Mean Value Theorem, where $\Image'$ lies between $\HighImage$ and $\Image$. In Equation (\ref{eq:temp}), since the value of $\Mask$ is identical inside each block, each block $(x,y)$ contributes the following value to Eq (\ref{eq:temp}):

{\footnotesize
\vspace{-0.2cm}
\begin{align}
& (1-\Mask_{x,y})\bigg\langle\sum_{(i,j)\in block_{x,y}} \frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}, (\HighImage_{i,j}-\LowImage_{i,j})\bigg\rangle_{\textrm{F}}\nonumber\\
\leq & \delta \cdot (1-\Mask_{x,y}) \cdot \sum_{(i,j)\in block_{x,y}} \bigg\Vert\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_1 \nonumber \\
= & \delta \cdot (1-\Mask_{x,y}) \cdot \AccuracyGradient_{x,y}.
\label{eq:temp3}
\end{align}
}
where $\delta$ denotes the maximum absolute value in $\HighImage_{i,j}-\LowImage_{i,j}$.
To minimize Eq~\ref{eq:temp3}, we have:

{
\vspace{-0.2cm}
\footnotesize
\begin{align}
\Mask^*_{x,y} =  top_c\big[\AccuracyGradient_{x,y}\big],
\label{eq:temp3}
\end{align}
}
where $top_c$ converts the top-$c$-largest elements in the matrix to $1$ and all other elements to $0$.

Thus, we can use $\Mask^*$ as the {\em ground truth} to train \AccuracyGradientModel.

\mypara{Training cost reduction analysis}
By generating the ground truth first and then training \AccuracyGradientModel, we only need to access the final DNN while generating the ground truth. Thus, the overhead of accessing the final DNN is now $1\times$, a $15\times$ reduction compared to training \AccuracyGradientModel through Eq~\ref{eq:idealized-objective}.


% This upper bound holds when the gradient of $\SimFunc(\DNN(\Image), \DNN(\HighImage))$ at $\Image$ is non-negative at all pixels in the block, which is a reasonable assumption since changing pixel values closer to the high quality encoding will likely make the inference result more similar to $\DNN(\Image)$.
% Now we assume lowering the encoding quality at every pixel will always lower the accuracy, thus Equation (\ref{eq:temp2}) is bounded by:
% \begin{align}
% &(1-\Mask_{x,y}) \nonumber\\
% \times&\bigg(\sum_{(i,j)\in block_{x,y}} \bigg\Vert\frac{\partial \SimFunc(\DNN(\Image), \DNN(\HighImage))}{\partial \Image}\bigg|_{i,j}\bigg\Vert_2\bigg) \nonumber\\
% \times& \bigg(\sum_{(i,j)\in block_{x,y}}\big\Vert\HighImage_{i,j}-\LowImage_{i,j}\big\Vert_2\bigg)
% \label{eq:temp3}
% \end{align}


% \mypara{Accuracy gradients (\Ags)} 
% From Eq (\ref{eq:temp3}), we can see that the key to approximating the optimal solution is the following value, which we call {\em accuracy gradients} or {\em \ag}, at each block $(x,y)$:

% {\footnotesize
% \begin{align}
% \AccuracyGradient(\LowImage)_{x,y} = \sum_{(i,j)\in block_{x,y}}\bigg\Vert\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_1.
% % \bigg\Vert\frac{\partial{\AccuracyFunc\circ \DNN(\textbf{V}), gt)}}{\partial \textbf{V}} \bigg|_{i,j}\bigg\Vert_2 \label{eq:acc-gradients}
% \end{align}
% }
% % which is essentially the gradients of the accuracy evaluation function at the point of specific encoding $\Image$. 
% %Given its importance, we call it the {\em accuracy gradients} or {\em \ag}.
% %Since the calculation of \ag in Eq (\ref{eq:acc-gradients}) still runs the DNN inference on the frame,

% In \S\ref{sec:training}, we will train a light-weight NN model to infer the block-level \ag values for each given frame.
% % \jc{question: is the accuracy gradient matrix same size of the grids or the image?}

% \myparashort{Rationale behind \ags}is three-fold:
% %The rationale of \ags is three-fold.
% \begin{packeditemize}
% \item \Ags naturally indicate which blocks should be in high quality. 
% If a block $(x,y)$ has a high value $\AccuracyGradient(\LowImage)_{x,y}$, then in order to minimize Eq (\ref{eq:objective}), $\Mask_{x,y}$ should be set to 1 (high quality); otherwise, $\Mask_{x,y}$ should be 0 (low quality).
% %The quality assignments based on the accuracy gradients preserve similar performance improvement as the idealized algorithm in \S\ref{subsec:idealized}. 
% %Figure~\ref{??} shows the quality assignment based on the idealized algorithm and the assignment based on accuracy gradients. 
% %We can see that in both assignments, \fillme
% %\jc{maybe a visualization?}
% \item \Ags are more amenable to learning than the binary masks returned by the idealized algorithm (\S\ref{subsec:idealized}), which frequently flip between 0 and 1 between neighboring blocks.
% %Ideally, we want to directly infer the binary masks returned by the idealized algorithm. 
% %However, these masks can flip between 0 and 1 frequently across neighboring blocks, making it hard to infer at times. 
% %The idealized algorithm can sometimes be very sensitive to \fillme, which gives rise to the quality assignment that changes frequently even between neighboring blocks, which can be prohibitively difficult to train the accuracy-gradient model on.
% In contrast, we found that the \ags have higher locality (nearby blocks have similar \ags). % and thus easier to learn with a small model.
% This is also supported by recent deep learning theories~\cite{xu2019frequency,xu2019training}.
% {\em This is why \name trains a shallow model to learn the \ag matrix, rather than the optimal binary mask.}
% \item \Ags share similar spirit with the widely used concept of saliency maps in the computer vision, but there is key distinction.
% While saliency indicates which regions have more influence on the DNN output, \ags indicate how much a change of a block's {\em encoding quality} brings the DNN output closer to the output on the original frame.
% %\item In addition, assigning quality by blocks still aligns with the (microblocks) used in classic codecs (H.264/265).
% %\jc{why not pixel level? our blocks align with the basic spatial units (microblocks) used in classic codecs like H.264/265.}
% \end{packeditemize}

\subsection{Hierarchical loss function}
\label{subsec:loss}



In training the \AccuracyGradientModel, \name uses the following loss function:
% \jc{equation}

{\footnotesize
\begin{align}
    \sum_{\lambda\in \Lambda} CrossEntropy(\AccuracyGradientModel(\RawImage), \mathbbm{1}(\AccuracyGradient(\LowImage) > \lambda)) \label{eq:loss-function}
\end{align}
}
where $\AccuracyGradientModel$ is the trained \AccuracyGradientModel, $\mathbbm{1}(\cdot)$ is the indicator function, $\RawImage$ is the original frame available before encoding, and $\Lambda$ is a set of thresholds with a logarithmic scale (in our experiment, we used 0.1 and 0.01).

While cross entropy loss is commonly used in deep learning, this particular form of loss function entails two design choices.


First, 
% thresholds ($\lambda$) tackle the imbalanced value distribution in $\AccuracyGradient(\LowImage)$.
$\AccuracyGradient(\LowImage)$ contains mostly low values (zeros or close to 0) while the some useful values are large ones, so if we use the traditional cross entropy loss (or mean square error) between $\AccuracyGradientModel$ and $\AccuracyGradient$ as the objective function, the resulting model will tend to produce mostly zeros. 
So to combat the data imbalance issue, we use a series of 
% In fact, the values in $\AccuracyGradient(\LowImage)$ roughly follow a log-normal distribution, 
%so in order to learn values at each percentile of the distribution, 
% we set a series of 
thresholds $\lambda$ at a logarithmic scale ($\AccuracyGradient(\LowImage)$ empirically follow a mixture of log-normal distributions), so that it explicitly teaches the $\AccuracyGradientModel$ model  to learn \ag values at each log scale. 
Though the use of these threshold is motivated by the log-normal-like shape of \ag values, it is effective at tackling the imbalance in the \ag distributions.
(While the same effect can be achieved by using the normal cross entropy over logarithmic \ag values, it is not feasible since many \ag values are zeros.)
%and does not depend on whether \ag values strictly follow a log-normal distribution. 
% We have found them to be effective at tackling the imbalance of saliency values.
% \jc{kuntai, why not just log the values first and then train it with normal cross entropy? is it because there are lots of zeros?}

Second, this loss function regulates \AccuracyGradientModel provides a hierarchical ground truths $\{\mathbbm{1}(\AccuracyGradient(\LowImage) > \lambda))\}_{\lambda in \Lambda}$ that enables \AccuracyGradientModel to learn a smooth transition from high \AccuracyGradient microblocks to low \AccuracyGradient microblocks. This will enable \AccuracyGradientModel to change the file size and accuracy smoothly when changing the two encoding parameters \AgThresh and \AreaThresh (defined in \S\ref{subsec:quality-assignment}).



% \jc{why $\AccuracyGradientModel$ is applied on $\HighImage$. To get more features}

% To see the reason behind this choice, let us first consider some other seemingly reasonable ones.

% 1. MSE
% $$
% \Vert \AccuracyGradientModel(\HighImage), \AccuracyGradient(\LowImage) \Vert_2^2
% $$
% \jc{accuracy gradient values are highly unbalanced, so MSE will tend to generate a all-zero mask, because most elements are small. in contrast, crossentropy will use $\lambda$ to filter out ??}

% 2. Cross entropy loss

% \begin{align*}
%     CrossEntropy(\AccuracyGradientModel(\HighImage), \AccuracyGradient(\LowImage))
% \end{align*}

% How to choose the threshold $\lambda$?
% The gradients in $\AccuracyGradient(\HighImage)$ follows a normal distribution in the logscale space.


% \jc{this is the place to show your lessons learned from prior tries of various loss functions}

% \jc{explain why not training a binary mask generator directly?}

% \jc{emphasize that we give more penalty to false negative than false positive}

%\begin{itemize}
%\item problem formulation: what to learn. how is it diff to region-proposal, background detection, etc
%\item problem 1: choice of labels (or loss function)
%\item strawman: \fillme. why it should work and why it didn't work
%\item our solution: 
%\item problem 2: choice of model architecture
%\item why not a custom model
%\item why vgg? any connection with classification
%\item choice of training data: same as the dnn (or user-defined)
%\end{itemize}



% \mypara{Training data}
% \name provides two options to obtain the training data of the accuracy-gradient model $\AccuracyGradientModel$. 
% \begin{packeditemize}
% \item First, the operator who provides the full DNN may share its training dataset (in many cases, this is a public dataset such as COCO or ImageNet).
% This way, the $\AccuracyGradientModel$ is trained on the same data the final DNN was trained on.\footnote{The intuition is that if the $\AccuracyGradientModel$ has a comparable complexity of the final DNN, then in theory, if $\AccuracyGradientModel$ is trained on the same dataset as the final DNN, it can very closely approximate the process of \ag calculation of Eq (\ref{eq:acc-gradients}).
% Thus when $\AccuracyGradientModel$ is based on a compact model, any error made by $\AccuracyGradientModel$ is likely caused by the model architecture, rather than any training data biases.
% Of course, this reasoning is no rigorous proof, but in lack of a dataset customized for training \AccuracyGradientModel, we believe this is a reasonable choice (as shown in \S\ref{sec:eval}). }
% \item An alternative choice of training data, sometimes used in prior work (~\cite{reducto,noscope}), is to train the \AccuracyGradientModel based on the frames sampled from the test video steam. 
% A benefit of this approach is that these sampled frames might share a similar data distribution with the real video stream. 
% \end{packeditemize}
% We will show the effectiveness of both choices in \S\ref{subsec:eval:micro}.




\subsection{Fast customization through transfer learning}

Nowadays, the server-side analytic DNN needs to frequently update itself to integrate latest computer vision techniques for better performance.
As a result, \name need to quickly customize its \AccuracygradientModel to cope with the new vision model.

Instead of training  \AccuracyGradientModel from scratch, we start from our \AccuracyGradientModel pretrained from the old server-side model and finetune it on the new server-side DNN.
The rationale behind this finetuning is two-fold:
\begin{packeditemize}
    \item A common design practice in computer vision community is to build new vision models based on those widely-used pretrained feature extractor~\cite{gao2021recent}. 
    As a result, the old server-side model and the new server-side model may share a common feature extractor.
    Thus, the \AccuracyGradientModel for the old model may somehow indirectly learn to preserve the fidelity of the features extracted from the feature extractor and thus may be useful for the new vision model.
    \item Even when the feature extractor of the new model is completely different from the old model, the last few layers of \AccuracyGradientModel also learns how to filter out the useless information and this experience is also useful for the \AccuracyGradientModel to handle new vision model.
\end{packeditemize}

By finetuning, the customization time of \name is within several minutes (see \S\ref{sec:eval} for further details).

==> technical.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\section{\hspace{-0.2cm}Towards a new video stack for video analytics}
\section{Overview of \name}
\label{sec:framework}

The previous section shows a substantial room for improvement by allocating quality level to fine-grained blocks. % based on how much impact each block has on the final DNN inference. 
A natural question then is how to build a concrete system to realize the benefits.
In this section, we derive the concept of accuracy gradients and sketch a near-optimal video stack based on accuracy gradients.
% begin with \kt{the choice of our accuracy function, followed by} an optimization framework for such a video stack  and introduce the key ideas behind our design. 

\begin{comment}
\subsection{Choosing accuracy function}
\kt{Feel that we need to add this part.}

Most of the evaluation metrics for vision applications (\eg mean average precision for object detection~\cite{coco}) is not differentiable, which prevent us to leverage the differentiability of the final DNN to further optimize accuracy.

To address this issue, we notice that at training stage, each neural network will minimize a {\em differentiable training loss} to maximize accuracy. Thus, we take the negative training loss of our accuracy function \SimFunc to derive the following insight.

% \tightsubsection{\hspace{-0.2cm}Framework for optimal quality assignment}

\end{comment}

\subsection{Accuracy gradients}
\label{subsec:ag}

The idealized algorithm introduced in \S\ref{subsec:idealized} requires running the final DNN multiple times on different encoded videos. 
To make it practical, 
%one needs to determine the quality assignment without running the DNN; instead, it 
one needs to ``derive'' the quality assignment from the pixel values of a frame.
%Formally, this problem can be framed in the following optimization problem.
%\jc{kuntai, please fill the formulation in here. please start from the formula of the idealized design point}
%\mypara{Optimization framework}
%To this end, we first rewrite the objective of the idealized algorithm in Eq (\ref{eq:idealized-objective}) (let $\Image=\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage,$ be the optimal solution) to minimizing the following value (the first term is independent on $\Mask$):
To this end, we first rewrite the objective of the idealized algorithm in Eq (\ref{eq:idealized-objective}) in a differentiable form as follows.
We notice that $\textrm{max}  ~~ \SimFunc(\DNN(\Image), \DNN(\HighImage))$ (where $\Image=\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage$)
is equivalent to the following (note that the first term of Eq~\ref{eq:objective} a constant to $\Mask$):


% To this end, we first rewrite the objective of the idealized algorithm in Eq (\ref{eq:idealized-objective}) $\textrm{max}  ~~ \SimFunc(\DNN(\Image), \DNN(\HighImage))$ (where $\Image=\Mask\times\HighImage+(\AllOnes-\Mask)\times\LowImage$)
% as follows: (note that the first term of Eq~\ref{eq:objective} a constant to $\Mask$):

{\footnotesize
\vspace{-0.2cm}
\begin{align}
\textrm{min} ~~~~ & \SimFunc(\DNN(\AllOnes\times\HighImage), \DNN(\HighImage))-\SimFunc(\DNN(\Image), \DNN(\HighImage)) \label{eq:objective}\\
= & \bigg\langle\frac{\partial \SimFunc(\DNN(\Image'), \DNN(\HighImage))}{\partial \Image'},(\AllOnes\times\HighImage - \Image)\bigg \rangle_{\textrm{F}} \label{eq:lagrange}\\
\approx & \bigg\langle\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage},(\AllOnes\times\HighImage - \Image)\bigg\rangle_{\textrm{F}} \label{eq:relax} \\
= & \bigg\langle\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage},(\AllOnes-\Mask)\times(\HighImage-\LowImage)\bigg\rangle_{\textrm{F}}, \label{eq:temp}
\end{align}
}
where $\langle\cdot,\cdot\rangle_{\textrm{F}}$ is the Frobenius inner product. 
Eq (\ref{eq:lagrange}) uses Lagrange's Mean Value Theorem, where $\Image'$ lies between $\HighImage$ and $\Image$. In Equation (\ref{eq:temp}), since the value of $\Mask$ is identical inside each block, each block $(x,y)$ contributes the following value to Eq (\ref{eq:temp}):
{\footnotesize
\vspace{-0.2cm}
\begin{align}
& (1-\Mask_{x,y})\bigg\langle\sum_{(i,j)\in block_{x,y}} \frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}, (\HighImage_{i,j}-\LowImage_{i,j})\bigg\rangle_{\textrm{F}}\nonumber\\
\leq & \delta \cdot (1-\Mask_{x,y}) \cdot \sum_{(i,j)\in block_{x,y}} \bigg\Vert\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_2, \label{eq:temp3}
\end{align}
}
where $\delta$ denotes the maximum element in $\HighImage_{i,j}-\LowImage_{i,j}$.
This upper bound holds when the gradient of $\SimFunc(\DNN(\Image), \DNN(\HighImage))$ at $\Image$ is non-negative at all pixels in the block, which is a reasonable assumption since changing pixel values closer to the high quality encoding will likely make the inference result more similar to $\DNN(\Image)$.
% Now we assume lowering the encoding quality at every pixel will always lower the accuracy, thus Equation (\ref{eq:temp2}) is bounded by:
% \begin{align}
% &(1-\Mask_{x,y}) \nonumber\\
% \times&\bigg(\sum_{(i,j)\in block_{x,y}} \bigg\Vert\frac{\partial \SimFunc(\DNN(\Image), \DNN(\HighImage))}{\partial \Image}\bigg|_{i,j}\bigg\Vert_2\bigg) \nonumber\\
% \times& \bigg(\sum_{(i,j)\in block_{x,y}}\big\Vert\HighImage_{i,j}-\LowImage_{i,j}\big\Vert_2\bigg)
% \label{eq:temp3}
% \end{align}


\mypara{Accuracy gradients (\Ags)} 
From Eq (\ref{eq:temp3}), we can see that the key to approximating the optimal solution is the following value, which we call {\em accuracy gradients} or {\em \ag}, at each block $(x,y)$:

{\footnotesize
\begin{align}
\AccuracyGradient(\LowImage)_{x,y} = \sum_{(i,j)\in block_{x,y}}\bigg\Vert\frac{\partial \SimFunc(\DNN(\LowImage), \DNN(\HighImage))}{\partial \LowImage}\bigg|_{i,j}\bigg\Vert_2. \label{eq:acc-gradients}
% \bigg\Vert\frac{\partial{\AccuracyFunc\circ \DNN(\textbf{V}), gt)}}{\partial \textbf{V}} \bigg|_{i,j}\bigg\Vert_2 \label{eq:acc-gradients}
\end{align}
}
% which is essentially the gradients of the accuracy evaluation function at the point of specific encoding $\Image$. 
%Given its importance, we call it the {\em accuracy gradients} or {\em \ag}.
%Since the calculation of \ag in Eq (\ref{eq:acc-gradients}) still runs the DNN inference on the frame,

In \S\ref{sec:training}, we will train a light-weight NN model to infer the block-level \ag values for each given frame.
% \jc{question: is the accuracy gradient matrix same size of the grids or the image?}

\myparashort{Rationale behind \ags}is three-fold:
%The rationale of \ags is three-fold.
\begin{packeditemize}
\item \Ags naturally indicate which blocks should be in high quality. 
If a block $(x,y)$ has a high value $\AccuracyGradient(\LowImage)_{x,y}$, then in order to minimize Eq (\ref{eq:objective}), $\Mask_{x,y}$ should be set to 1 (high quality); otherwise, $\Mask_{x,y}$ should be 0 (low quality).
%The quality assignments based on the accuracy gradients preserve similar performance improvement as the idealized algorithm in \S\ref{subsec:idealized}. 
%Figure~\ref{??} shows the quality assignment based on the idealized algorithm and the assignment based on accuracy gradients. 
%We can see that in both assignments, \fillme
%\jc{maybe a visualization?}
\item \Ags are more amenable to learning than the binary masks returned by the idealized algorithm (\S\ref{subsec:idealized}), which frequently flip between 0 and 1 between neighboring blocks.
%Ideally, we want to directly infer the binary masks returned by the idealized algorithm. 
%However, these masks can flip between 0 and 1 frequently across neighboring blocks, making it hard to infer at times. 
%The idealized algorithm can sometimes be very sensitive to \fillme, which gives rise to the quality assignment that changes frequently even between neighboring blocks, which can be prohibitively difficult to train the accuracy-gradient model on.
In contrast, we found that the \ags have higher locality (nearby blocks have similar \ags). % and thus easier to learn with a small model.
This is also supported by recent deep learning theories~\cite{xu2019frequency,xu2019training}.
{\em This is why \name trains a shallow model to learn the \ag matrix, rather than the optimal binary mask.}
\item \Ags share similar spirit with the widely used concept of saliency maps in the computer vision, but there is key distinction.
While saliency indicates which regions have more influence on the DNN output, \ags indicate how much a change of a block's {\em encoding quality} brings the DNN output closer to the output on the original frame.
%\item In addition, assigning quality by blocks still aligns with the (microblocks) used in classic codecs (H.264/265).
%\jc{why not pixel level? our blocks align with the basic spatial units (microblocks) used in classic codecs like H.264/265.}
\end{packeditemize}


\subsection{\Ag-based quality assignment}
\label{subsec:quality-assignment}

Given the matrix of \ags of a frame, \name then uses one of two parameters to decide which blocks in a frame should be encoded in high quality: 
\begin{packeditemize}
\item {\em \Ag threshold $\AgThresh$} means all blocks $(x,y)$ with $\AccuracyGradient(\LowImage)_{x,y}\geq\AgThresh$ will be encoded in high quality.
%\name picks a subset of blocks whose \ags based on Eq (\ref{eq:acc-gradients}) are over $\AgThresh$.
\item {\em High-quality area threshold $\AreaThresh$} sets the maximum number of high-quality blocks, by simply picking the top $\AreaThresh$ blocks with the highest \ags.
%\name picks the top $\AreaThresh$ blocks with the highest \ags.
\end{packeditemize} 
After a set of blocks are selected, \name then 
% the block-padding scale $\PadThresh$ to 
expands these selected blocks to each direction by $\PadThresh$ (by default 3) blocks (if they are not already selected).

Both $\AgThresh$ and $\AreaThresh$ allow users to navigate \name's accuracy-compression tradeoffs (lower $\AgThresh$ or higher $\AreaThresh$ increases the accuracy at the expense of encoding more blocks).
However, they have very different practical implications.
\begin{packeditemize}
\item When the \ag threshold $\AgThresh$ is set to a fixed value, \name will assign high quality to {\em all} low \ag blocks.
In effect, it {\em adapts the compression rate to content}, \eg when content is simple, it will compress more aggressively.
\item When the high-quality area threshold $\AreaThresh$ is set to a fixed value, \name will assign high quality to a {\em fixed} number of blocks.
As a result, it {\em adapts the accuracy to a target compression rate}.
\end{packeditemize} 
At a high level, the effects of $\AgThresh$ and $\AreaThresh$ in \name are analogous to variable bitrate (VBR) and constant bitrate (CBR) encoding (one adapts to content and one maintains constant bitrate).
However, we acknowledge that $\AgThresh$ and $\AreaThresh$ in our design do not directly tie to a target accuracy or fixed bitrate, which we will discuss in \S\ref{sec:discuss}.
Nonetheless, we will demonstrate how they can help adaptive streaming in \S\ref{subsec:eval:adaptive}.

%while minimizing compressed video size. 
%In contrast, the high-quality area threshold $\AreaThresh$ can be used to {\em control compressed video size} while maximizing accuracy. 

%\jc{can't control directy, but effective}

% In practice, we found tuning them result in a similar frontier of accuracy/compression tradeoffs, so we expose $\AgThresh$ as a tunable parameter to users (just as QP in MPEG/H.264) and empirically set $\PadThresh$ at 2 by default.


%it is straightforward to derive the optimal quality assignment on the given frame.
%\jc{Kuntai, please give the derivation}
%Recall that only $c$-many blocks will be encoded in high quality, we just need to pick $c$-many blocks with largest accuracy gradient value, encode them in high quality and encode remaining blocks in low quality.



\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{figs/overall-workflow.pdf}
    \tightcaption{Architecture and three phases of \name.}
    \label{fig:workflow}
    \vspace{-3mm}
\end{figure}

\subsection{Workflow of \name}

Figure~\ref{fig:workflow} depicts \name's workflow and the three APIs:

% \vspace{0.1cm}
% {\footnotesize
% \noindent
% {\bf \texttt{ag\_model = prepare(dnn\_func,acc\_func)}}\\
% {\bf \texttt{encoded\_video = ingest(ag\_model,*raw\_frame,param)}}\\
% {\bf \texttt{result = consume(encoded\_video,dnn)}}
% \vspace{0.1cm}
% }

\mypara{Preparation}
The analyst provides \name the final DNN with its accuracy function ({\footnotesize{\bf \texttt{acc\_func}}}), and \name trains a customized {\em \AccuracyGradientModel} ({\footnotesize{\bf \texttt{ag\_model}}}), which will predict the \ags on any new frame. 
%(similarity between DNN outputs on the high-quality frame and on the low-quality encoding)
%The accuracy function takes DNN's outputs on the high quality encoding and on the low quality encoding of a frame as input, and returns the similarity between them (which indicates accuracy as defined in \S\ref{??}).
%the accuracy of running the DNN on the encoded frame with respect to the result of running the DNN on the high quality image as the ``ground truth''. 
Optionally, the operator also provides a dataset to train the \AccuracyGradientModel; otherwise, \name can learn the \AccuracyGradientModel on a pre-determined number of video frames from the real video stream. 
We evaluate these choices in \S\ref{subsec:eval:micro}.
%As elaborated in \S\ref{??}, the choice of training data involves a tradeoff between accuracy-gradient model performance and real-time overhead. 

\vspace{0.1cm}
{\footnotesize
\noindent
{\bf \texttt{ag\_model = prepare(dnn\_func,acc\_func)}}
}

\mypara{Encoding} 
On each input frame, \name runs the customized \AccuracyGradientModel to get the \ag per block. 
The analyst can use the thresholds of $\AgThresh$ or $\AreaThresh$ ({\footnotesize{\bf \texttt{param}}}) to decide the quality assignment according to \S\ref{subsec:quality-assignment}.
% By setting the parameters, users can select tradeoff between accuracy and compression efficiency (file size). 
%The encoded video will then be saved together with a metafile that includes the quality assignment information.
Compared to H.264, a straightforward implementation of the encode function would involve an additional \AccuracyGradientModel model inference and multiple the encoding passes. 
\S\ref{sec:runtime} will discuss how \name reduces these additional overheads. 

\vspace{0.1cm}
{\footnotesize
\noindent
{\bf \texttt{encoded\_video = encode(ag\_model,*frame,param)}}
}

\mypara{Decoding}
Finally, \name decodes the video frames 
%and use the quality assignment information in the metafile to overlay the decoded high quality blocks on the low quality one. 
%The resulting frames are 
and then feed them to the DNN for inference whenever needed.
%As an further optimization to reduce inference time, the DNN can also use the quality sensitivity information in the metafile to filter out regions that are very unlikely to have useful information (\eg background).

\vspace{0.1cm}
{\footnotesize
\noindent
{\bf \texttt{result = decode(encoded\_video,dnn)}}
\vspace{0.1cm}
}

Though the workflow sketched in Figure~\ref{fig:workflow} is functionally sufficient,
%to encode videos with spatially different quality based on the notion of accuracy gradients, 
two challenges remain: 
(1) how to learn an accurate \AccuracyGradientModel (\S\ref{sec:training}); and (2) how to use it in real time for high accuracy and low encoding/decoding overhead (\S\ref{sec:runtime}).
We will address them in the next two sections.


%\begin{itemize}
%\item why the idealized design is impractical => automatically generating the quality assignment 
%\item an optimization framework for accuracy/compression tradeoffs
%\item key notion: a saliency map based on accuracy gradients
%\item why is it unique (diff to traditional saliency). aware of hq-lq diff
%\item why accuracy gradients naturally give rise to the three opportunities.
%\item walk-through an example (with API)
%\item challenges: (1) how to learn an accurate generator of accuracy gradients; and (2) how to use it in real time for high accuracy and low encoding/decoding overhead
%\item intuitively, why this problem is much simpler than final DNN. 
%\end{itemize}





%\section{Design of \name}


\section{Learning accuracy gradients in \name}
\label{sec:training}




\begin{comment}
First, it may be tempting to use an off-the-shelf background detector, a region proposal network or a segmentation network as the \AccuracyGradientModel. 
However, the \ag of a block indicates how much the inference result would change if the pixels in the block change from low quality encoding to high quality encoding, so  a small \ag does not necessarily mean the block is in the background (maybe part of an object that can be detected under both high and low quality).


However, the goal of an \AccuracyGradientModel differ in several aspects.
%First, the goal of an \AccuracyGradientModel may look similar to that of a background detector, a region proposal network or a segmentation network. However, they differ in several key aspects.
First, an \AccuracyGradientModel's output is per block, not per pixel, which has implications.
The \ag of a block indicates how much the inference result would change if the pixels in the block change from low quality encoding to high quality encoding. 
In other words, it captures both the importance of a region to the inference results and the magnitude of pixel value changes between different quality levels.
Thus, a low accuracy gradient does not necessarily mean the block is in the background (\eg part of an object that can be detected under both high and low quality).
In short, the accuracy-gradient model cannot directly reuse off-the-shelf models.
\end{comment}

%\jc{give a few examples, back ref to section 3}

Next, we present the design of the \AccuracyGradientModel architecture, loss function, and training data; and discuss the rationale of our design choices.


\subsection{Model architecture}

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/vgg11.pdf}
    \tightcaption{Schematic architecture of our \AccuracyGradientModel, where ``conv'' is convolution and ``pool'' is max pooling. }
    \label{fig:vgg11}
\end{figure}

% It is important to notice that the \ag of a block indicates how much the inference result would be changed by a change of the block's encoding quality.
% Thus, 
It is important to notice that the high-\ag blocks (as shown in \S\ref{subsec:analysis}) can be frequently misaligned with detection results (the bounding boxes or edges of objects).
As a result, we do not design the \AccuracyGradientModel based on region-proposal networks or cheap object detector (which are used in prior work that will be compared against in \S\ref{sec:eval}).
Instead, we use a custom shallow NN based on VGG11 as the architecture of the \AccuracyGradientModel. 
Figure~\ref{fig:vgg11} shows the model architecture.
% \jc{a few highlights on the model?}

The choice of this architecture is based on two reasons.
% On one hand, 
First, this model is much more compact than the alternatives that are still based on fully convolutional (FC) feature extractors.
To put it into perspective, our \AccuracyGradientModel has 160 GFLOPs, an 3.5x reduction compared to the typical cheap convolutional models (such as ResNet50), which contain 550 GFLOPs.
%\jc{any other metrics}
In addition, since the architecture in Figure~\ref{fig:vgg11} consists only of FC operations (in addition to a few batch normalization and activation), its computational overhead is proportional to the size of the input frame (\eg $4\times$ faster when the frame size is reduced by $2\times$ in each dimension). 
% On the other hand, 
% we have intuitive reasons (in addition to the empirical results in \S\ref{sec:eval}) to believe this architecture suffices to learn the task.
Second, we use this model,
% this architecture suffices to learn \ag values, 
because inferring \ags is functionally similar to running semantic segmentation on a low resolution image, to which FC operation is a natural fit~\cite{long2015fully}.
Moreover, compared to traditional segmentation tasks (where each label can be one of hundreds of classes), our task essentially assigns a binary label to each block: ultimately, the \AccuracyGradientModel output is not evaluated by how accurately each \ag is inferred, but whether the right set of blocks are selected to encode in high quality.\footnote{At first glance, it does appear that the \AccuracyGradientModel needs to approximate a highly complex mathematical procedure: after all calculating \ags in Eq (\ref{eq:acc-gradients}) involves the full DNN.
However, we believe this is not far fetched.
The matrix of \ag is mathematically the saliency of a DNN, and there is recent work in deep learning (\eg~\cite{dabkowski2017real}) that proposes relatively shallow models that quickly infer saliency of an arbitrary differentiable image classifier.
An intuitive explanation is that saliency inference is often used for purposes that do not depend on precise estimation of saliency on each pixel (\eg DNN interpretation or video encoding in our case), so they are inherently more tolerant to error than the task of the final DNN.
}
%our quality assignment only depends on whether accuracy gradient of a block is over a given threshold.

% We acknowledge that it is possible to design a custom DNN architecture for our \AccuracyGradientModel and train it from scratch.
That being said, our goal here is not to choose the ``optimal'' architecture; rather, \name takes a pragmatic choice of fine-tuning a pretrained VGG11~\cite{pytorch-model-zoo}, which can be done more efficiently than training a custom DNN model from scratch.
We will evaluate its inference and training cost in \S\ref{sec:eval}.

% rather, we want a light-weight \AccuracyGradientModel that is accurate enough to identify which regions should be in high quality.
% In designing the model, \name takes a pragmatic choice of fine-tuning a pretrained VGG11 model~\cite{pre-train model link}  which can be faster and more data efficient than training a clean-slate model in practice.


% \jc{why not customized model architecture?}


%On the other hand, any smaller model will have a CNN feature extractor smaller than most of the common ones, so one has to customize the model architecture and train the model from scratch. 
% \jc{1. it's easier than detection, etc
% 2. it's functionally similar to segmentation on a low-resolution image, and FC is known to be a good fit to segmentation.}
% \jc{explain please?}









\subsection{Loss function}
\label{subsec:loss}

In training the \AccuracyGradientModel, \name uses the following loss function:
% \jc{equation}

{\footnotesize
\begin{align}
    \sum_{\lambda\in \Lambda} CrossEntropy(\AccuracyGradientModel(\RawImage), \mathbbm{1}(\AccuracyGradient(\LowImage) > \lambda)) \label{eq:loss-function}
\end{align}
}
where $\AccuracyGradientModel$ is the trained \AccuracyGradientModel, $\mathbbm{1}(\cdot)$ is the indicator function, $\RawImage$ is the original frame available before encoding, and $\Lambda$ is a set of thresholds with a logarithmic scale (in our experiment, we used 0.1, 0.01, 0.001, etc).

While cross entropy loss is commonly used in deep learning, this particular form of loss function entails two design choices.
First, 
% thresholds ($\lambda$) tackle the imbalanced value distribution in $\AccuracyGradient(\LowImage)$.
$\AccuracyGradient(\LowImage)$ contains mostly low values (zeros or close to 0) while the some useful values are large ones, so if we use the traditional cross entropy loss (or mean square error) between $\AccuracyGradientModel$ and $\AccuracyGradient$ as the objective function, the resulting model will tend to produce mostly zeros. 
So to combat the data imbalance issue, we use a series of 
% In fact, the values in $\AccuracyGradient(\LowImage)$ roughly follow a log-normal distribution, 
%so in order to learn values at each percentile of the distribution, 
% we set a series of 
thresholds $\lambda$ at a logarithmic scale ($\AccuracyGradient(\LowImage)$ empirically follow a mixture of log-normal distributions), so that it explicitly teaches the $\AccuracyGradientModel$ model  to learn \ag values at each log scale. 
Though the use of these threshold is motivated by the log-normal-like shape of \ag values, it is effective at tackling the imbalance in the \ag distributions.
(While the same effect can be achieved by using the normal cross entropy over logarithmic \ag values, it is not feasible since many \ag values are zeros.)
%and does not depend on whether \ag values strictly follow a log-normal distribution. 
% We have found them to be effective at tackling the imbalance of saliency values.
% \jc{kuntai, why not just log the values first and then train it with normal cross entropy? is it because there are lots of zeros?}

Second, while a natural choice would be to minimize the loss between $\AccuracyGradientModel(\LowImage)$ and $\AccuracyGradient(\LowImage)$, we choose to use $\RawImage$ as the input to $\AccuracyGradientModel$, because the high quality frame $\RawImage$ preserves more information than $\LowImage$, which allows $\AccuracyGradientModel$ to learn and extract more features.
Moreover, $\RawImage$ is available during encoding, whereas to get the $\LowImage$ would require one additional encoding pass.



% \jc{why $\AccuracyGradientModel$ is applied on $\HighImage$. To get more features}

% To see the reason behind this choice, let us first consider some other seemingly reasonable ones.

% 1. MSE
% $$
% \Vert \AccuracyGradientModel(\HighImage), \AccuracyGradient(\LowImage) \Vert_2^2
% $$
% \jc{accuracy gradient values are highly unbalanced, so MSE will tend to generate a all-zero mask, because most elements are small. in contrast, crossentropy will use $\lambda$ to filter out ??}

% 2. Cross entropy loss

% \begin{align*}
%     CrossEntropy(\AccuracyGradientModel(\HighImage), \AccuracyGradient(\LowImage))
% \end{align*}

% How to choose the threshold $\lambda$?
% The gradients in $\AccuracyGradient(\HighImage)$ follows a normal distribution in the logscale space.


% \jc{this is the place to show your lessons learned from prior tries of various loss functions}

% \jc{explain why not training a binary mask generator directly?}

% \jc{emphasize that we give more penalty to false negative than false positive}

%\begin{itemize}
%\item problem formulation: what to learn. how is it diff to region-proposal, background detection, etc
%\item problem 1: choice of labels (or loss function)
%\item strawman: \fillme. why it should work and why it didn't work
%\item our solution: 
%\item problem 2: choice of model architecture
%\item why not a custom model
%\item why vgg? any connection with classification
%\item choice of training data: same as the dnn (or user-defined)
%\end{itemize}



\mypara{Training data}
\name provides two options to obtain the training data of the accuracy-gradient model $\AccuracyGradientModel$. 
\begin{packeditemize}
\item First, the operator who provides the full DNN may share its training dataset (in many cases, this is a public dataset such as COCO or ImageNet).
This way, the $\AccuracyGradientModel$ is trained on the same data the final DNN was trained on.\footnote{The intuition is that if the $\AccuracyGradientModel$ has a comparable complexity of the final DNN, then in theory, if $\AccuracyGradientModel$ is trained on the same dataset as the final DNN, it can very closely approximate the process of \ag calculation of Eq (\ref{eq:acc-gradients}).
Thus when $\AccuracyGradientModel$ is based on a compact model, any error made by $\AccuracyGradientModel$ is likely caused by the model architecture, rather than any training data biases.
Of course, this reasoning is no rigorous proof, but in lack of a dataset customized for training \AccuracyGradientModel, we believe this is a reasonable choice (as shown in \S\ref{sec:eval}). }
\item An alternative choice of training data, sometimes used in prior work (~\cite{reducto,noscope}), is to train the \AccuracyGradientModel based on the frames sampled from the test video steam. 
A benefit of this approach is that these sampled frames might share a similar data distribution with the real video stream. 
\end{packeditemize}
We will show the effectiveness of both choices in \S\ref{subsec:eval:micro}.


\begin{comment}


\subsection{Training data}
\label{subsec:training-data}

\name provides two options to obtain the training data of the accuracy-gradient model $\AccuracyGradientModel$. 
% Like in any ML models, the training data can affect both the accuracy and the generalizability of the accuracy-gradient model. \jc{this is not about generalizability!}
% In designing \name, we provide two options of obtaining the training data.

First, the operator who provides the full DNN may share its training dataset (in many cases, this is a public dataset such as COCO or ImageNet.)
This way, the $\AccuracyGradientModel$ can be trained on the same images that the final DNN was trained on.
% The reasoning of this choice is as follows.
The intuition is that if the $\AccuracyGradientModel$ has a comparable complexity of the final DNN, then in theory, if $\AccuracyGradientModel$ is trained on the same dataset as the final DNN, it can very closely approximate the process of \ag calculation of Eq (\ref{eq:acc-gradients}).
Thus when $\AccuracyGradientModel$ is based on a compact model, any error made by $\AccuracyGradientModel$ is likely caused by the model architecture, rather than any training data biases.
Of course, this reasoning is no rigorous proof, but in lack of a dataset customized for training \AccuracyGradientModel, we believe this is a reasonable choice (as shown in \S\ref{sec:eval}). 
%We show that the resulting model performs reasonably among videos that the final DNN works well.  

%A natural choice of training data is the same dataset used to train the DNN used for final inference. 
%In theory, this choice maximizes generalizability, because \jc{what's the rationale?}

The other choice of training data, sometimes used in prior work (~\cite{reducto,noscope}), is to train the \AccuracyGradientModel based on the frames sampled from the test video steam. 
A benefit of this approach is that these sampled frames might share a similar data distribution with the real video stream. 
We will show the effectiveness of both choices in \S\ref{subsec:eval:micro}.
%In practice, if training data of the full DNN is available, these two approach can be combined: one can first train $\AccuracyGradientModel$ on the operator-provided dataset in the preparation phase, and then fine-tune it with sampled frames from the test video streams. 
%\jc{a sentence to summarize the takeaway from eval}

\end{comment}



\section{Using accuracy gradients in \name}
\label{sec:runtime}

% Even if one successfully trains the accuracy gradient model, the challenge still remains when deploying it as part of a video stack.
% This section will introduce how \name addresses these issues. 


%\mypara{Speeding up encoding}
% Compared to the traditional video encoding, 
If we naively apply \AccuracyGradientModel in video encoding, each frame would involve one (light-weight) DNN inference (\AccuracyGradientModel) and two encoding passes, compared to only one encoding pass in the traditional codec. 
% Likewise, the decoding will involve two decoding processes per frame, instead of one.
In fairness, the computational cost of \name is much lower than some prior work that runs a large DNN on each frame occasionally~\cite{dds,awstream}, and it is not atypical for video analytics pipelines to run a light-weight model~\cite{vigil,canel2019scaling,reducto,glimpse,cloudseg} on each frame.
% object detector~\cite{vigil,canel2019scaling}, vision feature extractor~\cite{reducto}, object tracker~\cite{glimpse}, or super-resolution~\cite{cloudseg} on each frame. 
Nonetheless, the increased computational overheads compared to traditional codecs can hinder \name's deployment in resource-constrained devices.
% 's use as a generic video stack and can hinder its deployment in resource-constrained devices.
\name reduces the additional computational cost in two ways.

\subsection{Persistence of accuracy gradients}

% \kt{Mention enlargement}

\name runs the \AccuracyGradientModel only on sampled frames, rather than on each frame, and reuses it until the next sampled frame. 
The intuition here is that although the \ags do vary across frames, the quality assignment derived from it changes at much longer timescales. 
Figure~\ref{fig:assignment-persistence} shows that even if \name assigns quality per frame, on more than 90\% of the frames, the quality assignment of 90\% of the blocks remains the same in the next 30 frames. 


\begin{figure}
    \centering
    % \includegraphics[width=0.65\columnwidth]{figs/placeholder-assignment-persistence.pdf}
    
    \includegraphics[width=0.4\columnwidth]{figs/persistance.pdf}
    \tightcaption{The high quality blocks generated by more than 90\% of the frames can persist for over 30 consecutive frames.}
    \label{fig:assignment-persistence}
\end{figure}


% \jc{show some empirical evidence that the per-frame masks do evolve slowly}

We speculate that the relatively slow pace of change results from the conservative quality assignment by \name. 
% We speculate that the relatively slow pace of change 
% in quality accuracy-gradient matrix 
% results from the conservative predictions of the \AccuracyGradientModel. % and the relatively coarse granularity of grids.
% of the grids than pixels.
% While regions that must be encoded in high quality do move over time (\eg a moving object), we empirically found that the 
First, empirically we found that the \ag values generated by the \AccuracyGradientModel change smoothly across neighboring blocks.
As a side effect, many blocks surrounding the high-\ag blocks also have high \ag values, which means slightly more regions are encoded in high quality.
Second, \name adds $\gamma$ (by default, 3) blocks to each direction of a high-\ag block, which helps (though to a less extent than the first one) to stabilize the quality assignment.
% the inferred accuracy gradient matrices tend to encode slightly more regions in high quality.
% so even when a block is not assigned to high quality, it is 
% In addition, since the training process (introduced in \S\ref{??}) gives more penalty to false negatives (\fillme) than to false positives (\fillme). 
% As a consequence, the inferred accuracy gradient matrices tend to encode slightly more regions in high quality.
We acknowledge that re-using quality assignment can be problematic when objects move quickly and that these conservative estimates might lead to slightly inflated file sizes (as shown in the Dance dataset in Figure \ref{fig:eval-overall}). 
% Nonetheless, it does make it possible to reuse an accuracy-gradient matrix across neighboring frames.



\begin{figure}
    \centering
    % \includegraphics[width=0.9\columnwidth]{figs/placeholder-uniform-color.pdf}
    
    \includegraphics[width=0.95\columnwidth]{figs/fig10.pdf}
    \tightcaption{\kt{Using low quality to encode the background may introduce spurious objects, while encoding with uniform color will not.}Using uniform color to encode most of the blocks actually improves accuracy compared to using low quality which misleads the DNN to infer spurious results.}
    \label{fig:uniform-color}
\end{figure}

\subsection{Uniformly colored encoding}
\label{subsec:uniform}

% Besides reducing inference frequency of the \ag generator, 
To further reduce the encoding overhead, \name also uses uniform color as the low quality encoding to obviate the need to encode each frame twice (only high quality blocks need to be encoded).
At first sight, it seems to hurt accuracy, 
% but at first sight, this should hurt high accuracy, 
because the low-quality regions now provide no useful information outside the regions encoded in high quality.\footnote{We acknowledge that the two encoding passes could be avoided by using the RoI encoder, but the file size of RoI-encoded video will still be more than setting all non-high quality blocks in uniform coloring. 
% We did not use it since it is no longer readily supported in many off-the-shelf codec implementation~\cite{??}.
}
% , and the uniform coloring may appear ``unnatural'' to the DNN feature extractors and cause low accuracy.
However, it ignores several favorable properties of DNNs. 

First, many vision models, such as object detectors, naturally handle partially observed objects; \eg if half of a bus appears in the frame, an object detector still has enough features to detect it. 
% We have seen empirical evidence in our experiments too.
%that when an object is only partially encoded in high quality, object detection models can still detect them.
Second, using a single color to encode parts of a frame does not necessarily reduce accuracy.
Vision features extracted by FC layers are ``localized'', \ie changing the value of a pixel in theory does not change another region's FC-extracted features.
(This pattern may hold in the recent transformer-based vision models, but we have not verified it yet.)
That said, using a uniform color still may change the result of the batch normalization operation (which normalizes the feature matrices of the whole image).
% has two adverse effects: 
% (1) it may change the result of the batch normalization operation (which normalizes the feature matrices of the whole image); and % which does take the whole image into account, and 
% (2) it may still affect nearby FC-extracted features.
Somewhat surprisingly, we found that setting the non-high quality blocks in the {\em mean} pixel value (rather than an arbitrary color such as black) can effectively alleviate these issues, since batch normalization will not be affected. %, and it effectively ``smoothes'' the transition to high quality blocks (see Figure~\ref{fig:uniform-color}).
(This uniform color value can be stored with negligible overhead.)
% the uniform color is chosen in a way that \jc{kuntai, is this about normalization?}. \jc{also needs to mention that the uniform color can be retrieved from the encoded image so no additional meta data is needed}
% \kt{We do need to record the metadata (the mask). But for each frame, the mask only contain 45*60 booleans, and the mask is the same for 30 frames. The storage size is ~0.1KB per frame.}
Third, using low quality to encode non-high quality regions often cause DNN to output ``spurious'' inference results (see Figure~\ref{fig:uniform-color}).
In contrast, using a uniform color avoids such false positives. % the high-quality blocks picked by \name already contain enough blocks for DNN to make pretty accurate inference. 


\begin{comment}

there is in fact a tradeoff between using a low quality vs. uniform color to encode the non-high quality blocks.
Using a low quality to encode these regions might cause the DNN to output ``spurious'' inference results.
In contrast, since the high-quality blocks picked by \name already contain enough blocks for DNN to make pretty accurate inference. 
Setting the background in uniform color does not incur much cost on accuracy.
\end{comment}

We acknowledge that using the uniform color may {\em not} apply to all cases. 
% For instance, \jc{give a failure case}
That said, our design choice is driven by the observations of the set of DNNs under our study and we hope it can inspire future designs to improve its generalizability. 

% \jc{need to mention ROI encoding!}


%\subsection{Quality assignment based on accuracy gradients}
%
%\jc{threshold + enlargement}

%\jc{need to talk about how to deal adapt to bandwidth}



%\begin{itemize}
%\item solution (not running it per frame)
%\item choice of quality: we explore an extreme design point of uni-color background
%\item benefits: low bw for same acc, speed-up encoding/decoding \& inference
%\end{itemize}


%\mypara{Mitigating the effect of hard boundaries} 
%\begin{itemize}
%\item problem 1: inference accuracy over the black background can be low. example/reason(cnn)
%\item solution (smoothing?)
%\end{itemize}


\begin{figure}
    \centering
    % \includegraphics[width=0.95\columnwidth]{figs/placeholder-example.pdf}
    
    \includegraphics[width=0.95\columnwidth]{figs/walkthough.pdf}
    \tightcaption{Walkthrough of each stage in \name.}
    \label{fig:example}
    \vspace{-1mm}
\end{figure}


% \subsection{Putting the components together}

\subsection{Implementation}
Finally, we proceed to put the different design components together. 
Figure~\ref{fig:example} shows a concrete example to walk through the input and output of each step.
We implement \name on FFMPEG~\cite{ffmpeg}, with 4036 lines of python codes.
The DNN models are implemented in PyTorch (v1.7.1). 
We will open source the implementation upon publication of the work.

\begin{comment}
During encoding phase, \name receives 30 raw input frames every second and sends the last frame to the \AccuracyGradientModel.
\AccuracyGradientModel outputs the \AccuracyGradient of this frame.
\name then averages this \AccuracyGradient of this second with the last one for better estimation.
Based on this average \AccuracyGradient, we edit the frames: those parts that has high \AccuracyGradient score will be preserved, and other parts will be set to black (but the mean uniform color will be saved separately so that the decoded images can use the mean uniform color to improve accuracy, see \S\ref{subsec:uniform}).
We then feed these edited frames to the codec. The codec will buffer the frames during offline analysis and will immediately encode these frames for online streaming.
At decoding phase, \name decodes the video back to raw frames and reconstruct the blacked parts back to uniform color (RGB=(123.675, 116.28, 103.53) in our experiments) so that these parts will become black (RGB=(0,0,0)) after input preprocessing (\eg ImageNet normalization in ~\cite{pytorch-model-zoo,detectron2}). These reconstructed frames will be feeded into the final DNN to obtain analytic results.

\end{comment}

%\begin{itemize}
%\item challenges remain in two aspects
%\item problem 1: inference accuracy over the black background can be low. example/reason(cnn)
%\item solution (smoothing?)
%\item problem 2: overhead of running the generator per frame. 
%\item solution (not running it per frame)
%\item choice of quality: we explore an extreme design point of uni-color background
%\item benefits: low bw for same acc, speed-up encoding/decoding \& inference
%\end{itemize}

%\newpage
